Dynamic Term-Modal Logics for First-Order Epistemic Planning

Many classical planning frameworks are built on first-order languages. The first-order expressive power is desirable for compactly representing actions via schemas, and for specifying quantified conditions such as $\neg\exists x\mathsf{blocks\_door}(x)$. In contrast, several recent epistemic planning frameworks are built on propositional epistemic logic. The epistemic language is useful to describe planning problems involving higher-order reasoning or epistemic goals such as $K_{a}\neg\mathsf{problem}$. This paper develops a first-order version of Dynamic Epistemic Logic (DEL). In this framework, for example, $\exists xK_{x}\exists y\mathsf{blocks\_door}(y)$ is a formula. The formalism combines the strengths of DEL (higher-order reasoning) with those of first-order logic (lifted representation) to model multi-agent epistemic planning. The paper introduces an epistemic language with a possible-worlds semantics, followed by novel dynamics given by first-order action models and their execution via product updates. Taking advantage of the first-order machinery, epistemic action schemas are defined to provide compact, problem-independent domain descriptions, in the spirit of PDDL. Concerning metatheory, the paper defines axiomatic normal term-modal logics, shows a Canonical Model Theorem-like result which allows establishing completeness through frame characterization formulas, shows decidability for the finite agent case, and shows a general completeness result for the dynamic extension by reduction axioms.

==> pgfcirc.defines.tex <==

%% Options

%%%%%%%%%%%%
%% Dimensions

% coordinates
\newdimen\pgf@circ@res@up
\newdimen\pgf@circ@res@down
\newdimen\pgf@circ@res@zero
\newdimen\pgf@circ@res@left
\newdimen\pgf@circ@res@right
\newdimen\pgf@circ@res@other
\newdimen\pgf@circ@res@step
\newdimen\pgf@circ@res@temp
% inital thickness
\newdimen \pgfstartlinewidth

% arrow tips, ported over old arrows library (deprecated)
% see https://tex.stackexchange.com/questions/234084/latex-arrow-tip-with-arrows-meta-library
% this was the original definition of latex' tips, renamed to avoid clashes
%
\pgfarrowsdeclare{latexslim}{latexslim}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfarrowsleftextend{+-4\pgfutil@tempdima}
  \pgfarrowsrightextend{+6\pgfutil@tempdima}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfpathmoveto{\pgfqpoint{6\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{3.5\pgfutil@tempdima}{.5\pgfutil@tempdima}}
  {\pgfqpoint{-1\pgfutil@tempdima}{1.5\pgfutil@tempdima}}
  {\pgfqpoint{-4\pgfutil@tempdima}{3.75\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{-1.5\pgfutil@tempdima}{1\pgfutil@tempdima}}
  {\pgfqpoint{-1.5\pgfutil@tempdima}{-1\pgfutil@tempdima}}
  {\pgfqpoint{-4\pgfutil@tempdima}{-3.75\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{-1\pgfutil@tempdima}{-1.5\pgfutil@tempdima}}
  {\pgfqpoint{3.5\pgfutil@tempdima}{-.5\pgfutil@tempdima}}
  {\pgfqpoint{6\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqfill
}

\pgfarrowsdeclarereversed{latexslim reversed}{latexslim reversed}{latexslim}{latexslim}

%% Macro to fill or draw

\def\pgf@circ@draworfill{%
    \ifx\tikz@fillcolor\pgfutil@empty
        \pgfusepath{draw}
    \else
        \pgfsetfillcolor{\tikz@fillcolor}
        \pgfusepath{draw, fill}
    \fi
}

\def\pgf@circ@draworfillandclip{%
    \ifx\tikz@fillcolor\pgfutil@empty
        \pgfusepath{draw, clip}
    \else
        \pgfsetfillcolor{\tikz@fillcolor}
        \pgfusepath{draw, clip, fill}
    \fi
}

\def\pgf@circ@maybefill{%
    \ifx\tikz@fillcolor\pgfutil@empty
        \pgfusepath{discard}
    \else
        \pgfsetfillcolor{\tikz@fillcolor}
        \pgfusepath{fill}
    \fi
}
%% Keys

\long\def\pgf@circ@comment#1{}

\def\circuitikzbasekey{/tikz/circuitikz}

\pgfkeys{\circuitikzbasekey/.is family}

\def\circuitikzset#1{\pgfkeys{\circuitikzbasekey,#1}}
\let\ctikzset\circuitikzset
\def\ctikzvalof#1{\pgfkeysvalueof{\circuitikzbasekey/#1}}
\def\ctikzsetvalof#1#2{\pgfkeyssetvalue{\circuitikzbasekey/#1}{#2}}

\newif\ifpgf@circ@siunitx
\newif\ifpgf@circuit@compat
\newif\ifpgf@circ@oldvoltagedirection % default false
\newif\ifpgf@circ@explicitvdir
\newif\ifpgf@circ@fixbatteries

\ctikzset{voltage dir/.is choice}
\ctikzset{voltage dir/old/.code={\pgf@circ@oldvoltagedirectiontrue\pgf@circ@fixbatteriesfalse}}
\ctikzset{voltage dir/noold/.code={\pgf@circ@oldvoltagedirectionfalse\pgf@circ@fixbatteriesfalse}}
\ctikzset{voltage dir/RP/.code={\pgf@circ@oldvoltagedirectiontrue\pgf@circ@fixbatteriestrue}}
\ctikzset{voltage dir/EF/.code={\pgf@circ@oldvoltagedirectionfalse\pgf@circ@fixbatteriestrue}}
\tikzset{voltage dir/.style={circuitikz/voltage dir=#1}}


% Option ">" for twoports
\newif\ifpgf@circuit@inputarrow
\ctikzset{>/.add code={}{\pgf@circuit@inputarrowtrue}}
\ctikzset{inputarrow/.is choice}
\ctikzset{inputarrow/true/.code={\pgf@circuit@inputarrowtrue}}
\ctikzset{inputarrow/false/.code={\pgf@circuit@inputarrowfalse}}

% Option "boxed" for nodes and twoports
\newif\ifpgf@circuit@boxed
\pgfkeys{/tikz/boxed/.add code={}{\pgf@circuit@boxedtrue}}
\ctikzset{boxed/.add code={}{\pgf@circuit@boxedtrue}}
\pgfkeys{/tikz/box/.add code={}{\pgf@circuit@boxedtrue}}
\ctikzset{box/.add code={}{\pgf@circuit@boxedtrue}}

% Option "dashed" for nodes and twoports
\newif\ifpgf@circuit@dashed
\pgfkeys{/tikz/dashed/.add code={}{\pgf@circuit@dashedtrue}}
\ctikzset{dashed/.add code={}{\pgf@circuit@dashedtrue}}

% Option "t=*" for nodes
\pgfkeys{/tikz/t/.add code={}{\ctikzset{text=#1}}}

\ctikzset{current arrow scale/.initial=16}

\ctikzset{bipoles/.is family}
\ctikzset{bipoles/border margin/.initial=1.1}
\ctikzset{bipoles/thickness/.initial=2}
\ctikzset{tripoles/thickness/.initial=2}
\ctikzset{quadpoles/thickness/.initial=2}
\ctikzset{nodes width/.initial=.04}

% Base len for all circuitikz
\newdimen\pgf@circ@Rlen
\ctikzset{bipoles/length/.code={\pgf@circ@Rlen = #1}}
\pgf@circ@Rlen = 1.4cm

\ctikzset{monopoles/.is family}
\ctikzset{monopoles/ground/width/.initial=.25}
\ctikzset{monopoles/ground/connectionthickness/.initial=1}
\ctikzset{monopoles/ground/thickness/.initial=2}
\ctikzset{monopoles/rground/thickness/.initial=2}
\ctikzset{monopoles/tground/thickness/.initial=3}
\ctikzset{monopoles/vcc/width/.initial=.2}
\ctikzset{monopoles/match/width/.initial=.4}
\ctikzset{monopoles/chassis/width/.initial=.25}
\ctikzset{monopoles/alternative chassis/width/.initial=.25}
\ctikzset{monopoles/equipotentiality/width/.initial=.25}
\ctikzset{monopoles/tlinestub/width/.initial=.25}
\ctikzset{monopoles/antenna/width/.initial=.25}
\ctikzset{monopoles/antenna/label/xanchor/.initial=.4}
\ctikzset{monopoles/antenna/label/yanchor/.initial=.75}
\ctikzset{monopoles/txantenna/label/xanchor/.initial=.4}
\ctikzset{monopoles/txantenna/label/yanchor/.initial=.75}
\ctikzset{monopoles/txantenna/width/.initial=.25}
\ctikzset{monopoles/rxantenna/label/xanchor/.initial=.4}
\ctikzset{monopoles/rxantenna/label/yanchor/.initial=.75}
\ctikzset{monopoles/rxantenna/width/.initial=.25}
\ctikzset{monopoles/bareantenna/width/.initial=.25}
\ctikzset{monopoles/bareantenna/label/xanchor/.initial=1}
\ctikzset{monopoles/bareantenna/label/yanchor/.initial=0.5}
\ctikzset{monopoles/waves/width/.initial=0.5}
% microstrips
\ctikzset{bipoles/mstline/height/.initial=0.3}
\ctikzset{bipoles/mstline/width/.initial=1.2}
\pgfkeys{/tikz/mstlinelen/.add code={}{\ctikzset{bipoles/mstline/width=#1}}}
\ctikzset{monopoles/msport/width/.initial=.5}
\ctikzset{monopoles/msrstub/height/.initial=1.0}
\ctikzset{monopoles/msrstub/width/.initial=0.6}

% microphone and loudspeaker
\ctikzset{bipoles/loudspeaker/height/.initial=.8}
\ctikzset{bipoles/loudspeaker/depth/.initial=.3}
\ctikzset{bipoles/loudspeaker/width/.initial=.8}
\ctikzset{bipoles/mic/height/.initial=1.2}
\ctikzset{bipoles/mic/depth/.initial=.0}
\ctikzset{bipoles/mic/width/.initial=.8}

\ctikzset{bipoles/resistor/height/.initial=.3}
\ctikzset{bipoles/resistor/width/.initial=.8}
\ctikzset{bipoles/potentiometer/height/.initial=.8}
\ctikzset{bipoles/potentiometer/height 2/.initial=.3}
\ctikzset{bipoles/potentiometer/width/.initial=.8}
\ctikzset{bipoles/photoresistor/height/.initial=.6}
\ctikzset{bipoles/photoresistor/height 2/.initial=.3}
\ctikzset{bipoles/photoresistor/width/.initial=.8}
\ctikzset{bipoles/thermistor/main/.initial=.7}
\ctikzset{bipoles/thermistor/height/.initial=.428}%.3/.7
\ctikzset{bipoles/thermistorntc/width/.initial=.8}
\ctikzset{bipoles/thermistorntc/main/.initial=.7}
\ctikzset{bipoles/thermistorntc/height/.initial=.428}%.3/.7
\ctikzset{bipoles/thermistorntc/height 2/.initial=.75}%.3/.7
\ctikzset{bipoles/thermistorptc/width/.initial=.8}
\ctikzset{bipoles/thermistorptc/main/.initial=.7}
\ctikzset{bipoles/thermistorptc/height/.initial=.428}%.3/.7
\ctikzset{bipoles/thermistorptc/height 2/.initial=.75}%.3/.7
\ctikzset{bipoles/thermistor/width/.initial=.8}
\ctikzset{bipoles/varistor/main/.initial=.7}
\ctikzset{bipoles/varistor/height/.initial=.428}%.3/.7
\ctikzset{bipoles/varistor/width/.initial=.8}
\ctikzset{bipoles/vresistor/height/.initial=.6}
\ctikzset{bipoles/vresistor/width/.initial=.8}
\ctikzset{bipoles/cuteinductor/height/.initial=.3}
\ctikzset{bipoles/cuteinductor/lower coil height/.initial=.15}
\ctikzset{bipoles/cuteinductor/width/.initial=.6}
\ctikzset{bipoles/cuteinductor/coils/.initial=5}
\ctikzset{bipoles/cuteinductor/coil aspect/.initial=.5}%percentage of inductor width, which is covered by lower coil
%% Cute choke settings
\ctikzset{bipoles/cutechoke/height/.initial=.3}
\ctikzset{bipoles/cutechoke/lower coil height/.initial=.15}
\ctikzset{bipoles/cutechoke/width/.initial=.6}
\ctikzset{bipoles/cutechoke/coils/.initial=5}
\ctikzset{bipoles/cutechoke/coil aspect/.initial=.5}%percentage of choke width, which is covered by lower coil
\ctikzset{bipoles/cutechoke/cstep/.initial=.3}
\ctikzset{bipoles/cutechoke/cdist/.initial=1.3}
\ctikzset{bipoles/cutechoke/cthick/.initial=1}
\newif\ifpgf@circuit@bipole@twolines
\pgf@circuit@bipole@twolinesfalse
%
\ctikzset{bipoles/americaninductor/height/.initial=.3}
\ctikzset{bipoles/americaninductor/height 2/.initial=.1}
\ctikzset{bipoles/americaninductor/width/.initial=.8}
\ctikzset{bipoles/americaninductor/coils/.initial=4}
\ctikzset{bipoles/americaninductor/coil height/.initial=.15}
\ctikzset{bipoles/vcuteinductor/height/.initial=.6}
\ctikzset{bipoles/vcuteinductor/lower coil height/.initial=.3}
\ctikzset{bipoles/vcuteinductor/width/.initial=.6}
\ctikzset{bipoles/vcuteinductor/coils/.initial=5}
\ctikzset{bipoles/vcuteinductor/coil aspect/.initial=.5}%percentage of inductor width, which is covered by lower coil
\ctikzset{bipoles/vamericaninductor/height/.initial=.6}
\ctikzset{bipoles/vamericaninductor/height 2/.initial=.2}
\ctikzset{bipoles/vamericaninductor/width/.initial=.8}
\ctikzset{bipoles/vamericaninductor/coils/.initial=4}
\ctikzset{bipoles/vamericaninductor/coil height/.initial=.15}
\ctikzset{bipoles/esource/height/.initial=.60}
\ctikzset{bipoles/esource/width/.initial=.60}
\ctikzset{bipoles/pvsource/height/.initial=.60}
\ctikzset{bipoles/pvsource/width/.initial=.60}
\ctikzset{bipoles/isource/height/.initial=.60}
\ctikzset{bipoles/isource/width/.initial=.60}
\ctikzset{bipoles/oosource/height/.initial=.60}
\ctikzset{bipoles/oosource/width/.initial=.60}
\ctikzset{bipoles/oosource/circlesize/.initial=.65}%circlesize+circleoffset should be =1
\ctikzset{bipoles/oosource/circleoffset/.initial=.35}%circlesize+circleoffset should be =1
\ctikzset{bipoles/dcisource/height/.initial=.60}
\ctikzset{bipoles/dcisource/width/.initial=.60}
\ctikzset{bipoles/dcvsource/height/.initial=.60}
\ctikzset{bipoles/dcvsource/width/.initial=.60}
\ctikzset{bipoles/vsourcetri/height/.initial=.60}
\ctikzset{bipoles/vsourcetri/width/.initial=.60}
\ctikzset{bipoles/isourceam/height/.initial=.60}
\ctikzset{bipoles/isourceam/width/.initial=.60}
\ctikzset{bipoles/vsource/height/.initial=.60}
\ctikzset{bipoles/vsource/width/.initial=.60}
\ctikzset{bipoles/vsourceam/height/.initial=.60}
\ctikzset{bipoles/vsourceam/width/.initial=.60}
\ctikzset{bipoles/vsourceam/margin/.initial=.7}
\ctikzset{bipoles/isourcesin/height/.initial=.60}
\ctikzset{bipoles/isourcesin/width/.initial=.60}
\ctikzset{bipoles/vsourcesin/height/.initial=.60}
\ctikzset{bipoles/vsourcesin/width/.initial=.60}
\ctikzset{bipoles/vsourcesquare/height/.initial=.60}
\ctikzset{bipoles/vsourcesquare/width/.initial=.60}
\ctikzset{bipoles/cisource/height/.initial=.7}
\ctikzset{bipoles/cisource/width/.initial=.7}
\ctikzset{bipoles/cisourceam/height/.initial=.7}
\ctikzset{bipoles/cisourceam/width/.initial=.7}
\ctikzset{bipoles/cvsource/height/.initial=.7}
\ctikzset{bipoles/cvsource/width/.initial=.7}
\ctikzset{bipoles/cvsourceam/height/.initial=.7}
\ctikzset{bipoles/cvsourceam/width/.initial=.7}
\ctikzset{bipoles/cvsourceam/margin/.initial=.7}
\ctikzset{bipoles/cvsourceam/text scale/.initial=1}
\ctikzset{bipoles/cisourcesin/width/.initial=.7}
\ctikzset{bipoles/cvsourcesin/height/.initial=.7}
\ctikzset{bipoles/cvsourcesin/width/.initial=.7}
\ctikzset{bipoles/capacitor/height/.initial=.6}
\ctikzset{bipoles/capacitor/width/.initial=.2}
\ctikzset{bipoles/ecapacitor/height/.initial=.5}
\ctikzset{bipoles/ecapacitor/width/.initial=.2}
\ctikzset{bipoles/ecapacitor/font/.initial= \fontsize{6}{0}\selectfont\boldmath}
\ctikzset{bipoles/pcapacitor/height/.initial=.6}
\ctikzset{bipoles/pcapacitor/width/.initial=.2}
\ctikzset{bipoles/pcapacitor/bend width/.initial=1.1}
\ctikzset{bipoles/vcapacitor/height/.initial=.6}
\ctikzset{bipoles/vcapacitor/width/.initial=.5}
\ctikzset{bipoles/vcapacitor/capacitor width/.initial=.4}
\ctikzset{bipoles/piezoelectric/height/.initial=.7}
\ctikzset{bipoles/piezoelectric/width/.initial=.5}
\ctikzset{bipoles/battery/height/.initial=.6}
\ctikzset{bipoles/battery/width/.initial=.3}
\ctikzset{bipoles/battery1/height/.initial=.6}
\ctikzset{bipoles/battery1/width/.initial=.3}
\ctikzset{bipoles/battery2/height/.initial=.6}
\ctikzset{bipoles/battery2/width/.initial=.3}
\ctikzset{bipoles/diode/height/.initial=.50}
\ctikzset{bipoles/diode/width/.initial=.40}
\ctikzset{bipoles/bidirectionaldiode/height/.initial=1.1}
\ctikzset{bipoles/bidirectionaldiode/width/.initial=1}
\ctikzset{bipoles/bidirectionaldiode/diode width left/.initial=.3}
\ctikzset{bipoles/bidirectionaldiode/diode width right/.initial=.3}
\ctikzset{bipoles/varcap/height/.initial=.50}
\ctikzset{bipoles/varcap/width/.initial=.45}
\ctikzset{bipoles/spst/height/.initial=.35}
\ctikzset{bipoles/spst/width/.initial=.35}
\ctikzset{bipoles/spst/depth/.initial=.2}
\ctikzset{bipoles/nos/height/.initial=.3}
\ctikzset{bipoles/nos/width/.initial=.35}
\ctikzset{bipoles/nos/depth/.initial=.2}
\ctikzset{bipoles/ncs/height/.initial=.35}
\ctikzset{bipoles/ncs/width/.initial=.35}
\ctikzset{bipoles/ncs/depth/.initial=.2}
\ctikzset{bipoles/generic/height/.initial=.30}
\ctikzset{bipoles/generic/width/.initial=.80}
\ctikzset{bipoles/european gas filled surge arrester/height/.initial=.30}
\ctikzset{bipoles/european gas filled surge arrester/width/.initial=.80}
\ctikzset{bipoles/european gas filled surge arrester/inside/.initial=.30}
\ctikzset{bipoles/american gas filled surge arrester/height/.initial=.60}
\ctikzset{bipoles/american gas filled surge arrester/width/.initial=.60}
\ctikzset{bipoles/american gas filled surge arrester/inside/.initial=.15}
\ctikzset{bipoles/american gas filled surge arrester/dot x/.initial=.25}
\ctikzset{bipoles/american gas filled surge arrester/dot y/.initial=.45}
\ctikzset{bipoles/american gas filled surge arrester/size/.initial=.1}
\ctikzset{bipoles/fuse/height/.initial=.20}
\ctikzset{bipoles/fuse/width/.initial=.50}
\ctikzset{bipoles/afuse/height/.initial=.20}
\ctikzset{bipoles/afuse/width/.initial=.50}
\ctikzset{bipoles/generic potentiometer/height/.initial=.80}
\ctikzset{bipoles/generic potentiometer/height 2/.initial=.30}
\ctikzset{bipoles/generic potentiometer/width/.initial=.80}
\ctikzset{bipoles/ageneric/height/.initial=.30}
\ctikzset{bipoles/ageneric/width/.initial=.80}
\ctikzset{bipoles/memristor/height/.initial=.30}
\ctikzset{bipoles/memristor/wave height/.initial=.5}
\ctikzset{bipoles/memristor/width/.initial=.80}
\ctikzset{bipoles/tgeneric/height/.initial=.70}
\ctikzset{bipoles/tgeneric/width/.initial=.80}
\ctikzset{bipoles/tfullgeneric/height/.initial=.70}
\ctikzset{bipoles/tfullgeneric/width/.initial=.80}
\ctikzset{bipoles/fullgeneric/height/.initial=.30}
\ctikzset{bipoles/fullgeneric/width/.initial=.80}
\ctikzset{bipoles/open/height/.initial=.3} %necessary for curly voltages
\ctikzset{bipoles/open/width/.initial=.3} %necessary for curly voltages
\ctikzset{bipoles/open/voltage/straight label distance/.initial=0}
\ctikzset{bipoles/open/voltage/distance from node/.initial=.2}
\ctikzset{bipoles/short/height/.initial=0} %dummy height for voltage positioning
\ctikzset{bipoles/short/width/.initial=0} %dummy width for voltage positioning
%\ctikzset{bipoles/short/voltage/straight label distance/.initial=.2}
%\ctikzset{bipoles/short/voltage/distance from node/.initial=.5}
\ctikzset{bipoles/ammeter/height/.initial=.60}
\ctikzset{bipoles/ammeter/width/.initial=.60}
\ctikzset{bipoles/ohmmeter/height/.initial=.60}
\ctikzset{bipoles/ohmmeter/width/.initial=.60}
\ctikzset{bipoles/voltmeter/height/.initial=.60}
\ctikzset{bipoles/voltmeter/width/.initial=.60}
\ctikzset{bipoles/smeter/height/.initial=.60}
\ctikzset{bipoles/smeter/width/.initial=.60}
\ctikzset{bipoles/qmeter/depth/.initial=.40}
\ctikzset{bipoles/qmeter/height/.initial=.80}
\ctikzset{bipoles/qmeter/width/.initial=.60}
\ctikzset{bipoles/iloop/width/.initial=.40}
\ctikzset{bipoles/iloop/height/.initial=.60}
\ctikzset{bipoles/oscope/height/.initial=.60}
\ctikzset{bipoles/oscope/width/.initial=.60}
\ctikzset{bipoles/buffer/height/.initial=1}
\ctikzset{bipoles/buffer/width/.initial=1}
\ctikzset{bipoles/not port/width/.initial=1}
\ctikzset{bipoles/not port/height/.initial=.8}
\ctikzset{bipoles/not port/circle width/.initial=.15}
\ctikzset{bipoles/lamp/height/.initial=.60}
\ctikzset{bipoles/lamp/width/.initial=.60}
\ctikzset{bipoles/bulb/height/.initial=.8}
\ctikzset{bipoles/bulb/width/.initial=.8}
\ctikzset{bipoles/tline/height/.initial=.3}
\ctikzset{bipoles/tline/width/.initial=.8}
\ctikzset{bipoles/squid/height/.initial=.60}
\ctikzset{bipoles/squid/width/.initial=.60}
\ctikzset{bipoles/barrier/height/.initial=.60}
\ctikzset{bipoles/barrier/width/.initial=.60}
\ctikzset{bipoles/thermocouple/height/.initial=.250}
\ctikzset{bipoles/thermocouple/height 2/.initial=.60}
\ctikzset{bipoles/thermocouple/width/.initial=.140}
\ctikzset{bipoles/pushbutton/height/.initial=.5}
\ctikzset{bipoles/pushbutton/height 2/.initial=.2}
\ctikzset{bipoles/pushbutton/width/.initial=.50}

\ctikzset{bipoles/twoport/width/.initial=.7}
\ctikzset{bipoles/twoport/height/.initial=.7}
\ctikzset{bipoles/twoport/text/.initial=}
\ctikzset{bipoles/vco/width/.initial=.7}
\ctikzset{bipoles/bandpass/width/.initial=.7}
\ctikzset{bipoles/bandstop/width/.initial=.7}
\ctikzset{bipoles/highpass/width/.initial=.7}
\ctikzset{bipoles/lowpass/width/.initial=.7}
\ctikzset{bipoles/adc/width/.initial=.7}
\ctikzset{bipoles/dac/width/.initial=.7}
\ctikzset{bipoles/dsp/width/.initial=.7}
\ctikzset{bipoles/fft/width/.initial=.7}
\ctikzset{bipoles/amp/width/.initial=.7}
\ctikzset{bipoles/vamp/width/.initial=.7}
\ctikzset{bipoles/piattenuator/width/.initial=.7}
\ctikzset{bipoles/vpiattenuator/width/.initial=.7}
\ctikzset{bipoles/tattenuator/width/.initial=.7}
\ctikzset{bipoles/vtattenuator/width/.initial=.7}
\ctikzset{bipoles/phaseshifter/width/.initial=.7}
\ctikzset{bipoles/vphaseshifter/width/.initial=.7}
\ctikzset{bipoles/detector/width/.initial=.7}
% resistive sensor american style
\ctikzset{bipoles/resistivesens/height/.initial=.6}
\ctikzset{bipoles/resistivesens/width/.initial=.8}

% crossing wires
\ctikzset{bipoles/crossing/size/.initial=.2}

\newif\ifpgf@circuit@trans@depletiontype
\pgf@circuit@trans@depletiontypefalse

\newif\ifpgf@circuit@mos@arrows
\ctikzset{tripoles/mos style/.is choice}
\ctikzset{tripoles/mos style/no arrows/.code={\pgf@circuit@mos@arrowsfalse}}
\ctikzset{tripoles/mos style/arrows/.code={\pgf@circuit@mos@arrowstrue}}

% Option solderdot for fet
\newif\ifpgf@circuit@fet@solderdot
\pgfkeys{/tikz/solderdot/.add code={}{\pgf@circuit@fet@solderdottrue}}
\ctikzset{solderdot/.add code={}{\pgf@circuit@fet@solderdottrue}}
\pgfkeys{/tikz/nosolderdot/.add code={}{\pgf@circuit@fet@solderdotfalse}}
\ctikzset{nosolderdot/.add code={}{\pgf@circuit@fet@solderdotfalse}}

% Option bodydiode for fet
\newif\ifpgf@circuit@fet@bodydiode
\pgfkeys{/tikz/bodydiode/.add code={}{\pgf@circuit@fet@bodydiodetrue}}
\ctikzset{bodydiode/.add code={}{\pgf@circuit@fet@bodydiodetrue}}
\pgfkeys{/tikz/nobodydiode/.add code={}{\pgf@circuit@fet@bodydiodefalse}}
\ctikzset{nobodydiode/.add code={}{\pgf@circuit@fet@bodydiodefalse}}

% Option draw fet without gate connection
\newif\ifpgf@circuit@bpt@drawgate
\pgf@circuit@bpt@drawgatetrue
\pgfkeys{/tikz/nogate/.add code={}{\pgf@circuit@bpt@drawgatefalse}}
\ctikzset{nogate/.add code={}{\pgf@circuit@bpt@drawgatefalse}}
\pgfkeys{/tikz/nobase/.add code={}{\pgf@circuit@bpt@drawgatefalse}}
\ctikzset{nobase/.add code={}{\pgf@circuit@bpt@drawgatefalse}}

% Option draw bpt without base connection
\newif\ifpgf@circuit@bpt@drawbase
\pgf@circuit@bpt@drawbasetrue
\pgfkeys{/tikz/nobase/.add code={}{\pgf@circuit@bpt@drawbasefalse}}
\ctikzset{nobase/.add code={}{\pgf@circuit@bpt@drawbasefalse}}
\pgfkeys{/tikz/nogate/.add code={}{\pgf@circuit@bpt@drawbasefalse}}
\ctikzset{nogate/.add code={}{\pgf@circuit@bpt@drawbasefalse}}

% Option draw bpt with optical input
\newif\ifpgf@circuit@bpt@drawphoto
\pgf@circuit@bpt@drawphotofalse
\pgfkeys{/tikz/photo/.add code={}{\pgf@circuit@bpt@drawphototrue}}
\ctikzset{photo/.add code={}{\pgf@circuit@bpt@drawphototrue}}
\pgfkeys{/tikz/photo/.add code={}{\pgf@circuit@bpt@drawphototrue}}
\ctikzset{photo/.add code={}{\pgf@circuit@bpt@drawphototrue}}

% Option draw pmos with empty circle
\newif\ifpgf@circuit@pmos@emptycircle
\newif\ifpgf@circuit@pmos@emptycircle
\pgf@circuit@pmos@emptycirclefalse
\pgfkeys{/tikz/emptycircle/.add code={}{\pgf@circuit@pmos@emptycircletrue}}
\ctikzset{tripoles/pmos style/emptycircle/.add code={}{\pgf@circuit@pmos@emptycircletrue}}


\newif\ifpgf@circuit@trans@ntype
\pgf@circuit@trans@ntypetrue %default true
%\newif\ifpgf@circuit@trans@ptype
%\ctikzset{tripoles/nmos/.add code={\pgf@circuit@trans@ntypetrue}}
\ctikzset{tripoles/nmos/width/.initial=.7}
\ctikzset{tripoles/nmos/gate height/.initial=.35}
\ctikzset{tripoles/nmos/base height/.initial=.5}
\ctikzset{tripoles/nmos/conn height/.initial=0}
\ctikzset{tripoles/nmos/height/.initial=1.1}
\ctikzset{tripoles/nmos/base width/.initial=.5}
\ctikzset{tripoles/nmos/gate width/.initial=.62}
\ctikzset{tripoles/nmos/arrow pos/.initial=.6}
\ctikzset{tripoles/nmos/bodydiode scale/.initial=.3}
\ctikzset{tripoles/nmos/bodydiode distance/.initial=.3}
\ctikzset{tripoles/nmos/bodydiode conn/.initial=.6}
\ctikzset{tripoles/nmos/curr direction/.initial=1}

\ctikzset{tripoles/pmos/width/.initial=.7}
\ctikzset{tripoles/pmos/gate height/.initial=.35}
\ctikzset{tripoles/pmos/base height/.initial=.5}
\ctikzset{tripoles/pmos/conn height/.initial=0}
\ctikzset{tripoles/pmos/height/.initial=1.1}
\ctikzset{tripoles/pmos/base width/.initial=.5}
\ctikzset{tripoles/pmos/gate width/.initial=.62}
\ctikzset{tripoles/pmos/arrow pos/.initial=.4}
\ctikzset{tripoles/pmos/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pmos/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pmos/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pmos/curr direction/.initial=-1}

\ctikzset{tripoles/hemt/width/.initial=.7}
\ctikzset{tripoles/hemt/gate height/.initial=.35}
\ctikzset{tripoles/hemt/base height/.initial=.5}
\ctikzset{tripoles/hemt/conn height/.initial=0}
\ctikzset{tripoles/hemt/height/.initial=1.1}
\ctikzset{tripoles/hemt/base width/.initial=.5}
\ctikzset{tripoles/hemt/gate width/.initial=.62}
\ctikzset{tripoles/hemt/bodydiode scale/.initial=.3}
\ctikzset{tripoles/hemt/bodydiode distance/.initial=.3}
\ctikzset{tripoles/hemt/bodydiode conn/.initial=.6}
\ctikzset{tripoles/hemt/curr direction/.initial=1}

\ctikzset{tripoles/nfet/width/.initial=.7}
\ctikzset{tripoles/nfet/gate height/.initial=.35}
\ctikzset{tripoles/nfet/base height/.initial=.5}
\ctikzset{tripoles/nfet/conn height/.initial=0}
\ctikzset{tripoles/nfet/height/.initial=1.1}
\ctikzset{tripoles/nfet/base width/.initial=.5}
\ctikzset{tripoles/nfet/gate width/.initial=.62}
\ctikzset{tripoles/nfet/bodydiode scale/.initial=.3}
\ctikzset{tripoles/nfet/bodydiode distance/.initial=.3}
\ctikzset{tripoles/nfet/bodydiode conn/.initial=.6}
\ctikzset{tripoles/nfet/curr direction/.initial=1}

\ctikzset{tripoles/pfet/width/.initial=.7}
\ctikzset{tripoles/pfet/gate height/.initial=.35}
\ctikzset{tripoles/pfet/base height/.initial=.5}
\ctikzset{tripoles/pfet/conn height/.initial=0}
\ctikzset{tripoles/pfet/height/.initial=1.1}
\ctikzset{tripoles/pfet/base width/.initial=.5}
\ctikzset{tripoles/pfet/gate width/.initial=.62}
\ctikzset{tripoles/pfet/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pfet/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pfet/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pfet/curr direction/.initial=-1}

\ctikzset{tripoles/nigfete/width/.initial=.7}
\ctikzset{tripoles/nigfete/gate height/.initial=.35}
\ctikzset{tripoles/nigfete/base height/.initial=.5}
\ctikzset{tripoles/nigfete/conn height/.initial=.35}
\ctikzset{tripoles/nigfete/height/.initial=1.1}
\ctikzset{tripoles/nigfete/base width/.initial=.5}
\ctikzset{tripoles/nigfete/gate width/.initial=.62}
\ctikzset{tripoles/nigfete/bodydiode scale/.initial=.3}
\ctikzset{tripoles/nigfete/bodydiode distance/.initial=.3}
\ctikzset{tripoles/nigfete/bodydiode conn/.initial=.6}
\ctikzset{tripoles/nigfete/curr direction/.initial=1}

\ctikzset{tripoles/nigfetd/width/.initial=.7}
\ctikzset{tripoles/nigfetd/gate height/.initial=.35}
\ctikzset{tripoles/nigfetd/base height/.initial=.5}
\ctikzset{tripoles/nigfetd/conn height/.initial=.35}
\ctikzset{tripoles/nigfetd/height/.initial=1.1}
\ctikzset{tripoles/nigfetd/base width/.initial=.5}
\ctikzset{tripoles/nigfetd/gate width/.initial=.62}
\ctikzset{tripoles/nigfetd/bodydiode scale/.initial=.3}
\ctikzset{tripoles/nigfetd/bodydiode distance/.initial=.3}
\ctikzset{tripoles/nigfetd/bodydiode conn/.initial=.6}
\ctikzset{tripoles/nigfetd/curr direction/.initial=1}

\ctikzset{tripoles/nigfetebulk/width/.initial=.7}
\ctikzset{tripoles/nigfetebulk/gate height/.initial=.35}
\ctikzset{tripoles/nigfetebulk/base height/.initial=.5}
\ctikzset{tripoles/nigfetebulk/conn height/.initial=.35}
\ctikzset{tripoles/nigfetebulk/height/.initial=1.1}
\ctikzset{tripoles/nigfetebulk/base width/.initial=.5}
\ctikzset{tripoles/nigfetebulk/gate width/.initial=.62}
\ctikzset{tripoles/nigfetebulk/bodydiode scale/.initial=.3}
\ctikzset{tripoles/nigfetebulk/bodydiode distance/.initial=.3}
\ctikzset{tripoles/nigfetebulk/bodydiode conn/.initial=.6}
\ctikzset{tripoles/nigfetebulk/curr direction/.initial=1}

\ctikzset{tripoles/pigfete/width/.initial=.7}
\ctikzset{tripoles/pigfete/gate height/.initial=.35}
\ctikzset{tripoles/pigfete/base height/.initial=.5}
\ctikzset{tripoles/pigfete/conn height/.initial=.35}
\ctikzset{tripoles/pigfete/height/.initial=1.1}
\ctikzset{tripoles/pigfete/base width/.initial=.5}
\ctikzset{tripoles/pigfete/gate width/.initial=.62}
\ctikzset{tripoles/pigfete/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pigfete/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pigfete/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pigfete/curr direction/.initial=-1}

\ctikzset{tripoles/pigfetd/width/.initial=.7}
\ctikzset{tripoles/pigfetd/gate height/.initial=.35}
\ctikzset{tripoles/pigfetd/base height/.initial=.5}
\ctikzset{tripoles/pigfetd/conn height/.initial=.35}
\ctikzset{tripoles/pigfetd/height/.initial=1.1}
\ctikzset{tripoles/pigfetd/base width/.initial=.5}
\ctikzset{tripoles/pigfetd/gate width/.initial=.62}
\ctikzset{tripoles/pigfetd/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pigfetd/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pigfetd/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pigfetd/curr direction/.initial=-1}

\ctikzset{tripoles/pigfetebulk/width/.initial=.7}
\ctikzset{tripoles/pigfetebulk/gate height/.initial=.35}
\ctikzset{tripoles/pigfetebulk/conn height/.initial=.35}
\ctikzset{tripoles/pigfetebulk/base height/.initial=.5}
\ctikzset{tripoles/pigfetebulk/height/.initial=1.1}
\ctikzset{tripoles/pigfetebulk/base width/.initial=.5}
\ctikzset{tripoles/pigfetebulk/gate width/.initial=.62}
\ctikzset{tripoles/pigfetebulk/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pigfetebulk/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pigfetebulk/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pigfetebulk/curr direction/.initial=-1}

\ctikzset{tripoles/npn/width/.initial=.6}
\ctikzset{tripoles/npn/base height/.initial=.45}
\ctikzset{tripoles/npn/base height 2/.initial=.15}
\ctikzset{tripoles/npn/base height/.initial=.4}
\ctikzset{tripoles/npn/conn height/.initial=0}
\ctikzset{tripoles/npn/height/.initial=1.1}
\ctikzset{tripoles/npn/base width/.initial=.5}
\ctikzset{tripoles/npn/arrow pos/.initial=.5}
\ctikzset{tripoles/npn/bodydiode scale/.initial=.3}
\ctikzset{tripoles/npn/bodydiode distance/.initial=.3}
\ctikzset{tripoles/npn/bodydiode conn/.initial=.6}
\ctikzset{tripoles/npn/curr direction/.initial=1}

\ctikzset{tripoles/pnp/width/.initial=.6}
\ctikzset{tripoles/pnp/base height/.initial=.45}
\ctikzset{tripoles/pnp/base height 2/.initial=.15}
\ctikzset{tripoles/pnp/base height/.initial=.4}
\ctikzset{tripoles/pnp/conn height/.initial=0}
\ctikzset{tripoles/pnp/height/.initial=1.1}
\ctikzset{tripoles/pnp/base width/.initial=.5}
\ctikzset{tripoles/pnp/arrow pos/.initial=.5}
\ctikzset{tripoles/pnp/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pnp/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pnp/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pnp/curr direction/.initial=-1}

\ctikzset{tripoles/pigbt/width/.initial=.6}
\ctikzset{tripoles/pigbt/gate height/.initial=.45}
\ctikzset{tripoles/pigbt/gate height 2/.initial=.15}
\ctikzset{tripoles/pigbt/base height/.initial=.4}
\ctikzset{tripoles/pigbt/conn height/.initial=0}
\ctikzset{tripoles/pigbt/height/.initial=1.1}
\ctikzset{tripoles/pigbt/gate width/.initial=.62}
\ctikzset{tripoles/pigbt/base width/.initial=.5}
\ctikzset{tripoles/pigbt/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pigbt/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pigbt/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pigbt/curr direction/.initial=-1}

\ctikzset{tripoles/nigbt/width/.initial=.6}
\ctikzset{tripoles/nigbt/gate height/.initial=.45}
\ctikzset{tripoles/nigbt/gate height 2/.initial=.15}
\ctikzset{tripoles/nigbt/base height/.initial=.4}
\ctikzset{tripoles/nigbt/conn height/.initial=0}
\ctikzset{tripoles/nigbt/height/.initial=1.1}
\ctikzset{tripoles/nigbt/gate width/.initial=.62}
\ctikzset{tripoles/nigbt/base width/.initial=.5}
\ctikzset{tripoles/nigbt/bodydiode scale/.initial=.3}
\ctikzset{tripoles/nigbt/bodydiode distance/.initial=.3}
\ctikzset{tripoles/nigbt/bodydiode conn/.initial=.6}
\ctikzset{tripoles/nigbt/curr direction/.initial=1}

\ctikzset{tripoles/Lpigbt/width/.initial=.6}
\ctikzset{tripoles/Lpigbt/gate height/.initial=.45}
\ctikzset{tripoles/Lpigbt/gate height 2/.initial=.15}
\ctikzset{tripoles/Lpigbt/base height/.initial=.4}
\ctikzset{tripoles/Lpigbt/conn height/.initial=.4}
\ctikzset{tripoles/Lpigbt/height/.initial=1.1}
\ctikzset{tripoles/Lpigbt/gate width/.initial=.62}
\ctikzset{tripoles/Lpigbt/base width/.initial=.5}
\ctikzset{tripoles/Lpigbt/bodydiode scale/.initial=.3}
\ctikzset{tripoles/Lpigbt/bodydiode distance/.initial=.3}
\ctikzset{tripoles/Lpigbt/bodydiode conn/.initial=.6}
\ctikzset{tripoles/Lpigbt/curr direction/.initial=-1}

\ctikzset{tripoles/Lnigbt/width/.initial=.6}
\ctikzset{tripoles/Lnigbt/gate height/.initial=.45}
\ctikzset{tripoles/Lnigbt/gate height 2/.initial=.15}
\ctikzset{tripoles/Lnigbt/base height/.initial=.4}
\ctikzset{tripoles/Lnigbt/conn height/.initial=.4}
\ctikzset{tripoles/Lnigbt/height/.initial=1.1}
\ctikzset{tripoles/Lnigbt/gate width/.initial=.62}
\ctikzset{tripoles/Lnigbt/base width/.initial=.5}
\ctikzset{tripoles/Lnigbt/bodydiode scale/.initial=.3}
\ctikzset{tripoles/Lnigbt/bodydiode distance/.initial=.3}
\ctikzset{tripoles/Lnigbt/bodydiode conn/.initial=.6}
\ctikzset{tripoles/Lnigbt/curr direction/.initial=1}

\ctikzset{tripoles/njfet/width/.initial=.7}
\ctikzset{tripoles/njfet/gate height/.initial=.5}
\ctikzset{tripoles/njfet/gate height 2/.initial=.35}
\ctikzset{tripoles/njfet/gate width/.initial=.5}
\ctikzset{tripoles/njfet/conn height/.initial=.35}
\ctikzset{tripoles/njfet/height/.initial=1.1}
\ctikzset{tripoles/njfet/bodydiode scale/.initial=.3}
\ctikzset{tripoles/njfet/bodydiode distance/.initial=.3}
\ctikzset{tripoles/njfet/bodydiode conn/.initial=.6}
\ctikzset{tripoles/njfet/curr direction/.initial=1}

\ctikzset{tripoles/pjfet/width/.initial=.7}
\ctikzset{tripoles/pjfet/gate height/.initial=.5}
\ctikzset{tripoles/pjfet/gate height 2/.initial=.35}
\ctikzset{tripoles/pjfet/gate width/.initial=.5}
\ctikzset{tripoles/pjfet/conn height/.initial=.35}
\ctikzset{tripoles/pjfet/height/.initial=1.1}
\ctikzset{tripoles/pjfet/bodydiode scale/.initial=.3}
\ctikzset{tripoles/pjfet/bodydiode distance/.initial=.3}
\ctikzset{tripoles/pjfet/bodydiode conn/.initial=.6}
\ctikzset{tripoles/pjfet/curr direction/.initial=-1}

\ctikzset{tripoles/isfet/width/.initial=1}
\ctikzset{tripoles/isfet/gate height/.initial=.35}
\ctikzset{tripoles/isfet/base height/.initial=.5}
\ctikzset{tripoles/isfet/height/.initial=1.1}
\ctikzset{tripoles/isfet/base width/.initial=.3}
\ctikzset{tripoles/isfet/gate width/.initial=.5}
\ctikzset{tripoles/isfet/conn height/.initial=0}
\ctikzset{tripoles/isfet/wave width/.initial=.16}
\ctikzset{tripoles/isfet/wave amp/.initial=.06}
\ctikzset{tripoles/isfet/waves y sep/.initial=.22}
\ctikzset{tripoles/isfet/waves x sep/.initial=.8}
\ctikzset{tripoles/isfet/bodydiode scale/.initial=.3}
\ctikzset{tripoles/isfet/bodydiode distance/.initial=.3}
\ctikzset{tripoles/isfet/bodydiode conn/.initial=.6}
\ctikzset{tripoles/isfet/curr direction/.initial=1}

\newif\ifpgf@circuit@europeanlogicport
\ctikzset{logic ports/.is choice}
\ctikzset{logic ports/european/.code= {\pgf@circuit@europeanlogicporttrue
    \tikzset{and port/.style={shape=european and port}}
    \tikzset{or port/.style={shape=european or port}}
    \tikzset{xor port/.style={shape=european xor port}}
    \tikzset{not port/.style={shape=european not port}}
    \tikzset{nand port/.style={shape=european nand port}}
    \tikzset{nor port/.style={shape=european nor port}}
    \tikzset{xnor port/.style={shape=european xnor port}}
    } }
\ctikzset{logic ports/american/.code= {\pgf@circuit@europeanlogicportfalse
    \tikzset{and port/.style={shape=american and port}}
    \tikzset{or port/.style={shape=american or port}}
    \tikzset{xor port/.style={shape=american xor port}}
    \tikzset{not port/.style={shape=american not port}}
    \tikzset{nand port/.style={shape=american nand port}}
    \tikzset{nor port/.style={shape=american nor port}}
    \tikzset{xnor port/.style={shape=american xnor port}}
    } }

\ctikzset{logic ports origin/.is choice}
\ctikzset{logic ports origin/legacy/.code= {
    \ctikzset{tripoles/american and port/origin/.initial=0.8}
    \ctikzset{tripoles/american nand port/origin/.initial=0.8}
    \ctikzset{tripoles/american nor port/origin/.initial=0.8}
    \ctikzset{tripoles/american or port/origin/.initial=0.8}
    \ctikzset{tripoles/american xor port/origin/.initial=0.8}
    \ctikzset{tripoles/american xnor port/origin/.initial=0.8}
    \ctikzset{tripoles/european and port/origin/.initial=0.8}
    \ctikzset{tripoles/european nand port/origin/.initial=0.8}
    \ctikzset{tripoles/european or port/origin/.initial=0.8}
    \ctikzset{tripoles/european nor port/origin/.initial=0.8}
    \ctikzset{tripoles/european xor port/origin/.initial=0.8}
    \ctikzset{tripoles/european xnor port/origin/.initial=0.8}
    \ctikzset{tripoles/european not port/origin/.initial=0.8}
    }
}
\ctikzset{logic ports origin/center/.code= {
    \ctikzset{tripoles/american and port/origin/.initial=0}
    \ctikzset{tripoles/american nand port/origin/.initial=0}
    \ctikzset{tripoles/american nor port/origin/.initial=0}
    \ctikzset{tripoles/american or port/origin/.initial=0}
    \ctikzset{tripoles/american xor port/origin/.initial=0}
    \ctikzset{tripoles/american xnor port/origin/.initial=0}
    \ctikzset{tripoles/european and port/origin/.initial=0}
    \ctikzset{tripoles/european nand port/origin/.initial=0}
    \ctikzset{tripoles/european or port/origin/.initial=0}
    \ctikzset{tripoles/european nor port/origin/.initial=0}
    \ctikzset{tripoles/european xor port/origin/.initial=0}
    \ctikzset{tripoles/european xnor port/origin/.initial=0}
    \ctikzset{tripoles/european not port/origin/.initial=0}
    }
}


\ctikzset{tripoles/american and port/width/.initial=1.1}
\ctikzset{tripoles/american and port/height/.initial=.8}
\ctikzset{tripoles/american and port/port width/.initial=.7}
\ctikzset{tripoles/american and port/input height/.initial=.5}
\ctikzset{tripoles/american nand port/width/.initial=1.1}
\ctikzset{tripoles/american nand port/height/.initial=.8}
\ctikzset{tripoles/american nand port/port width/.initial=.7}
\ctikzset{tripoles/american nand port/circle width/.initial=.15}
\ctikzset{tripoles/american nand port/input height/.initial=.5}
\ctikzset{tripoles/american or port/width/.initial=1.1}
\ctikzset{tripoles/american or port/height/.initial=.8}
\ctikzset{tripoles/american or port/port width/.initial=.7}
\ctikzset{tripoles/american or port/input height/.initial=.5}
\ctikzset{tripoles/american or port/input skip/.initial=.25}
\ctikzset{tripoles/american or port/aaa/.initial=.6}
\ctikzset{tripoles/american or port/bbb/.initial=.4}
\ctikzset{tripoles/american or port/ccc/.initial=.5}
\ctikzset{tripoles/american or port/ddd/.initial=.0}
\ctikzset{tripoles/american nor port/width/.initial=1.1}
\ctikzset{tripoles/american nor port/height/.initial=.8}
\ctikzset{tripoles/american nor port/port width/.initial=.7}
\ctikzset{tripoles/american nor port/input height/.initial=.5}
\ctikzset{tripoles/american nor port/input skip/.initial=.25}
\ctikzset{tripoles/american nor port/circle width/.initial=.15}
\ctikzset{tripoles/american nor port/aaa/.initial=.6}
\ctikzset{tripoles/american nor port/bbb/.initial=.4}
\ctikzset{tripoles/american nor port/ccc/.initial=.5}
\ctikzset{tripoles/american nor port/ddd/.initial=.0}
\ctikzset{tripoles/american xor port/width/.initial=1.1}
\ctikzset{tripoles/american xor port/height/.initial=.8}
\ctikzset{tripoles/american xor port/port width/.initial=.7}
\ctikzset{tripoles/american xor port/input height/.initial=.5}
\ctikzset{tripoles/american xor port/input skip/.initial=.15}
\ctikzset{tripoles/american xor port/distance/.initial=.1}
\ctikzset{tripoles/american xnor port/width/.initial=1.1}
\ctikzset{tripoles/american xnor port/height/.initial=.8}
\ctikzset{tripoles/american xnor port/port width/.initial=.7}
\ctikzset{tripoles/american xnor port/input height/.initial=.5}
\ctikzset{tripoles/american xnor port/input skip/.initial=.15}
\ctikzset{tripoles/american xnor port/distance/.initial=.1}
\ctikzset{tripoles/american xnor port/circle width/.initial=.15}
\ctikzset{tripoles/american and port/origin/.initial=0.8}
\ctikzset{tripoles/american and port/inputs/.initial=2}
% variable number of inputs
\ctikzset{tripoles/american nand port/origin/.initial=0.8}
\ctikzset{tripoles/american nand port/inputs/.initial=2}
\ctikzset{tripoles/american nor port/origin/.initial=0.8}
\ctikzset{tripoles/american nor port/inputs/.initial=2}
\ctikzset{tripoles/american nor port/angle/.initial=70}
\ctikzset{tripoles/american nor port/inner/.initial=0.3}
\ctikzset{tripoles/american or port/origin/.initial=0.8}
\ctikzset{tripoles/american or port/inputs/.initial=2}
\ctikzset{tripoles/american or port/angle/.initial=70}
\ctikzset{tripoles/american or port/inner/.initial=0.3}
\ctikzset{tripoles/american xor port/origin/.initial=0.8}
\ctikzset{tripoles/american xor port/inputs/.initial=2}
\ctikzset{tripoles/american xor port/angle/.initial=70}
\ctikzset{tripoles/american xor port/inner/.initial=0.3}
\ctikzset{tripoles/american xnor port/origin/.initial=0.8}
\ctikzset{tripoles/american xnor port/inputs/.initial=2}
\ctikzset{tripoles/american xnor port/angle/.initial=70}
\ctikzset{tripoles/american xnor port/inner/.initial=0.3}

\ctikzset{tripoles/european and port/width/.initial=1.4}
\ctikzset{tripoles/european and port/height/.initial=.65}
\ctikzset{tripoles/european and port/reserved/.initial=.6}
\ctikzset{tripoles/european and port/input height/.initial=.6}
\ctikzset{tripoles/european or port/width/.initial=1.4}
\ctikzset{tripoles/european or port/height/.initial=.65}
\ctikzset{tripoles/european or port/reserved/.initial=.6}
\ctikzset{tripoles/european or port/input height/.initial=.6}
\ctikzset{tripoles/european xor port/width/.initial=1.4}
\ctikzset{tripoles/european xor port/height/.initial=.65}
\ctikzset{tripoles/european xor port/reserved/.initial=.6}
\ctikzset{tripoles/european xor port/input height/.initial=.6}
\ctikzset{tripoles/european nand port/width/.initial=1.4}
\ctikzset{tripoles/european nand port/not height/.initial=.3}
\ctikzset{tripoles/european nand port/not width/.initial=.8}
\ctikzset{tripoles/european nand port/height/.initial=.65}
\ctikzset{tripoles/european nand port/reserved/.initial=.6}
\ctikzset{tripoles/european nand port/input height/.initial=.6}
\ctikzset{tripoles/european not port/width/.initial=1.4}
\ctikzset{tripoles/european not port/not height/.initial=.3}
\ctikzset{tripoles/european not port/not width/.initial=.8}
\ctikzset{tripoles/european not port/height/.initial=.65}
\ctikzset{tripoles/european not port/reserved/.initial=.6}
\ctikzset{tripoles/european not port/input height/.initial=0}
\ctikzset{tripoles/european xnor port/width/.initial=1.4}
\ctikzset{tripoles/european xnor port/not height/.initial=.3}
\ctikzset{tripoles/european xnor port/not width/.initial=.8}
\ctikzset{tripoles/european xnor port/height/.initial=.65}
\ctikzset{tripoles/european xnor port/reserved/.initial=.6}
\ctikzset{tripoles/european xnor port/input height/.initial=.6}
\ctikzset{tripoles/european nor port/width/.initial=1.4}
\ctikzset{tripoles/european nor port/not height/.initial=.3}
\ctikzset{tripoles/european nor port/not width/.initial=.8}
\ctikzset{tripoles/european nor port/height/.initial=.65}
\ctikzset{tripoles/european nor port/reserved/.initial=.6}
\ctikzset{tripoles/european nor port/input height/.initial=.6}
% variable number of inputs
\ctikzset{tripoles/european and port/origin/.initial=0.8}
\ctikzset{tripoles/european and port/inputs/.initial=2}
\ctikzset{tripoles/european nand port/origin/.initial=0.8}
\ctikzset{tripoles/european nand port/inputs/.initial=2}
\ctikzset{tripoles/european or port/origin/.initial=0.8}
\ctikzset{tripoles/european or port/inputs/.initial=2}
\ctikzset{tripoles/european nor port/origin/.initial=0.8}
\ctikzset{tripoles/european nor port/inputs/.initial=2}
\ctikzset{tripoles/european xor port/origin/.initial=0.8}
\ctikzset{tripoles/european xor port/inputs/.initial=2}
\ctikzset{tripoles/european xnor port/origin/.initial=0.8}
\ctikzset{tripoles/european xnor port/inputs/.initial=2}
\ctikzset{tripoles/european not port/origin/.initial=0.8}
\ctikzset{tripoles/european not port/inputs/.initial=1}%
%%% parameters that are not used anymore after multi-input
%%% gates --- left for compatibility of source code.
\ctikzset{tripoles/american xor port/aaa/.initial=.6}
\ctikzset{tripoles/american xor port/bbb/.initial=.4}
\ctikzset{tripoles/american xor port/ccc/.initial=.5}
\ctikzset{tripoles/american xor port/ddd/.initial=.0}
\ctikzset{tripoles/american xnor port/aaa/.initial=.6}
\ctikzset{tripoles/american xnor port/bbb/.initial=.4}
\ctikzset{tripoles/american xnor port/ccc/.initial=.5}
\ctikzset{tripoles/american xnor port/ddd/.initial=.0}
% switches for logic gates
%
\pgfkeys{/tikz/number inputs/.initial=0}
\pgfkeys{/tikz/number inputs/.default=0}
%
% switches for op amps
% changing input polarity
%
\newif\ifpgf@circuit@oa@iplusup\pgf@circuit@oa@iplusupfalse
\pgfkeys{/tikz/noinv input up/.add code={}{\pgf@circuit@oa@iplusuptrue}}
\ctikzset{noinv input up/.add code={}{\pgf@circuit@oa@iplusuptrue}}
\pgfkeys{/tikz/input noinv down/.add code={}{\pgf@circuit@oa@iplusupfalse}}
\ctikzset{input noinv down/.add code={}{\pgf@circuit@oa@iplusupfalse}}
%
% changing output polarity (for fully diff objects)
%
\newif\ifpgf@circuit@oa@oplusup\pgf@circuit@oa@oplusuptrue
\pgfkeys{/tikz/noinv output up/.add code={}{\pgf@circuit@oa@oplusuptrue}}
\ctikzset{noinv output up/.add code={}{\pgf@circuit@oa@oplusuptrue}}
\pgfkeys{/tikz/noinv output down/.add code={}{\pgf@circuit@oa@oplusupfalse}}
\ctikzset{noinv output down/.add code={}{\pgf@circuit@oa@oplusupfalse}}
%
\ctikzset{tripoles/op amp/width/.initial=1.7}
\ctikzset{tripoles/op amp/port width/.initial=.7}
\ctikzset{tripoles/op amp/height/.initial=1.4}
\ctikzset{tripoles/op amp/input height/.initial=.5}
\ctikzset{tripoles/op amp/up pos/.initial=.45}
\ctikzset{tripoles/op amp/font/.initial= \fontsize{10}{12}\selectfont\boldmath}%absolute font size needed!
\ctikzset{tripoles/en amp/width/.initial=1.7}
\ctikzset{tripoles/en amp/port width/.initial=.7}
\ctikzset{tripoles/en amp/height/.initial=1.6}
\ctikzset{tripoles/en amp/input height/.initial=.3}
\ctikzset{tripoles/en amp/up pos/.initial=.45}
\ctikzset{tripoles/en amp/font/.initial= \fontsize{10}{12}\selectfont}%absolute font size needed!
\ctikzset{tripoles/en amp/font2/.initial= \fontsize{12}{14}\selectfont}%absolute font size needed!
\ctikzset{tripoles/en amp/text/.initial={$\mathstrut{\triangleright}\,{\infty}$}}
\tikzset{
    en amp text/.code = {
        \ctikzsetvalof{tripoles/en amp/text}{#1}
    },
    en amp text A/.code = {
        \ctikzsetvalof{tripoles/en amp/text}{$\mathstrut{\triangleright}\,\mathrm{A}$}
    },
}
\ctikzset{tripoles/gm amp/width/.initial=1.7}
\ctikzset{tripoles/gm amp/port width/.initial=.7}
\ctikzset{tripoles/gm amp/height/.initial=1.4}
\ctikzset{tripoles/gm amp/input height/.initial=.5}
\ctikzset{tripoles/gm amp/up pos/.initial=.45}
\ctikzset{tripoles/inst amp/width/.initial=1.7} % instrumentation amplifier, simple
\ctikzset{tripoles/inst amp/port width/.initial=.7}
\ctikzset{tripoles/inst amp/height/.initial=1.4}
\ctikzset{tripoles/inst amp/input height/.initial=.5}
\ctikzset{tripoles/inst amp/up pos/.initial=.4}
\ctikzset{tripoles/inst amp/refv pos/.initial=.7}
\ctikzset{tripoles/inst amp/font/.initial= \fontsize{10}{0}\selectfont\boldmath}%absolute font size needed!
\ctikzset{tripoles/fd inst amp/width/.initial=1.7} % instrumentation amplifier, diff output
\ctikzset{tripoles/fd inst amp/port width/.initial=.7}
\ctikzset{tripoles/fd inst amp/height/.initial=1.4}
\ctikzset{tripoles/fd inst amp/input height/.initial=.5}
\ctikzset{tripoles/fd inst amp/up pos/.initial=.4}
\ctikzset{tripoles/fd inst amp/refv pos/.initial=.7}
\ctikzset{tripoles/fd inst amp/font/.initial= \fontsize{10}{0}\selectfont\boldmath}%absolute font size needed!
\ctikzset{tripoles/inst amp ra/width/.initial=2.4} % instrumentation amplifier with ra gain resistance added
\ctikzset{tripoles/inst amp ra/port width/.initial=.7}
\ctikzset{tripoles/inst amp ra/height/.initial=2.9}
\ctikzset{tripoles/inst amp ra/input height/.initial=.7}
\ctikzset{tripoles/inst amp ra/up pos/.initial=.4}
\ctikzset{tripoles/inst amp ra/refv pos/.initial=.7}
\ctikzset{tripoles/inst amp ra/ra pos/.initial=.6}
\ctikzset{tripoles/inst amp ra/font/.initial= \fontsize{10}{0}\selectfont\boldmath}%absolute font size needed!
\ctikzset{tripoles/plain amp/width/.initial=1.7}
\ctikzset{tripoles/plain amp/port width/.initial=.7}
\ctikzset{tripoles/plain amp/height/.initial=1.4}
\ctikzset{tripoles/plain amp/input height/.initial=.5}
\ctikzset{tripoles/plain amp/up pos/.initial=.45}

\ctikzset{tripoles/thyristor/height/.initial=1.10}
\ctikzset{tripoles/thyristor/height 2/.initial=.5}
\ctikzset{tripoles/thyristor/width/.initial=1.0}
\ctikzset{tripoles/thyristor/diode height/.initial=.5}
\ctikzset{tripoles/thyristor/diode width left/.initial=.4}
\ctikzset{tripoles/thyristor/diode width right/.initial=.3}

\ctikzset{tripoles/triac/height/.initial=1.1}
\ctikzset{tripoles/triac/width/.initial=1}
\ctikzset{tripoles/triac/diode width left/.initial=.3}
\ctikzset{tripoles/triac/diode width right/.initial=.3}

%% Cute switches
\ctikzset{bipoles/cuteswitch/height/.initial=.6}
\ctikzset{bipoles/cuteswitch/height 2/.initial=.2}
\ctikzset{bipoles/cuteswitch/width/.initial=.50}
\ctikzset{bipoles/cuteswitch/thickness/.initial=1}

\ctikzset{tripoles/spdt/width/.initial=.85}
\ctikzset{tripoles/spdt/height/.initial=.45}
\ctikzset{tripoles/spdt/margin/.initial=.45}

\ctikzset{tripoles/toggleswitch/height/.initial=.8}
\ctikzset{tripoles/toggleswitch/height 2/.initial=.0}
\ctikzset{tripoles/toggleswitch/width/.initial=.80}

\ctikzset{tripoles/mixer/width/.initial=0.7}
\ctikzset{tripoles/adder/width/.initial=0.7}
\ctikzset{tripoles/circulator/width/.initial=.7}
\ctikzset{tripoles/oscillator/width/.initial=.7}


\ctikzset{tripoles/wilkinson/height/.initial=1.3}
\ctikzset{tripoles/wilkinson/width/.initial=1.3}

\ctikzset{quadpoles/transformer/width/.initial=1.5}
\ctikzset{quadpoles/transformer/width1/.initial=.4}
\ctikzset{quadpoles/transformer/height/.initial=1.5}
\ctikzset{quadpoles/transformer/height1/.initial=.8}
\ctikzset{quadpoles/transformer core/width/.initial=1.5}
\ctikzset{quadpoles/transformer core/height/.initial=1.5}
\ctikzset{quadpoles/transformer core/core height/.initial=.5}
\ctikzset{quadpoles/transformer core/core width/.initial=.05}
\ctikzset{quadpoles/gyrator/width/.initial=1.5}
\ctikzset{quadpoles/gyrator/height/.initial=1.5}
\ctikzset{quadpoles/fourport/width/.initial=1.3}
\ctikzset{quadpoles/fourport/height/.initial=1.3}
\ctikzset{quadpoles/coupler/width/.initial=1.3}
\ctikzset{quadpoles/coupler/height/.initial=1.3}
\ctikzset{quadpoles/coupler2/width/.initial=1.3}
\ctikzset{quadpoles/coupler2/height/.initial=1.3}

\ctikzset{/tikz/circuitikz/tripoles/magnetron/width/.initial=1}

%
% multipoles
%
\ctikzset{multipoles/thickness/.initial=2}
\ctikzset{multipoles/font/.initial=\tiny}
% DIP (dual in line package) chips
\ctikzset{multipoles/dipchip/width/.initial=1.2}
\ctikzset{multipoles/dipchip/num pins/.initial=8}
\ctikzset{multipoles/dipchip/pin spacing/.initial=0.4}
\pgfkeys{/tikz/num pins/.add code={}{\ctikzset{multipoles/dipchip/num pins=#1}}}
% QFP (quad flat package) chips
\ctikzset{multipoles/qfpchip/num pins/.initial=8}
\ctikzset{multipoles/qfpchip/pin spacing/.initial=0.4}
\pgfkeys{/tikz/num pins/.add code={}{\ctikzset{multipoles/qfpchip/num pins=#1}}}
% chip numbers
\newif\ifpgf@circuit@chip@shownumbers\pgf@circuit@chip@shownumberstrue
\pgfkeys{/tikz/show numbers/.add code={}{\pgf@circuit@chip@shownumberstrue}}
\ctikzset{show numbers/.add code={}{\pgf@circuit@chip@shownumberstrue}}
\pgfkeys{/tikz/hide numbers/.add code={}{\pgf@circuit@chip@shownumbersfalse}}
\ctikzset{hide numbers/.add code={}{\pgf@circuit@chip@shownumbersfalse}}
\newif\ifpgf@circuit@chip@straightnumbers\pgf@circuit@chip@straightnumberstrue
\pgfkeys{/tikz/straight numbers/.add code={}{\pgf@circuit@chip@straightnumberstrue}}
\ctikzset{straight numbers/.add code={}{\pgf@circuit@chip@straightnumberstrue}}
\pgfkeys{/tikz/rotated numbers/.add code={}{\pgf@circuit@chip@straightnumbersfalse}}
\ctikzset{rotated numbers/.add code={}{\pgf@circuit@chip@straightnumbersfalse}}
% external chip pins
\ctikzset{multipoles/external pins thickness/.initial=1}
\ctikzset{multipoles/external pins width/.initial=0.2}
\ctikzset{multipoles/external pad fraction/.initial=0}
\pgfkeys{/tikz/external pins width/.add code={}{\ctikzset{multipoles/external pins width=#1}}}
\pgfkeys{/tikz/external pad fraction/.add code={}{\ctikzset{multipoles/external pad fraction=#1}}}
% topmarks
\newif\ifpgf@circuit@chip@topmark\pgf@circuit@chip@topmarktrue
\pgfkeys{/tikz/topmark/.add code={}{\pgf@circuit@chip@topmarktrue}}
\ctikzset{topmark/.add code={}{\pgf@circuit@chip@topmarktrue}}
\pgfkeys{/tikz/no topmark/.add code={}{\pgf@circuit@chip@topmarkfalse}}
\ctikzset{no topmark/.add code={}{\pgf@circuit@chip@topmarkfalse}}



% %Mechanical section
\ctikzset{/tikz/circuitikz/tripoles/elmech/height/.initial=.8}
\ctikzset{/tikz/circuitikz/tripoles/elmech/width/.initial=.6}
\ctikzset{bipoles/spring/height/.initial=.5}
\ctikzset{bipoles/spring/width/.initial=.5}
\ctikzset{bipoles/mass/height/.initial=.55}
\ctikzset{bipoles/mass/box height/.initial=.4}
\ctikzset{bipoles/mass/width/.initial=.5}

\ctikzset{bipoles/damper/height/.initial=.35}
\ctikzset{bipoles/damper/length/.initial=.3}
\ctikzset{bipoles/damper/width/.initial=.4}


\ctikzset{bipole/.is family}
\ctikzset{bipole/kind/.initial = }
\ctikzset{bipole/name/.initial = }
\newif\ifpgf@circuit@bipole@isvoltage
\ctikzset{bipole/is voltage/.is if=pgf@circuit@bipole@isvoltage}
\newif\ifpgf@circuit@bipole@voltageoutsideofsymbol
\ctikzset{bipole/is voltageoutsideofsymbol/.is if=pgf@circuit@bipole@voltageoutsideofsymbol}
\newif\ifpgf@circuit@bipole@strokedsymbol
\ctikzset{bipole/is strokedsymbol/.is if=pgf@circuit@bipole@strokedsymbol}
\newif\ifpgf@circuit@bipole@iscurrent
\ctikzset{bipole/is current/.is if=pgf@circuit@bipole@iscurrent}

\ctikzset{bipole/voltage/.is family}
\newif\ifpgf@circuit@bipole@voltage@backward
\ctikzset{bipole/voltage/direction/.is choice}
\ctikzset{bipole/voltage/direction/forward/.code={\pgf@circuit@bipole@voltage@backwardfalse}}
\ctikzset{bipole/voltage/direction/backward/.code={\pgf@circuit@bipole@voltage@backwardtrue}}
\newif\ifpgf@circuit@bipole@voltage@below
\ctikzset{bipole/voltage/position/.is choice}
\ctikzset{bipole/voltage/position/above/.code={\pgf@circuit@bipole@voltage@belowfalse}}
\ctikzset{bipole/voltage/position/below/.code={\pgf@circuit@bipole@voltage@belowtrue}}

\ctikzset{bipole/voltage/label/unit/.initial=}
\ctikzset{bipole/voltage/label/name/.initial=}

\ctikzset{bipole/current/.is family}
\newif\ifpgf@circuit@bipole@current@backward
\ctikzset{bipole/current/direction/.is choice}
\ctikzset{bipole/current/direction/forward/.code={\pgf@circuit@bipole@current@backwardfalse}}
\ctikzset{bipole/current/direction/backward/.code={\pgf@circuit@bipole@current@backwardtrue}}
\newif\ifpgf@circuit@bipole@current@before
\ctikzset{bipole/current/x position/.is choice}
\ctikzset{bipole/current/x position/after/.code={\pgf@circuit@bipole@current@beforefalse}}
\ctikzset{bipole/current/x position/before/.code={\pgf@circuit@bipole@current@beforetrue}}
\newif\ifpgf@circuit@bipole@current@below
\ctikzset{bipole/current/y position/.is choice}
\ctikzset{bipole/current/y position/above/.code={\pgf@circuit@bipole@current@belowfalse}}
\ctikzset{bipole/current/y position/below/.code={\pgf@circuit@bipole@current@belowtrue}}
\ctikzset{bipole/current/label/unit/.initial=}
\ctikzset{bipole/current/label/name/.initial=}

\ctikzset{bipole/flow/.is family}
\newif\ifpgf@circuit@bipole@flow@backward
\ctikzset{bipole/flow/direction/.is choice}
\ctikzset{bipole/flow/direction/forward/.code={\pgf@circuit@bipole@flow@backwardfalse}}
\ctikzset{bipole/flow/direction/backward/.code={\pgf@circuit@bipole@flow@backwardtrue}}
\newif\ifpgf@circuit@bipole@flow@before
\ctikzset{bipole/flow/x position/.is choice}
\ctikzset{bipole/flow/x position/after/.code={\pgf@circuit@bipole@flow@beforefalse}}
\ctikzset{bipole/flow/x position/before/.code={\pgf@circuit@bipole@flow@beforetrue}}
\newif\ifpgf@circuit@bipole@flow@below
\ctikzset{bipole/flow/y position/.is choice}
\ctikzset{bipole/flow/y position/above/.code={\pgf@circuit@bipole@flow@belowfalse}}
\ctikzset{bipole/flow/y position/below/.code={\pgf@circuit@bipole@flow@belowtrue}}
\ctikzset{bipole/flow/label/unit/.initial=}
\ctikzset{bipole/flow/label/name/.initial=}
\ctikzset{flow/distance/.initial = .5}
\ctikzset{flow/offset/.initial = .2}%distance between flow-arrow and conductor


\ctikzset{bipole/label/.is family}
\ctikzset{bipole/label/position/.initial=90}
\ctikzset{bipole/label/unit/.initial=}
\ctikzset{bipole/label/name/.initial=}
\ctikzset{bipole/annotation/.is family}
\ctikzset{bipole/annotation/position/.initial=-90}
\ctikzset{bipole/annotation/unit/.initial=}
\ctikzset{bipole/annotation/name/.initial=}
\ctikzset{bipole/nodes/.is family}
\ctikzset{bipole/nodes/left/.is choice}
\ctikzset{bipole/nodes/left/none/.code={\ctikzsetvalof{bipole/nodes/left}{none}}}
\ctikzset{bipole/nodes/left/empty/.code={\ctikzsetvalof{bipole/nodes/left}{empty}}}
\ctikzset{bipole/nodes/left/full/.code={\ctikzsetvalof{bipole/nodes/left}{full}}}
\ctikzset{bipole/nodes/left/diamond/.code={\ctikzsetvalof{bipole/nodes/left}{diamond}}}
\ctikzset{bipole/nodes/left/rectjoinfill/.code={\ctikzsetvalof{bipole/nodes/left}{rectjoinfill}}}
\ctikzset{bipole/nodes/right/.is choice}
\ctikzset{bipole/nodes/right/none/.code={\ctikzsetvalof{bipole/nodes/right}{none}}}
\ctikzset{bipole/nodes/right/empty/.code={\ctikzsetvalof{bipole/nodes/right}{empty}}}
\ctikzset{bipole/nodes/right/full/.code={\ctikzsetvalof{bipole/nodes/right}{full}}}
\ctikzset{bipole/nodes/right/diamond/.code={\ctikzsetvalof{bipole/nodes/right}{diamond}}}
\ctikzset{bipole/nodes/right/rectjoinfill/.code={\ctikzsetvalof{bipole/nodes/right}{rectjoinfill}}}

\newif\ifpgf@circuit@europeanresistor
\ctikzset{resistor/.is choice}
\ctikzset{resistor/american/.code = \pgf@circuit@europeanresistorfalse }
\ctikzset{resistor/european/.code = \pgf@circuit@europeanresistortrue }

\ctikzset{inductor/.is choice}
\ctikzset{inductor/cute/.code={\ctikzsetvalof{inductor}{cute}}}
\ctikzset{inductor/european/.code={\ctikzsetvalof{inductor}{european}}}
\ctikzset{inductor/american/.code={\ctikzsetvalof{inductor}{american}}}

\newif\ifpgf@circuit@strokediode
\newif\ifpgf@circuit@fulldiode
\pgf@circuit@strokediodefalse
\pgf@circuit@fulldiodefalse

\ctikzset{diode/.is choice}
\ctikzset{diode/empty/.code = \pgf@circuit@fulldiodefalse\pgf@circuit@strokediodefalse}%default
\ctikzset{diode/full/.code = \pgf@circuit@fulldiodetrue }
\ctikzset{diode/stroke/.code = \pgf@circuit@strokediodetrue}

\tikzset{full diodes/.style = { \circuitikzbasekey/diode = full }}
\tikzset{empty diodes/.style = { \circuitikzbasekey/diode = empty }}
\tikzset{stroke diodes/.style = { \circuitikzbasekey/diode = stroke }}

\ctikzset{thickness/.initial=2}
\ctikzset{color/.initial=black}
\pgfkeys{/tikz/color/.add code={}{\ctikzset{color={#1}}}}

\newif\ifpgf@circ@siunitx
\newif\ifpgf@circ@siunitx@res

\ctikzset{straight/.is choice}
\ctikzset{straightvoltage value/.initial=true}
\ctikzset{straight/true/.code = {\pgf@circuit@bipole@voltage@straighttrue}}
\ctikzset{straight/false/.code = {\pgf@circuit@bipole@voltage@straightfalse}}
\ctikzset{straightvoltage/.style = {/tikz/circuitikz/straight=true}}
\newif\ifpgf@circuit@bipole@voltage@straight
\ctikzset{bipole/straight/.is if=pgf@circuit@bipole@voltage@straight}


\ctikzset{voltage/.is family}
\ctikzset{voltage/distance from node/.initial=.5} %\pgf@circ@Rlen units
\ctikzset{voltage/distance from line/.initial=.08} % pos, tra 0 e 1
\ctikzset{voltage/bump a/.initial=1.2}
\ctikzset{voltage/bump b/.initial=1.5}
\ctikzset{voltage/shift/.initial=0.0} % shift form the cable of voltage symbols
\ctikzset{voltage shift/.style={voltage/shift=#1}}
\tikzset{voltage shift/.style={\circuitikzbasekey/voltage/shift=#1}}
\ctikzset{voltage/european label distance/.initial=1.4}
\ctikzset{voltage/american label distance/.initial=1.1}
% shaping the +/- sign, see pgfcircvoltage.tex
\ctikzset{voltage/american font/.initial={}}
\ctikzset{voltage/american plus/.initial={$+$}}
\ctikzset{voltage/american minus/.initial={$-$}}

% special cases
\ctikzset{bipoles/generic/voltage/distance from node/.initial=.4}
\ctikzset{bipoles/generic/voltage/bump b/.initial=2}
\ctikzset{bipoles/generic/voltage/european label distance/.initial=1.8}
%\ctikzset{bipoles/thermocouple/voltage/distance from node/.initial=.3}
\ctikzset{bipoles/thermocouple/voltage/bump b/.initial=2.2}
\ctikzset{bipoles/thermocouple/voltage/european label distance/.initial=1.5}
\ctikzset{bipoles/ageneric/voltage/distance from node/.initial=.4}
\ctikzset{bipoles/ageneric/voltage/bump b/.initial=2}
\ctikzset{bipoles/ageneric/voltage/european label distance/.initial=1.8}
\ctikzset{bipoles/fullgeneric/voltage/distance from node/.initial=.4}
\ctikzset{bipoles/fullgeneric/voltage/bump b/.initial=2}
\ctikzset{bipoles/fullgeneric/voltage/european label distance/.initial=1.8}
\ctikzset{bipoles/memristor/voltage/distance from node/.initial=.4}
\ctikzset{bipoles/memristor/voltage/bump b/.initial=2}
\ctikzset{bipoles/memristor/voltage/european label distance/.initial=1.8}
%\ctikzset{bipoles/tline/voltage/distance from node/.initial=.2}
\ctikzset{bipoles/tline/voltage/bump b/.initial=2.4}
\ctikzset{bipoles/tline/voltage/european label distance/.initial=2.1}
%\ctikzset{bipoles/varistor/voltage/distance from node/.initial=.2}
\ctikzset{bipoles/varistor/voltage/bump b/.initial=2.4}
\ctikzset{bipoles/varistor/voltage/european label distance/.initial=2}
%\ctikzset{bipoles/photoresistor/voltage/distance from node/.initial=.2}
\ctikzset{bipoles/photoresistor/voltage/bump b/.initial=2}
\ctikzset{bipoles/photoresistor/voltage/european label distance/.initial=1.8}
%\ctikzset{bipoles/thermistor/voltage/distance from node/.initial=.2}
\ctikzset{bipoles/thermistor/voltage/bump b/.initial=2.4}
\ctikzset{bipoles/thermistor/voltage/european label distance/.initial=2}
%\ctikzset{bipoles/thermistorntc/voltage/distance from node/.initial=.2}
\ctikzset{bipoles/thermistorntc/voltage/bump b/.initial=1.6}
%\ctikzset{bipoles/thermistorptc/voltage/distance from node/.initial=.2}
\ctikzset{bipoles/thermistorptc/voltage/bump b/.initial=1.6}

\ctikzset{current/.is family}
\ctikzset{current/distance/.initial = .5}


\tikzset{american currents/.style = { \circuitikzbasekey/current = american } }
\tikzset{european currents/.style = { \circuitikzbasekey/current = european } }
\tikzset{american voltages/.style = { \circuitikzbasekey/voltage = american } }
\tikzset{european voltages/.style = { \circuitikzbasekey/voltage = european } }
\tikzset{american resistors/.style = { \circuitikzbasekey/resistor = american } }
\tikzset{european resistors/.style = { \circuitikzbasekey/resistor = european } }

\newif\ifpgf@circuit@europeangfsurgearrester
\ctikzset{gas filled surge arrester choice/.is choice}
\ctikzset{gas filled surge arrester choice/european/.code= {\pgf@circuit@europeangfsurgearrestertrue } }
\ctikzset{gas filled surge arrester choice/american/.code= {\pgf@circuit@europeangfsurgearresterfalse } }

\tikzset{american gas filled surge arrester set/.style = { \circuitikzbasekey/gas filled surge arrester choice=american } }
\tikzset{european gas filled surge arrester set/.style = { \circuitikzbasekey/gas filled surge arrester choice=european } }
\tikzset{american inductors/.style = { \circuitikzbasekey/inductor = american } }
\tikzset{european inductors/.style = { \circuitikzbasekey/inductor = european } }
\tikzset{cute inductors/.style = { \circuitikzbasekey/inductor = cute } }
\tikzset{american ports/.style = { \circuitikzbasekey/logic ports = american } }
\tikzset{european ports/.style = { \circuitikzbasekey/logic ports = european } }
\tikzset{european/.style = { european currents, european voltages, european resistors, european inductors, european ports, european gas filled surge arrester set} }
\tikzset{american/.style = { american currents, american voltages, american resistors, american inductors, american ports, american gas filled surge arrester set} }
\tikzset{cute/.style = { european currents, european voltages, american resistors, cute inductors, american ports } }

% I should try to make the tree clearer (this voltage conflicts with the options above)

\newif\ifpgf@circuit@europeanvoltage
\ctikzset{voltage/.is choice}
\ctikzset{voltage/american/.code = {\pgf@circuit@europeanvoltagefalse } }
\ctikzset{voltage/european/.code = {\pgf@circuit@europeanvoltagetrue } }

\newif\ifpgf@circuit@europeancurrent
\ctikzset{current/.is choice}
\ctikzset{current/american/.code = \pgf@circuit@europeancurrentfalse }
\ctikzset{current/european/.code = \pgf@circuit@europeancurrenttrue }

% noise sources
\ctikzset{bipoles/noise sources/fillcolor/.initial=gray!50}

\ctikzset{label/align/.is choice}
\ctikzset{label/align/straight/.code={\ctikzsetvalof{label/align}{straight}}}
\ctikzset{label/align/rotate/.code={\ctikzsetvalof{label/align}{rotate}}}
\ctikzset{label/align/smart/.code={\ctikzsetvalof{label/align}{smart}}}

%%%%%%%%%% new
\pgfkeys{\circuitikzbasekey/.search also={/tikz}}


==> pgfcircbipoles.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the files gpl-3.0_license.txt and lppl-1-3c_license.txt for more details.

%% Generic macro for defining a bipole shape
% #1 - additional anchors
% #2 - lower y-size of the bipole (from the center).
% #3 - #shape is the name of the shape
% #4 - upper y-size of the bipole (from the center)
% #5 - width of the bipole
% #6 - macros drawing the bipole


\long\def\pgfcircdeclarebipole#1#2#3#4#5#6{
    \pgfdeclareshape{#3shape}{

        \savedanchor{\northeast}{
            \pgf@y=#4\pgf@circ@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=#5\pgf@circ@Rlen
            \pgf@x=.5\pgf@x
        }
        \savedanchor{\northeastborder}{
            \pgf@y=#4\pgf@circ@Rlen
            \pgf@y=.5\pgf@y
            \pgf@y=\ctikzvalof{bipoles/border margin}\pgf@y
            \pgf@x=#5\pgf@circ@Rlen
            \pgf@x=.5\pgf@x
            \pgf@x=\ctikzvalof{bipoles/border margin}\pgf@x
        }
        \savedanchor{\southwestborder}{
            \pgf@y=-#2\pgf@circ@Rlen
            \pgf@y=.5\pgf@y
            \pgf@y=\ctikzvalof{bipoles/border margin}\pgf@y
            \pgf@x=-#5\pgf@circ@Rlen
            \pgf@x=.5\pgf@x
            \pgf@x=\ctikzvalof{bipoles/border margin}\pgf@x
        }
        \savedanchor{\southwest}{
            \pgf@y=-#2\pgf@circ@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=-#5\pgf@circ@Rlen
            \pgf@x=.5\pgf@x
        }
        \savedanchor{\centerpoint}{
            \pgf@circ@res@down=-#2\pgf@circ@Rlen
            \pgf@circ@res@up=#4\pgf@circ@Rlen
            \pgfpointorigin
            \pgf@y=\pgf@circ@res@up
            \advance\pgf@y by\pgf@circ@res@down
            \pgf@y=.5\pgf@y
        }
        \anchor{center}{\pgfpointorigin}
        \anchor{n}{
            \northeast
            \pgf@x=0cm
        }
        \anchor{north east}{
            \northeast
        }
        \anchor{north west}{
            \northeast
            \pgf@x=-\pgf@x
        }
        \anchor{ne}{
            \northeast
        }
        \anchor{nw}{
            \northeast
            \pgf@x=-\pgf@x
        }
        \anchor{e}{
            \northeast
            \pgf@y=0cm
        }
        \anchor{s}{
            \southwest
            \pgf@x=0cm
        }
        \anchor{south east}{
            \southwest
            \pgf@x=-\pgf@x
        }
        \anchor{south west}{
            \southwest
        }
        \anchor{se}{
            \southwest
            \pgf@x=-\pgf@x
        }
        \anchor{sw}{
            \southwest
        }
        \anchor{w}{
            \southwest
            \pgf@y=0cm
        }
        \anchor{north}{
            \northeast
            \pgf@x=0cm
        }
        \anchor{east}{
            \northeast
            \pgf@y=0cm
        }
        \anchor{south}{
            \southwest
            \pgf@x=0cm
        }
        \anchor{west}{
            \southwest
            \pgf@y=0cm
        }
        \anchor{right}{
            \northeast
            \pgf@y=0cm
        }
        \anchor{above}{
            \northeast
            \pgf@x=0cm
        }
        \anchor{left}{
            \southwest
            \pgf@y=0cm
        }
        \anchor{below}{
            \southwest
            \pgf@x=0cm
        }
        \anchor{a}{
            \northeast
            \pgf@y=0cm
        }
        \anchor{b}{
            \southwest
            \pgf@y=0cm
        }
        \savedanchor{\textanchor}{%
            \pgf@y=\ht\pgfnodeparttextbox
            \pgf@x=-.5\wd\pgfnodeparttextbox
        }
        \anchor{text}{
            \textanchor
        }
        \anchorborder{%
            \ifpgf@circuit@bipole@inverted
                \pgf@circ@res@left=-\pgf@x
                \pgf@circ@res@right=-\pgf@y
            \else
                \pgf@circ@res@left=\pgf@x
                \pgf@circ@res@right=\pgf@y
            \fi
            \ifdim\pgf@circ@res@right>0cm
                \pgfpointborderrectangle{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@right}}{\northeastborder}
            \else
                \southwestborder
                \pgfpointborderrectangle{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@right}}{\pgfpoint{-\pgf@x}{-\pgf@y}}
            \fi
        }

        #1

        \backgroundpath{
            \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

            \northeast
            \pgf@circ@res@up = \pgf@y
            \pgf@circ@res@zero = 0cm
            \pgf@circ@res@left = -\pgf@x
            \pgf@circ@res@right = \pgf@x
            \southwest
            \pgf@circ@res@down = \pgf@y

            \pgfstartlinewidth=\pgflinewidth
            \pgfsetcornersarced{\pgfpointorigin}% do not use rounded corners!
            #6

            \pgfsetlinewidth{\pgfstartlinewidth}
        }
    }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Standard bipole shapes declarations

%% Resistor
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/resistor/height}}
{resistor}
{\ctikzvalof{bipoles/resistor/height}}
{\ctikzvalof{bipoles/resistor/width}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgftransformationadjustments
    \pgfmathsetlength{\pgf@circ@res@step}{\ctikzvalof{bipoles/resistor/width}\pgf@circ@Rlen+\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}
    \divide \pgf@circ@res@step by 12

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@up}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@up}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@up}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
    \advance\pgf@circ@res@other by \pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@zero}}
    \pgfsetbeveljoin
    \pgfusepath{draw}
}



%% Variable resistor
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/vresistor/height}}
{vresistor}
{\ctikzvalof{bipoles/vresistor/height}}
{\ctikzvalof{bipoles/vresistor/width}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgftransformationadjustments
    \pgfmathsetlength{\pgf@circ@res@step}{\ctikzvalof{bipoles/resistor/width}\pgf@circ@Rlen+\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}
    \divide \pgf@circ@res@step by 12

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{\pgf@circ@res@zero}}

    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@up}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@down}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@up}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@down}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@up}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@down}}
    \advance\pgf@circ@res@other by \pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@zero}}
    \pgfsetbeveljoin
    \pgfusepath{draw}

    \pgfscope
        \pgfsetarrowsend{latexslim}
        \pgfpathmoveto{\pgfpoint{.4\pgf@circ@res@other}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{-.4\pgf@circ@res@other}{\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}



%% Capacitor

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/capacitor/height}}
{capacitor}
{\ctikzvalof{bipoles/capacitor/height}}
{\ctikzvalof{bipoles/capacitor/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/capacitor/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 5

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfusepath{draw}

}

%% Capacitive sensor
\pgfcircdeclarebipole
{\anchor{label}{%
        \southwest
        \pgf@x=2.6\pgf@x
        \pgf@y=1.4\pgf@y
    }%
}
{\ctikzvalof{bipoles/capacitor/height}}
{capacitivesens}
{\ctikzvalof{bipoles/capacitor/height}}
{\ctikzvalof{bipoles/capacitor/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/capacitor/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 5

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfusepath{draw}
    \pgfscope
        \pgfpathmoveto{\pgfpoint{2.6\pgf@circ@res@right}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{-2.6\pgf@circ@res@right}{1.4\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{-4.4\pgf@circ@res@right}{1.4\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Polar Capacitor

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/pcapacitor/height}}
{polarcapacitor}
{\ctikzvalof{bipoles/pcapacitor/height}}
{\ctikzvalof{bipoles/pcapacitor/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/pcapacitor/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 5

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgfscope
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left+ \ctikzvalof{bipoles/pcapacitor/bend width}\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgftransformrotate{-90}
        \pgfpathsine{\pgfpoint{\pgf@circ@res@up}{-\ctikzvalof{bipoles/pcapacitor/bend width}\pgf@circ@res@left}}
        \pgfpathcosine{\pgfpoint{\pgf@circ@res@up}{\ctikzvalof{bipoles/pcapacitor/bend width}\pgf@circ@res@left}}
        \pgfusepath{draw}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfusepath{draw}

}

%% Electrolytic Capacitor

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/ecapacitor/height}}
{ecapacitor}
{\ctikzvalof{bipoles/ecapacitor/height}}
{\ctikzvalof{bipoles/ecapacitor/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/ecapacitor/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 5
    \pgfsetrectcap
    % % % Draw plus pole
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgf@circ@draworfill
    % % Draw minus pole
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfsetfillcolor{black}
    \pgfusepath{draw,fill}
    \pgfsetfillcolor{black}
    % % plus pole annotation
    \pgftext[right,at=\pgfpoint{1.2\pgf@circ@res@left}{.6\pgf@circ@res@up}]
    {\pgfkeysvalueof{/tikz/circuitikz/bipoles/ecapacitor/font} $+$}
}

%% Battery

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/battery/height}}
{battery}
{\ctikzvalof{bipoles/battery/height}}
{\ctikzvalof{bipoles/battery/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/battery/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 6

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \ifpgf@circ@fixbatteries
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{.5\pgf@circ@res@down}}

        \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@step}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{-\pgf@circ@res@step}{\pgf@circ@res@down}}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{.5\pgf@circ@res@down}}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \else
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}

        \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@step}{.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{-\pgf@circ@res@step}{.5\pgf@circ@res@down}}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@down}}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{.5\pgf@circ@res@down}}
    \fi
    \pgfusepath{draw}
}


%% Battery 1 % poles with equl thickness

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/battery1/height}}
{battery1}
{\ctikzvalof{bipoles/battery1/height}}
{\ctikzvalof{bipoles/battery1/width}}
{
    \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@right}{0}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0}}
    \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@left}{0}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \ifpgf@circ@fixbatteries
        \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@right}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.33\pgf@circ@res@right}{\pgf@circ@res@down}}

        \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@left}{.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.33\pgf@circ@res@left}{.5\pgf@circ@res@down}}
    \else
        \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@right}{.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.33\pgf@circ@res@right}{.5\pgf@circ@res@down}}

        \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.33\pgf@circ@res@left}{\pgf@circ@res@down}}
    \fi
    \pgfusepath{draw}
}

%% Battery 2 % negative pole thicker

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/battery2/height}}
{battery2}
{\ctikzvalof{bipoles/battery2/height}}
{\ctikzvalof{bipoles/battery2/width}}
{
    \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@right}{0}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0}}
    \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@left}{0}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \ifpgf@circ@fixbatteries
        \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@right}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.33\pgf@circ@res@right}{\pgf@circ@res@down}}
        \pgfusepath{draw}
        \pgfsetlinewidth{3\pgflinewidth}
        \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@left}{.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.33\pgf@circ@res@left}{.5\pgf@circ@res@down}}
    \else
        \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.33\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfusepath{draw}
        \pgfsetlinewidth{3\pgflinewidth}
        \pgfpathmoveto{\pgfpoint{.33\pgf@circ@res@right}{.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.33\pgf@circ@res@right}{.5\pgf@circ@res@down}}
    \fi
    \pgfusepath{draw}
}


%% cute inductor

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/cuteinductor/lower coil height}}
{cuteinductor}
{\ctikzvalof{bipoles/cuteinductor/height}}
{\ctikzvalof{bipoles/cuteinductor/width}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgftransformationadjustments

    \pgfmathsetlength{\pgf@circ@res@other}%width of small coil
    {0.5*\ctikzvalof{bipoles/cuteinductor/coil aspect}*\ctikzvalof{bipoles/cuteinductor/width}*\pgf@circ@Rlen/(\ctikzvalof{bipoles/cuteinductor/coils}-1)}


    \pgfmathsetlength{\pgf@circ@res@step}
    {(\ctikzvalof{bipoles/cuteinductor/width}*\pgf@circ@Rlen+\pgfhorizontaltransformationadjustment\pgflinewidth+(\ctikzvalof{bipoles/cuteinductor/coils}-1)*2*\pgf@circ@res@other)/\ctikzvalof{bipoles/cuteinductor/coils}/2}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth}}%correct value would be 0.5 but arcs are not really flat, therefore 0.4 is better is (almost) all cases
    \foreach \x in {2,...,\ctikzvalof{bipoles/cuteinductor/coils}}
    {
        \pgfpatharc{180}{0}{\pgf@circ@res@step and \pgf@circ@res@up}
        \pgfpatharc{0}{-180}{\pgf@circ@res@other and -\pgf@circ@res@down}
    }
    \pgfpatharc{180}{0}{\pgf@circ@res@step and \pgf@circ@res@up}
    \pgfsetbuttcap
    \pgfsetbeveljoin
    \pgfusepath{stroke}
}

%% cute inductive sensor

\pgfcircdeclarebipole
{%
{% anchor for labelling the type of dependency
    \anchor{label}{%
        \southwest
        \pgf@x=0.8\pgf@x
        \pgf@y=2.6\pgf@y
    }%
}}
{\ctikzvalof{bipoles/cuteinductor/lower coil height}}
{scuteinductor}
{\ctikzvalof{bipoles/cuteinductor/height}}
{\ctikzvalof{bipoles/cuteinductor/width}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgftransformationadjustments

    \pgfmathsetlength{\pgf@circ@res@other}%width of small coil
    {0.5*\ctikzvalof{bipoles/cuteinductor/coil aspect}*\ctikzvalof{bipoles/cuteinductor/width}*\pgf@circ@Rlen/(\ctikzvalof{bipoles/cuteinductor/coils}-1)}


    \pgfmathsetlength{\pgf@circ@res@step}
    {(\ctikzvalof{bipoles/cuteinductor/width}*\pgf@circ@Rlen+\pgfhorizontaltransformationadjustment\pgflinewidth+(\ctikzvalof{bipoles/cuteinductor/coils}-1)*2*\pgf@circ@res@other)/\ctikzvalof{bipoles/cuteinductor/coils}/2}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth}}%correct value would be 0.5 but arcs are not really flat, therefore 0.4 is better is (almost) all cases
    \foreach \x in {2,...,\ctikzvalof{bipoles/cuteinductor/coils}}
    {
        \pgfpatharc{180}{0}{\pgf@circ@res@step and \pgf@circ@res@up}
        \pgfpatharc{0}{-180}{\pgf@circ@res@other and -\pgf@circ@res@down}
    }
    \pgfpatharc{180}{0}{\pgf@circ@res@step and \pgf@circ@res@up}
    \pgfsetbuttcap
    \pgfsetbeveljoin
    \pgfusepath{stroke}
    \pgfscope
        \pgfpathmoveto{\pgfpoint{.8\pgf@circ@res@right}{2\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{-.8\pgf@circ@res@right}{2.6\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{-1.6\pgf@circ@res@right}{2.6\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}

%% cute choke

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/cutechoke/lower coil height}}
{cutechoke}
{\ctikzvalof{bipoles/cutechoke/height}}
{\ctikzvalof{bipoles/cutechoke/width}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgftransformationadjustments

    \pgfmathsetlength{\pgf@circ@res@other}%width of small coil
    {0.5*\ctikzvalof{bipoles/cutechoke/coil aspect}*\ctikzvalof{bipoles/cutechoke/width}*\pgf@circ@Rlen/(\ctikzvalof{bipoles/cutechoke/coils}-1)}


    \pgfmathsetlength{\pgf@circ@res@step}
    {(\ctikzvalof{bipoles/cutechoke/width}*\pgf@circ@Rlen+\pgfhorizontaltransformationadjustment\pgflinewidth+(\ctikzvalof{bipoles/cutechoke/coils}-1)*2*\pgf@circ@res@other)/\ctikzvalof{bipoles/cutechoke/coils}/2}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth}}%correct value would be 0.5 but arcs are not really flat, therefore 0.4 is better is (almost) all cases
    \foreach \x in {2,...,\ctikzvalof{bipoles/cutechoke/coils}}
    {
        \pgfpatharc{180}{0}{\pgf@circ@res@step and \pgf@circ@res@up}
        \pgfpatharc{0}{-180}{\pgf@circ@res@other and -\pgf@circ@res@down}
    }
    \pgfpatharc{180}{0}{\pgf@circ@res@step and \pgf@circ@res@up}
    \pgfsetbuttcap
    \pgfsetbeveljoin
    \pgfusepath{stroke}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth+\ctikzvalof{bipoles/cutechoke/cdist}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth+\ctikzvalof{bipoles/cutechoke/cdist}\pgf@circ@res@up}}
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}*\ctikzvalof{bipoles/cutechoke/cthick}\pgfstartlinewidth}
    \pgfusepath{stroke}

    \ifpgf@circuit@bipole@twolines
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth+\ctikzvalof{bipoles/cutechoke/cdist}\pgf@circ@res@up+\ctikzvalof{bipoles/cutechoke/cstep}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth+\ctikzvalof{bipoles/cutechoke/cdist}\pgf@circ@res@up+\ctikzvalof{bipoles/cutechoke/cstep}\pgf@circ@res@up}}
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}*\ctikzvalof{bipoles/cutechoke/cthick}\pgfstartlinewidth}
        \pgfusepath{stroke}
    \fi
}

%% variable cute inductor

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/vcuteinductor/lower coil height}}
{vcuteinductor}
{\ctikzvalof{bipoles/vcuteinductor/height}}
{\ctikzvalof{bipoles/vcuteinductor/width}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgftransformationadjustments

    \pgfmathsetlength{\pgf@circ@res@other}%width of small coil
    {0.5*\ctikzvalof{bipoles/vcuteinductor/coil aspect}*\ctikzvalof{bipoles/vcuteinductor/width}*\pgf@circ@Rlen/(\ctikzvalof{bipoles/vcuteinductor/coils}-1)}


    \pgfmathsetlength{\pgf@circ@res@step}
    {(\ctikzvalof{bipoles/vcuteinductor/width}*\pgf@circ@Rlen+\pgfhorizontaltransformationadjustment\pgflinewidth+(\ctikzvalof{bipoles/vcuteinductor/coils}-1)*2*\pgf@circ@res@other)/\ctikzvalof{bipoles/vcuteinductor/coils}/2}

    \pgfscope
        \pgfsetarrowsend{latexslim}
        \pgfpathmoveto{\pgfpoint{.4\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@right}{\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth}}%correct value would be 0.5 but arcs are not really flat, therefore 0.4 is better is (almost) all cases
    \foreach \x in {2,...,\ctikzvalof{bipoles/vcuteinductor/coils}}
    {
        \pgfpatharc{180}{0}{\pgf@circ@res@step and .5\pgf@circ@res@up}
        \pgfpatharc{0}{-180}{\pgf@circ@res@other and -.5\pgf@circ@res@down}
    }
    \pgfpatharc{180}{0}{\pgf@circ@res@step and .5\pgf@circ@res@up}
    \pgfsetbuttcap
    \pgfsetbeveljoin
    \pgfusepath{stroke}
}
%% american inductor

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/americaninductor/height 2}}
{americaninductor}
{\ctikzvalof{bipoles/americaninductor/height}}
{\ctikzvalof{bipoles/americaninductor/width}}
{
    \pgf@circ@res@step=\ctikzvalof{bipoles/americaninductor/width}\pgf@circ@Rlen
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgftransformationadjustments
    \advance \pgf@circ@res@step by \pgfhorizontaltransformationadjustment\pgflinewidth
    \divide \pgf@circ@res@step by \ctikzvalof{bipoles/americaninductor/coils}
    \divide \pgf@circ@res@step by 2
    \pgf@circ@res@other = \ctikzvalof{bipoles/americaninductor/coil height}\pgf@circ@Rlen

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth}}%correct value would be 0.5 but arcs are not really flat, therefore 0.4 is better is (almost) all cases
    \foreach \x in {1,...,\ctikzvalof{bipoles/americaninductor/coils}}
    {
        \pgfpatharc{180}{0}{\pgf@circ@res@step and  \pgf@circ@res@other}
    }
    \pgfsetbuttcap
    \pgfsetbeveljoin
    \pgfusepath{stroke}
}


%% american inductive sensor

\pgfcircdeclarebipole
{%
{% anchor for labelling the type of dependency
    \anchor{label}{%
        \southwest
        \pgf@x=0.8\pgf@x
        \pgf@y=2.6\pgf@y
    }%
}}
{\ctikzvalof{bipoles/americaninductor/height 2}}
{samericaninductor}
{\ctikzvalof{bipoles/americaninductor/height}}
{\ctikzvalof{bipoles/americaninductor/width}}
{
    \pgf@circ@res@step=\ctikzvalof{bipoles/americaninductor/width}\pgf@circ@Rlen
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgftransformationadjustments
    \advance \pgf@circ@res@step by \pgfhorizontaltransformationadjustment\pgflinewidth
    \divide \pgf@circ@res@step by \ctikzvalof{bipoles/americaninductor/coils}
    \divide \pgf@circ@res@step by 2
    \pgf@circ@res@other = \ctikzvalof{bipoles/americaninductor/coil height}\pgf@circ@Rlen

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth}}%correct value would be 0.5 but arcs are not really flat, therefore 0.4 is better is (almost) all cases
    \foreach \x in {1,...,\ctikzvalof{bipoles/americaninductor/coils}}
    {
        \pgfpatharc{180}{0}{\pgf@circ@res@step and  \pgf@circ@res@other}
    }
    \pgfsetbuttcap
    \pgfsetbeveljoin
    \pgfusepath{stroke}
    \pgfscope
        \pgfpathmoveto{\pgfpoint{.8\pgf@circ@res@right}{2\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{-.8\pgf@circ@res@right}{2.6\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{-1.6\pgf@circ@res@right}{2.6\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}

%% variable american inductor

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/vamericaninductor/height 2}}
{vamericaninductor}
{\ctikzvalof{bipoles/vamericaninductor/height}}
{\ctikzvalof{bipoles/vamericaninductor/width}}
{
    \pgf@circ@res@step=\ctikzvalof{bipoles/vamericaninductor/width}\pgf@circ@Rlen
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgftransformationadjustments
    \advance \pgf@circ@res@step by \pgfhorizontaltransformationadjustment\pgflinewidth
    \divide \pgf@circ@res@step by \ctikzvalof{bipoles/vamericaninductor/coils}
    \divide \pgf@circ@res@step by 2
    \pgf@circ@res@other = \ctikzvalof{bipoles/vamericaninductor/coil height}\pgf@circ@Rlen

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{-\pgfverticaltransformationadjustment*0.4*\pgfstartlinewidth}}%correct value would be 0.5 but arcs are not really flat, therefore 0.4 is better is (almost) all cases
    \foreach \x in {1,...,\ctikzvalof{bipoles/vamericaninductor/coils}}
    {
        \pgfpatharc{180}{0}{\pgf@circ@res@step and  \pgf@circ@res@other}
    }
    \pgfsetbuttcap
    \pgfsetbeveljoin
    \pgfusepath{stroke}

    \pgfscope
        \pgfsetarrowsend{latexslim}
        \pgfpathmoveto{\pgfpoint{.4\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{-.4\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}


%% Independent voltage source

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/vsource/height}}
{vsource}
{\ctikzvalof{bipoles/vsource/height}}
{\ctikzvalof{bipoles/vsource/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfusepath{draw}
}


%% Independent voltage source - American style

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/vsourceam/height}}
{vsourceAM}
{\ctikzvalof{bipoles/vsourceam/height}}
{\ctikzvalof{bipoles/vsourceam/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill
    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
    \ifpgf@circ@oldvoltagedirection
        \pgftext[bottom,rotate=90,y=\ctikzvalof{bipoles/vsourceam/margin}\pgf@circ@res@down]{$+$}
        \pgftext[top,rotate=90,y=\ctikzvalof{bipoles/vsourceam/margin}\pgf@circ@res@up]{$-$}
    \else
        \pgftext[bottom,rotate=90,y=\ctikzvalof{bipoles/vsourceam/margin}\pgf@circ@res@down]{$-$}
        \pgftext[top,rotate=90,y=\ctikzvalof{bipoles/vsourceam/margin}\pgf@circ@res@up]{$+$}
    \fi
}



%% Independent sinusoidal voltage source

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/vsourcesin/height}}
{vsourcesin}
{\ctikzvalof{bipoles/vsourcesin/height}}
{\ctikzvalof{bipoles/vsourcesin/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill

    \pgf@circ@res@up = .5\pgf@circ@res@up
    \pgfscope
        \pgftransformrotate{90}
        \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@up}{0cm}}
        \pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
        \pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}

% Square Voltage source -  contributed by Alistair Kwan
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/vsourcesquare/height}}
{vsourcesquare}
{\ctikzvalof{bipoles/vsourcesquare/height}}
{\ctikzvalof{bipoles/vsourcesquare/width}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill
    \pgf@circ@res@up = .5\pgf@circ@res@up
    \pgfscope
        \pgftransformrotate{90}
        \pgfpathmoveto{\pgfpoint{-1\pgf@circ@res@up}{0cm}}
        \pgfpathlineto{\pgfpoint{-1\pgf@circ@res@up}{1\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0\pgf@circ@res@up}{1\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0\pgf@circ@res@up}{-1\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{1\pgf@circ@res@up}{-1\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{1\pgf@circ@res@up}{0\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}

% Triangle Voltage source - contributed by Ralf Farkas
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/vsourcetri/height}}
{vsourcetri}
{\ctikzvalof{bipoles/vsourcetri/height}}
{\ctikzvalof{bipoles/vsourcetri/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill

    \pgf@circ@res@up = .5\pgf@circ@res@up
    \pgfscope
        \pgftransformrotate{90}
        \pgfpathmoveto{\pgfpoint{-1\pgf@circ@res@up}{0cm}}
        \pgfpathlineto{\pgfpoint{-0.5\pgf@circ@res@up}{0.75\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@up}{-0.75\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{1\pgf@circ@res@up}{0\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}


%% PV Source
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/pvsource/height}}
{pvsource}
{\ctikzvalof{bipoles/pvsource/height}}
{\ctikzvalof{bipoles/pvsource/width}}
{
    \pgfpointorigin
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@up}}
    \pgf@circ@draworfill

    \pgfpathmoveto{\pgfpoint{.15\pgf@circ@res@right}{0}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0}}
    \pgfpathmoveto{\pgfpoint{.15\pgf@circ@res@left}{0}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{.15\pgf@circ@res@left}{.4\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.15\pgf@circ@res@left}{.4\pgf@circ@res@down}}

    \pgfpathmoveto{\pgfpoint{.15\pgf@circ@res@right}{.6\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.15\pgf@circ@res@right}{.6\pgf@circ@res@down}}
    \pgfusepath{draw}

    %Arrow Part
    \pgfscope
        \pgfsetarrowsend{latex}
        \pgfpathmoveto{\pgfpointadd{\pgfpoint{.3\pgf@circ@res@left}{0}}{\pgfpointpolar{-45}{2.2\pgf@circ@res@up}}}
        \pgfpathlineto{\pgfpointadd{\pgfpoint{.3\pgf@circ@res@left}{0}}{\pgfpointpolar{-45}{1.3\pgf@circ@res@up}}}
        \pgfusepath{draw}
        \pgfpathmoveto{\pgfpointadd{\pgfpoint{0}{0.3\pgf@circ@res@up}}{\pgfpointpolar{-45}{2.2\pgf@circ@res@up}}}
        \pgfpathlineto{\pgfpointadd{\pgfpoint{0}{0.3\pgf@circ@res@up}}{\pgfpointpolar{-45}{1.3\pgf@circ@res@up}}}
        \pgfusepath{draw}
    \endpgfscope

}

%% Empty Source
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/esource/height}}
{esource}
{\ctikzvalof{bipoles/esource/height}}
{\ctikzvalof{bipoles/esource/width}}
{
    \pgfpointorigin
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill
}

%% DC Current Source with open shape
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/dcisource/height}}
{dcisource}
{\ctikzvalof{bipoles/dcisource/height}}
{\ctikzvalof{bipoles/dcisource/width}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@maybefill
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0}}\pgfpatharc{0}{90}{0.85\pgf@circ@res@right and \pgf@circ@res@up}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0}}\pgfpatharc{0}{-90}{0.85\pgf@circ@res@right and \pgf@circ@res@up}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0}}\pgfpatharc{180}{270}{0.85\pgf@circ@res@right and \pgf@circ@res@up}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0}}\pgfpatharc{180}{90}{0.85\pgf@circ@res@right and \pgf@circ@res@up}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{.7\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfusepath{draw}
    \pgfscope
        \pgftransformshift{\pgfpoint{.5\pgf@circ@res@right}{\pgf@circ@res@zero}}
        \pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
    \endpgfscope
}

%% DC-Voltage source
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/dcvsource/height}}
{dcvsource}
{\ctikzvalof{bipoles/dcvsource/height}}
{\ctikzvalof{bipoles/dcvsource/width}}
{
    \pgfpointorigin
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill
    \pgfpathmoveto{\pgfpoint{.2\pgf@circ@res@up}{.5\pgf@circ@res@left}}
    \pgfpathlineto{\pgfpoint{.2\pgf@circ@res@up}{.5\pgf@circ@res@right}}
    \pgfpathmoveto{\pgfpoint{.2\pgf@circ@res@down}{.5\pgf@circ@res@left}}
    \pgfpathlineto{\pgfpoint{.2\pgf@circ@res@down}{.5\pgf@circ@res@right}}
    \pgfusepath{draw}
}


%% Independent current source

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/isource/height}}
{isource}
{\ctikzvalof{bipoles/isource/height}}
{\ctikzvalof{bipoles/isource/width}}
{
    \pgfpointorigin
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@down}}
    \pgf@circ@draworfill
}

%% Independent double oo source

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/oosource/height}}
{oosource}
{\ctikzvalof{bipoles/oosource/height}}
{\ctikzvalof{bipoles/oosource/width}}
{
    \pgfpointorigin
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathcircle{\pgfpoint{\ctikzvalof{bipoles/oosource/circleoffset}\pgf@circ@res@left}{0}}
        {\ctikzvalof{bipoles/oosource/circlesize}\pgf@circ@res@left}
    \pgf@circ@maybefill
    \pgfpathcircle{\pgfpoint{\ctikzvalof{bipoles/oosource/circleoffset}\pgf@circ@res@right}{0}}
        {\ctikzvalof{bipoles/oosource/circlesize}\pgf@circ@res@right}
    \pgf@circ@draworfill
    \pgfpathcircle{\pgfpoint{\ctikzvalof{bipoles/oosource/circleoffset}\pgf@circ@res@left}{0}}
        {\ctikzvalof{bipoles/oosource/circlesize}\pgf@circ@res@left}
    \pgfusepath{draw}
}


%% Independent current source - American

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/isourceam/height}}
{isourceAM}
{\ctikzvalof{bipoles/isourceam/height}}
{\ctikzvalof{bipoles/isourceam/width}}
{
    \pgfpointorigin
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill

    \pgfpathmoveto{\pgfpoint{.7\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfusepath{draw}
    \pgfscope
        \pgftransformshift{\pgfpoint{.5\pgf@circ@res@right}{\pgf@circ@res@zero}}
        \pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
    \endpgfscope
}


%% Independent sinusoidal current source

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/isource/height}}
{isourcesin}
{\ctikzvalof{bipoles/isource/height}}
{\ctikzvalof{bipoles/isource/width}}
{
    \pgfpointorigin
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill

    \pgf@circ@res@up = .5\pgf@circ@res@up
    \pgfscope
        \pgftransformrotate{90}
        \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@up}{0cm}}
        \pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
        \pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope

}


%% Controlled voltage source

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/cvsource/height}}
{cvsource}
{\ctikzvalof{bipoles/cvsource/height}}
{\ctikzvalof{bipoles/cvsource/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
    \pgfpathclose
    \pgf@circ@draworfill

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfusepath{draw}
}




%% Controlled voltage source - American
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/cvsourceam/height}}
{cvsourceAM}
{\ctikzvalof{bipoles/cvsourceam/height}}
{\ctikzvalof{bipoles/cvsourceam/width}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
    \pgfpathclose
    \pgf@circ@draworfill

    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
    \ifpgf@circ@oldvoltagedirection
        \pgftext[bottom,rotate=90,y=\ctikzvalof{bipoles/cvsourceam/margin}\pgf@circ@res@left]{$+$}
        \pgftext[top,rotate=90,y=\ctikzvalof{bipoles/cvsourceam/margin}\pgf@circ@res@right]{$-$}
    \else
        \pgftext[bottom,rotate=90,y=\ctikzvalof{bipoles/cvsourceam/margin}\pgf@circ@res@left]{$-$}
        \pgftext[top,rotate=90,y=\ctikzvalof{bipoles/cvsourceam/margin}\pgf@circ@res@right]{$+$}
    \fi
}


%% Controlled sinusoidal voltage source
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/cvsourcesin/height}}
{cvsourcesin}
{\ctikzvalof{bipoles/cvsourcesin/height}}
{\ctikzvalof{bipoles/cvsourcesin/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgfscope
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
        \pgfpathclose
        \pgf@circ@draworfill
    \endpgfscope

    \pgf@circ@res@up = .5\pgf@circ@res@up
    \pgfscope
        \pgftransformrotate{90}
        \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@up}{0cm}}
        \pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
        \pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}



%% Controlled sinusoidal current source

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/cvsourcesin/height}}
{cisourcesin}
{\ctikzvalof{bipoles/cvsourcesin/height}}
{\ctikzvalof{bipoles/cvsourcesin/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgfscope
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
        \pgfpathclose
        \pgf@circ@draworfill
    \endpgfscope

    \pgf@circ@res@up = .5\pgf@circ@res@up
    \pgfscope
        \pgftransformrotate{90}
        \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@up}{0cm}}
        \pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
        \pgfpathsine{\pgfpoint{.5\pgf@circ@res@up}{-.5\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Controlled current source

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/cisource/height}}
{cisource}
{\ctikzvalof{bipoles/cisource/height}}
{\ctikzvalof{bipoles/cisource/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
    \pgfpathclose
    \pgf@circ@draworfill

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
    \pgfusepath{draw}
}


%% Controlled current source - American

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/cisourceam/height}}
{cisourceAM}
{\ctikzvalof{bipoles/cisourceam/height}}
{\ctikzvalof{bipoles/cisourceam/width}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
    \pgfpathclose
    \pgf@circ@draworfill
    \pgfpathmoveto{\pgfpoint{.7\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfusepath{draw}
    \pgfscope
        \pgftransformshift{\pgfpoint{.5\pgf@circ@res@right}{\pgf@circ@res@zero}}
        \pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
    \endpgfscope
}

%% Cute Independent voltage source

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/vsource/height}}
{vsourceC}
{\ctikzvalof{bipoles/vsource/height}}
{\ctikzvalof{bipoles/vsource/width}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill
    \pgfmathsetmacro{\@@thicker}{3*\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}}
    \pgfsetlinewidth{\@@thicker\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfsetroundcap\pgfusepath{draw}
}
%% Cute Independent current source

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/isource/height}}
{isourceC}
{\ctikzvalof{bipoles/isource/height}}
{\ctikzvalof{bipoles/isource/width}}
{
    \pgfpointorigin
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill
    \pgfmathsetmacro{\@@thicker}{3*\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}}
    \pgfsetlinewidth{\@@thicker\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{.6\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{.6\pgf@circ@res@down}}
    \pgfsetroundcap\pgfusepath{draw}
}
%% Cute Controlled voltage source

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/cvsource/height}}
{cvsourceC}
{\ctikzvalof{bipoles/cvsource/height}}
{\ctikzvalof{bipoles/cvsource/width}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@draworfill
    \pgfmathsetmacro{\@@thicker}{3*\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}}
    \pgfsetlinewidth{\@@thicker\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfsetroundcap\pgfusepath{draw}
}

%% Cute Controlled current source

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/cisource/height}}
{cisourceC}
{\ctikzvalof{bipoles/cisource/height}}
{\ctikzvalof{bipoles/cisource/width}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@draworfill
    \pgfmathsetmacro{\@@thicker}{3*\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}}
    \pgfsetlinewidth{\@@thicker\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@zero}{.6\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@zero}{.6\pgf@circ@res@down}}
    \pgfsetroundcap\pgfusepath{draw}
}

%%  Noise voltage source

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/vsource/height}}
{vsourceN}
{\ctikzvalof{bipoles/vsource/height}}
{\ctikzvalof{bipoles/vsource/width}}
{
    \pgfscope
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
        \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
        %
        \pgf@circ@res@step=0.125\pgf@circ@Rlen\relax
        \edef\pgf@noise@temp{dashed}
        \edef\pgf@noise@fill{\pgfkeysvalueof{/tikz/circuitikz/bipoles/noise sources/fillcolor}}
        \ifx\pgf@noise@temp\pgf@noise@fill
            % fillable in this case
            \pgf@circ@draworfillandclip
            \pgfmathsetmacro{\thinner}{.5*\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}}
            \pgfsetlinewidth{\thinner\pgfstartlinewidth}
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \advance\pgf@circ@res@up by \pgf@circ@res@step\advance\pgf@circ@res@down by \pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \advance\pgf@circ@res@up by \pgf@circ@res@step\advance\pgf@circ@res@down by \pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \advance\pgf@circ@res@up by \pgf@circ@res@step\advance\pgf@circ@res@down by \pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            %
            \advance\pgf@circ@res@up by -4\pgf@circ@res@step \advance\pgf@circ@res@down by -4\pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \advance\pgf@circ@res@up by -\pgf@circ@res@step\advance\pgf@circ@res@down by -\pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \advance\pgf@circ@res@up by -\pgf@circ@res@step\advance\pgf@circ@res@down by -\pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \pgfusepath{draw}
        \else
            \pgfsetfillcolor{\pgf@noise@fill}
            \pgfusepath{draw,fill}
        \fi
    \endpgfscope
    \pgfmathsetmacro{\@@thicker}{3*\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}}
    \pgfsetlinewidth{\@@thicker\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfsetroundcap\pgfusepath{draw}
}
%% Noise current source

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/isource/height}}
{isourceN}
{\ctikzvalof{bipoles/isource/height}}
{\ctikzvalof{bipoles/isource/width}}
{
    \pgfpointorigin
    \pgfscope
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
        \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
        %
        \pgf@circ@res@step=0.125\pgf@circ@Rlen\relax
        \edef\pgf@noise@temp{dashed}
        \edef\pgf@noise@fill{\pgfkeysvalueof{/tikz/circuitikz/bipoles/noise sources/fillcolor}}
        \ifx\pgf@noise@temp\pgf@noise@fill
            % fillable in this case
            \pgf@circ@draworfillandclip
            \pgfmathsetmacro{\thinner}{.5*\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}}
            \pgfsetlinewidth{\thinner\pgfstartlinewidth}
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \advance\pgf@circ@res@up by \pgf@circ@res@step\advance\pgf@circ@res@down by \pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \advance\pgf@circ@res@up by \pgf@circ@res@step\advance\pgf@circ@res@down by \pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \advance\pgf@circ@res@up by \pgf@circ@res@step\advance\pgf@circ@res@down by \pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            %
            \advance\pgf@circ@res@up by -4\pgf@circ@res@step \advance\pgf@circ@res@down by -4\pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \advance\pgf@circ@res@up by -\pgf@circ@res@step\advance\pgf@circ@res@down by -\pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \advance\pgf@circ@res@up by -\pgf@circ@res@step\advance\pgf@circ@res@down by -\pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \pgfusepath{draw}
        \else
            \pgfsetfillcolor{\pgf@noise@fill}
            \pgfusepath{draw,fill}
        \fi
    \endpgfscope
    \pgfmathsetmacro{\@@thicker}{3*\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}}
    \pgfsetlinewidth{\@@thicker\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{.6\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{.6\pgf@circ@res@down}}
    \pgfsetroundcap\pgfusepath{draw}
}
%% Black generic diode

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/diode/height}}
{fulldiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgfscope
        \pgftransformxshift{\pgf@circ@res@left}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfusepath{draw,fill}
    \endpgfscope
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% Black Zener diode

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/diode/height}}
{fullzdiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgfscope
        \pgftransformxshift{\pgf@circ@res@left}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfusepath{draw,fill}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Black alternative zigzag Zener diode
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/diode/height}}
{fullzzdiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgfscope
        \pgftransformxshift{\pgf@circ@res@left}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfusepath{draw,fill}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-1.8\pgf@circ@res@left}{\pgf@circ@res@down-0.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-0.2\pgf@circ@res@left}{\pgf@circ@res@up-0.5\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Black Schottky diode

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/diode/height}}
{fullsdiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfscope
        \pgftransformxshift{\pgf@circ@res@left}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfusepath{draw,fill}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{.6\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-1.4\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-1.4\pgf@circ@res@left}{.6\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope

}

%% Black tunnel diode

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/diode/height}}
{fulltdiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfscope
        \pgftransformxshift{\pgf@circ@res@left}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfusepath{draw,fill}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Black light emitting diode

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/diode/height}}
{fulllediode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfscope
        \pgftransformxshift{\pgf@circ@res@left}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfusepath{draw,fill}
    \endpgfscope
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfsetarrowsend{latexslim}
    \pgfpathmoveto{\pgfpoint{-0.4\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{2\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.2\pgf@circ@res@right}{0.8\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{1.2\pgf@circ@res@right}{1.8\pgf@circ@res@up}}
    \pgfusepath{draw}

}

%% Black photodiode

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/diode/height}}
{fullpdiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfscope
        \pgftransformxshift{\pgf@circ@res@left}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfusepath{draw,fill}
    \endpgfscope
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfsetarrowsstart{latexslim}
    \pgfpathmoveto{\pgfpoint{-0.4\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{2\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.2\pgf@circ@res@right}{0.8\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{1.2\pgf@circ@res@right}{1.8\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% Black varcap

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/varcap/height}}
{fullvarcap}
{\ctikzvalof{bipoles/varcap/height}}
{\ctikzvalof{bipoles/varcap/width}}
{
    \pgf@circ@res@temp=\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
    \pgfsetlinewidth{\pgf@circ@res@temp}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{0pt}}
    \pgfusepath{draw,fill}
    %
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{\pgf@circ@res@up}}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% Code for the diode triangle
\def\pgf@circ@basicdiodeshape{
    % \pgfscope
        \pgftransformxshift{\pgf@circ@res@left}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfpathclose
        \pgf@circ@draworfill
        \pgfscope
            % to allow filling, we need to draw explicitily the stroke here.
            \pgfsetlinewidth{\pgfstartlinewidth}
            \ifpgf@circuit@bipole@strokedsymbol
                \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{0pt}}
                \pgfpathlineto{\pgfpoint{0pt}{0pt}}
                \pgfusepath{draw}
            \fi
        \endpgfscope
    % \endpgfscope
}


%% Empty generic diode

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/diode/height}}
{emptydiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfscope
        \pgf@circ@basicdiodeshape
    \endpgfscope
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% Empty Zener diode

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/diode/height}}
{emptyzdiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgfscope
        \pgf@circ@basicdiodeshape
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-0.6\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Empty alternative zigzag Zener diode
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/diode/height}}
{emptyzzdiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgfscope
        \pgf@circ@basicdiodeshape
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-1.8\pgf@circ@res@left}{\pgf@circ@res@down-0.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-0.2\pgf@circ@res@left}{\pgf@circ@res@up-0.5\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}
%% Empty Schottky diode

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/diode/height}}
{emptysdiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfscope
        \pgf@circ@basicdiodeshape
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{.6\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-1.4\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-1.4\pgf@circ@res@left}{.6\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope

}

%% Empty tunnel diode

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/diode/height}}
{emptytdiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfscope
        \pgf@circ@basicdiodeshape
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-.6\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Empty light emitting diode

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/diode/height}}
{emptylediode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfscope
        \pgf@circ@basicdiodeshape
    \endpgfscope
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfsetarrowsend{latexslim}
    \pgfpathmoveto{\pgfpoint{-0.4\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{2\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.2\pgf@circ@res@right}{0.8\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{1.2\pgf@circ@res@right}{1.8\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% Empty photodiode

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/diode/height}}
{emptypdiode}
{\ctikzvalof{bipoles/diode/height}}
{\ctikzvalof{bipoles/diode/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfscope
        \pgf@circ@basicdiodeshape
    \endpgfscope
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfsetarrowsstart{latexslim}
    \pgfpathmoveto{\pgfpoint{-0.4\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{2\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.2\pgf@circ@res@right}{0.8\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{1.2\pgf@circ@res@right}{1.8\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% Empty varcap

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/varcap/height}}
{emptyvarcap}
{\ctikzvalof{bipoles/varcap/height}}
{\ctikzvalof{bipoles/varcap/width}}
{
    \pgf@circ@res@temp=\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
    \pgfsetlinewidth{\pgf@circ@res@temp}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
    % \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{0pt}}
    \pgfpathclose
    \pgf@circ@draworfill
    \pgfscope
        % to allow filling, we need to draw explicitily the stroke here.
        \pgfsetlinewidth{\pgfstartlinewidth}
        \ifpgf@circuit@bipole@strokedsymbol
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{0pt}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfusepath{draw}
        \fi
    \endpgfscope
    %
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-2\pgf@circ@res@temp}{\pgf@circ@res@up}}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% Empty bidirectionaldiode

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/bidirectionaldiode/height}}{emptybidirectionaldiode}{\ctikzvalof{bipoles/bidirectionaldiode/height}}{\ctikzvalof{bipoles/bidirectionaldiode/width}}
{

	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

        \pgf@circ@res@other = \ctikzvalof{bipoles/bidirectionaldiode/diode width left}\pgf@circ@res@left
        \pgf@circ@res@step = \ctikzvalof{bipoles/bidirectionaldiode/diode width right}\pgf@circ@res@right

	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
	\pgfpathlineto{\pgfpoint{0.95\pgf@circ@res@step}{0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}

	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
	\pgfpathlineto{\pgfpoint{0.95\pgf@circ@res@other}{-0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}

        \pgf@circ@draworfill
	% \pgfusepath{draw}

	\pgfsetlinewidth{\pgfstartlinewidth}

	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0pt}}

	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}

	\pgfusepath{draw}

}


%% Full bidirectionaldiode

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/bidirectionaldiode/height}}
{fullbidirectionaldiode}
{\ctikzvalof{bipoles/bidirectionaldiode/height}}
{\ctikzvalof{bipoles/bidirectionaldiode/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgf@circ@res@other = \ctikzvalof{bipoles/bidirectionaldiode/diode width left}\pgf@circ@res@left
    \pgf@circ@res@step = \ctikzvalof{bipoles/bidirectionaldiode/diode width right}\pgf@circ@res@right

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{0.95\pgf@circ@res@step}{0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
    \pgfpathlineto{\pgfpoint{0.95\pgf@circ@res@other}{-0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}

    \pgfusepath{draw, fill}

    \pgfsetlinewidth{\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0pt}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}

    \pgfusepath{draw}

}

%% (Closing) SPST
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/spst/depth}}
{cspst}
{\ctikzvalof{bipoles/spst/height}}
{\ctikzvalof{bipoles/spst/width}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgfscope
        \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathmoveto{\pgfpointpolar{90}{1.2\pgf@circ@res@right}}
        \pgfpatharc{90}{-20}{1.2\pgf@circ@res@right}
        \pgfsetarrowsend{latexslim}
        \pgfsetbeveljoin
        \pgfusepath{draw}
    \endpgfscope
}

%% Opening SPST
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/spst/depth}}
{ospst}
{\ctikzvalof{bipoles/spst/height}}
{\ctikzvalof{bipoles/spst/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgfscope
        \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathmoveto{\pgfpointpolar{-10}{1.2\pgf@circ@res@right}}
        \pgfpatharc{-10}{90}{1.2\pgf@circ@res@right}
        \pgfsetarrowsend{latexslim}
        \pgfsetbeveljoin
        \pgfusepath{draw}
    \endpgfscope
}

%% Normal open Switch
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/nos/depth}}
{nos}
{\ctikzvalof{bipoles/nos/height}}
{\ctikzvalof{bipoles/nos/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{.9\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfsetbuttcap
    \pgfusepath{draw}
}

%% Normal closed Switch
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/ncs/depth}}
{ncs}
{\ctikzvalof{bipoles/ncs/height}}
{\ctikzvalof{bipoles/ncs/width}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{.9\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{.2\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{.2\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% Push Button
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/pushbutton/height 2}}
{pushbutton}
{\ctikzvalof{bipoles/pushbutton/height}}
{\ctikzvalof{bipoles/pushbutton/width}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{.5\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{.5\pgf@circ@res@up}}
    \pgfpathmoveto{\pgfpoint{0}{.5\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0}{\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfnode{ocirc}{center}{}{}{\pgfusepath{draw}}
    \pgftransformshift{\pgfpoint{2\pgf@circ@res@right}{0pt}}
    \pgfnode{ocirc}{center}{}{}{\pgfusepath{draw}}
}

%% Normally closed Push Button
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/pushbutton/height 2}}
{ncpushbutton}
{\ctikzvalof{bipoles/pushbutton/height}}
{\ctikzvalof{bipoles/pushbutton/width}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    % This is the radius of the "ocirc" shape (see pgfcircshapes.tex)
    \pgf@circ@res@temp=\pgfkeysvalueof{/tikz/circuitikz/nodes width}\pgf@circ@Rlen
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{-\pgf@circ@res@temp}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{-\pgf@circ@res@temp}}
    \pgfpathmoveto{\pgfpoint{0}{-\pgf@circ@res@temp}}
    \pgfpathlineto{\pgfpoint{0}{\pgf@circ@res@up}}
    \pgfusepath{draw}
    %
    \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfnode{ocirc}{center}{}{}{\pgfusepath{draw}}
    \pgftransformshift{\pgfpoint{2\pgf@circ@res@right}{0pt}}
    \pgfnode{ocirc}{center}{}{}{\pgfusepath{draw}}
}
% cute switch "to" shapes help function
% #1 -> name
% #2 -> barposition
% #3 -> arrowcode
\long\def\pgfcircdeclarecutesw#1#2#3{
    \pgfcircdeclarebipole
    {
        \savedanchor\midlever{
            % these values are calculated when we create the definition of the shape.
            \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/cuteswitch/height}\pgf@circ@Rlen
            \pgf@circ@res@temp=\pgfkeysvalueof{/tikz/circuitikz/nodes width}\pgf@circ@Rlen
            \pgf@circ@res@temp=\ctikzvalof{bipoles/cuteswitch/thickness}\pgf@circ@res@temp
            \pgf@circ@res@down = -.5\pgf@y
            \pgf@circ@res@up = .5\pgf@y
            \pgfextracty{\pgf@circ@res@other}{#2}
            \pgf@x=0pt
            \pgf@y=.5\pgf@circ@res@other
        }
        % mid of the lever, to stack switches
        \anchor{mid}{\midlever}
        \anchor{out}{\northeast \pgf@y=0cm}
        \anchor{in}{\southwest\pgf@y=0cm}
    }
    {\ctikzvalof{bipoles/cuteswitch/height 2}}
    {#1}
    {\ctikzvalof{bipoles/cuteswitch/height}}
    {\ctikzvalof{bipoles/cuteswitch/width}}{
        \pgfscope
        % This is the radius of the "ocirc" shape (see pgfcircshapes.tex)
        \pgf@circ@res@temp=\pgfkeysvalueof{/tikz/circuitikz/nodes width}\pgf@circ@Rlen
        \pgf@circ@res@temp=\ctikzvalof{bipoles/cuteswitch/thickness}\pgf@circ@res@temp
        \pgfsetlinewidth{2\pgf@circ@res@temp}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{#2}
        \pgfsetroundcap\pgfusepath{draw}
        \endpgfscope
        \pgfscope % arrow
        #3
        \endpgfscope
        \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfnode{ocirc}{center}{}{}{\pgfusepath{draw}}
        \pgftransformshift{\pgfpoint{2\pgf@circ@res@right}{0pt}}
        \pgfnode{ocirc}{center}{}{}{\pgfusepath{draw}}
    }
}

%% closed cute switch
\pgfcircdeclarecutesw{cuteclosedswitch}
    {\pgfpoint{\pgf@circ@res@right}{1.5\pgf@circ@res@temp}}
    {}

%% open cute switch
\pgfcircdeclarecutesw{cuteopenswitch}
    {\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    {}

%% closing cute switch
\pgfcircdeclarecutesw{cuteclosingswitch}
    {\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    {
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}} % in node
    \pgfpathmoveto{\pgfpointpolar{70}{1.2\pgf@circ@res@right}}
    \pgfpatharc{70}{-10}{1.2\pgf@circ@res@right}
    \pgfsetarrowsend{latexslim}
    \pgfusepath{draw}
    }

%% opening cute switch
\pgfcircdeclarecutesw{cuteopeningswitch}
    {\pgfpoint{\pgf@circ@res@right}{1.5\pgf@circ@res@temp}}
    {
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}} % in node
    \pgfpathmoveto{\pgfpointpolar{-10}{1.2\pgf@circ@res@right}}
    \pgfpatharc{-10}{60}{1.2\pgf@circ@res@right}
    \pgfsetarrowsend{latexslim}
    \pgfusepath{draw}
    }


% % METERINGSHAPE
    \long\def\drawmeteringcircle{
        \def\pgf@circ@temp{right}
        \ifx\tikz@res@label@pos\pgf@circ@temp
            \pgf@circ@res@step=-1.2\pgf@circ@res@up
        \else
            \def\pgf@circ@temp{below}
            \ifx\tikz@res@label@pos\pgf@circ@temp
                \pgf@circ@res@step=-1.2\pgf@circ@res@up
            \else
                \pgf@circ@res@step=1.2\pgf@circ@res@up
            \fi
        \fi
        %draw connections to circle
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
        \pgfpathlineto{\pgfpoint{.9\pgf@circ@res@left}{\pgf@circ@res@zero}}
        \pgfpathmoveto{\pgfpoint{.9\pgf@circ@res@right}{\pgf@circ@res@zero}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
        \pgfusepath{draw}
        %draw circle
        \pgfscope
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
            \pgfpathcircle{\pgfpointorigin}{.9\pgf@circ@res@up}
            \pgf@circ@draworfill
        \endpgfscope
        %draw arrow
        \pgfscope
            \pgfsetarrowsend{latex}
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
            \pgfpathlineto{\pgfpoint{-\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfusepath{draw}
        \endpgfscope
    }
%AMPEREMETER
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/ammeter/height}}
{ammeter}
{\ctikzvalof{bipoles/ammeter/height}}
{\ctikzvalof{bipoles/ammeter/width}}
{
    \drawmeteringcircle
    \pgfnode{circle}{center}{\textbf{A}}{}{}
}
%OHMMETER
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/ohmmeter/height}}
{ohmmeter}
{\ctikzvalof{bipoles/ohmmeter/height}}
{\ctikzvalof{bipoles/ohmmeter/width}}
{
    \drawmeteringcircle
    \pgfnode{circle}{center}{\boldmath$\Omega$}{}{}
}
%VOLTMETER
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/voltmeter/height}}
{voltmeter}
{\ctikzvalof{bipoles/voltmeter/height}}
{\ctikzvalof{bipoles/voltmeter/width}}
{
    \drawmeteringcircle
    \pgfnode{circle}{center}{\textbf{V}}{}{}

}

% oscilloscope, suggested by @nobrl https://github.com/circuitikz/circuitikz/issues/176
\pgfcircdeclarebipole
{
    \anchor{in 1}{\southwest\pgf@y=0.75\pgf@y\pgf@x=0.4\pgf@x}
    \anchor{in 2}{\southwest\pgf@y=0.75\pgf@y\pgf@x=-0.4\pgf@x}
    % put the node text above and centered
    \anchor{text}{\pgfextracty{\pgf@circ@res@up}{\northeast}
        \pgfpoint{-.5\wd\pgfnodeparttextbox}{
            \dimexpr.5\dp\pgfnodeparttextbox+.5\ht\pgfnodeparttextbox+\pgf@circ@res@up\relax
        }
    }
}
{\ctikzvalof{bipoles/oscope/height}}
{oscope}
{\ctikzvalof{bipoles/oscope/height}}
{\ctikzvalof{bipoles/oscope/width}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfextracty{\pgf@circ@res@up}{\northeast}
    \pgfextractx{\pgf@circ@res@right}{\northeast}
    \pgfextractx{\pgf@circ@res@left}{\southwest}
    \pgfextracty{\pgf@circ@res@down}{\southwest}
    \pgfmathsetlength{\pgf@circ@res@step}{0.25*\pgf@circ@res@up}
    \pgfscope
        \pgfsetcornersarced{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@step}}
        \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
        % this would create a round (analog?) scope...
        % \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
        \pgf@circ@draworfill
    \endpgfscope
    % get the rotation
    \pgfgettransformentries\a\b\temp\temp\temp\temp
    \pgfmathsetmacro{\rot}{-atan2(\b,\a)}
    % and unrotate the scope
    \pgfscope
        \pgftransformrotate{\rot}
        % grid
        \pgfscope
            \pgfsetlinewidth{0.5\pgfstartlinewidth}
            \pgfpathmoveto{\pgfpoint{0.75\pgf@circ@res@left}{0.25\pgf@circ@res@down}}
            \pgfpathgrid[stepx=\pgf@circ@res@step, stepy=\pgf@circ@res@step]%
            {\pgfpoint{0.75\pgf@circ@res@left}{0.5\pgf@circ@res@down}}
            {\pgfpoint{0.75\pgf@circ@res@right}{0.5\pgf@circ@res@up}}
            \pgfsetstrokeopacity{0.5}
            \pgfusepath{draw}
        \endpgfscope
        % function displayed, thanks to
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
        \pgfpathmoveto{\pgfpoint{0.75\pgf@circ@res@left}{0.25\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{0.05\pgf@circ@res@left}{0.25\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0.05\pgf@circ@res@left}{0.25\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{0.65\pgf@circ@res@right}{0.25\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0.65\pgf@circ@res@right}{0.25\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}
%% Short circuit

%%% NOTICE that the short is really NOT drawn; we trust the fact that its
%%% natural length is zero.
\pgfcircdeclarebipole
{}
{0}
{short}
{0}
{0}
{ }

%% Open circuit

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/open/height}}
{open}
{\ctikzvalof{bipoles/open/height}}
{\ctikzvalof{bipoles/open/width}}
{ }

%% Generic bipole - used as resistor by some (bleah)

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/generic/height}}
{generic}
{\ctikzvalof{bipoles/generic/height}}
{\ctikzvalof{bipoles/generic/width}}
{
    \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgf@circ@draworfill
}


%% fuse

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/fuse/height}}
{fuse}
{\ctikzvalof{bipoles/fuse/height}}
{\ctikzvalof{bipoles/fuse/width}}
{

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0}}
    \pgfusepath{draw}

    \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgf@circ@draworfill
}



%% Generic bipole, filled - used as inductor by some

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/fullgeneric/height}}
{fullgeneric}
{\ctikzvalof{bipoles/fullgeneric/height}}
{\ctikzvalof{bipoles/fullgeneric/width}}
{
    \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgfusepath{draw,fill}
}

%% Generic sensor, filled - used as inductive sensor by some

\pgfcircdeclarebipole
{{% anchor for labelling the type of dependency
    \anchor{label}{%
        \southwest
        \pgf@x=0.4\pgf@x
        \pgf@y=2\pgf@y
    }%
}}
{\ctikzvalof{bipoles/fullgeneric/height}}
{sfullgeneric}
{\ctikzvalof{bipoles/fullgeneric/height}}
{\ctikzvalof{bipoles/fullgeneric/width}}
{

    \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfusepath{draw,fill}
    %\pgfscope
    \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@left}{-2\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{2\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{2\pgf@circ@res@down}}
    \pgfusepath{draw}
    %\endpgfscope
}


%% Generic asymmetric bipole

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/ageneric/height}}
{ageneric}
{\ctikzvalof{bipoles/ageneric/height}}
{\ctikzvalof{bipoles/ageneric/width}}
{
    \pgfscope
        \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
        \pgf@circ@draworfill
    \endpgfscope

    \pgfpathrectanglecorners{\pgfpoint{.7\pgf@circ@res@right}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfusepath{stroke,fill}
}


%% asymmetric fuse

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/afuse/height}}
{afuse}
{\ctikzvalof{bipoles/afuse/height}}
{\ctikzvalof{bipoles/afuse/width}}
{
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0}}
    \pgfusepath{draw}

    \pgfscope
        \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
        \pgf@circ@draworfill
    \endpgfscope

    \pgfpathrectanglecorners{\pgfpoint{.7\pgf@circ@res@right}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfusepath{stroke,fill}
}




%% Memristor

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/memristor/height}}
{memristor}
{\ctikzvalof{bipoles/memristor/height}}
{\ctikzvalof{bipoles/memristor/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/resistor/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 14

    \pgfscope
        \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
        \pgf@circ@draworfill
    \endpgfscope
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{.72*\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{.72*\pgf@circ@res@left}{\ctikzvalof{bipoles/memristor/wave height}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.35*\pgf@circ@res@left}{\ctikzvalof{bipoles/memristor/wave height}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.35*\pgf@circ@res@left}{-\ctikzvalof{bipoles/memristor/wave height}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{-.05*\pgf@circ@res@left}{-\ctikzvalof{bipoles/memristor/wave height}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{-.05*\pgf@circ@res@left}{\ctikzvalof{bipoles/memristor/wave height}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.42*\pgf@circ@res@right}{\ctikzvalof{bipoles/memristor/wave height}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.42*\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{.8*\pgf@circ@res@right}{0pt}}

    \pgfusepath{draw}

    \pgfpathrectanglecorners{\pgfpoint{.7\pgf@circ@res@right}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfusepath{stroke,fill}
}




%% Generic empty tunable

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/tgeneric/height}}
{tgeneric}
{\ctikzvalof{bipoles/tgeneric/height}}
{\ctikzvalof{bipoles/tgeneric/width}}
{
    \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{.4\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{.4\pgf@circ@res@down}}
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgf@circ@draworfill
    \pgfscope
        \pgfsetarrowsend{latexslim}
        \pgfpathmoveto{\pgfpoint{.5\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{-.5\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}

%% Photoresistor

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/photoresistor/height 2}}
{photoresistor}
{\ctikzvalof{bipoles/photoresistor/height}}
{\ctikzvalof{bipoles/photoresistor/width}}
{
    \pgfscope
        \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}{\pgfpoint{\pgf@circ@res@right}{-\pgf@circ@res@down}}
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
        \pgf@circ@draworfill
    \endpgfscope

    \pgfscope
        \pgfsetarrowsend{latexslim}
        \pgfpathmoveto{\pgfpoint{.7\pgf@circ@res@right}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.3\pgf@circ@res@right}{-1.2\pgf@circ@res@down}}
        \pgfusepath{draw}
        \pgfpathmoveto{\pgfpoint{.45\pgf@circ@res@right}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.05\pgf@circ@res@right}{-1.2\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}




%% Thermistor
\pgfcircdeclarebipole
{{% anchor for labelling the type of dependency
    \anchor{label}{%
        \southwest
        \pgf@x=0.4\pgf@x
        \pgf@y=1.2\pgf@y
    }%
}}
{\ctikzvalof{bipoles/thermistor/height}}
{thermistor}
{\ctikzvalof{bipoles/thermistor/height}}
{\ctikzvalof{bipoles/thermistor/width}}
{
    \pgfscope
    \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thermistor/main}\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{-\pgfkeysvalueof{/tikz/circuitikz/bipoles/thermistor/main}\pgf@circ@res@up}}
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgf@circ@draworfill
    \endpgfscope

    %\pgfscope
    \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@left}{-\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{1.2\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{1.2\pgf@circ@res@down}}
    \pgfusepath{draw}
    %\endpgfscope
}


%% Thermistor PTC
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/thermistorptc/height 2}}
{thermistorptc}
{\ctikzvalof{bipoles/thermistorptc/height}}
{\ctikzvalof{bipoles/thermistorptc/width}}
{
    \pgfscope
        \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thermistorptc/main}\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{-\pgfkeysvalueof{/tikz/circuitikz/bipoles/thermistorptc/main}\pgf@circ@res@up}}
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
        \pgf@circ@draworfill
    \endpgfscope
    \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{-\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{-\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgftext[top,x=.85\pgf@circ@res@left,y=.75\pgf@circ@res@down]{\tiny$\vartheta$}
    \pgfsetarrowsend{latexslim}
    \pgfpathmoveto{\pgfpoint{.62\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{.62\pgf@circ@res@left}{.7\pgf@circ@res@down}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{.45\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{.45\pgf@circ@res@left}{.7\pgf@circ@res@down}}
    \pgfusepath{draw}
}

%% Thermistor NTC
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/thermistorntc/height 2}}
{thermistorntc}
{\ctikzvalof{bipoles/thermistorntc/height}}
{\ctikzvalof{bipoles/thermistorntc/width}}
{
    \pgfscope
        \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thermistorntc/main}\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{-\pgfkeysvalueof{/tikz/circuitikz/bipoles/thermistorntc/main}\pgf@circ@res@up}}
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
        \pgf@circ@draworfill
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{-\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{-\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgftext[top,x=.85\pgf@circ@res@left,y=.75\pgf@circ@res@down]{\tiny$\vartheta$}
    \pgfsetarrowsend{latexslim}
    \pgfpathmoveto{\pgfpoint{.62\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{.62\pgf@circ@res@left}{.7\pgf@circ@res@down}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{.45\pgf@circ@res@left}{.7\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{.45\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfusepath{draw}
}

%% thermocouple
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/thermocouple/height 2}}
{thermocouple}
{\ctikzvalof{bipoles/thermocouple/height}}
{\ctikzvalof{bipoles/thermocouple/width}}
{

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{.5\pgf@circ@res@down}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{.5\pgf@circ@res@down}}
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathlineto{\pgfpoint{0}{\pgf@circ@res@down}}
    \pgfusepath{draw}
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{0}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{.5\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0}}
    \pgfusepath{draw}
}

%% Varistor
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/varistor/height}}
{varistor}
{\ctikzvalof{bipoles/varistor/height}}
{\ctikzvalof{bipoles/varistor/width}}
{
    \pgfscope
        \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/bipoles/varistor/main}\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{-\pgfkeysvalueof{/tikz/circuitikz/bipoles/varistor/main}\pgf@circ@res@up}}
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
        \pgf@circ@draworfill
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@left}{-\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfusepath{draw}

    \pgftext[top,x=.65\pgf@circ@res@left,y=1.2\pgf@circ@res@down]{{\tiny\textsf{U}}}
}



%% Generic full tunable

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/tfullgeneric/height}}
{tfullgeneric}
{\ctikzvalof{bipoles/tfullgeneric/height}}
{\ctikzvalof{bipoles/tfullgeneric/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/resistor/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 14

    \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{.4\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{.4\pgf@circ@res@down}}
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfusepath{draw,fill}

    \pgfscope
        \pgfsetarrowsend{latexslim}
        \pgfpathmoveto{\pgfpoint{.5\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{-.5\pgf@circ@res@left}{\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}







%% Variable Capacitor

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/vcapacitor/height}}
{vcapacitor}
{\ctikzvalof{bipoles/vcapacitor/height}}
{\ctikzvalof{bipoles/vcapacitor/width}}
{
    %\pgf@circ@res@step = \ctikzvalof{bipoles/vcapacitor/width}\pgf@circ@Rlen
    \pgf@circ@res@step = \ctikzvalof{bipoles/vcapacitor/capacitor width} \pgf@circ@res@right

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@step}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{-\pgf@circ@res@step}{\pgf@circ@res@down}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@down}}
    \pgfusepath{draw}

    \pgfscope
        \pgfsetarrowsend{latexslim}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{-\pgf@circ@res@step}{0pt}}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{0pt}}
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfusepath{draw}
}


%% Piezoelectric Element

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/piezoelectric/height}}
{piezoelectric}
{\ctikzvalof{bipoles/piezoelectric/height}}
{\ctikzvalof{bipoles/piezoelectric/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/piezoelectric/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 5

    %% Outer markings
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfusepath{draw}

    %% Inner Box
    \pgfscope
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
        \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left+4}{\pgf@circ@res@up-1}}{\pgfpoint{\pgf@circ@res@right-4}{\pgf@circ@res@down+1}}
        \pgf@circ@draworfill
    \endpgfscope
}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Handling of terminals


%% Easily usable styles

\ctikzset{o-o/.style = {\circuitikzbasekey/bipole/nodes/left=empty, \circuitikzbasekey/bipole/nodes/right=empty}}
\ctikzset{-o/.style = {\circuitikzbasekey/bipole/nodes/left=none, \circuitikzbasekey/bipole/nodes/right=empty}}
\ctikzset{o-/.style = {\circuitikzbasekey/bipole/nodes/left=empty, \circuitikzbasekey/bipole/nodes/right=none}}
\ctikzset{*-o/.style = {\circuitikzbasekey/bipole/nodes/left=full, \circuitikzbasekey/bipole/nodes/right=empty}}
\ctikzset{o-*/.style = {\circuitikzbasekey/bipole/nodes/left=empty, \circuitikzbasekey/bipole/nodes/right=full}}
\ctikzset{d-o/.style = {\circuitikzbasekey/bipole/nodes/left=diamond, \circuitikzbasekey/bipole/nodes/right=empty}}
\ctikzset{o-d/.style = {\circuitikzbasekey/bipole/nodes/left=empty, \circuitikzbasekey/bipole/nodes/right=diamond}}
\ctikzset{*-/.style = {\circuitikzbasekey/bipole/nodes/left=full, \circuitikzbasekey/bipole/nodes/right=none}}
\ctikzset{-*/.style = {\circuitikzbasekey/bipole/nodes/left=none, \circuitikzbasekey/bipole/nodes/right=full}}
\ctikzset{d-/.style = {\circuitikzbasekey/bipole/nodes/left=diamond, \circuitikzbasekey/bipole/nodes/right=none}}
\ctikzset{-d/.style = {\circuitikzbasekey/bipole/nodes/left=none, \circuitikzbasekey/bipole/nodes/right=diamond}}
\ctikzset{*-*/.style = {\circuitikzbasekey/bipole/nodes/left=full, \circuitikzbasekey/bipole/nodes/right=full}}
\ctikzset{d-*/.style = {\circuitikzbasekey/bipole/nodes/left=diamond, \circuitikzbasekey/bipole/nodes/right=full}}
\ctikzset{*-d/.style = {\circuitikzbasekey/bipole/nodes/left=full, \circuitikzbasekey/bipole/nodes/right=diamond}}
\ctikzset{d-d/.style = {\circuitikzbasekey/bipole/nodes/left=diamond, \circuitikzbasekey/bipole/nodes/right=diamond}}

\ctikzset{.-/.style = {\circuitikzbasekey/bipole/nodes/left=rectjoinfill, \circuitikzbasekey/bipole/nodes/right=none}}
\ctikzset{.-*/.style = {\circuitikzbasekey/bipole/nodes/left=rectjoinfill, \circuitikzbasekey/bipole/nodes/right=full}}
\ctikzset{.-o/.style = {\circuitikzbasekey/bipole/nodes/left=rectjoinfill, \circuitikzbasekey/bipole/nodes/right=empty}}
\ctikzset{.-d/.style = {\circuitikzbasekey/bipole/nodes/left=rectjoinfill, \circuitikzbasekey/bipole/nodes/right=diamond}}
\ctikzset{-./.style = {\circuitikzbasekey/bipole/nodes/left=none, \circuitikzbasekey/bipole/nodes/right=rectjoinfill}}
\ctikzset{o-./.style = {\circuitikzbasekey/bipole/nodes/left=empty, \circuitikzbasekey/bipole/nodes/right=rectjoinfill}}
\ctikzset{*-./.style = {\circuitikzbasekey/bipole/nodes/left=full, \circuitikzbasekey/bipole/nodes/right=rectjoinfill}}
\ctikzset{d-./.style = {\circuitikzbasekey/bipole/nodes/left=diamond, \circuitikzbasekey/bipole/nodes/right=rectjoinfill}}
\ctikzset{.-./.style = {\circuitikzbasekey/bipole/nodes/left=rectjoinfill, \circuitikzbasekey/bipole/nodes/right=rectjoinfill}}

\tikzset{reversed/.style = {\circuitikzbasekey/bipole/inverted=true}}


%% The output routine

\def\drawpoles{
	\pgfextra{ \edef\pgf@circ@temp{\ctikzvalof{bipole/nodes/left}} \def\pgf@temp{diamond}  }
	\ifx\pgf@temp\pgf@circ@temp
		 (\tikztostart) node[diamondpole] {}
	\else
		\pgfextra{ \def\pgf@temp{empty}  }
		\ifx\pgf@temp\pgf@circ@temp
			 (\tikztostart) node[ocirc] {}
		\else
			\pgfextra{  \def\pgf@temp{full}  }
			\ifx\pgf@temp\pgf@circ@temp
				(\tikztostart) node[circ] {}
			\else
				\pgfextra{ \def\pgf@temp{rectjoinfill} }
				\ifx\pgf@temp\pgf@circ@temp
				 (\tikztostart) node[rectjoinfill] {}
				\else
				\fi
			\fi
		\fi
	\fi
	\pgfextra{ \edef\pgf@circ@temp{\ctikzvalof{bipole/nodes/right}} \def\pgf@temp{diamond}  }
	\ifx\pgf@temp\pgf@circ@temp
		 (\tikztotarget) node[diamondpole] {}
	\else
		\pgfextra{ \def\pgf@temp{empty}  }
		\ifx\pgf@temp\pgf@circ@temp
			 (\tikztotarget) node[ocirc] {}
		\else
			\pgfextra{  \def\pgf@temp{full}  }
			\ifx\pgf@temp\pgf@circ@temp
				(\tikztotarget) node[circ] {}
			\else
				\pgfextra{ \def\pgf@temp{rectjoinfill} }
				\ifx\pgf@temp\pgf@circ@temp
				 (\tikztotarget) node[rectjoinfill] {}
				\else
				\fi
			\fi
		\fi
	\fi
}



%% Lamp

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/lamp/height}}
{lamp}
{\ctikzvalof{bipoles/lamp/height}}
{\ctikzvalof{bipoles/lamp/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill
    \pgfpathmoveto{\pgfpoint{.7071*\pgf@circ@res@left}{.7071*\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.7071*\pgf@circ@res@right}{.7071*\pgf@circ@res@down}}
    \pgfpathmoveto{\pgfpoint{.7071*\pgf@circ@res@left}{.7071*\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{.7071*\pgf@circ@res@right}{.7071*\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% bulb
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/bulb/height}}
{bulb}
{\ctikzvalof{bipoles/bulb/height}}
{\ctikzvalof{bipoles/bulb/width}}
{%
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{0.8\pgf@circ@res@up}}{\pgfpoint{0.8\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{0.4\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpatharc{0}{-180}{0.4*\pgf@circ@res@left}
    \pgfsetbeveljoin
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfusepath{draw}
}


% transmission line

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/tline/height}}
{tline}
{\ctikzvalof{bipoles/tline/height}}
{\ctikzvalof{bipoles/tline/width}}
{
    \pgf@circ@res@step=.2\pgf@circ@res@right % half x axis
    \begin{pgftransparencygroup}
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@step}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left+\pgf@circ@res@step}{\pgf@circ@res@up}}
        \pgfpatharc{-90}{90}{-\pgf@circ@res@step and -\pgf@circ@res@up}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@step}{\pgf@circ@res@down}}
        \pgf@circ@draworfill
        \pgfpathellipse{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@step}{0pt}}
        {\pgfpoint{\pgf@circ@res@step}{0pt}}{\pgfpoint{0pt}{-\pgf@circ@res@up}}
        \pgf@circ@draworfill
    \end{pgftransparencygroup}
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right-\pgf@circ@res@step}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfusepath{stroke}
}

% microstrip transmission line

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/mstline/height}}
{mstline}
{\ctikzvalof{bipoles/mstline/height}}
{\ctikzvalof{bipoles/mstline/width}}
{
    \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfsetlinewidth{\ctikzvalof{bipoles/thickness}\pgfstartlinewidth}
    \pgf@circ@draworfill
}
%% SQUID added by Cor Molenaar 5 March 2010

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/squid/height}}
{squid}
{\ctikzvalof{bipoles/squid/height}}
{\ctikzvalof{bipoles/squid/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgfpathmoveto{\pgfpoint{0.35*\pgf@circ@res@left}{1.35*\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.35*\pgf@circ@res@right}{0.65*\pgf@circ@res@up}}
    \pgfpathmoveto{\pgfpoint{0.35*\pgf@circ@res@left}{0.65*\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.35*\pgf@circ@res@right}{1.35*\pgf@circ@res@up}}
    \pgfpathmoveto{\pgfpoint{0.35*\pgf@circ@res@left}{1.35*\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.35*\pgf@circ@res@right}{0.65*\pgf@circ@res@down}}
    \pgfpathmoveto{\pgfpoint{0.35*\pgf@circ@res@left}{0.65*\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.35*\pgf@circ@res@right}{1.35*\pgf@circ@res@down}}

    \pgfusepath{draw}
}



% Generic barrier added by Cor Molenaar 5 March 2010

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/barrier/height}}
{barrier}
{\ctikzvalof{bipoles/barrier/height}}
{\ctikzvalof{bipoles/barrier/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{0.35*\pgf@circ@res@left}{0.35*\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.35*\pgf@circ@res@right}{0.35*\pgf@circ@res@down}}
    \pgfpathmoveto{\pgfpoint{0.35*\pgf@circ@res@left}{0.35*\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.35*\pgf@circ@res@right}{0.35*\pgf@circ@res@up}}

    \pgfusepath{draw}
}


% Contributed by Danilo Piazzalunga

\pgfdeclareshape{buffer}
{
    \anchor{center}{\pgfpointorigin}
    \savedanchor\northwest{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/buffer/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/bipoles/buffer/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{east}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{west}{ \northwest \pgf@y=0pt }
    \anchor{south}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{north}{ \northwest \pgf@x=0pt }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \savedanchor\left{%
        \pgf@y=0pt
    }
    \anchor{in}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }

    \anchor{text}{\pgfpoint{-.5\wd\pgfnodeparttextbox}{\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox}}

    \backgroundpath{
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}


        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfscope
            \pgfsetlinewidth{2\pgflinewidth}
            \pgftransformxshift{.7\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=.7\pgf@circ@res@step

            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
            \pgfpathclose
            \pgf@circ@draworfill
        \endpgfscope


        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@left}{0pt}}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{0pt}}

        \pgfusepath{draw}

    }
}





\pgfdeclareshape{plain amp}
{
    \anchor{center}{\pgfpointorigin}
    \savedanchor\northwest{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{east}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{west}{ \northwest \pgf@y=0pt }
    \anchor{south}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{north}{ \northwest \pgf@x=0pt }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \savedanchor\left{%
        \pgf@y=0pt
    }
    \savedanchor\inOne{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/input height}\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{-}{
        \inOne
    }
    \anchor{+}{
        \inOne
        \pgf@y=-\pgf@y
    }
    \savedanchor\up{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfpointlineattime{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/up pos}}{
            \pgfpoint{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/port width}\pgf@circ@res@left}
        {\pgf@circ@res@up}}
        {\pgfpoint{.7\pgf@circ@res@right}{0pt}}
    }
    \anchor{up}{
        \up
    }
    \anchor{down}{
        \up
        \pgf@y=-\pgf@y
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }

    \anchor{text}{\pgfpoint{-.5\wd\pgfnodeparttextbox}{\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox}}

    \backgroundpath{
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x

        \pgfscope
            \pgfsetlinewidth{2\pgflinewidth}
            \pgftransformxshift{.7\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=.7\pgf@circ@res@step

            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
            \pgfpathclose
            \pgf@circ@draworfill
        \endpgfscope
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/input height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/port width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/input height}\pgf@circ@res@up}}


        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/input height}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/port width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/plain amp/input height}\pgf@circ@res@down}}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{0pt}}

        \pgfusepath{draw}





    }
}


%% Draw the two-port fillable box
\def\pgf@circ@twoportbox{
    \pgfscope
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
        \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
        \pgf@circ@draworfill
    \endpgfscope
}

%% Generic two port box
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/twoport/height}}
{twoport}
{\ctikzvalof{bipoles/twoport/height}}
{\ctikzvalof{bipoles/twoport/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/twoport/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step
    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi
    % draw outer box
    \pgf@circ@twoportbox
    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 135 \ifnum \pgfcircmathresult < 225
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner symbol
    \pgftext[center,x=0,y=0]{\ctikzvalof{bipoles/twoport/text}}

}

%% voltage controled oscillator
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/vco/width}}
{vco}
{\ctikzvalof{bipoles/twoport/width}}
{\ctikzvalof{bipoles/vco/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/vco/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi
    % draw circle
    \pgfscope
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
        \pgfpathcircle{\pgfpoint{0}{0}} {\pgf@circ@res@step}
        \pgf@circ@draworfill
    \endpgfscope
    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 134 \ifnum \pgfcircmathresult < 225  % 134 degree, because >= 135 is not possible
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 224 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner sine waves
    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-.5\pgf@circ@res@step}{0\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}

}

%% bandpass filter
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/bandpass/width}}
{bandpass}
{\ctikzvalof{bipoles/bandpass/width}}
{\ctikzvalof{bipoles/bandpass/width}}
{

    \pgf@circ@res@step = \ctikzvalof{bipoles/bandpass/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 134 \ifnum \pgfcircmathresult < 225  % 134 degree, because >= 135 is not possible
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 224 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner symbol
    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetarrows{-} %never draw arrows
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0.5\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{-0.15\pgf@circ@res@step}{0.35\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{0.15\pgf@circ@res@step}{0.65\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{-0.5\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{-0.15\pgf@circ@res@step}{-0.65\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{0.15\pgf@circ@res@step}{-0.35\pgf@circ@res@step}}
    \pgfusepath{draw}
}

%% bandstop filter
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/bandstop/width}}
{bandstop}
{\ctikzvalof{bipoles/bandstop/width}}
{\ctikzvalof{bipoles/bandstop/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/bandstop/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 134 \ifnum \pgfcircmathresult < 225% 134 degree, because >= 135 is not possible
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 224 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner symbol
    \pgfsetdash{}{0pt}% always draw solid line for inner symbol
    \pgfsetarrows{-}%never draw arrows
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0.5\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{-0.15\pgf@circ@res@step}{-0.15\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{0.15\pgf@circ@res@step}{0.15\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{-0.5\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}
}

%% highpass filter
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/highpass/width}}
{highpass}
{\ctikzvalof{bipoles/highpass/width}}
{\ctikzvalof{bipoles/highpass/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/highpass/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 134 \ifnum \pgfcircmathresult < 225  % 134 degree, because >= 135 is not possible
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 224 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner symbol
    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetarrows{-} %never draw arrows
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0.5\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{-0.15\pgf@circ@res@step}{-0.15\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{0.15\pgf@circ@res@step}{0.15\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{-0.5\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{-0.15\pgf@circ@res@step}{-0.65\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{0.15\pgf@circ@res@step}{-0.35\pgf@circ@res@step}}
    \pgfusepath{draw}
}

%% lowpass filter
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/lowpass/width}}
{lowpass}
{\ctikzvalof{bipoles/lowpass/width}}
{\ctikzvalof{bipoles/lowpass/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/lowpass/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 134 \ifnum \pgfcircmathresult < 225  % 134 degree, because >= 135 is not possible
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 224 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner symbol
    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetarrows{-} %never draw arrows
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0.5\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{-0.15\pgf@circ@res@step}{0.35\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{0.15\pgf@circ@res@step}{0.65\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{-0.15\pgf@circ@res@step}{-0.15\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{0.15\pgf@circ@res@step}{0.15\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{-0.5\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathsine{\pgfpoint{.25\pgf@circ@res@step}{-.25\pgf@circ@res@step}}
    \pgfpathcosine{\pgfpoint{.25\pgf@circ@res@step}{.25\pgf@circ@res@step}}
    \pgfusepath{draw}
}

%% ADC
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/adc/width}}
{adc}
{\ctikzvalof{bipoles/adc/width}}
{\ctikzvalof{bipoles/adc/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/adc/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\texti{A}
    \def\textii{D}
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \def\texti{D}
        \def\textii{A}
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 134 \ifnum \pgfcircmathresult < 225  % 134 degree, because >= 135 is not possible
        \def\texti{D}
        \def\textii{A}
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
        \def\texti{A}
        \def\textii{D}
    \fi\fi

    % draw inner symbol
    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetarrows{-} %never draw arrows
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgftext[center,x=0.45\pgf@circ@res@left,y=0.45\pgf@circ@res@up]{\textsf{\texti}}
    \pgftext[center,x=0.45\pgf@circ@res@right,y=0.45\pgf@circ@res@down]{\textsf{\textii}}
}

%% DAC
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/dac/width}}
{dac}
{\ctikzvalof{bipoles/dac/width}}
{\ctikzvalof{bipoles/dac/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/dac/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\texti{D}
    \def\textii{A}
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \def\texti{A}
        \def\textii{D}
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 134 \ifnum \pgfcircmathresult < 225  % 134 degree, because >= 135 is not possible
        \def\texti{A}
        \def\textii{D}
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
        \def\texti{D}
        \def\textii{A}
    \fi\fi

    % draw inner symbol
    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetarrows{-} %never draw arrows
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgftext[center,x=0.45\pgf@circ@res@left,y=0.45\pgf@circ@res@up]{\textsf{\texti}}
    \pgftext[center,x=0.45\pgf@circ@res@right,y=0.45\pgf@circ@res@down]{\textsf{\textii}}
}

%% DSP
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/dsp/width}}
{dsp}
{\ctikzvalof{bipoles/dsp/width}}
{\ctikzvalof{bipoles/dsp/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/dsp/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 135 \ifnum \pgfcircmathresult < 225
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner symbol
    \pgftext[center,x=0,y=0]{\textsf{DSP}}
}

%% FFT
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/fft/width}}
{fft}
{\ctikzvalof{bipoles/fft/width}}
{\ctikzvalof{bipoles/fft/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/fft/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 135 \ifnum \pgfcircmathresult < 225
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner symbol
    \pgftext[center,x=0,y=0]{\textsf{FFT}}
}

%% Amplifier
\pgfcircdeclarebipole
{}
{
    \ifpgf@circuit@boxed
        \ctikzvalof{bipoles/twoport/width}
    \else
        \ctikzvalof{bipoles/amp/width}
    \fi
}
{amp}
{
    \ifpgf@circuit@boxed
        \ctikzvalof{bipoles/twoport/width}
    \else
        \ctikzvalof{bipoles/amp/width}
    \fi
}
{
    \ifpgf@circuit@boxed
        \ctikzvalof{bipoles/twoport/width}
    \else
        \ctikzvalof{bipoles/amp/width}
    \fi
}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/amp/width}\pgf@circ@Rlen

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \ifpgf@circuit@boxed
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
        \pgfnode{box}{center}{}{pgf@box}{\pgfusepath{draw}}
    \pgf@circ@draworfill
    \fi

    % draw input arrow
    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    \ifpgf@circuit@boxed
        \pgfsetlinewidth{\pgfstartlinewidth}
        \pgfsetdash{}{0pt}	% draw solid line for inner symbol if no box is drawn
        \pgf@circ@res@step=.7\pgf@circ@res@step % scale amp symbol when inside a box
    \else
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \fi

    \pgfsetarrows{-} %never draw arrows
    \pgfsetlinewidth{\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0.55\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@step}{0}}
    \pgfpathlineto{\pgfpoint{-0.5\pgf@circ@res@step}{-0.55\pgf@circ@res@step}}

    \pgfpathclose
    \pgf@circ@draworfill

    % draw inner text
    \pgftext[center,x=-0.12\pgf@circ@res@step,y=0]{\ctikzvalof{bipoles/twoport/text}}
}


%% variable amplifier
\pgfcircdeclarebipole
{}
{
    \ifpgf@circuit@boxed
        \ctikzvalof{bipoles/twoport/width}
    \else
        \ctikzvalof{bipoles/amp/width}
    \fi
}
{vamp}
{
    \ifpgf@circuit@boxed
        \ctikzvalof{bipoles/twoport/width}
    \else
        \ctikzvalof{bipoles/amp/width}
    \fi
}
{
    \ifpgf@circuit@boxed
        \ctikzvalof{bipoles/twoport/width}
    \else
        \ctikzvalof{bipoles/amp/width}
    \fi
}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/amp/width}\pgf@circ@Rlen

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \ifpgf@circuit@boxed
        \pgfnode{box}{center}{}{pgf@box}{\pgfusepath{draw}}
    \fi

    % draw input arrow
    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    \ifpgf@circuit@boxed
        \pgfsetlinewidth{\pgfstartlinewidth}
        \pgfsetdash{}{0pt}	% draw solid line for inner symbol if no box is drawn
        \pgf@circ@res@step=.7\pgf@circ@res@step % scale amp symbol when inside a box
    \else
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \fi


    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetarrows{-} %never draw arrows
    \pgfsetlinewidth{\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{0.55\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@step}{0}}
    \pgfpathlineto{\pgfpoint{-0.5\pgf@circ@res@step}{-0.55\pgf@circ@res@step}}

    \pgfpathclose
    \pgf@circ@draworfill

    % draw inner text
    \pgftext[center,x=-0.12\pgf@circ@res@step,y=0]{\ctikzvalof{bipoles/twoport/text}}

    % draw arrow
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfsetarrowsend{latex}
    \pgfpathmoveto{\pgfpoint{-0.8\pgf@circ@res@step}{-0.5\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@step}{0.6\pgf@circ@res@step}}
    \pgfusepath{draw}
}

%% pi attenuator
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/piattenuator/width}}
{piattenuator}
{\ctikzvalof{bipoles/piattenuator/width}}
{\ctikzvalof{bipoles/piattenuator/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/piattenuator/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner symbol
    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetarrows{-} %never draw arrows
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{0.4\pgf@circ@res@left}{0.4\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.4\pgf@circ@res@left}{0.4\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.4\pgf@circ@res@right}{0.4\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.4\pgf@circ@res@right}{0.4\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.6\pgf@circ@res@left}{0.4\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{0.4\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% variable pi attenuator
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/vpiattenuator/width}}
{vpiattenuator}
{\ctikzvalof{bipoles/vpiattenuator/width}}
{\ctikzvalof{bipoles/vpiattenuator/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/vpiattenuator/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner symbol
    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetarrows{-} %never draw arrows
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{0.4\pgf@circ@res@left}{0.4\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.4\pgf@circ@res@left}{0.4\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.4\pgf@circ@res@right}{0.4\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.4\pgf@circ@res@right}{0.4\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.6\pgf@circ@res@left}{0.4\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{0.4\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgfsetarrowsend{latex}
    \pgfpathmoveto{\pgfpoint{0.7\pgf@circ@res@left}{0.5\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.7\pgf@circ@res@right}{0.8\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% T attenuator
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/tattenuator/width}}
{tattenuator}
{\ctikzvalof{bipoles/tattenuator/width}}
{\ctikzvalof{bipoles/tattenuator/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/tattenuator/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner symbol
    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetarrows{-} %never draw arrows
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{0pt}{0.4\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0pt}{0.4\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.6\pgf@circ@res@left}{0.4\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{0.4\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% variable T attenuator
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/vtattenuator/width}}
{vtattenuator}
{\ctikzvalof{bipoles/vtattenuator/width}}
{\ctikzvalof{bipoles/vtattenuator/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/vtattenuator/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % draw inner symbol
    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetarrows{-} %never draw arrows
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{0pt}{0.4\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0pt}{0.4\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.6\pgf@circ@res@left}{0.4\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.6\pgf@circ@res@right}{0.4\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgfsetarrowsend{latex}
    \pgfpathmoveto{\pgfpoint{0.7\pgf@circ@res@left}{0.5\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.7\pgf@circ@res@right}{0.8\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% phase shifter
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/phaseshifter/width}}
{phaseshifter}
{\ctikzvalof{bipoles/phaseshifter/width}}
{\ctikzvalof{bipoles/phaseshifter/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/phaseshifter/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 135 \ifnum \pgfcircmathresult < 225
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % inner symbol
    \pgftext[center,x=0,y=0]{\Large$\varphi$}
}

%% variable phase shifter
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/phaseshifter/width}}
{vphaseshifter}
{\ctikzvalof{bipoles/vphaseshifter/width}}
{\ctikzvalof{bipoles/vphaseshifter/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/vphaseshifter/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % rotate inner symbol
    \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
    \ifnum \pgfcircmathresult > 45 \ifnum \pgfcircmathresult < 135
        \pgftransformrotate{270}
    \fi\fi
    \ifnum \pgfcircmathresult > 135 \ifnum \pgfcircmathresult < 225
        \pgftransformrotate{180}
    \fi\fi
    \ifnum \pgfcircmathresult > 225 \ifnum \pgfcircmathresult < 315
        \pgftransformrotate{90}
    \fi\fi

    % inner symbol
    \pgftext[center,x=0,y=0]{\Large$\varphi$}

    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfsetarrowsend{latex}
    \pgfpathmoveto{\pgfpoint{0.75\pgf@circ@res@left}{0.65\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.7\pgf@circ@res@right}{0.65\pgf@circ@res@up}}
    \pgfusepath{draw}
}

%% detector
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/detector/width}}
{detector}
{\ctikzvalof{bipoles/detector/width}}
{\ctikzvalof{bipoles/detector/width}}
{
    \pgf@circ@res@step = \ctikzvalof{bipoles/detector/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 2

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step

    \ifpgf@circuit@dashed
        \pgfsetdash{{0.1cm}{0.1cm}}{0cm}
    \fi

    % draw outer box
    \pgf@circ@twoportbox

    \ifpgf@circuit@inputarrow
        {
            \advance \pgf@circ@res@left by -.5\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{inputarrow}{tip}{}{pgf@inputarrow}{\pgfusepath{fill}}
        }
    \fi

    % draw inner stuff
    \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
    \pgfsetarrows{-} %never draw arrows
    \pgfsetlinewidth{0.8\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{0.75\pgf@circ@res@left}{0}}
    \pgfpathlineto{\pgfpoint{0.75\pgf@circ@res@right}{0}}
    \pgfusepath{draw}

    \ifpgf@circuit@fulldiode
        \pgfmathparse{2\pgf@circ@res@up / \pgf@circ@Rlen / \ctikzvalof{bipoles/generic/width}}
        \pgftransformscale{\pgfmathresult}
        \pgfnode{fulldiodeshape}{center}{}{pgf@fulldiode}{\pgfusepath{fill}}
    \else
        \pgfmathparse{2\pgf@circ@res@up / \pgf@circ@Rlen / \ctikzvalof{bipoles/resistor/width}}
        \pgftransformscale{\pgfmathresult}
        \pgfnode{emptydiodeshape}{center}{}{pgf@emptydiode}{\pgfusepath{fill}}
    \fi

}




%% european gas filled surge arrester

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/european gas filled surge arrester/height}}
{european gas filled surge arrester}
{\ctikzvalof{bipoles/european gas filled surge arrester/height}}
{\ctikzvalof{bipoles/european gas filled surge arrester/width}}
{

    %\pgf@circ@res@step = \ctikzvalof{bipoles/resistor/width}\pgf@circ@Rlen
    %\divide \pgf@circ@res@step by 14

    \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgf@circ@draworfill

    \pgfscope
        \pgfsetarrowsend{latexslim}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/bipoles/european gas filled surge arrester/inside}\pgf@circ@res@left}{0pt}}
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
        \pgfusepath{draw}

    \endpgfscope
}




%% american gas filled surge arrester

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/american gas filled surge arrester/height}}
{american gas filled surge arrester}
{\ctikzvalof{bipoles/american gas filled surge arrester/height}}
{\ctikzvalof{bipoles/american gas filled surge arrester/width}}{

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpointorigin	\pgf@circ@res@other =  \pgf@x  \advance \pgf@circ@res@other by -\pgf@circ@res@up
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@zero}}
    \pgfusepath{draw}

    \pgfscope
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
        \pgfpathcircle{\pgfpointorigin}{.9\pgf@circ@res@up}
        \pgf@circ@draworfill
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
    \pgfusepath{draw}

    \pgfscope
        \pgfsetarrowsend{latex}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
        \pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/bipoles/american gas filled surge arrester/inside}\pgf@circ@res@right}{\pgf@circ@res@zero}}
        \pgfusepath{draw}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
        \pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/bipoles/american gas filled surge arrester/inside}\pgf@circ@res@left}{\pgf@circ@res@zero}}
        \pgfusepath{draw}
    \endpgfscope{}

    \pgfcircle{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/bipoles/american gas filled surge arrester/dot x}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/bipoles/american gas filled surge arrester/dot y}\pgf@circ@res@down}}{\pgfkeysvalueof{/tikz/circuitikz/bipoles/american gas filled surge arrester/size}\pgf@circ@res@down}
    \pgfusepath{fill}
}

% % MECHANICAL SYMBOLS

%% mechanical capacitance - stiffness/spring

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/spring/height}}{spring}{\ctikzvalof{bipoles/spring/height}}{\ctikzvalof{bipoles/spring/width}}{
	\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
	\pgftransformationadjustments

	\pgfmathsetlength{\pgf@circ@res@step}
	{(\ctikzvalof{bipoles/spring/width}*\pgf@circ@Rlen+\pgfhorizontaltransformationadjustment*.5*\pgflinewidth)/16}

	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{\pgf@circ@res@zero}}
	\pgfsetcornersarced{\pgfpoint{.5\pgf@circ@res@up}{.5\pgf@circ@res@up}}
	\pgf@circ@res@other = \pgf@circ@res@left
	\advance\pgf@circ@res@other by \pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@up}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@up}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@up}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@up}}
	\advance\pgf@circ@res@other by 2\pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
	\advance\pgf@circ@res@other by \pgf@circ@res@step
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@zero}}
	\pgfsetbuttcap
	\pgfsetbeveljoin
	\pgfusepath{stroke}
}

%% mechanical inductance - mass
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/mass/box height}}
{mass}
{\ctikzvalof{bipoles/mass/height}}
{\ctikzvalof{bipoles/mass/width}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgftransformationadjustments
    \pgfpathrectangle{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
        {\pgfpoint{-2\pgf@circ@res@down}{-2\pgf@circ@res@down}}
    \pgf@circ@draworfill

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfsetrectcap
    \pgfsetmiterjoin
    \pgfusepath{stroke}
}

%% mechanical resistor - damper
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/damper/height}}
{damper}
{\ctikzvalof{bipoles/damper/height}}
{\ctikzvalof{bipoles/damper/width}}
{
    \pgfpathrectanglecorners{\pgfpoint{\ctikzvalof{bipoles/damper/length}\pgf@circ@res@right}{\pgf@circ@res@down}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgf@circ@maybefill

    % line into the damper
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
    \pgfpathlineto{\pgfpoint{\ctikzvalof{bipoles/damper/length}\pgf@circ@res@right}
        {\pgf@circ@res@zero}}
    \pgfusepath{stroke}

    % damper box
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}

    \pgfsetrectcap
    \pgfsetmiterjoin
    \pgfusepath{stroke}

    % damper vertical element
    \pgfpathmoveto{\pgfpoint{\ctikzvalof{bipoles/damper/length}\pgf@circ@res@right}
        {.8\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\ctikzvalof{bipoles/damper/length}\pgf@circ@res@right}
        {.8\pgf@circ@res@up}}
    \pgfsetbuttcap
    \pgfusepath{stroke}

}
%% mechanical viscoelastic element, suggested by @alex
%% in https://tex.stackexchange.com/questions/484268/combined-spring-damper-in-circuitikz
\pgfcircdeclarebipole
{}                                   % extra anchors
{\ctikzvalof{bipoles/damper/height}} % depth (under the path line)
{viscoe}                             % name
{\ctikzvalof{bipoles/damper/height}} % height (above the path line)
{\ctikzvalof{bipoles/damper/width}}  % width
{ % draw the bipole
    \pgfpathrectanglecorners{\pgfpoint{\ctikzvalof{bipoles/damper/length}\pgf@circ@res@right}{\pgf@circ@res@down}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgf@circ@maybefill

    % spring into the damper
    \pgfscope
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
        \pgfsetcornersarced{\pgfpoint{.25\pgf@circ@res@up}{.25\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.75\pgf@circ@res@left}{.75\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.5\pgf@circ@res@left}{-.75\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.25\pgf@circ@res@left}{.75\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{-.75\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{\ctikzvalof{bipoles/damper/length}\pgf@circ@res@right}{.75\pgf@circ@res@up}}
        \pgfusepath{stroke}
    \endpgfscope
    % damper box
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}

    \pgfsetrectcap
    \pgfsetmiterjoin
    \pgfusepath{stroke}

    % damper vertical element
    \pgfpathmoveto{\pgfpoint{\ctikzvalof{bipoles/damper/length}\pgf@circ@res@right}
        {.8\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\ctikzvalof{bipoles/damper/length}\pgf@circ@res@right}
        {.8\pgf@circ@res@up}}
    \pgfsetbuttcap
    \pgfusepath{stroke}

}


\pgfcircdeclarebipole
{% anchor for labelling the type of dependency
    \anchor{label}{%
        \southwest
        \pgf@x=0.4\pgf@x
    }%
}
{\ctikzvalof{bipoles/resistivesens/height}}
{resistivesens}
{\ctikzvalof{bipoles/resistivesens/height}}
{\ctikzvalof{bipoles/resistivesens/width}}
{%
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgftransformationadjustments
    \pgfmathsetlength{\pgf@circ@res@step}{\ctikzvalof{bipoles/resistor/width}\pgf@circ@Rlen+\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}
    \divide \pgf@circ@res@step by 12

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{\pgf@circ@res@zero}}

    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@up}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@down}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@up}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@down}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@up}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@down}}
    \advance\pgf@circ@res@other by \pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@zero}}
    \pgfsetbeveljoin
    \pgfusepath{draw}

    \pgfscope
        \pgfpathmoveto{\pgfpoint{.4\pgf@circ@res@other}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{-.4\pgf@circ@res@other}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{-.9\pgf@circ@res@other}{\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}

%% crossing bipole (but see also nodes)
\pgfcircdeclarebipole
    {}
    {\ctikzvalof{bipoles/crossing/size}}
    {crossing}
    {\ctikzvalof{bipoles/crossing/size}}
    {\ctikzvalof{bipoles/crossing/size}}{
        \pgfscope
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@zero}}
        \pgfpathlineto{\pgfpoint{0.4\pgf@circ@res@left}{\pgf@circ@res@zero}}
        \pgfpatharc{0}{-180}{0.4*\pgf@circ@res@left}
        \pgfsetbeveljoin
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@zero}}
        \pgfusepath{draw}
        \endpgfscope
    }

%% loudspeaker and microphone

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/loudspeaker/depth}}
{loudspeaker}
{\ctikzvalof{bipoles/loudspeaker/height}}
{\ctikzvalof{bipoles/loudspeaker/width}}{

    \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{.4\pgf@circ@res@up}}
    {\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathmoveto{\pgfpoint{0.5\pgf@circ@res@left}{.4\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.8\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.8\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@right}{.4\pgf@circ@res@up}}
    \pgfpathclose
    \pgfsetlinewidth{\ctikzvalof{bipoles/thickness}\pgfstartlinewidth}
    \pgf@circ@draworfill
}

\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/mic/depth}}
{mic}
{\ctikzvalof{bipoles/mic/height}}
{\ctikzvalof{bipoles/mic/width}}{

    \pgfscope
    \pgfsetlinewidth{\ctikzvalof{bipoles/thickness}\pgfstartlinewidth}
    \pgfpathcircle{\pgfpoint{0pt}{.6\pgf@circ@res@up}}{.4\pgf@circ@res@up}
    \pgf@circ@draworfill
    \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}
    \endpgfscope
    \pgfscope
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{-.2\pgf@circ@res@up}{0pt}}
    % 0.25358 is 0.6-0.4*cos(30)
    \pgfpathlineto{\pgfpoint{-.2\pgf@circ@res@up}{.25358\pgf@circ@res@up}}
    \pgfpathmoveto{\pgfpoint{.2\pgf@circ@res@up}{.25358\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.2\pgf@circ@res@up}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfusepath{draw}

    \pgfusepath{draw}
    \endpgfscope
}

% generic round meter with always horizontal text, no arrow
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/esource/height}}
{rmeter}
{\ctikzvalof{bipoles/esource/height}}
{\ctikzvalof{bipoles/esource/width}}
{
    \pgfpointorigin
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill
    % draw the text label
    % get the rotation
    \pgfgettransformentries\a\b\temp\temp\temp\temp
    \pgfmathsetmacro{\rot}{-atan2(\b,\a)}
    % and unrotate the scope
    \pgfscope
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
        \pgftransformrotate{\rot}
        \pgftext[center,x=0,y=0]{\ctikzvalof{bipoles/twoport/text}}
    \endpgfscope
}

% generic round meter with always horizontal text, with arrow
\pgfcircdeclarebipole
{}
{\ctikzvalof{bipoles/esource/height}}
{rmeterwa}
{\ctikzvalof{bipoles/esource/height}}
{\ctikzvalof{bipoles/esource/width}}
{
    \pgfpointorigin
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgf@circ@draworfill
    % draw the text label
    % get the rotation
    \pgfgettransformentries\a\b\temp\temp\temp\temp
    \pgfmathsetmacro{\rot}{-atan2(\b,\a)}
    % and unrotate the scope
    \pgfscope
        \pgftransformrotate{\rot}
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
        \pgfsetlinewidth{\pgfstartlinewidth}
        % arrow: create  a center hole to have better visual
        \pgfscope
            % clipping path: first a rectangle bigger then the shape
            % to avoid problems with the line thickness
            \pgfpathrectanglecorners{\pgfpoint{2\pgf@circ@res@left}{2\pgf@circ@res@down}}
            {\pgfpoint{2\pgf@circ@res@right}{2\pgf@circ@res@up}}
            % next open a circle into it
            \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{.6\pgf@circ@res@up}}{\pgfpoint{.6\pgf@circ@res@left}{0}}
            % do the difference and clip before drawing
            \pgfseteorule
            \pgfusepath{clip}
            \pgfsetarrowsend{latexslim}
            % the arrow is better if it has a bit of breath and it's not 45º
            \pgfpathmoveto{\pgfpoint{.8\pgf@circ@res@left}{1.2\pgf@circ@res@down}}
            \pgfpathlineto{\pgfpoint{.8\pgf@circ@res@right}{1.2\pgf@circ@res@up}}
            \pgfusepath{draw}
        \endpgfscope
        \pgftext[center]{\ctikzvalof{bipoles/twoport/text}}
    \endpgfscope
}

% generic square meter with always horizontal text
\pgfcircdeclarebipole
{
    \anchor{in 1}{\southwest\pgf@y=0.75\pgf@y\pgf@x=0.4\pgf@x}
    \anchor{in 2}{\southwest\pgf@y=0.75\pgf@y\pgf@x=-0.4\pgf@x}
    % put the node text above and centered
    \anchor{text}{\pgfextracty{\pgf@circ@res@up}{\northeast}
        \pgfpoint{-.5\wd\pgfnodeparttextbox}{
            \dimexpr.5\dp\pgfnodeparttextbox+.5\ht\pgfnodeparttextbox+\pgf@circ@res@up\relax
        }
    }
}
{\ctikzvalof{bipoles/smeter/height}}
{smeter}
{\ctikzvalof{bipoles/smeter/height}}
{\ctikzvalof{bipoles/smeter/width}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgfextracty{\pgf@circ@res@up}{\northeast}
    \pgfextractx{\pgf@circ@res@right}{\northeast}
    \pgfextractx{\pgf@circ@res@left}{\southwest}
    \pgfextracty{\pgf@circ@res@down}{\southwest}
    \pgfmathsetlength{\pgf@circ@res@step}{0.25*\pgf@circ@res@up}
    \pgfscope
        \pgfsetcornersarced{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@step}}
        \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
        \pgf@circ@draworfill
    \endpgfscope
    % get the rotation
    \pgfgettransformentries\a\b\temp\temp\temp\temp
    \pgfmathsetmacro{\rot}{-atan2(\b,\a)}
    % and unrotate the scope
    \pgfscope
        \pgftransformrotate{\rot}
        % the metering window
        \pgfscope
            \def\@starta{105}\def\@stopa{75}
            \pgfsetlinewidth{\pgfstartlinewidth}
            \pgftransformshift{\pgfpoint{0pt}{-1.8\pgf@circ@res@up}}
            \pgfpathmoveto{\pgfpointpolar{\@starta}{2\pgf@circ@res@up}}
            \pgfpatharc{\@starta}{\@stopa}{2\pgf@circ@res@up}
            \pgfpathlineto{\pgfpointpolar{\@stopa}{2.5\pgf@circ@res@up}}
            \pgfpatharc{\@stopa}{\@starta}{2.5\pgf@circ@res@up}
            \pgfclosepath
            \pgfpathmoveto{\pgfpointpolar{80}{2\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpointpolar{80}{2.4\pgf@circ@res@up}}
            \pgfusepath{draw}
        \endpgfscope
        \pgftext[center, y=0.5\pgf@circ@res@down]{\ctikzvalof{bipoles/twoport/text}}
    \endpgfscope
}

% probles qucs style:
% #1 : name
% #2 : extra code
\long\def\pgfcirc@qucsprobe#1#2{
    \pgfcircdeclarebipole
    {
        \anchor{v+}{\southwest\pgf@x=0.6\pgf@x}
        \anchor{v-}{\southwest\pgf@x=-0.6\pgf@x}
        % put the node text above and centered
        \anchor{text}{\pgfextracty{\pgf@circ@res@up}{\northeast}
            \pgfpoint{-.5\wd\pgfnodeparttextbox}{
                \dimexpr.5\dp\pgfnodeparttextbox+.5\ht\pgfnodeparttextbox+\pgf@circ@res@up\relax
            }
        }
    }
    {\ctikzvalof{bipoles/qmeter/depth}}
    {#1}
    {\ctikzvalof{bipoles/qmeter/height}}
    {\ctikzvalof{bipoles/qmeter/width}}
    {
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
        \pgfextracty{\pgf@circ@res@up}{\northeast}
        \pgfextractx{\pgf@circ@res@right}{\northeast}
        \pgfextractx{\pgf@circ@res@left}{\southwest}
        \pgfextracty{\pgf@circ@res@down}{\southwest}
        \pgfmathsetlength{\pgf@circ@res@step}{0.25*\pgf@circ@res@up}
        \pgfscope
            \pgfscope
                \pgfsetcornersarced{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@step}}
                \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
            \pgf@circ@draworfill
            \endpgfscope
            \def\@starta{103}\def\@stopa{77}
            \pgfsetlinewidth{\pgfstartlinewidth}
            \pgfscope
                \pgftransformshift{\pgfpoint{0pt}{-1.7\pgf@circ@res@up}}
                \pgfpathmoveto{\pgfpointpolar{\@starta}{2.1\pgf@circ@res@up}}
                \pgfpatharc{\@starta}{\@stopa}{2.1\pgf@circ@res@up}
                \pgfpathlineto{\pgfpointpolar{\@stopa}{2.5\pgf@circ@res@up}}
                \pgfpatharc{\@stopa}{\@starta}{2.5\pgf@circ@res@up}
                \pgfclosepath
                \pgfpathmoveto{\pgfpointpolar{83}{2.1\pgf@circ@res@up}}
                \pgfpathlineto{\pgfpointpolar{83}{2.4\pgf@circ@res@up}}
                \pgfusepath{draw}
                \pgf@circ@draworfill
            \endpgfscope
            #2
        \endpgfscope
    }
}

\pgfcirc@qucsprobe{qiprobe}{
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfusepath{draw}
    \pgfnode{currarrow}{center}{}{}{}
}

\pgfcirc@qucsprobe{qvprobe}{
    \pgfmathsetlength{\pgf@circ@res@other}{\pgfkeysvalueof{/tikz/circuitikz/nodes width}*\pgf@circ@Rlen}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@left}{0pt}}
    \pgfpathcircle{\pgfpoint{.6\pgf@circ@res@left+\pgf@circ@res@other}{0pt}}{\pgf@circ@res@other}
    \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathcircle{\pgfpoint{.6\pgf@circ@res@right-\pgf@circ@res@other}{0pt}}{\pgf@circ@res@other}
    \pgfusepath{draw}
    \pgfscope
        % "+" and "-", drawn so that they scale correctly
        \pgfsetlinewidth{2\pgfstartlinewidth}
        \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left+\pgf@circ@res@other}{-1.5\pgf@circ@res@other}}
        \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@left+\pgf@circ@res@other}{-3.5\pgf@circ@res@other}}
        \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left+0\pgf@circ@res@other}{-2.5\pgf@circ@res@other}}
        \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@left+2\pgf@circ@res@other}{-2.5\pgf@circ@res@other}}
        \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@right+0\pgf@circ@res@other}{-2.5\pgf@circ@res@other}}
        \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@right-2\pgf@circ@res@other}{-2.5\pgf@circ@res@other}}
        \pgfusepath{draw}
    \endpgfscope
}

\pgfcirc@qucsprobe{qpprobe}{
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfusepath{draw}
    \pgfnode{currarrow}{center}{}{}{}
    \pgfmathsetlength{\pgf@circ@res@other}{\pgfkeysvalueof{/tikz/circuitikz/nodes width}*\pgf@circ@Rlen}
    \pgfpathcircle{\pgfpoint{.6\pgf@circ@res@left}{-3\pgf@circ@res@other}}{\pgf@circ@res@other}
    \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left}{-4\pgf@circ@res@other}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathcircle{\pgfpoint{.6\pgf@circ@res@right}{-3\pgf@circ@res@other}}{\pgf@circ@res@other}
    \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@right}{-4\pgf@circ@res@other}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfusepath{draw}
    \pgfscope
        % "+" and "-", drawn so that they scale correctly
        \pgfsetlinewidth{2\pgfstartlinewidth}
        \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left+3\pgf@circ@res@other}{-2\pgf@circ@res@other}}
        \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@left+3\pgf@circ@res@other}{-4\pgf@circ@res@other}}
        \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left+2\pgf@circ@res@other}{-3\pgf@circ@res@other}}
        \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@left+4\pgf@circ@res@other}{-3\pgf@circ@res@other}}
        \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@right-4\pgf@circ@res@other}{-3\pgf@circ@res@other}}
        \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@right-2\pgf@circ@res@other}{-3\pgf@circ@res@other}}
        \pgfusepath{draw}
    \endpgfscope
}


% current loop for oscope and similar: stylized

\pgfcircdeclarebipole
{
    \anchor{i}{\northeast\pgf@x=0pt\relax}
    \anchor{text}{
        \pgfextracty{\pgf@circ@res@up}{\northeast}
        \pgfextractx{\pgf@circ@res@left}{\northeast}
        \pgfpoint{-.5\wd\pgfnodeparttextbox+\pgf@circ@res@left}{
            \dimexpr.5\dp\pgfnodeparttextbox+.5\ht\pgfnodeparttextbox+\pgf@circ@res@up\relax
        }
    }
}
{\ctikzvalof{bipoles/iloop/height}}
{iloop}
{\ctikzvalof{bipoles/iloop/height}}
{\ctikzvalof{bipoles/iloop/width}}
{
    \pgfextracty{\pgf@circ@res@up}{\northeast}
    \pgfextractx{\pgf@circ@res@right}{\northeast}
    \pgf@circ@res@down=-\pgf@circ@res@up
    \pgf@circ@res@left=-\pgf@circ@res@right
    \pgfscope
        \pgfstartlinewidth=\pgflinewidth
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
        % external ellipse
        \pgfscope
            \pgfsetlinewidth{\ctikzvalof{bipoles/thickness}\pgflinewidth}
            % clipping path: first a rectangle bigger then the shape
            % to avoid problems with the line thickness
            \pgfpathrectanglecorners{\pgfpoint{2\pgf@circ@res@left}{2\pgf@circ@res@down}}
            {\pgfpoint{2\pgf@circ@res@right}{2\pgf@circ@res@up}}
            % next the opening to the left
            \pgfpathrectanglecorners{\pgfpoint{2\pgf@circ@res@left}{.1\pgf@circ@res@down}}
            {\pgfpoint{0pt}{.1\pgf@circ@res@up}}
            % do the difference and clip before drawing
            \pgfseteorule
            \pgfusepath{clip}
            \pgfpathellipse{\pgfpointorigin}{
                \pgfpoint{0pt}{0.8\pgf@circ@res@up}}{
            \pgfpoint{0.4\pgf@circ@res@right}{0pt}}
            \pgfusepath{draw}
        \endpgfscope
        % internal wire
        \pgfsetlinewidth{\pgfstartlinewidth}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0.3\pgf@circ@res@right}{0pt}}
        \pgfpathmoveto{\pgfpoint{0.5\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        % and the contact line up
        \pgfpathmoveto{\pgfpoint{0pt}{0.8\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}


% current loop for oscope and similar: real (double connection)

\pgfcircdeclarebipole
{
    \anchor{i+}{
        \pgfextracty{\pgf@circ@res@up}{\northeast}
        \pgfextractx{\pgf@circ@res@right}{\northeast}
        \pgf@circ@res@step=0.4\pgf@circ@res@right
        \pgf@circ@res@other=0.8\pgf@circ@res@up
        \pgfpointpolar{105}{\pgf@circ@res@step and \pgf@circ@res@other}
        \pgf@y=\pgf@circ@res@up
    }
    \anchor{i-}{
        \pgfextracty{\pgf@circ@res@up}{\northeast}
        \pgfextractx{\pgf@circ@res@right}{\northeast}
        \pgf@circ@res@step=0.4\pgf@circ@res@right
        \pgf@circ@res@other=0.8\pgf@circ@res@up
        \pgfpointpolar{75}{\pgf@circ@res@step and \pgf@circ@res@other}
        \pgf@y=\pgf@circ@res@up
    }
    \anchor{text}{
        \pgfextracty{\pgf@circ@res@up}{\northeast}
        \pgfextractx{\pgf@circ@res@left}{\northeast}
        \pgfpoint{-.5\wd\pgfnodeparttextbox+\pgf@circ@res@left}{
            \dimexpr.5\dp\pgfnodeparttextbox+.5\ht\pgfnodeparttextbox+\pgf@circ@res@up\relax
        }
    }
}
{\ctikzvalof{bipoles/iloop/height}}
{iloop2}
{\ctikzvalof{bipoles/iloop/height}}
{\ctikzvalof{bipoles/iloop/width}}
{
    \pgfextracty{\pgf@circ@res@up}{\northeast}
    \pgfextractx{\pgf@circ@res@right}{\northeast}
    \pgf@circ@res@down=-\pgf@circ@res@up
    \pgf@circ@res@left=-\pgf@circ@res@right
    % must be the same than internal i+ and i- anchors definition
    \pgf@circ@res@step=0.4\pgf@circ@res@right
    \pgf@circ@res@other=0.8\pgf@circ@res@up
    \def\@plus{\pgfpointpolar{105}{\pgf@circ@res@step and \pgf@circ@res@other}}
    \def\@minus{\pgfpointpolar{75}{\pgf@circ@res@step and \pgf@circ@res@other}}
    \pgfscope
        \pgfstartlinewidth=\pgflinewidth
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
        % external ellipse
        \pgfscope
            \pgfsetlinewidth{\ctikzvalof{bipoles/thickness}\pgflinewidth}
            % clipping path: first a rectangle bigger then the shape
            % to avoid problems with the line thickness
            \pgfpathrectanglecorners{\pgfpoint{2\pgf@circ@res@left}{2\pgf@circ@res@down}}
            {\pgfpoint{2\pgf@circ@res@right}{2\pgf@circ@res@up}}
            % next the opening to the left
            \pgfpathrectanglecorners{\pgfpoint{2\pgf@circ@res@left}{.1\pgf@circ@res@down}}
            {\pgfpoint{0pt}{.1\pgf@circ@res@up}}
            % do the difference and clip before drawing
            \pgfseteorule
            \pgfusepath{clip}
            \pgfpathmoveto{\@plus}
            \pgfpatharc{105}{435}{\pgf@circ@res@step and \pgf@circ@res@other}
            \pgfusepath{draw}
        \endpgfscope
        % internal wire
        \pgfsetlinewidth{\pgfstartlinewidth}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0.3\pgf@circ@res@right}{0pt}}
        \pgfpathmoveto{\pgfpoint{0.5\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        % and the contact line up
        % I use ...left and ---right as temporal lengths here to avoid defining more
        \pgfextractx{\pgf@circ@res@left}{\@plus}
        \pgfextractx{\pgf@circ@res@right}{\@minus}
        \pgfpathmoveto{\@plus}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
        \pgfpathmoveto{\@minus}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope
}

% end of pgfcircbipoles.tex


==> pgfcirccurrent.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the files gpl-3.0_license.txt and lppl-1-3c_license.txt for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Current handling

%% Options
\ctikzset{i^>/.style = {
        i = #1,
        \circuitikzbasekey/bipole/current/direction = forward,
        \circuitikzbasekey/bipole/current/x position = after,
        \circuitikzbasekey/bipole/current/y position = above
    }
}

\ctikzset{i_>/.style = {
        i = #1,
        \circuitikzbasekey/bipole/current/direction = forward,
        \circuitikzbasekey/bipole/current/x position = after,
        \circuitikzbasekey/bipole/current/y position = below
    }
}

\ctikzset{i>^/.style = {
        i = #1,
        \circuitikzbasekey/bipole/current/direction = forward,
        \circuitikzbasekey/bipole/current/x position = before,
        \circuitikzbasekey/bipole/current/y position = above
    }
}

\ctikzset{i>_/.style = {
        i = #1,
        \circuitikzbasekey/bipole/current/direction = forward,
        \circuitikzbasekey/bipole/current/x position = before,
        \circuitikzbasekey/bipole/current/y position = below
    }
}

\ctikzset{i^</.style = {
        i = #1,
        \circuitikzbasekey/bipole/current/direction = backward,
        \circuitikzbasekey/bipole/current/x position = after,
        \circuitikzbasekey/bipole/current/y position = above
    }
}

\ctikzset{i_</.style = {
        i = #1,
        \circuitikzbasekey/bipole/current/direction = backward,
        \circuitikzbasekey/bipole/current/x position = after,
        \circuitikzbasekey/bipole/current/y position = below
    }
}

\ctikzset{i<^/.style = {
        i = #1,
        \circuitikzbasekey/bipole/current/direction = backward,
        \circuitikzbasekey/bipole/current/x position = before,
        \circuitikzbasekey/bipole/current/y position = above
    }
}

\ctikzset{i<_/.style = {
        i = #1,
        \circuitikzbasekey/bipole/current/direction = backward,
        \circuitikzbasekey/bipole/current/x position = before,
        \circuitikzbasekey/bipole/current/y position = below
    }
}

\ctikzset{i/.code = {
        \pgfkeys{\circuitikzbasekey/bipole/current/direction = forward,
            \circuitikzbasekey/bipole/current/x position = after,
        \circuitikzbasekey/bipole/current/y position = above }
        \pgfkeys{/tikz/circuitikz/bipole/current/label/name=#1}
        \ctikzsetvalof{bipole/current/label/unit}{}
        \ifpgf@circ@siunitx
            \pgf@circ@handleSI{#1}
            \ifpgf@circ@siunitx@res
                \edef\pgf@temp{\pgf@circ@handleSI@val}
                \pgfkeyslet{/tikz/circuitikz/bipole/current/label/name}{\pgf@temp}
                \edef\pgf@temp{\pgf@circ@handleSI@unit}
                \pgfkeyslet{/tikz/circuitikz/bipole/current/label/unit}{\pgf@temp}
            \else
        \fi
        \else
    \fi
    %reverse current direction for voltage sources
    \ifpgf@circ@oldvoltagedirection\else
        \ifpgf@circuit@bipole@isvoltage
            \ifpgf@circuit@bipole@voltage@backward
                \pgfkeys{\circuitikzbasekey/bipole/current/direction = forward,
                    \circuitikzbasekey/bipole/current/x position = after,
                \circuitikzbasekey/bipole/current/y position = below }
            \else
                \pgfkeys{\circuitikzbasekey/bipole/current/direction = backward,
                    \circuitikzbasekey/bipole/current/x position = before,
                \circuitikzbasekey/bipole/current/y position = above }
            \fi\fi\fi
    }
}

\ifpgf@circ@oldvoltagedirection
    \ctikzset{i</.style = { i = #1, \circuitikzbasekey/bipole/current/direction = backward } }
\else
    \ctikzset{i</.style = { i = #1, \circuitikzbasekey/bipole/current/direction = backward, \circuitikzbasekey/bipole/current/x position = before } }
\fi
\ctikzset{i_/.style = { i = #1, \circuitikzbasekey/bipole/current/y position = below } }
\ctikzset{i>/.style = {i = #1, \circuitikzbasekey/bipole/current/direction = forward } }
\ctikzset{i^/.style = { i= #1, \circuitikzbasekey/bipole/current/y position = above } }

%% Output routine
\def\pgf@circ@drawcurrent{
    \pgfextra{
        \edef\pgf@circ@ffffff{\pgf@circ@direction}
        \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@ffffff\pgf@nil}

        \ifnum\pgfcircmathresult >4 \ifnum\pgfcircmathresult <86
        \ifpgf@circuit@bipole@current@below
            \def\pgf@circ@dir{north west} \else \def\pgf@circ@dir{south east}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >85 \ifnum\pgfcircmathresult <95
        \ifpgf@circuit@bipole@current@below
            \def\pgf@circ@dir{west} \else \def\pgf@circ@dir{east}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >94 \ifnum\pgfcircmathresult <176
        \ifpgf@circuit@bipole@current@below
            \def\pgf@circ@dir{south west}\else \def\pgf@circ@dir{north east}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >175 \ifnum\pgfcircmathresult <185
        \ifpgf@circuit@bipole@current@below
            \def\pgf@circ@dir{south}\else\def\pgf@circ@dir{north}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >184 \ifnum\pgfcircmathresult <266
        \ifpgf@circuit@bipole@current@below
            \def\pgf@circ@dir{south east}\else\def\pgf@circ@dir{north west}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >265 \ifnum\pgfcircmathresult <275
        \ifpgf@circuit@bipole@current@below
            \def\pgf@circ@dir{east}\else \def\pgf@circ@dir{west}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >274 \ifnum\pgfcircmathresult <356
        \ifpgf@circuit@bipole@current@below
            \def\pgf@circ@dir{north east}\else\def\pgf@circ@dir{south west}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult <5
        \ifpgf@circuit@bipole@current@below
            \def\pgf@circ@dir{north}\else\def\pgf@circ@dir{south}
        \fi
        \fi
        \ifnum\pgfcircmathresult >355
        \ifpgf@circuit@bipole@current@below
            \def\pgf@circ@dir{north}\else\def\pgf@circ@dir{south}
        \fi
    \fi

    \ifpgf@circuit@bipole@current@below
        \def\pgf@circ@bipole@current@label@where{-90}
    \else
        \def\pgf@circ@bipole@current@label@where{+90}
    \fi
    }

    \pgfextra{\def\pgf@temp{short}\edef\pgf@circ@temp{\ctikzvalof{bipole/kind}}}
    \ifx\pgf@circ@temp\pgf@temp%draw current at a short at middle of the line
        (\tikztostart)--(\tikztotarget)
    \else% normal bipole or source
        \ifpgf@circuit@bipole@current@before
            (\tikztostart)--(anchorstartnode)
        \else
            (anchorendnode)--(\tikztotarget)
        \fi
    \fi
    \ifpgf@circuit@bipole@current@backward
        \pgfextra{
            \pgfmathsubtract{\pgf@circ@ffffff}{180}
            \edef\pgf@circ@ffffff{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
        }
    \fi
    coordinate[currarrow,pos=\ctikzvalof{current/distance},rotate=\pgf@circ@ffffff](Iarrow)
    (Iarrow.\pgf@circ@bipole@current@label@where) node[anchor=\pgf@circ@dir]{\pgf@circ@finallabels{current/label}}
}

\endinput


==> pgfcircflow.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the files gpl-3.0_license.txt and lppl-1-3c_license.txt for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% flow handling

%% Options
\ctikzset{f^>/.style = {
        f = #1,
        \circuitikzbasekey/bipole/flow/direction = forward,
        \circuitikzbasekey/bipole/flow/x position = after,
        \circuitikzbasekey/bipole/curflowrent/y position = above
    }
}

\ctikzset{f_>/.style = {
        f = #1,
        \circuitikzbasekey/bipole/flow/direction = forward,
        \circuitikzbasekey/bipole/flow/x position = after,
        \circuitikzbasekey/bipole/flow/y position = below
    }
}

\ctikzset{f>^/.style = {
        f = #1,
        \circuitikzbasekey/bipole/flow/direction = forward,
        \circuitikzbasekey/bipole/flow/x position = before,
        \circuitikzbasekey/bipole/flow/y position = above
    }
}

\ctikzset{f>_/.style = {
        f = #1,
        \circuitikzbasekey/bipole/flow/direction = forward,
        \circuitikzbasekey/bipole/flow/x position = before,
        \circuitikzbasekey/bipole/flow/y position = below
    }
}

\ctikzset{f^</.style = {
        f = #1,
        \circuitikzbasekey/bipole/flow/direction = backward,
        \circuitikzbasekey/bipole/flow/x position = after,
        \circuitikzbasekey/bipole/flow/y position = above
    }
}

\ctikzset{f_</.style = {
        f = #1,
        \circuitikzbasekey/bipole/flow/direction = backward,
        \circuitikzbasekey/bipole/flow/x position = after,
        \circuitikzbasekey/bipole/flow/y position = below
    }
}

\ctikzset{f<^/.style = {
        f = #1,
        \circuitikzbasekey/bipole/flow/direction = backward,
        \circuitikzbasekey/bipole/flow/x position = before,
        \circuitikzbasekey/bipole/flow/y position = above
    }
}

\ctikzset{f<_/.style = {
        f = #1,
        \circuitikzbasekey/bipole/flow/direction = backward,
        \circuitikzbasekey/bipole/flow/x position = before,
        \circuitikzbasekey/bipole/flow/y position = below
    }
}

\ctikzset{f</.style = { f = #1, \circuitikzbasekey/bipole/flow/direction = backward} }
\ctikzset{f_/.style = { f = #1, \circuitikzbasekey/bipole/flow/y position = below } }
\ctikzset{f>/.style = { f = #1, \circuitikzbasekey/bipole/flow/direction = forward } }
\ctikzset{f^/.style = { f = #1, \circuitikzbasekey/bipole/flow/y position = above } }

\ctikzset{f/.code = {
        \pgfkeys{\circuitikzbasekey/bipole/flow/direction = forward,
            \circuitikzbasekey/bipole/flow/x position = after,
        \circuitikzbasekey/bipole/flow/y position = above }
        \pgfkeys{/tikz/circuitikz/bipole/flow/label/name=#1}
        \ctikzsetvalof{bipole/flow/label/unit}{}
        \ifpgf@circ@siunitx
            \pgf@circ@handleSI{#1}
            \ifpgf@circ@siunitx@res
                \edef\pgf@temp{\pgf@circ@handleSI@val}
                \pgfkeyslet{/tikz/circuitikz/bipole/flow/label/name}{\pgf@temp}
                \edef\pgf@temp{\pgf@circ@handleSI@unit}
                \pgfkeyslet{/tikz/circuitikz/bipole/flow/label/unit}{\pgf@temp}
            \else
        \fi
        \else
    \fi
}
}

%% Output routine
\def\pgf@circ@drawflow{
    \pgfextra{
        \edef\pgf@circ@ffffff{\pgf@circ@direction}
        \def\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@ffffff\pgf@nil}

        \ifnum\pgfcircmathresult >4 \ifnum\pgfcircmathresult <86
                \ifpgf@circuit@bipole@flow@below
                        \def\pgf@circ@dir{north west} \else \def\pgf@circ@dir{south east}
                \fi
        \fi\fi
        \ifnum\pgfcircmathresult >85 \ifnum\pgfcircmathresult <95
                \ifpgf@circuit@bipole@flow@below
                        \def\pgf@circ@dir{west} \else \def\pgf@circ@dir{east}
                \fi
        \fi\fi
        \ifnum\pgfcircmathresult >94 \ifnum\pgfcircmathresult <176
                \ifpgf@circuit@bipole@flow@below
                         \def\pgf@circ@dir{south west}\else \def\pgf@circ@dir{north east}
                \fi
        \fi\fi
        \ifnum\pgfcircmathresult >175 \ifnum\pgfcircmathresult <185
                \ifpgf@circuit@bipole@flow@below
                          \def\pgf@circ@dir{south}\else\def\pgf@circ@dir{north}
                \fi
        \fi\fi
        \ifnum\pgfcircmathresult >184 \ifnum\pgfcircmathresult <266
                \ifpgf@circuit@bipole@flow@below
                         \def\pgf@circ@dir{south east}\else\def\pgf@circ@dir{north west}
                \fi
        \fi\fi
        \ifnum\pgfcircmathresult >265 \ifnum\pgfcircmathresult <275
                \ifpgf@circuit@bipole@flow@below
                         \def\pgf@circ@dir{east}\else \def\pgf@circ@dir{west}
                \fi
        \fi\fi
        \ifnum\pgfcircmathresult >274 \ifnum\pgfcircmathresult <356
                \ifpgf@circuit@bipole@flow@below
                          \def\pgf@circ@dir{north east}\else\def\pgf@circ@dir{south west}
                \fi
        \fi\fi
        \ifnum\pgfcircmathresult <5
                \ifpgf@circuit@bipole@flow@below
                         \def\pgf@circ@dir{north}\else\def\pgf@circ@dir{south}
                \fi
        \fi
        \ifnum\pgfcircmathresult >355
                \ifpgf@circuit@bipole@flow@below
                         \def\pgf@circ@dir{north}\else\def\pgf@circ@dir{south}
                \fi
        \fi

        \ifpgf@circuit@bipole@flow@below
                \def\pgf@circ@bipole@flow@label@where{-90}
        \else
                \def\pgf@circ@bipole@flow@label@where{+90}
        \fi
    }

    \pgfextra{\def\pgf@temp{short}\edef\pgf@circ@temp{\ctikzvalof{bipole/kind}}}
    \ifx\pgf@circ@temp\pgf@temp%draw flow at a short at middle of the line
        (\tikztostart)--(\tikztotarget)
    \else% normal bipole or source
        \ifpgf@circuit@bipole@flow@before
            (\tikztostart)--(anchorstartnode)
        \else
            (anchorendnode)--(\tikztotarget)
        \fi
    \fi
    \pgfextra{
        \ifpgf@circuit@bipole@flow@backward
            \ifpgf@circuit@bipole@flow@below
                \def\flow@offset{\ctikzvalof{flow/offset}\pgf@circ@Rlen}
            \else
                \def\flow@offset{-\ctikzvalof{flow/offset}\pgf@circ@Rlen}
            \fi
            \pgfmathsubtract{\pgf@circ@ffffff}{180}
            \edef\pgf@circ@ffffff{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
            \else
            \ifpgf@circuit@bipole@flow@below
                \def\flow@offset{-\ctikzvalof{flow/offset}\pgf@circ@Rlen}
            \else
                \def\flow@offset{\ctikzvalof{flow/offset}\pgf@circ@Rlen}
            \fi
        \fi
    }
    coordinate[flowarrow,pos=\ctikzvalof{flow/distance},rotate=\pgf@circ@ffffff,yshift=\flow@offset](Farrowpos)
    (Farrowpos.\pgf@circ@bipole@flow@label@where) node[anchor=\pgf@circ@dir]{ \pgf@circ@finallabels{flow/label}}
}

\endinput


==> pgfcirclabel.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the files gpl-3.0_license.txt and lppl-1-3c_license.txt for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Bipole label positioning

%% Options
\ctikzset{label/.style = { l=#1 } }
\ctikzset{l/.code = {
        \pgfkeys{/tikz/circuitikz/bipole/label/name=#1}
        \ctikzsetvalof{bipole/label/unit}{}
        \ifpgf@circ@siunitx
            \pgf@circ@handleSI{#1}
            \ifpgf@circ@siunitx@res
                \edef\pgf@temp{\pgf@circ@handleSI@val}
                \pgfkeyslet{/tikz/circuitikz/bipole/label/name}{\pgf@temp}
                \edef\pgf@temp{\pgf@circ@handleSI@unit}
                \pgfkeyslet{/tikz/circuitikz/bipole/label/unit}{\pgf@temp}
            \else
        \fi
        \else
    \fi
}}

\ctikzset{label above/.code = {
        l=#1,
    \circuitikzbasekey/bipole/label/position=90 }
}

\ctikzset{l^/.style = {
        l=#1,
    \circuitikzbasekey/bipole/label/position=90 }
}

\ctikzset{label below/.code = {
        l=#1,
    \circuitikzbasekey/bipole/label/position=-90 }
}

\ctikzset{l_/.style = {
        l=#1,
    \circuitikzbasekey/bipole/label/position=-90 }
}

\ctikzset{annotation/.style = { a=#1 } }
\ctikzset{a/.code = {
    \pgfkeys{/tikz/circuitikz/bipole/annotation/name=#1}
    \ctikzsetvalof{bipole/annotation/unit}{}
    \ifpgf@circ@siunitx
        \pgf@circ@handleSI{#1}
        \ifpgf@circ@siunitx@res
            \edef\pgf@temp{\pgf@circ@handleSI@val}
            \pgfkeyslet{/tikz/circuitikz/bipole/annotation/name}{\pgf@temp}
            \edef\pgf@temp{\pgf@circ@handleSI@unit}
            \pgfkeyslet{/tikz/circuitikz/bipole/annotation/unit}{\pgf@temp}
        \else
        \fi
    \else
    \fi
}}

\ctikzset{annotation above/.code = {
        a=#1,
    \circuitikzbasekey/bipole/annotation/position=90 }
}

\ctikzset{a^/.style = {
        a=#1,
    \circuitikzbasekey/bipole/annotation/position=90 }
}

\ctikzset{annotation below/.code = {
        a=#1,
    \circuitikzbasekey/bipole/annotation/position=-90 }
}
\ctikzset{a_/.style = {
        a=#1,
    \circuitikzbasekey/bipole/annotation/position=-90 }
}

% This is to adjust spacing for the labels so that they are not cramped on components
\def\pgf@circ@ls{.75ex} % labelspace to have just one point to change

\def\pgf@circ@drawlabels#1{
    \pgfextra{
        % This function will be called with argument #1 equal
        % to "label" or "annotation" form pgfcircpath.tex.
        % pgf@circ@direction is the direction of the path,
        % its value is set in pgfcircpath.tex
        \pgfmathsubtract{\pgf@circ@direction}{90}
        \pgfmathround{\pgfmathresult} % avoid precision loss errors
        \edef\pgf@circ@labanc{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}

        \edef\pgf@circ@temp{\ctikzvalof{bipole/#1/position}}
        \ifnum \pgf@circ@temp < 0
                \pgfmathadd{\pgf@circ@labanc}{180}
                \edef\pgf@circ@labanc{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
        \fi
        \ifpgf@circuit@bipole@inverted
                \pgfmathadd{\pgf@circ@temp}{180} %If shape is inverted, use opposite anchor
                \edef\pgf@circ@temp{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
        \fi

        \ifnum \ctikzvalof{mirror value} = -1
                \pgfmathadd{\pgf@circ@temp}{180} %If shape is mirrored, use opposite anchor
                \edef\pgf@circ@temp{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
        \fi
    }
    %Firstly, place a coordinate directly at the edge of the shape
    (\ctikzvalof{bipole/name}.\pgf@circ@temp) coordinate (labelcoor)
    %now decide, which labels should be drawn
    \pgfextra{
            \edef\pgf@temp{\ctikzvalof{label/align}}
            \def\pgf@circ@temp{straight}
    }
    \ifx\pgf@temp\pgf@circ@temp %straight
            \pgf@circ@drawreglabels{#1}
    \else
            \pgfextra{\def\pgf@circ@temp{rotate}}
            \ifx\pgf@temp\pgf@circ@temp %rotate
                    \pgf@circ@drawrotlabels{#1}
            \else% smart
                    \pgf@circ@drawsmartlabels{#1}
            \fi
    \fi
}


\def\pgf@circ@drawsmartlabels#1{
    \pgfextra{
        \pgfmathmod{\pgf@circ@direction}{90}
        \edef\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
    }
    \ifnum \pgfcircmathresult > 20
    \ifnum \pgfcircmathresult < 70
        \pgf@circ@drawrotlabels{#1}
    \else
        \pgf@circ@drawreglabels{#1}
    \fi
    \else
        \pgf@circ@drawreglabels{#1}
    \fi
    }


\def\pgf@circ@drawrotlabels#1{
    \pgfextra{
        % scale the distances in function of zoom, so that they are not
        % dependent on it but on font size. Thanks to @marmot
        % https://tex.stackexchange.com/a/476018/38080
        % the coeffcient is adjusted so that the distance is more or less
        % the same for rotated labels and straight ones (although it will
        % depend on the font, so it's not exact).
        \pgfgettransformentries{\tmp}{\tmp}{\tmp}{\myscale}{\tmp}{\tmp}
        \pgfmathsetlength\pgf@circ@res@temp{1.5*\pgf@circ@ls/\myscale}
        \ifnum \ctikzvalof{bipole/#1/position}>0
        %we need some more space for placement below, due to mid-anchor
            \else % we do not have <= in \ifnum...
                \pgf@circ@res@temp=1.5\pgf@circ@res@temp
        \fi
        %Calculate rotation of the label from direction and strip decimals
        \edef\pgfcirclabrot{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
        % rotate the label at second or third quadrant:
        \ifnum \pgfcirclabrot > 90 \ifnum \pgfcirclabrot < 270
                \pgfmathsubtract{\pgf@circ@direction}{180}
                \edef\pgfcirclabrot{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
                %invert the space relationships due to rotated strings
                \ifnum \ctikzvalof{bipole/#1/position}>0
                        \pgf@circ@res@temp=1.5\pgf@circ@res@temp
                \fi
        \fi\fi
        \pgfmathparse{\ctikzvalof{bipole/#1/position}>0?\pgf@circ@direction+90:\pgf@circ@direction-90}
        \edef\pgf@circ@labposangle{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
    }
    % reset cm is not working correctly here
    (labelcoor)++(\pgf@circ@labposangle:\the\pgf@circ@res@temp) coordinate(labelcoor)
    node[anchor=mid, rotate=\pgfcirclabrot](\ctikzvalof{bipole/name}#1){\pgf@circ@finallabels{#1}}
}

\def\pgf@circ@drawreglabels#1{
    %Now calculate all shape positions
    %Use mid-anchor at x-axis and base-anchor at y-axis, respectively.
    %All points between will be addressed by angled-anchors:
    \pgfextra{
        % scale ex-distance to make it independent on scale
        % thanks @marmot see https://tex.stackexchange.com/a/476018/38080
        \pgfgettransformentries{\tmp}{\tmp}{\tmp}{\myscale}{\tmp}{\tmp}
        \pgfmathsetlength\pgf@circ@res@temp{\pgf@circ@ls/\myscale}
        \pgfmathadd{\pgf@circ@labanc}{90}
        \pgfmathround{\pgfmathresult}
        \def\pgf@circ@labanctext{\pgf@circ@labanc}
        \edef\pgf@circ@temp{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
        \pgfmathparse{mod(\pgf@circ@temp,180)>135?mod(\pgf@circ@temp,180)-180:mod(\pgf@circ@temp,180)}
        \edef\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgfmathresult\pgf@nil}
    }
    %Values around 90 are at both y-axis
    \ifnum \pgfcircmathresult > 84 \ifnum \pgfcircmathresult< 96
        \pgfextra{\edef\pgf@circ@labpos{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}}
        \ifnum \pgf@circ@labpos > 180
            \ifnum \ctikzvalof{bipole/#1/position} > 0
                    \pgfextra{\def\pgf@circ@labanctext{mid west}}
            \else
                    \pgfextra{\def\pgf@circ@labanctext{mid east}}
            \fi
        \else
            \ifnum \ctikzvalof{bipole/#1/position} > 0
                    \pgfextra{\def\pgf@circ@labanctext{mid east}}
            \else
                    \pgfextra{\def\pgf@circ@labanctext{mid west}}
            \fi
        \fi
    \fi\fi
    %Values between -5 and 5 are at pos /neg x-axis
    \pgfextra{\def\uffa{}\newdimen\realshift\realshift=\dimexpr1pt\relax}
        \ifnum \pgfcircmathresult <6 \ifnum \pgfcircmathresult > -6
            \ifnum \ctikzvalof{bipole/#1/position} < 0
                \ifnum \pgf@circ@labanc > 90
                    % using base coordinate instead of south to naturally align
                    % symbols with descendants; but this invalidate the effect of
                    % the inner sep, so recover it by shifting the anchor
                    % reset cm is not working sometime, use @marmot solution
                    % see https://tex.stackexchange.com/a/476018/38080
                    (labelcoor) ++(-\pgf@circ@labanc:\pgf@circ@res@temp) coordinate(labelcoor)
                    \pgfextra{\def\pgf@circ@labanctext{base}}%base
                \else
                    \pgfextra{\def\pgf@circ@labanctext{north}}%north
                \fi
             \else
                \ifnum \pgf@circ@labanc < 90
                    % shift, as above
                    (labelcoor) ++(-\pgf@circ@labanc:\pgf@circ@res@temp) coordinate(labelcoor)
                    \pgfextra{\def\pgf@circ@labanctext{base}}%base
                \else
                    \ifnum \pgf@circ@labanc > 180
                        % this shouldn't  happen, but somehow it does (270 degree anchors)
                        % shift, as above
                        (labelcoor) ++(-\pgf@circ@labanc:\pgf@circ@res@temp) coordinate(labelcoor)
                         \pgfextra{\def\pgf@circ@labanctext{base}}%base
                    \else
                      \pgfextra{\def\pgf@circ@labanctext{north}}%north
                   \fi
                \fi
            \fi
        \fi\fi
    (labelcoor) node[anchor=\pgf@circ@labanctext,
        inner sep=0.5\pgf@circ@res@temp, outer sep=0pt,
        ](\ctikzvalof{bipole/name}#1){\strut\pgf@circ@finallabels{#1}%
    }
}

\def\pgf@circ@finallabels#1{%
    \edef\pgf@temp{}%
    \edef\pgf@circ@temp{\ctikzvalof{bipole/#1/unit}}%
    \ifx\pgf@temp\pgf@circ@temp%
        \ctikzvalof{bipole/#1/name}%
    \else%
        $\SI{\ctikzvalof{bipole/#1/name}}{\ctikzvalof{bipole/#1/unit}}$%
    \fi%
}

\ctikzset{text/.style = { t=#1 } }
\ctikzset{t/.code = {
        \ctikzsetvalof{bipoles/twoport/text}{#1}
}}

%%%% Stacked labels
%
% stacked labels by Romano Giannetti romano@rgtti.com
% heavily based on Claudo Fiandrinos's https://tex.stackexchange.com/a/65792/38080
% \expandafter trick inspired by Matthew Leingang's https://tex.stackexchange.com/a/12272/38080
%
% labels are in a tabular, globally aligned:
%        vertically with key l2 valign (default c)
%        c: center t: top b: bottom
%        horizontally with key l2 align (default l)
%        l: left c: centered r: right
% you can switch sides using l2_=... and l2^=...
% syntax is l2_ = line1 and line2 (same for l2^)
%
\ctikzset{%
    l2 valign/.store in=\ltwo@valign, l2 valign=c,
    l2 halign/.store in=\ltwo@halign, l2 halign=l,
}
\ctikzset{l2base/.code n args={2}{
  \pgfkeys{/tikz/circuitikz/bipole/label/name=%
        \bgroup
        \setlength{\tabcolsep}{2pt}%
        \def\ltwo@tabu{\tabular[\ltwo@valign]}%
        \expandafter\ltwo@tabu\expandafter{\ltwo@halign}%
        #1\\ #2%
        \endtabular
        \egroup
    }%
    \ctikzsetvalof{bipole/label/unit}{}
    \ifpgf@circ@siunitx
        \pgf@circ@handleSI{#2}
        \ifpgf@circ@siunitx@res
            \edef\pgf@temp{\pgf@circ@handleSI@val}
            \pgfkeyslet{/tikz/circuitikz/bipole/label/name}{\pgf@temp}
            \edef\pgf@temp{\pgf@circ@handleSI@unit}
            \pgfkeyslet{/tikz/circuitikz/bipole/label/unit}{\pgf@temp}
        \else
        \fi
    \else
    \fi
}}
\ctikzset{l2/.style args={#1 and #2}{
        l2base={#1}{#2},
    \circuitikzbasekey/bipole/label/position=90 }
}
\ctikzset{l2 above/.style args={#1 and #2}{
        l2base={#1}{#2},
    \circuitikzbasekey/bipole/label/position=90 }
}
\ctikzset{l2^/.style args={#1 and #2}{
        l2base={#1}{#2},
    \circuitikzbasekey/bipole/label/position=90 }
}
\ctikzset{l2 below/.style args={#1 and #2}{
        l2base={#1}{#2},
    \circuitikzbasekey/bipole/label/position=-90 }
}
\ctikzset{l2_/.style args={#1 and #2}{
        l2base={#1}{#2},
    \circuitikzbasekey/bipole/label/position=-90 }
}

\endinput


==> pgfcircmonopoles.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the files gpl-3.0_license.txt and lppl-1-3c_license.txt for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Monopoles

%% Ground symbol
% #1 -> name
% #2 -> width
% #3 -> depth
% #4 -> code
\long\def\pgf@circ@declareground#1#2#3#4{
    \pgfdeclareshape{#1}{
        \savedanchor{\southeast}{
            \pgf@x=\ctikzvalof{monopoles/ground/width}\pgf@circ@Rlen
            \pgf@x=#2\pgf@x
            \pgf@y=\ctikzvalof{monopoles/ground/width}\pgf@circ@Rlen
            \pgf@y=-#3\pgf@y
        }
        \anchor{north}{\pgfpointorigin}
        \anchor{north east}{\southeast\pgf@y=0pt\relax}
        \anchor{east}{\southeast\pgf@y=.5\pgf@y}
        \anchor{south east}{\southeast}
        \anchor{south}{\southeast\pgf@x=0pt\relax}
        \anchor{south west}{\southeast\pgf@x=-\pgf@x}
        \anchor{west}{\southeast\pgf@y=.5\pgf@y\pgf@x=-\pgf@x}
        \anchor{north west}{\southeast\pgf@y=0pt\pgf@x=-\pgf@x}
        \anchor{left}{\pgfpointorigin}
        \anchor{right}{\pgfpointorigin}
        \anchor{center}{\pgfpointorigin}
        \behindforegroundpath{
            \pgf@circ@res@step=\ctikzvalof{monopoles/ground/width}\pgf@circ@Rlen
            \pgfscope
                \pgfstartlinewidth=\pgflinewidth
                #4
            \endpgfscope
        }
    }
}


\pgf@circ@declareground{ground}{0.6}{1.6}{
    \pgfsetlinewidth{\ctikzvalof{monopoles/ground/connectionthickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpoint{0pt}{-1.2\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgfsetlinewidth{\ctikzvalof{monopoles/ground/thickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-.6\pgf@circ@res@step}{-1.2\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@step}{-1.2\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{-.4\pgf@circ@res@step}{-1.4\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@step}{-1.4\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{-.25\pgf@circ@res@step}{-1.6\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.25\pgf@circ@res@step}{-1.6\pgf@circ@res@step}}
    \pgfusepath{draw}
}



\pgf@circ@declareground{rground}{0.6}{1}{
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfstartlinewidth=\pgflinewidth
    \pgfsetlinewidth{\ctikzvalof{monopoles/rground/thickness}\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{-.6\pgf@circ@res@step}{-\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@step}{-\pgf@circ@res@step}}
    \pgfsetroundcap\pgfusepath{draw}
}

\pgf@circ@declareground{tground}{0.6}{0}{
    \pgfpathmoveto{\pgfpointorigin}
    \pgfusepath{draw}

    \pgfstartlinewidth=\pgflinewidth
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/monopoles/tground/thickness}\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{-.6\pgf@circ@res@step}{0pt}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@step}{0pt}}
    \pgfusepath{draw}
}

\pgf@circ@declareground{sground}{0.6}{1.8}{
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfstartlinewidth=\pgflinewidth
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{-.6\pgf@circ@res@step}{-\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@step}{-\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{0}{-1.8\pgf@circ@res@step}}
    \pgfpathclose
    \pgf@circ@draworfill
}

% noiseless ground
\pgf@circ@declareground{nground}{0.9}{1.6}{
    \pgfsetlinewidth{\ctikzvalof{monopoles/ground/connectionthickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpoint{0pt}{-1.2\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgfsetlinewidth{\ctikzvalof{monopoles/ground/thickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-.6\pgf@circ@res@step}{-1.2\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@step}{-1.2\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{-.4\pgf@circ@res@step}{-1.4\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@step}{-1.4\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{-.25\pgf@circ@res@step}{-1.6\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.25\pgf@circ@res@step}{-1.6\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.9\pgf@circ@res@step}{-1.6\pgf@circ@res@step}}
    \pgfpatharc{0}{180}{0.9\pgf@circ@res@step}
    \pgfusepath{draw}
}

% protective ground
\pgf@circ@declareground{pground}{0.9}{1.8}{
    \pgfsetlinewidth{\ctikzvalof{monopoles/ground/connectionthickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpoint{0pt}{-1\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgfsetlinewidth{\ctikzvalof{monopoles/ground/thickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-.6\pgf@circ@res@step}{-1\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.6\pgf@circ@res@step}{-1\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{-.4\pgf@circ@res@step}{-1.2\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@step}{-1.2\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{-.25\pgf@circ@res@step}{-1.4\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.25\pgf@circ@res@step}{-1.4\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgfpathcircle{\pgfpoint{0pt}{-0.9\pgf@circ@res@step}}{0.9\pgf@circ@res@step}
    \pgfusepath{draw}
}

% chassis ground
\pgf@circ@declareground{cground}{1}{2}{
    \pgfsetlinewidth{\ctikzvalof{monopoles/ground/connectionthickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpoint{0pt}{-1.5\pgf@circ@res@step}}
    \pgfusepath{draw}
    \pgfsetlinewidth{\ctikzvalof{monopoles/ground/thickness}\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-1.00\pgf@circ@res@step}{-2.10\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{-0.75\pgf@circ@res@step}{-1.50\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{ 0.75\pgf@circ@res@step}{-1.50\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{ 0.50\pgf@circ@res@step}{-2.10\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{ 0.00\pgf@circ@res@step}{-1.50\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{-0.25\pgf@circ@res@step}{-2.10\pgf@circ@res@step}}
    \pgfusepath{draw}
}

% Contributed by @fotesan https://github.com/fotesan

\pgf@circ@declareground{eground}{1.1}{1.7}{
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfstartlinewidth=\pgflinewidth
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/monopoles/tground/thickness}\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{-1\pgf@circ@res@step}{-\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{1\pgf@circ@res@step}{-\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-1.1\pgf@circ@res@step}{-1.7\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{-.6\pgf@circ@res@step}{-1\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{-.6\pgf@circ@res@step}{-1.7\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{-.1\pgf@circ@res@step}{-1\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{-.1\pgf@circ@res@step}{-1.7\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@step}{-1\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{.4\pgf@circ@res@step}{-1.7\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.9\pgf@circ@res@step}{-1\pgf@circ@res@step}}
    \pgfusepath{draw}
}

\pgf@circ@declareground{eground2}{1.1}{1.7}{
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfstartlinewidth=\pgflinewidth
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/monopoles/tground/thickness}\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{-1\pgf@circ@res@step}{-\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{1\pgf@circ@res@step}{-\pgf@circ@res@step}}
    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{-1.1\pgf@circ@res@step}{-1.7\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{-.4\pgf@circ@res@step}{-1\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{-.45\pgf@circ@res@step}{-1.7\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.25\pgf@circ@res@step}{-1\pgf@circ@res@step}}
    \pgfpathmoveto{\pgfpoint{.2\pgf@circ@res@step}{-1.7\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{.9\pgf@circ@res@step}{-1\pgf@circ@res@step}}
    \pgfusepath{draw}
}

% Contributed by Leonardo Azzinnari
\pgfdeclareshape{tlinestub}{
    \savedanchor{\northeast}{%
        \pgf@circ@res@step = \ctikzvalof{bipoles/tline/width} \pgf@circ@Rlen
        \pgf@x=1.625\pgf@circ@res@step
        \pgf@circ@res@step = \ctikzvalof{bipoles/tline/width} \pgf@circ@Rlen
        \pgf@y=.25\pgf@circ@res@step%
    }
    % the center is on the left side of the shape for facility of usage
    \anchor{north}{\northeast\pgf@x=0.5\pgf@x\relax}
    \anchor{east}{\northeast\pgf@y=0cm\relax}
    \anchor{south}{\northeast\pgf@y=-\pgf@y \pgf@x=0.5\pgf@x\relax}
    \anchor{west}{\pgfpointorigin}
    \anchor{north east}{\northeast}
    \anchor{north west}{\northeast\pgf@x=0cm\relax}
    \anchor{south east}{\northeast\pgf@y=-\pgf@y}
    \anchor{south west}{\northeast\pgf@x=0cm\pgf@y=-\pgf@y}
    \anchor{center}{\pgfpointorigin}
    \behindforegroundpath{
        \pgfstartlinewidth=\pgflinewidth

        \pgf@circ@res@step=\ctikzvalof{bipoles/tline/width} \pgf@circ@Rlen

        \pgfscope\begin{pgftransparencygroup}
            \pgfpathellipse{\pgfpoint{0.5\pgf@circ@res@step}{0\pgf@circ@res@step}}{\pgfpoint{0.125\pgf@circ@res@step}{0\pgf@circ@res@step}}{\pgfpoint{0\pgf@circ@res@step}{0.25\pgf@circ@res@step}}
            \pgf@circ@maybefill
            \pgfpathmoveto{\pgfpoint{0.5\pgf@circ@res@step}{0.25\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{1.5\pgf@circ@res@step}{0.25\pgf@circ@res@step}}
            \pgfpatharc{90}{-90}{0.125\pgf@circ@res@step and 0.25\pgf@circ@res@step}
            \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@step}{-0.25\pgf@circ@res@step}}
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
            \pgf@circ@draworfill
            \pgfpathellipse{\pgfpoint{0.5\pgf@circ@res@step}{0\pgf@circ@res@step}}{\pgfpoint{0.125\pgf@circ@res@step}{0\pgf@circ@res@step}}{\pgfpoint{0\pgf@circ@res@step}{0.25\pgf@circ@res@step}}
            \pgfusepath{draw}
        \end{pgftransparencygroup} \endpgfscope
        \pgfpathmoveto{\pgfpointorigin}
        \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@step}{0pt}}
        \pgfusepath{draw}
    }
}

%% New antennas without tails

% main body
\def\pgf@circ@antennabody{%
    \pgfstartlinewidth=\pgflinewidth
    \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
    \pgf@circ@res@step=\ctikzvalof{monopoles/bareantenna/width}\pgf@circ@Rlen
    \pgfscope
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
        \pgfpathmoveto{\pgfpointorigin}
        \pgfpathlineto{\pgfpoint{-\pgf@circ@res@step}{2\pgf@circ@res@step}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{2\pgf@circ@res@step}}
        \pgfsetbeveljoin
        \pgfpathclose
        \pgf@circ@draworfill
    \endpgfscope
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpoint{0pt}{2\pgf@circ@res@step}}
    \pgfusepath{draw}
}

% Waves for the antennas.
\def\pgf@circ@antennawaves{%
    \pgfscope
    % define a triangle for clipping the waves
    \pgfpathmoveto{\pgfpoint{0pt}{\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{4.2\pgf@circ@res@step}{3\pgf@circ@res@step}}
    \pgfpathlineto{\pgfpoint{4.2\pgf@circ@res@step}{-1\pgf@circ@res@step}}
    \pgfpathclose
    \pgfusepath{clip}
    % ...and build the waves as clipped circles
    \c@pgf@counta=8\pgf@circ@res@other=0.5\pgf@circ@res@step
    \pgfmathloop%
    \ifnum\c@pgf@counta>2
        \pgfpathcircle{\pgfpoint{0pt}{\pgf@circ@res@step}}{\the\c@pgf@counta*\pgf@circ@res@other}
        \advance\c@pgf@counta-1\relax%
        \repeatpgfmathloop
        \pgfusepath{draw}
    \endpgfscope
}


% additional shape with the waves
\pgfdeclareshape{waves}{
    \anchor{center}{\pgfpointorigin}
    \savedanchor{\northeast}{
        \pgf@circ@res@step=\ctikzvalof{monopoles/waves/width}\pgf@circ@Rlen
        \pgf@x=\pgf@circ@res@step
        \pgf@y=\pgf@circ@res@step
    }
    \anchor{text}{
        \northeast
        \pgf@y=\dimexpr\pgf@y+.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox\relax
    }
    \anchor{top}{\northeast\pgf@x=0pt}
    \anchor{right}{\northeast\pgf@y=0pt}
    \anchor{left}{\northeast\pgf@x=-\pgf@x\pgf@y=0pt}
    \anchor{bottom}{\northeast\pgf@y=-\pgf@y\pgf@x=0pt}
    \anchor{north}{\northeast\pgf@x=0pt}
    \anchor{north east}{\northeast}
    \anchor{east}{\northeast\pgf@y=0pt}
    \anchor{south east}{\northeast\pgf@y=-\pgf@y}
    \anchor{south}{\northeast\pgf@y=-\pgf@y\pgf@x=0pt}
    \anchor{south west}{\northeast\pgf@y=-\pgf@y\pgf@x=-\pgf@x}
    \anchor{west}{\northeast\pgf@x=-\pgf@x\pgf@y=0pt}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x}
    \behindforegroundpath{
        \pgf@circ@res@step=\ctikzvalof{monopoles/waves/width}\pgf@circ@Rlen
        \pgf@circ@res@step=0.5\pgf@circ@res@step
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
        \pgfscope
        % define a triangle for clipping the waves
        \pgfpathmoveto{\pgfpoint{-2\pgf@circ@res@step}{0pt}}
        \pgfpathlineto{\pgfpoint{2.1\pgf@circ@res@step}{2\pgf@circ@res@step}}
        \pgfpathlineto{\pgfpoint{2.1\pgf@circ@res@step}{-2\pgf@circ@res@step}}
        \pgfpathclose
        \pgfusepath{clip}
        % ...and build the waves as clipped circles
        \c@pgf@counta=8\pgf@circ@res@other=0.5\pgf@circ@res@step
        \pgfmathloop%
        \ifnum\c@pgf@counta>1
            \pgfpathcircle{\pgfpoint{-2\pgf@circ@res@step}{0pt}}{\the\c@pgf@counta*\pgf@circ@res@other}
            \advance\c@pgf@counta-1\relax%
            \repeatpgfmathloop
            \pgfusepath{draw}
        \endpgfscope
    }
}

% the three types of antennas: simple, TX, RX. Notice that you can flip them...

\pgfdeclareshape{bareantenna}{
    \anchor{center}{\pgfpointorigin}
    \savedanchor{\northeast}{
        \pgf@circ@res@step=\ctikzvalof{monopoles/bareantenna/width}\pgf@circ@Rlen
        \pgf@x=\pgf@circ@res@step
        \pgf@y=2\pgf@circ@res@step
    }
    \anchor{text}{
        \northeast
        \pgf@x=\ctikzvalof{monopoles/bareantenna/label/xanchor}\pgf@x
        \pgf@y=\ctikzvalof{monopoles/bareantenna/label/yanchor}\pgf@y
        \pgf@y=\dimexpr\pgf@y+.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox\relax
    }
    \anchor{top}{\northeast\pgf@x=0pt}
    \anchor{right}{\northeast\pgf@y=0.5\pgf@y}
    \anchor{left}{\northeast\pgf@x=-\pgf@x\pgf@y=0.5\pgf@y}
    \anchor{bottom}{\pgfpointorigin}
    \anchor{north}{\northeast\pgf@x=0pt}
    \anchor{east}{\northeast\pgf@y=0.5\pgf@y}
    \anchor{west}{\northeast\pgf@x=-\pgf@x\pgf@y=0.5\pgf@y}
    \anchor{south}{\pgfpointorigin}
    \anchor{north east}{\northeast}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x}
    \anchor{south east}{\northeast\pgf@y=0pt\relax}
    \anchor{south west}{\northeast\pgf@y=0pt\pgf@x=-\pgf@x}
    \behindforegroundpath{
        \pgf@circ@antennabody
    }
}

\pgfdeclareshape{bareTXantenna}{
    \anchor{center}{\pgfpointorigin}
    \savedanchor{\northeast}{
        \pgf@circ@res@step=\ctikzvalof{monopoles/bareantenna/width}\pgf@circ@Rlen
        \pgf@x=\pgf@circ@res@step
        \pgf@y=2\pgf@circ@res@step
    }
    \anchor{text}{
        \northeast
        \pgf@x=\ctikzvalof{monopoles/bareantenna/label/xanchor}\pgf@x
        \pgf@y=\ctikzvalof{monopoles/bareantenna/label/yanchor}\pgf@y
        \pgf@x=\dimexpr-\pgf@x-\wd\pgfnodeparttextbox\relax
        \pgf@y=\dimexpr\pgf@y+.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox\relax
    }
    \anchor{waves}{
        \northeast
        \pgf@circ@res@step=\ctikzvalof{monopoles/bareantenna/width}\pgf@circ@Rlen
        \pgf@x=4.2\pgf@circ@res@step
        \pgf@y=\pgf@circ@res@step
    }
    \anchor{top}{\northeast\pgf@x=0pt}
    \anchor{right}{\northeast\pgf@y=0.5\pgf@y}
    \anchor{left}{\northeast\pgf@x=-\pgf@x\pgf@y=0.5\pgf@y}
    \anchor{bottom}{\pgfpointorigin}
    \anchor{north}{\northeast\pgf@x=0pt}
    \anchor{east}{\northeast\pgf@y=0.5\pgf@y}
    \anchor{west}{\northeast\pgf@x=-\pgf@x\pgf@y=0.5\pgf@y}
    \anchor{south}{\pgfpointorigin}
    \anchor{north east}{\northeast}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x}
    \anchor{south east}{\northeast\pgf@y=0pt\relax}
    \anchor{south west}{\northeast\pgf@y=0pt\pgf@x=-\pgf@x}
    \behindforegroundpath{
        \pgf@circ@antennabody
        \pgf@circ@antennawaves
    }
}

\pgfdeclareshape{bareRXantenna}{
    \anchor{center}{\pgfpointorigin}
    \savedanchor{\northeast}{
        \pgf@circ@res@step=\ctikzvalof{monopoles/bareantenna/width}\pgf@circ@Rlen
        \pgf@x=\pgf@circ@res@step
        \pgf@y=2\pgf@circ@res@step
    }
    \anchor{text}{
        \northeast
        \pgf@x=\ctikzvalof{monopoles/bareantenna/label/xanchor}\pgf@x
        \pgf@y=\ctikzvalof{monopoles/bareantenna/label/yanchor}\pgf@y
        \pgf@y=\dimexpr\pgf@y+.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox\relax
    }
    \anchor{waves}{
        \northeast
        \pgf@circ@res@step=\ctikzvalof{monopoles/bareantenna/width}\pgf@circ@Rlen
        \pgf@x=-4.2\pgf@circ@res@step
        \pgf@y=\pgf@circ@res@step
    }
    \anchor{top}{\northeast\pgf@x=0pt}
    \anchor{right}{\northeast\pgf@y=0.5\pgf@y}
    \anchor{left}{\northeast\pgf@x=-\pgf@x\pgf@y=0.5\pgf@y}
    \anchor{bottom}{\pgfpointorigin}
    \anchor{north}{\northeast\pgf@x=0pt}
    \anchor{east}{\northeast\pgf@y=0.5\pgf@y}
    \anchor{west}{\northeast\pgf@x=-\pgf@x\pgf@y=0.5\pgf@y}
    \anchor{south}{\pgfpointorigin}
    \anchor{north east}{\northeast}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x}
    \anchor{south east}{\northeast\pgf@y=0pt\relax}
    \anchor{south west}{\northeast\pgf@y=0pt\pgf@x=-\pgf@x}
    \behindforegroundpath{
        \pgf@circ@antennabody
        \pgftransformxshift{-5.2\pgf@circ@res@step}
        \pgf@circ@antennawaves
    }
}

% Microstrip monopoles

\pgfdeclareshape{mslstub}{
    \savedanchor{\southeast}{
        \pgf@x=\ctikzvalof{bipoles/mstline/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
        \pgf@y=\ctikzvalof{bipoles/mstline/height}\pgf@circ@Rlen
        \pgf@y=-.5\pgf@y
    }
    \savedanchor{\northwest}{
        \pgf@x=\ctikzvalof{bipoles/mstline/width}\pgf@circ@Rlen
        \pgf@x=-.5\pgf@x
        \pgf@y=\ctikzvalof{bipoles/mstline/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
    }
    \anchor{north}{\northwest\pgf@x=0pt\relax}
    \anchor{north east}{\northwest\pgf@x=-\pgf@x}
    \anchor{east}{\southeast\pgf@y=0pt\relax}
    \anchor{south east}{\southeast}
    \anchor{south}{\southeast\pgf@x=0pt\relax}
    \anchor{south west}{\southeast\pgf@x=-\pgf@x}
    \anchor{west}{\northwest\pgf@y=0pt\relax}
    \anchor{north west}{\northwest}
    %
    \anchor{center}{\northwest\pgf@y=0pt\relax}
    \anchor{left}{\northwest\pgf@y=0pt\relax}
    \anchor{right}{\southeast\pgf@y=0pt\relax}
    % put the node text above and centered
    \anchor{text}{\pgfextracty{\pgf@circ@res@up}{\northwest}
        \pgfpoint{-.5\wd\pgfnodeparttextbox}{
            \dimexpr.5\dp\pgfnodeparttextbox+.5\ht\pgfnodeparttextbox+\pgf@circ@res@up\relax
        }
    }
    \behindbackgroundpath{
        \pgfextracty{\pgf@circ@res@up}{\northwest}
        \pgfextractx{\pgf@circ@res@right}{\southeast}
        \pgfextractx{\pgf@circ@res@left}{\northwest}
        \pgfextracty{\pgf@circ@res@down}{\southeast}
        \pgfmathsetlength{\pgf@circ@res@step}{0.25*\pgf@circ@res@up}
        \pgfstartlinewidth=\pgflinewidth
        \pgfscope
            \pgfsetlinewidth{\ctikzvalof{bipoles/thickness}\pgfstartlinewidth}
            \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \pgf@circ@draworfill
        \endpgfscope
    }
}

\pgfdeclareshape{msrstub}{
    \savedanchor{\southeast}{
        \pgf@x=\ctikzvalof{monopoles/msrstub/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
        \pgf@y=0pt\relax
    }
    \savedanchor{\northwest}{
        \pgf@x=\ctikzvalof{monopoles/msrstub/width}\pgf@circ@Rlen
        \pgf@x=-.5\pgf@x
        \pgf@y=\ctikzvalof{monopoles/msrstub/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
    }
    \anchor{north}{\northwest\pgf@x=0pt\relax}
    \anchor{north east}{\northwest\pgf@x=-\pgf@x}
    \anchor{east}{\southeast\pgf@y=0pt\relax}
    \anchor{south east}{\southeast}
    \anchor{south}{\southeast\pgf@x=0pt\relax}
    \anchor{south west}{\southeast\pgf@x=-\pgf@x}
    \anchor{west}{\northwest\pgf@y=0pt\relax}
    \anchor{north west}{\northwest}
    %
    \anchor{center}{\pgfpointorigin}
    \anchor{left}{\pgfpointorigin}
    \anchor{right}{\pgfpointorigin}
    % put the node text above and centered
    \anchor{text}{\pgfextracty{\pgf@circ@res@up}{\northwest}
        \pgfpoint{-.5\wd\pgfnodeparttextbox}{
            \dimexpr.5\dp\pgfnodeparttextbox+.5\ht\pgfnodeparttextbox+\pgf@circ@res@up\relax
        }
    }
    \behindbackgroundpath{
        \pgfextracty{\pgf@circ@res@up}{\northwest}
        \pgfextractx{\pgf@circ@res@right}{\southeast}
        \pgfextractx{\pgf@circ@res@left}{\northwest}
        \pgfextracty{\pgf@circ@res@down}{\southeast}
        \pgfmathsetlength{\pgf@circ@res@step}{0.25*\pgf@circ@res@up}
        \pgfstartlinewidth=\pgflinewidth
        \pgfscope
            \pgfpathmoveto{\pgfpointorigin}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@step}}
            \pgfusepath{draw}
            \pgfsetlinewidth{\ctikzvalof{bipoles/thickness}\pgfstartlinewidth}
            \pgfpathmoveto{\pgfpointpolar{135}{\pgf@circ@res@step}}
            \pgfpatharc{135}{45}{\pgf@circ@res@step}
            \pgfpathlineto{\pgfpointpolar{45}{\pgf@circ@res@up}}
            \pgfpatharc{45}{135}{\pgf@circ@res@up}
            \pgfclosepath
            % \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \pgf@circ@draworfill
        \endpgfscope
    }
}

\pgfdeclareshape{msport}{
    \savedanchor{\southeast}{
        \pgf@x=\ctikzvalof{monopoles/msport/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
        \pgf@y=\ctikzvalof{bipoles/mstline/height}\pgf@circ@Rlen
        \pgf@y=-.5\pgf@y
    }
    \savedanchor{\northwest}{
        \pgf@x=\ctikzvalof{monopoles/msport/width}\pgf@circ@Rlen
        \pgf@x=-.5\pgf@x
        \pgf@y=\ctikzvalof{bipoles/mstline/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
    }
    \anchor{north}{\northwest\pgf@x=0pt\relax}
    \anchor{north east}{\northwest\pgf@x=-\pgf@x}
    \anchor{east}{\southeast\pgf@y=0pt\relax}
    \anchor{south east}{\southeast}
    \anchor{south}{\southeast\pgf@x=0pt\relax}
    \anchor{south west}{\southeast\pgf@x=-\pgf@x}
    \anchor{west}{\northwest\pgf@y=0pt\relax}
    \anchor{north west}{\northwest}
    %
    \anchor{center}{\northwest\pgf@y=0pt\relax}
    \anchor{left}{\northwest\pgf@y=0pt\relax}
    \anchor{right}{\southeast\pgf@y=0pt\relax}
    % put the node text above and centered
    \anchor{text}{\pgfextracty{\pgf@circ@res@up}{\northwest}
        \pgfpoint{-.5\wd\pgfnodeparttextbox}{
            \dimexpr-.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox\relax
        }
    }
    \behindbackgroundpath{
        \pgfextracty{\pgf@circ@res@up}{\northwest}
        \pgfextractx{\pgf@circ@res@right}{\southeast}
        \pgfextractx{\pgf@circ@res@left}{\northwest}
        \pgfextracty{\pgf@circ@res@down}{\southeast}
        \pgfmathsetlength{\pgf@circ@res@step}{0.5*\pgf@circ@res@up}
        \pgfstartlinewidth=\pgflinewidth
        \pgfscope
            \pgfsetlinewidth{\ctikzvalof{bipoles/thickness}\pgfstartlinewidth}
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@left+\pgf@circ@res@step}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@left+\pgf@circ@res@step}{\pgf@circ@res@down}}
            \pgfpathclose
            \pgf@circ@draworfill
        \endpgfscope
    }
}
% Legacy antennas (with tails)

\def\pgf@circ@shift@antenna@xy#1#2{%
    \pgf@circ@res@step=\ctikzvalof{monopoles/antenna/width}\pgf@circ@Rlen
    \pgf@y=\dimexpr\pgf@y+#2\pgf@circ@res@step
    \pgf@x=\dimexpr\pgf@x+#1\pgf@circ@res@step
\relax}

\pgfdeclareshape{antenna}{
    \anchor{center}{\pgfpointorigin}
    \savedanchor{\northeast}{
        \pgf@circ@res@step=\ctikzvalof{monopoles/antenna/width}\pgf@circ@Rlen
        \pgf@x=\pgf@circ@res@step%-0.5\pgflinewidth
        \pgf@y=4\pgf@circ@res@step
    }
    \anchor{north}{\northeast\pgf@x=0cm\pgf@circ@shift@antenna@xy{0}{2}}
    \anchor{east}{\northeast\pgf@y=0cm\pgf@circ@shift@antenna@xy{0}{3}\relax}
    \anchor{south}{\northeast\pgf@y=-\pgf@y \pgf@x=0cm\pgf@circ@shift@antenna@xy{0}{4}\relax}
    \anchor{west}{\northeast\pgf@y=0cm\pgf@x=-\pgf@x\pgf@circ@shift@antenna@xy{0}{3}}
    \anchor{north east}{\northeast\pgf@circ@shift@antenna@xy{0}{2}}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x\pgf@circ@shift@antenna@xy{0}{2}}
    \anchor{south east}{\northeast\pgf@y=-\pgf@y\pgf@circ@shift@antenna@xy{0}{4}}
    \anchor{south west}{\northeast\pgf@y=-\pgf@y\pgf@x=-\pgf@x\pgf@circ@shift@antenna@xy{0}{4}}
    \anchor{text}{
        \northeast
        \pgf@x=\ctikzvalof{monopoles/antenna/label/xanchor}\pgf@x
        \pgf@y=\ctikzvalof{monopoles/antenna/label/yanchor}\pgf@y
    }
    \behindforegroundpath{
        \pgfstartlinewidth=\pgflinewidth
        \pgf@circ@res@step=\ctikzvalof{monopoles/antenna/width}\pgf@circ@Rlen

        \pgftransformxshift{ -4\pgf@circ@res@step }

        \pgfpathmoveto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{0pt}}
        \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}

        \pgfusepath{draw}

        \pgfscope
            \pgfpathmoveto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{5\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{4\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{3\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
            \pgfusepath{draw}
        \endpgfscope
        \pgfsetlinewidth{\pgfstartlinewidth}

    }
}


\pgfdeclareshape{txantenna}{
    \anchor{center}{\pgfpointorigin}
    \savedanchor{\northeast}{
        \pgf@circ@res@step=\ctikzvalof{monopoles/antenna/width}\pgf@circ@Rlen
        \pgf@x=\pgf@circ@res@step%-0.5\pgflinewidth
        \pgf@y=4\pgf@circ@res@step
    }
    \anchor{north}{\northeast\pgf@x=0cm\pgf@circ@shift@antenna@xy{2}{2}}
    \anchor{east}{\northeast\pgf@y=0cm\pgf@circ@shift@antenna@xy{4}{3}\relax}
    \anchor{south}{\northeast\pgf@y=-\pgf@y \pgf@x=0cm\pgf@circ@shift@antenna@xy{2}{4}\relax}
    \anchor{west}{\northeast\pgf@y=0cm\pgf@x=-\pgf@x\pgf@circ@shift@antenna@xy{1}{3}}
    \anchor{north east}{\northeast\pgf@circ@shift@antenna@xy{4}{2}}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x\pgf@circ@shift@antenna@xy{1}{2}}
    \anchor{south east}{\northeast\pgf@y=-\pgf@y\pgf@circ@shift@antenna@xy{4}{4}}
    \anchor{south west}{\northeast\pgf@y=-\pgf@y\pgf@x=-\pgf@x\pgf@circ@shift@antenna@xy{1}{4}}
    \anchor{text}{
        \northeast
        \pgf@x=\ctikzvalof{monopoles/txantenna/label/xanchor}\pgf@x
        \pgf@y=\ctikzvalof{monopoles/txantenna/label/yanchor}\pgf@y
    }
    \behindforegroundpath{
        \pgfstartlinewidth=\pgflinewidth
        \pgf@circ@res@step=\ctikzvalof{monopoles/txantenna/width}\pgf@circ@Rlen

        \pgfpathmoveto{\pgfpointorigin}
        \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step}{0pt}}
        \pgfpathmoveto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{0pt}}
        \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}

        \pgfusepath{draw}

        \pgfscope
            \pgfpathmoveto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{5\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{4\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{3\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
            \pgfusepath{draw}
        \endpgfscope
        \pgfpathmoveto{\pgfpoint{5.5\pgf@circ@res@step}{6\pgf@circ@res@step}}
        %        \pgfpatharc{60}{-60}{\pgf@circ@res@step and \pgf@circ@res@step}
        \pgfpatharc{30}{-30}{2\pgf@circ@res@step}         \pgfpathmoveto{\pgfpoint{6\pgf@circ@res@step}{6.25\pgf@circ@res@step}}
        \pgfpatharc{30}{-30}{2.5\pgf@circ@res@step}
        \pgfpathmoveto{\pgfpoint{6.5\pgf@circ@res@step}{6.5\pgf@circ@res@step}}
        \pgfpatharc{30}{-30}{3\pgf@circ@res@step}
        \pgfpathmoveto{\pgfpoint{7\pgf@circ@res@step}{6.75\pgf@circ@res@step}}
        \pgfpatharc{30}{-30}{3.5\pgf@circ@res@step}
        \pgfpathmoveto{\pgfpoint{7.5\pgf@circ@res@step}{7\pgf@circ@res@step}}
        \pgfpatharc{30}{-30}{4\pgf@circ@res@step}
        \pgfusepath{draw}
        \pgfsetlinewidth{\pgfstartlinewidth}

    }
}


\pgfdeclareshape{rxantenna}{
    \anchor{center}{\pgfpointorigin}
    \savedanchor{\northeast}{
        \pgf@circ@res@step=\ctikzvalof{monopoles/antenna/width}\pgf@circ@Rlen
        \pgf@x=\pgf@circ@res@step%-0.5\pgflinewidth
        \pgf@y=4\pgf@circ@res@step
    }
    \anchor{north}{\northeast\pgf@x=0cm\pgf@circ@shift@antenna@xy{2}{2}}
    \anchor{east}{\northeast\pgf@y=0cm\pgf@circ@shift@antenna@xy{4}{3}\relax}
    \anchor{south}{\northeast\pgf@y=-\pgf@y \pgf@x=0cm\pgf@circ@shift@antenna@xy{2}{4}\relax}
    \anchor{west}{\northeast\pgf@y=0cm\pgf@x=-\pgf@x\pgf@circ@shift@antenna@xy{1}{3}}
    \anchor{north east}{\northeast\pgf@circ@shift@antenna@xy{4}{2}}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x\pgf@circ@shift@antenna@xy{1}{2}}
    \anchor{south east}{\northeast\pgf@y=-\pgf@y\pgf@circ@shift@antenna@xy{4}{4}}
    \anchor{south west}{\northeast\pgf@y=-\pgf@y\pgf@x=-\pgf@x\pgf@circ@shift@antenna@xy{1}{4}}
    \anchor{text}{
        \northeast
        \pgf@x=\ctikzvalof{monopoles/rxantenna/label/xanchor}\pgf@x
        \pgf@y=\ctikzvalof{monopoles/rxantenna/label/yanchor}\pgf@y
    }
    \behindforegroundpath{
        \pgfstartlinewidth=\pgflinewidth
        \pgf@circ@res@step=\ctikzvalof{monopoles/rxantenna/width}\pgf@circ@Rlen

        \pgfpathmoveto{\pgfpointorigin}
        \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step}{0pt}}
        \pgfpathmoveto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{0pt}}
        \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}

        \pgfusepath{draw}

        \pgfscope
            \pgfpathmoveto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{5\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{4\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{3\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{4\pgf@circ@res@step-0.5\pgflinewidth}{6\pgf@circ@res@step}}
            \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
            \pgfusepath{draw}
        \endpgfscope

        \pgfpathmoveto{\pgfpoint{6\pgf@circ@res@step}{7\pgf@circ@res@step}}
        %             \pgfpatharc{60}{-60}{\pgf@circ@res@step and \pgf@circ@res@step}
        \pgfpatharc{150}{210}{4\pgf@circ@res@step}              \pgfpathmoveto{\pgfpoint{6.5\pgf@circ@res@step}{6.75\pgf@circ@res@step}}
        \pgfpatharc{150}{210}{3.5\pgf@circ@res@step}
        \pgfpathmoveto{\pgfpoint{7\pgf@circ@res@step}{6.5\pgf@circ@res@step}}
        \pgfpatharc{150}{210}{3\pgf@circ@res@step}
        \pgfpathmoveto{\pgfpoint{7.5\pgf@circ@res@step}{6.25\pgf@circ@res@step}}
        \pgfpatharc{150}{210}{2.5\pgf@circ@res@step}
        \pgfpathmoveto{\pgfpoint{8\pgf@circ@res@step}{6\pgf@circ@res@step}}
        \pgfpatharc{150}{210}{2\pgf@circ@res@step}
        \pgfusepath{draw}
        \pgfsetlinewidth{\pgfstartlinewidth}

    }
}

% Vcc
\pgfdeclareshape{vcc}{
    \savedanchor{\northeast}{%
        \pgf@circ@res@step=\ctikzvalof{monopoles/vcc/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@circ@res@step
        \pgf@y=3\pgf@x%
    }
    \anchor{north}{\northeast\pgf@x=0cm\relax}
    \anchor{east}{\northeast\pgf@y=0.5\pgf@y\relax}
    \anchor{south}{\pgfpointorigin}
    \anchor{west}{\northeast\pgf@y=0.5\pgf@y\pgf@x=-\pgf@x}
    \anchor{north east}{\northeast}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x}
    \anchor{south east}{\northeast\pgf@y=0pt\relax}
    \anchor{south west}{\northeast\pgf@y=0pt\pgf@x=-\pgf@x}
    \anchor{center}{\pgfpointorigin}
    \anchor{text}{
        \pgf@circ@res@step=\ctikzvalof{monopoles/vcc/width}\pgf@circ@Rlen
        \pgfpathmoveto{\pgfpoint{-.5\wd\pgfnodeparttextbox}{2\pgf@circ@res@step+2\ht\pgfnodeparttextbox}}
        \pgfpathmoveto{\pgfpoint{.5\wd\pgfnodeparttextbox}{2\pgf@circ@res@step+2\ht\pgfnodeparttextbox}}
        \pgf@x=0pt
        \pgf@y=2\pgf@circ@res@step
        \advance \pgf@y by 0.5\ht\pgfnodeparttextbox
        \pgf@x=-.5\wd\pgfnodeparttextbox
    }
    \behindforegroundpath{
        \pgf@circ@res@step=\ctikzvalof{monopoles/vcc/width}\pgf@circ@Rlen
        \pgfscope
            \pgfpathmoveto{\pgfpointorigin}
            \pgfpathlineto{\pgfpoint{0pt}{1.5\pgf@circ@res@step}}
            \pgfusepath{draw}

            \pgfstartlinewidth=\pgflinewidth
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

            \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{.8\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{0}{1.5\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@step}{.8\pgf@circ@res@step}}
            \pgfusepath{draw}

            \pgfsetlinewidth{\pgfstartlinewidth}

        \endpgfscope
    }

}

% Vee
\pgfdeclareshape{vee}{
    \savedanchor{\northeast}{%
        \pgf@circ@res@step=\ctikzvalof{monopoles/vcc/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@circ@res@step
        \pgf@y=-3\pgf@x%
    }
    \anchor{south}{\northeast\pgf@x=0cm\relax}
    \anchor{east}{\northeast\pgf@y=0.5\pgf@y\relax}
    \anchor{north}{\pgfpointorigin}
    \anchor{west}{\northeast\pgf@y=0.5\pgf@y\pgf@x=-\pgf@x}
    \anchor{south east}{\northeast}
    \anchor{south west}{\northeast\pgf@x=-\pgf@x}
    \anchor{north east}{\northeast\pgf@y=0pt\relax}
    \anchor{north west}{\northeast\pgf@y=0pt\pgf@x=-\pgf@x}
    \anchor{center}{\pgfpointorigin}
    \anchor{text}{
        \pgf@circ@res@step=\ctikzvalof{monopoles/vcc/width}\pgf@circ@Rlen
        \pgfpathmoveto{\pgfpoint{-.5\wd\pgfnodeparttextbox}{-2\pgf@circ@res@step-2\ht\pgfnodeparttextbox}}
        \pgfpathmoveto{\pgfpoint{.5\wd\pgfnodeparttextbox}{-2\pgf@circ@res@step-2\ht\pgfnodeparttextbox}}
        \pgf@x=0pt
        \pgf@y=-2\pgf@circ@res@step
        \advance \pgf@y by -1.5\ht\pgfnodeparttextbox
        \pgf@x=-.5\wd\pgfnodeparttextbox
    }

    \behindforegroundpath{
        \pgf@circ@res@step=\ctikzvalof{monopoles/vcc/width}\pgf@circ@Rlen

        \pgfscope
            \pgfpathmoveto{\pgfpointorigin}
            \pgfpathlineto{\pgfpoint{0pt}{-1.5\pgf@circ@res@step}}
            \pgfusepath{draw}

            \pgfstartlinewidth=\pgflinewidth
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

            \pgfpathmoveto{\pgfpoint{-0.5\pgf@circ@res@step}{-.8\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{0}{-1.5\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@step}{-.8\pgf@circ@res@step}}
            \pgfusepath{draw}
            \pgfsetlinewidth{\pgfstartlinewidth}

        \endpgfscope
    }

}


% match
\pgfdeclareshape{match}{
    \savedanchor{\northeast}{%
        \pgf@circ@res@step = \ctikzvalof{monopoles/match/width} \pgf@circ@Rlen
        \pgf@x=2\pgf@circ@res@step
        \pgf@circ@res@step = \ctikzvalof{monopoles/match/width} \pgf@circ@Rlen
        \pgf@y=.5\pgf@circ@res@step%
    }
    % the center is on the left side of the shape for facility of usage
    \anchor{north}{\northeast\pgf@x=0.5\pgf@x\relax}
    \anchor{east}{\northeast\pgf@y=0cm\relax}
    \anchor{south}{\northeast\pgf@y=0pt\pgf@x=0.5\pgf@x\relax}
    \anchor{west}{\pgfpointorigin}
    \anchor{north east}{\northeast}
    \anchor{north west}{\northeast\pgf@x=0cm\relax}
    \anchor{south east}{\northeast\pgf@y=0pt\relax}
    \anchor{south west}{\pgfpointorigin}
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{text}{
        \pgf@x=\ctikzvalof{monopoles/match/width}\pgf@circ@Rlen
        \pgf@x=1.5\pgf@x
        \advance \pgf@x by -.5\wd\pgfnodeparttextbox
        \pgf@y=-1.5\ht\pgfnodeparttextbox
    }
    \behindforegroundpath{
        \pgf@circ@res@step=\ctikzvalof{monopoles/match/width}\pgf@circ@Rlen

        \pgfscope
            \pgfpathmoveto{\pgfpointorigin}
            \pgfpathlineto{\pgfpoint{2\pgf@circ@res@step}{0pt}}
            \pgfusepath{draw}

            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
            \pgfpathlineto{\pgfpoint{2\pgf@circ@res@step}{0.5\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{2\pgf@circ@res@step}{0}}
            \pgfusepath{fill}

            \pgfsetlinewidth{\pgfstartlinewidth}

        \endpgfscope
    }
}

\endinput


==> pgfcircmultipoles.tex <==
% Copyright 2007-2009 by Massimo Redaelli
% Copyright 2019 by Romano Giannetti
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the files gpl-3.0_license.txt and lppl-1-3c_license.txt for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Multipoles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% counters for pin accounting...
\newcount\pgf@circ@count@c
\newcount\pgf@circ@count@b
\def\pgf@circ@dip@pin@shift{0.5}
\def\pgf@circ@qfp@pin@shift{0.25}

% derived from https://tex.stackexchange.com/a/146753/38080
% original author Mark Wibrow
% Thanks also to John Kormylo https://tex.stackexchange.com/a/372996/38080
% a lot of thanks to @marmot  for the un-rotation hint
% https://tex.stackexchange.com/a/473571/38080

% DIP (dual in line package) chips

\pgfdeclareshape{dipchip}{
    \savedanchor\centerpoint{%
        \pgf@x=-.5\wd\pgfnodeparttextbox%
        \pgf@y=-.5\ht\pgfnodeparttextbox%
        \advance\pgf@y by+.5\dp\pgfnodeparttextbox%
    }%
    \savedanchor\origin{\pgfpoint{0pt}{0pt}}
    \anchor{center}{\origin}
    \anchor{text}{\centerpoint}% to adjust text
    \saveddimen\height{%
        \pgfmathsetlength\pgf@x{((\pgfkeysvalueof{/tikz/circuitikz/multipoles/dipchip/num pins})
        *\pgfkeysvalueof{/tikz/circuitikz/multipoles/dipchip/pin spacing})*\pgf@circ@Rlen/2}%
    }%
    \saveddimen{\chipspacing}{\pgfmathsetlength\pgf@x{\pgf@circ@Rlen*\pgfkeysvalueof{/tikz/circuitikz/multipoles/dipchip/pin spacing}}}
    \saveddimen{\width}{\pgfmathsetlength\pgf@x{\pgf@circ@Rlen*\pgfkeysvalueof{/tikz/circuitikz/multipoles/dipchip/width}}}
    \saveddimen{\extshift}{\pgfmathsetlength\pgf@x{\pgf@circ@Rlen*\pgfkeysvalueof{/tikz/circuitikz/multipoles/external pins width}}}
    % standard anchors
    \savedanchor\northwest{%
        \pgfmathsetlength\pgf@y{0.5*((\pgfkeysvalueof{/tikz/circuitikz/multipoles/dipchip/num pins})
        *\pgfkeysvalueof{/tikz/circuitikz/multipoles/dipchip/pin spacing})*\pgf@circ@Rlen/2}%
        \pgfmathsetlength\pgf@x{-0.5*\pgf@circ@Rlen*\pgfkeysvalueof{/tikz/circuitikz/multipoles/dipchip/width}}
    }
    \anchor{dot}{\northwest
        \pgfmathsetlength\pgf@x{\pgf@x + 0.3*\chipspacing}
        \pgfmathsetlength\pgf@y{\pgf@y - 0.3*\chipspacing}
    }
    \anchor{nw}{\northwest}
    \anchor{ne}{\northwest\pgf@x=-\pgf@x}
    \anchor{se}{\northwest\pgf@x=-\pgf@x\pgf@y=-\pgf@y}
    \anchor{sw}{\northwest\pgf@y=-\pgf@y}
    \anchor{north west}{\northwest}
    \anchor{north east}{\northwest\pgf@x=-\pgf@x}
    \anchor{south east}{\northwest\pgf@x=-\pgf@x \pgf@y=-\pgf@y}
    \anchor{south west}{\northwest\pgf@y=-\pgf@y}
    \anchor{n}{\northwest\pgf@x=0pt }
    \anchor{e}{\northwest\pgf@x=-\pgf@x\pgf@y=0pt }
    \anchor{s}{\northwest\pgf@x=0pt\pgf@y=-\pgf@y}
    \anchor{w}{\northwest\pgf@y=0pt }
    \anchor{north}{\northwest\pgf@x=0pt }
    \anchor{east}{\northwest\pgf@x=-\pgf@x\pgf@y=0pt }
    \anchor{south}{\northwest\pgf@x=0pt\pgf@y=-\pgf@y}
    \anchor{west}{\northwest\pgf@y=0pt }
    % start drawing
    \backgroundpath{%
        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgf@circ@res@step = \pgfkeysvalueof{/tikz/circuitikz/multipoles/dipchip/pin spacing}\pgf@circ@Rlen
        \pgf@circ@res@other = \pgfkeysvalueof{/tikz/circuitikz/multipoles/external pins width}\pgf@circ@Rlen
        \pgfscope% (for the line width)
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/multipoles/thickness}\pgflinewidth}
        \pgfpathrectanglecorners{\pgfpoint{-\width/2}{-\height/2}}{\pgfpoint{\width/2}{\height/2}}%
        \pgf@circ@draworfill
        %% upside mark
        \ifpgf@circuit@chip@topmark
            \pgfpathmoveto{\pgfpoint{0.2*\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpatharc{0}{180}{0.2*\pgf@circ@res@left}
        \fi
        \pgfusepath{stroke}%
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
        % Adding the pin number
        \ifpgf@circuit@chip@shownumbers
            \c@pgf@counta=\pgfkeysvalueof{/tikz/circuitikz/multipoles/dipchip/num pins}%
            \divide\c@pgf@counta by 2 \pgf@circ@count@b=\c@pgf@counta
            % thanks to @marmot: https://tex.stackexchange.com/a/473571/38080
            \ifpgf@circuit@chip@straightnumbers
                \pgfgettransformentries\a\b\temp\temp\temp\temp
                \pgfmathsetmacro{\rot}{-atan2(\b,\a)}
                \pgfmathtruncatemacro{\quadrant}{mod(4+int(360+(\rot+45)/90),4)}
            \else
                \pgfmathsetmacro{\rot}{0}
                \pgfmathsetmacro{\quadrant}{0}
            \fi
            \def\pgf@circ@strut{\vrule width 0pt height 1em depth 0.4em\relax}
            \def\mytext{\pgfkeysvalueof{/tikz/circuitikz/multipoles/font}\space\pgf@circ@strut\the\pgf@circ@count@c\space}
            \pgfmathloop%
            \ifnum\c@pgf@counta>0
                \ifcase\quadrant % rotation 0
                    % left
                    \pgf@circ@count@c=\c@pgf@counta
                    \pgftext[left,
                        at=\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % right
                    \pgf@circ@count@c=\numexpr2*\pgf@circ@count@b-\c@pgf@counta+1\relax
                    \pgftext[right,
                        at=\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                \or % rotation -90
                    % left
                    \pgf@circ@count@c=\c@pgf@counta
                    \pgftext[top,
                        at=\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % right
                    \pgf@circ@count@c=\numexpr2*\pgf@circ@count@b-\c@pgf@counta+1\relax
                    \pgftext[bottom,
                        at=\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                \or %rotation 180
                    % left
                    \pgf@circ@count@c=\c@pgf@counta
                    \pgftext[right,
                        at=\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % right
                    \pgf@circ@count@c=\numexpr2*\pgf@circ@count@b-\c@pgf@counta+1\relax
                    \pgftext[left,
                        at=\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                \or % rotation +90
                    % left
                    \pgf@circ@count@c=\c@pgf@counta
                    \pgftext[bottom,
                        at=\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % right
                    \pgf@circ@count@c=\numexpr2*\pgf@circ@count@b-\c@pgf@counta+1\relax
                    \pgftext[top,
                        at=\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                \fi
                \advance\c@pgf@counta-1\relax%
                \repeatpgfmathloop
            \fi
            \endpgfscope
            \ifdim\pgf@circ@res@other>0pt
            \pgfscope
                \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/multipoles/external pins thickness}\pgflinewidth}
                \c@pgf@counta=\pgfkeysvalueof{/tikz/circuitikz/multipoles/dipchip/num pins}%
                \divide\c@pgf@counta by 2 \pgf@circ@count@b=\c@pgf@counta
                \pgfmathloop%
                \ifnum\c@pgf@counta>0
                    \edef\padfrac{\pgfkeysvalueof{/tikz/circuitikz/multipoles/external pad fraction}}
                    \ifnum\padfrac>0
                        \pgf@circ@res@temp=\pgf@circ@res@step\divide\pgf@circ@res@temp by \padfrac
                        % left side pads
                        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgf@circ@res@other}{\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgf@circ@res@other}{-\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{-\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                        % right side pads
                        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right+\pgf@circ@res@other}{\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right+\pgf@circ@res@other}{-\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{-\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                    \else
                        % left side pins
                        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgf@circ@res@other}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                        % right side pins
                        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right+\pgf@circ@res@other}{\pgf@circ@res@up+(\pgf@circ@dip@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                    \fi
                    \advance\c@pgf@counta by -1\relax%
                \repeatpgfmathloop
                \pgfusepath{stroke}
            \endpgfscope
            \fi
        }%
        % \pgf@sh@s@<name of the shape here> contains all the code for the shape
        % and is executed just before a node is drawn.
        \pgfutil@g@addto@macro\pgf@sh@s@dipchip{%
            % Start with the maximum pin number and go backwards.
            % If the anchor is undefined, create it. Otherwise stop.
            \c@pgf@counta=\pgfkeysvalueof{/tikz/circuitikz/multipoles/dipchip/num pins}%
            \divide\c@pgf@counta by 2 \pgf@circ@count@b=\c@pgf@counta
            \pgfmathloop%
            \ifnum\c@pgf@counta>0
                % left side, pins 1..npins/2
                % we will create two anchors per pin: the "normal one" like `pin 1` for the
                % electrical contact, and the "border one" like `bpin 1` for labels.
                % they will coincide if `external pins width` is set to 0.
                \expandafter\xdef\csname pgf@anchor@dipchip@bpin\space\the\c@pgf@counta\endcsname{%
                    \noexpand\pgf@circ@chippinanchorLB{\the\c@pgf@counta}%
                }
                \expandafter\xdef\csname pgf@anchor@dipchip@pin\space\the\c@pgf@counta\endcsname{%
                    \noexpand\pgf@circ@chippinanchorL{\the\c@pgf@counta}%
                }
                % right side
                \pgf@circ@count@c=\numexpr2*\pgf@circ@count@b-\c@pgf@counta+1\relax
                \expandafter\xdef\csname pgf@anchor@dipchip@bpin\space\the\pgf@circ@count@c\endcsname{%
                    \noexpand\pgf@circ@chippinanchorRB{\the\c@pgf@counta}%
                }%
                \expandafter\xdef\csname pgf@anchor@dipchip@pin\space\the\pgf@circ@count@c\endcsname{%
                    \noexpand\pgf@circ@chippinanchorR{\the\c@pgf@counta}%
                }%
                \advance\c@pgf@counta by -1\relax%
                \repeatpgfmathloop%
            }%
        }

% QFP (quad flat package) chips

\pgfdeclareshape{qfpchip}{
    \savedanchor\centerpoint{%
        \pgf@x=-.5\wd\pgfnodeparttextbox%
        \pgf@y=-.5\ht\pgfnodeparttextbox%
        \advance\pgf@y by+.5\dp\pgfnodeparttextbox%
    }%
    \savedanchor\origin{\pgfpoint{0pt}{0pt}}
    \anchor{center}{\origin}
    \anchor{text}{\centerpoint}% to adjust text
    \saveddimen\height{%
        \pgfmathsetlength\pgf@x{((\pgfkeysvalueof{/tikz/circuitikz/multipoles/qfpchip/num pins}+2)
        *\pgfkeysvalueof{/tikz/circuitikz/multipoles/qfpchip/pin spacing})*\pgf@circ@Rlen/4}%
    }%
    \saveddimen\width{%
        \pgfmathsetlength\pgf@x{((\pgfkeysvalueof{/tikz/circuitikz/multipoles/qfpchip/num pins}+2)
        *\pgfkeysvalueof{/tikz/circuitikz/multipoles/qfpchip/pin spacing})*\pgf@circ@Rlen/4}%
    }%
    \saveddimen{\chipspacing}{\pgfmathsetlength\pgf@x{\pgf@circ@Rlen*\pgfkeysvalueof{/tikz/circuitikz/multipoles/qfpchip/pin spacing}}}
    \saveddimen{\extshift}{\pgfmathsetlength\pgf@x{\pgf@circ@Rlen*\pgfkeysvalueof{/tikz/circuitikz/multipoles/external pins width}}}
    % standard anchors
    \savedanchor\northwest{%
        \pgfmathsetlength\pgf@y{0.5*((\pgfkeysvalueof{/tikz/circuitikz/multipoles/qfpchip/num pins}+2)
        *\pgfkeysvalueof{/tikz/circuitikz/multipoles/qfpchip/pin spacing})*\pgf@circ@Rlen/4}%
        \pgf@x=-\pgf@y
    }
    \anchor{dot}{\northwest
        \pgfmathsetlength\pgf@x{\pgf@x + 0.3*\chipspacing}
        \pgfmathsetlength\pgf@y{\pgf@y - 0.3*\chipspacing}
    }
    \anchor{nw}{\northwest}
    \anchor{ne}{\northwest\pgf@x=-\pgf@x}
    \anchor{se}{\northwest\pgf@x=-\pgf@x\pgf@y=-\pgf@y}
    \anchor{sw}{\northwest\pgf@y=-\pgf@y}
    \anchor{north west}{\northwest}
    \anchor{north east}{\northwest\pgf@x=-\pgf@x}
    \anchor{south east}{\northwest\pgf@x=-\pgf@x \pgf@y=-\pgf@y}
    \anchor{south west}{\northwest\pgf@y=-\pgf@y}
    \anchor{n}{\northwest\pgf@x=0pt }
    \anchor{e}{\northwest\pgf@x=-\pgf@x\pgf@y=0pt }
    \anchor{s}{\northwest\pgf@x=0pt\pgf@y=-\pgf@y}
    \anchor{w}{\northwest\pgf@y=0pt }
    \anchor{north}{\northwest\pgf@x=0pt }
    \anchor{east}{\northwest\pgf@x=-\pgf@x\pgf@y=0pt }
    \anchor{south}{\northwest\pgf@x=0pt\pgf@y=-\pgf@y}
    \anchor{west}{\northwest\pgf@y=0pt }
    % start drawing
    \backgroundpath{%
        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgf@circ@res@step = \pgfkeysvalueof{/tikz/circuitikz/multipoles/qfpchip/pin spacing}\pgf@circ@Rlen
        \pgf@circ@res@other = \pgfkeysvalueof{/tikz/circuitikz/multipoles/external pins width}\pgf@circ@Rlen
        \pgfscope% (for the line width)
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/multipoles/thickness}\pgflinewidth}
        %% upside mark
        \ifpgf@circuit@chip@topmark
            \pgfpathmoveto{\pgfpoint{-\width/2}{\height/2-\pgf@circ@res@step/2}}
            \pgfpathlineto{\pgfpoint{-\width/2+\pgf@circ@res@step/2}{\height/2}}
        \else
            \pgfpathmoveto{\pgfpoint{-\width/2}{\height/2}}
        \fi
        %% rest of the shape
        \pgfpathlineto{\pgfpoint{\width/2}{\height/2}}
        \pgfpathlineto{\pgfpoint{\width/2}{-\height/2}}
        \pgfpathlineto{\pgfpoint{-\width/2}{-\height/2}}
        \pgfpathclose
        \pgf@circ@draworfill
        % Adding the pin number
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
        \ifpgf@circuit@chip@shownumbers
            \c@pgf@counta=\pgfkeysvalueof{/tikz/circuitikz/multipoles/qfpchip/num pins}%
            \divide\c@pgf@counta by 4 \pgf@circ@count@b=\c@pgf@counta
            % thanks to @marmot: https://tex.stackexchange.com/a/473571/38080
            \ifpgf@circuit@chip@straightnumbers
                \pgfgettransformentries\a\b\temp\temp\temp\temp
                \pgfmathsetmacro{\rot}{-atan2(\b,\a)}
                \pgfmathtruncatemacro{\quadrant}{mod(4+int(360+(\rot+45)/90),4)}
            \else
                \pgfmathsetmacro{\rot}{0}
                \pgfmathsetmacro{\quadrant}{0}
            \fi
            \def\pgf@circ@strut{\vrule width 0pt height 1em depth 0.4em\relax}
            \def\mytext{\pgfkeysvalueof{/tikz/circuitikz/multipoles/font}\space\pgf@circ@strut\the\pgf@circ@count@c\space}
            \pgfmathloop%
            \ifnum\c@pgf@counta>0
                \ifcase\quadrant % rotation 0
                    % left
                    \pgf@circ@count@c=\c@pgf@counta
                    \pgftext[left,
                        at=\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % bottom
                    \pgf@circ@count@c=\numexpr\pgf@circ@count@b+\c@pgf@counta\relax
                    \pgftext[bottom,
                        at=\pgfpoint{\pgf@circ@res@left-(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}{\pgf@circ@res@down},
                        rotate=\rot]{\mytext}
                    % right
                    \pgf@circ@count@c=\numexpr3*\pgf@circ@count@b-\c@pgf@counta+1\relax
                    \pgftext[right,
                        at=\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % top
                    \pgf@circ@count@c=\numexpr3*\pgf@circ@count@b+\c@pgf@counta\relax
                    \pgftext[top,
                        at=\pgfpoint{\pgf@circ@res@right+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}{\pgf@circ@res@up},
                        rotate=\rot]{\mytext}
                \or % rotation -90
                    % left
                    \pgf@circ@count@c=\c@pgf@counta
                    \pgftext[top,
                        at=\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % bottom
                    \pgf@circ@count@c=\numexpr\pgf@circ@count@b+\c@pgf@counta\relax
                    \pgftext[left,
                        at=\pgfpoint{\pgf@circ@res@left-(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}{\pgf@circ@res@down},
                        rotate=\rot]{\mytext}
                    % right
                    \pgf@circ@count@c=\numexpr3*\pgf@circ@count@b-\c@pgf@counta+1\relax
                    \pgftext[bottom,
                        at=\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % top
                    \pgf@circ@count@c=\numexpr3*\pgf@circ@count@b+\c@pgf@counta\relax
                    \pgftext[right,
                        at=\pgfpoint{\pgf@circ@res@right+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}{\pgf@circ@res@up},
                        rotate=\rot]{\mytext}
                \or %rotation 180
                    % left
                    \pgf@circ@count@c=\c@pgf@counta
                    \pgftext[right,
                        at=\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % bottom
                    \pgf@circ@count@c=\numexpr\pgf@circ@count@b+\c@pgf@counta\relax
                    \pgftext[top,
                        at=\pgfpoint{\pgf@circ@res@left-(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}{\pgf@circ@res@down},
                        rotate=\rot]{\mytext}
                    % right
                    \pgf@circ@count@c=\numexpr3*\pgf@circ@count@b-\c@pgf@counta+1\relax
                    \pgftext[left,
                        at=\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % top
                    \pgf@circ@count@c=\numexpr3*\pgf@circ@count@b+\c@pgf@counta\relax
                    \pgftext[bottom,
                        at=\pgfpoint{\pgf@circ@res@right+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}{\pgf@circ@res@up},
                        rotate=\rot]{\mytext}
                \or % rotation +90
                    % left
                    \pgf@circ@count@c=\c@pgf@counta
                    \pgftext[bottom,
                        at=\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % bottom
                    \pgf@circ@count@c=\numexpr\pgf@circ@count@b+\c@pgf@counta\relax
                    \pgftext[right,
                        at=\pgfpoint{\pgf@circ@res@left-(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}{\pgf@circ@res@down},
                        rotate=\rot]{\mytext}
                    % right
                    \pgf@circ@count@c=\numexpr3*\pgf@circ@count@b-\c@pgf@counta+1\relax
                    \pgftext[top,
                        at=\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step},
                        rotate=\rot]{\mytext}
                    % top
                    \pgf@circ@count@c=\numexpr3*\pgf@circ@count@b+\c@pgf@counta\relax
                    \pgftext[left,
                        at=\pgfpoint{\pgf@circ@res@right+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}{\pgf@circ@res@up},
                        rotate=\rot]{\mytext}
                \fi
                \advance\c@pgf@counta-1\relax%
                \repeatpgfmathloop
            \fi
            \endpgfscope
            \ifdim\pgf@circ@res@other>0pt
            \pgfscope
                \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/multipoles/external pins thickness}\pgflinewidth}
                \c@pgf@counta=\pgfkeysvalueof{/tikz/circuitikz/multipoles/qfpchip/num pins}%
                \divide\c@pgf@counta by 4 \pgf@circ@count@b=\c@pgf@counta
                \pgfmathloop%
                \ifnum\c@pgf@counta>0
                    \edef\padfrac{\pgfkeysvalueof{/tikz/circuitikz/multipoles/external pad fraction}}
                    \ifnum\padfrac>0
                        \pgf@circ@res@temp=\pgf@circ@res@step\divide\pgf@circ@res@temp by \padfrac
                        % left side pads
                        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgf@circ@res@other}{\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgf@circ@res@other}{-\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{-\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                        % bottom side pads
                        \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@temp+\pgf@circ@res@left-(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}{\pgf@circ@res@down}}
                        \pgfpathlineto{\pgfpoint{-\pgf@circ@res@temp+\pgf@circ@res@left-(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}{\pgf@circ@res@down-\pgf@circ@res@other}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@temp+\pgf@circ@res@left-(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}{\pgf@circ@res@down-\pgf@circ@res@other}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@temp+\pgf@circ@res@left-(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}{\pgf@circ@res@down}}
                        % right side pads
                        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right+\pgf@circ@res@other}{\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right+\pgf@circ@res@other}{-\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{-\pgf@circ@res@temp+\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                        % top side pads
                        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@temp+\pgf@circ@res@right+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}{\pgf@circ@res@up}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@temp+\pgf@circ@res@right+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}{\pgf@circ@res@up+\pgf@circ@res@other}}
                        \pgfpathlineto{\pgfpoint{-\pgf@circ@res@temp+\pgf@circ@res@right+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}{\pgf@circ@res@up+\pgf@circ@res@other}}
                        \pgfpathlineto{\pgfpoint{-\pgf@circ@res@temp+\pgf@circ@res@right+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}{\pgf@circ@res@up}}
                    \else
                        % left side pins
                        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgf@circ@res@other}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                        % bottom side pins
                        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}{\pgf@circ@res@down}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}{\pgf@circ@res@down-\pgf@circ@res@other}}
                        % right side pins
                        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right+\pgf@circ@res@other}{\pgf@circ@res@up+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}}
                        % top side pins
                        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}{\pgf@circ@res@up}}
                        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right+(\pgf@circ@qfp@pin@shift-\the\c@pgf@counta)*\pgf@circ@res@step}{\pgf@circ@res@up+\pgf@circ@res@other}}
                    \fi
                    \advance\c@pgf@counta-1\relax%
                \repeatpgfmathloop
                \pgfusepath{stroke}
            \endpgfscope
            \fi
        }%
        % \pgf@sh@s@<name of the shape here> contains all the code for the shape
        % and is executed just before a node is drawn.
        \pgfutil@g@addto@macro\pgf@sh@s@qfpchip{%
            % Start with the maximum pin number and go backwards.
            % If the anchor is undefined, create it. Otherwise stop.
            \c@pgf@counta=\pgfkeysvalueof{/tikz/circuitikz/multipoles/qfpchip/num pins}%
            \divide\c@pgf@counta by 4 \pgf@circ@count@b=\c@pgf@counta
            \pgfmathloop%
            \ifnum\c@pgf@counta>0
                % left side; 1..npins/4
                \expandafter\xdef\csname pgf@anchor@qfpchip@pin\space\the\c@pgf@counta\endcsname{%
                    \noexpand\pgf@circ@chippinanchorQL{\the\c@pgf@counta}%
                }
                \expandafter\xdef\csname pgf@anchor@qfpchip@bpin\space\the\c@pgf@counta\endcsname{%
                    \noexpand\pgf@circ@chippinanchorQLB{\the\c@pgf@counta}%
                }
                % bottom side;
                \pgf@circ@count@c=\numexpr2*\pgf@circ@count@b-\c@pgf@counta+1\relax
                \expandafter\xdef\csname pgf@anchor@qfpchip@pin\space\the\pgf@circ@count@c\endcsname{%
                    \noexpand\pgf@circ@chippinanchorQB{\the\c@pgf@counta}%
                }
                \expandafter\xdef\csname pgf@anchor@qfpchip@bpin\space\the\pgf@circ@count@c\endcsname{%
                    \noexpand\pgf@circ@chippinanchorQBB{\the\c@pgf@counta}%
                }
                % right side; 2*npins/4+1, 3*npins/4
                \pgf@circ@count@c=\numexpr3*\pgf@circ@count@b-\c@pgf@counta+1\relax
                \expandafter\xdef\csname pgf@anchor@qfpchip@pin\space\the\pgf@circ@count@c\endcsname{%
                    \noexpand\pgf@circ@chippinanchorQR{\the\c@pgf@counta}%
                }
                \expandafter\xdef\csname pgf@anchor@qfpchip@bpin\space\the\pgf@circ@count@c\endcsname{%
                    \noexpand\pgf@circ@chippinanchorQRB{\the\c@pgf@counta}%
                }
                % top side
                \pgf@circ@count@c=\numexpr3*\pgf@circ@count@b+\c@pgf@counta\relax
                \expandafter\xdef\csname pgf@anchor@qfpchip@pin\space\the\pgf@circ@count@c\endcsname{%
                    \noexpand\pgf@circ@chippinanchorQT{\the\c@pgf@counta}%
                }
                \expandafter\xdef\csname pgf@anchor@qfpchip@bpin\space\the\pgf@circ@count@c\endcsname{%
                    \noexpand\pgf@circ@chippinanchorQTB{\the\c@pgf@counta}%
                }
                \advance\c@pgf@counta-1\relax%
                \repeatpgfmathloop%
            }%
        }

%% anchors for DIP
\def\pgf@circ@chippinanchorR#1{%
  % When this macro is called,
  % \extshift, \height and \chipspacing will be defined.
    \pgfpoint{\width/2+\extshift}{\height/2+(\pgf@circ@dip@pin@shift-#1)*\chipspacing}%
}
\def\pgf@circ@chippinanchorL#1{%
  % When this macro is called,
  % \extshift, \height and \chipspacing will be defined.
    \pgfpoint{-\width/2-\extshift}{\height/2+(\pgf@circ@dip@pin@shift-#1)*\chipspacing}%
}
\def\pgf@circ@chippinanchorRB#1{%
  % When this macro is called,
  % \extshift, \height and \chipspacing will be defined.
    \pgfpoint{\width/2}{\height/2+(\pgf@circ@dip@pin@shift-#1)*\chipspacing}%
}
\def\pgf@circ@chippinanchorLB#1{%
  % When this macro is called,
  % \extshift, \height and \chipspacing will be defined.
    \pgfpoint{-\width/2}{\height/2+(\pgf@circ@dip@pin@shift-#1)*\chipspacing}%
}

%% anchors for QFP
\def\pgf@circ@chippinanchorQR#1{%
  % When this macro is called,
  % \extshift, \height and \chipspacing will be defined.
    \pgfpoint{\width/2+\extshift}{\height/2+(\pgf@circ@qfp@pin@shift-#1)*\chipspacing}%
}
\def\pgf@circ@chippinanchorQL#1{%
  % When this macro is called,
  % \extshift, \height and \chipspacing will be defined.
    \pgfpoint{-\width/2-\extshift}{\height/2+(\pgf@circ@qfp@pin@shift-#1)*\chipspacing}%
}
\def\pgf@circ@chippinanchorQT#1{%
  % When this macro is called,
  % \extshift, \height and \chipspacing will be defined.
    \pgfpoint{\width/2+(\pgf@circ@qfp@pin@shift-#1)*\chipspacing}{\height/2+\extshift}%
}
\def\pgf@circ@chippinanchorQB#1{%
  % When this macro is called,
  % \extshift, \height and \chipspacing will be defined.
    \pgfpoint{\width/2+(\pgf@circ@qfp@pin@shift-#1)*\chipspacing}{-\height/2-\extshift}%
}
\def\pgf@circ@chippinanchorQRB#1{%
  % When this macro is called,
  % \extshift, \height and \chipspacing will be defined.
    \pgfpoint{\width/2}{\height/2+(\pgf@circ@qfp@pin@shift-#1)*\chipspacing}%
}
\def\pgf@circ@chippinanchorQLB#1{%
  % When this macro is called,
  % \extshift, \height and \chipspacing will be defined.
    \pgfpoint{-\width/2}{\height/2+(\pgf@circ@qfp@pin@shift-#1)*\chipspacing}%
}
\def\pgf@circ@chippinanchorQTB#1{%
  % When this macro is called,
  % \extshift, \height and \chipspacing will be defined.
    \pgfpoint{\width/2+(\pgf@circ@qfp@pin@shift-#1)*\chipspacing}{\height/2}%
}
\def\pgf@circ@chippinanchorQBB#1{%
  % When this macro is called,
  % \extshift, \height and \chipspacing will be defined.
    \pgfpoint{\width/2+(\pgf@circ@qfp@pin@shift-#1)*\chipspacing}{-\height/2}%
}



==> pgfcircpath.tex <==

\def\pgf@circ@direction{0.0}

% Names
\ctikzset{name/.style = { n=#1 } } %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%@@@
\ctikzset{n/.code = {
	\pgfkeys{/tikz/circuitikz/bipole/name=#1}
}}

% Reflect the node along
\ctikzset{mirrored/.is choice}
\ctikzset{mirror value/.initial=1}
\ctikzset{mirrored/true/.code = {\ctikzsetvalof{mirror value}{-1}} }
\ctikzset{mirrored/false/.code = {\ctikzsetvalof{mirror value}{1}} }
\ctikzset{mirror/.style = {/tikz/circuitikz/mirrored=true}}

% Invert node along path
\ctikzset{inverted/.is choice}
\ctikzset{invert value/.initial=1}
\ctikzset{inverted/true/.code = {\ctikzsetvalof{invert value}{-1}\pgf@circuit@bipole@invertedtrue}}
\ctikzset{inverted/false/.code = {\ctikzsetvalof{invert value}{1}\pgf@circuit@bipole@invertedfalse}}
\ctikzset{invert/.style = {/tikz/circuitikz/inverted=true}}
\newif\ifpgf@circuit@bipole@inverted
\ctikzset{bipole/inverted/.is if=pgf@circuit@bipole@inverted}


\newif\ifpgf@circuit@bipole@voltage@backward
\ctikzset{bipole/voltage/direction/.is choice}
\ctikzset{bipole/voltage/direction/forward/.code={\pgf@circuit@bipole@voltage@backwardfalse}}
\ctikzset{bipole/voltage/direction/backward/.code={\pgf@circuit@bipole@voltage@backwardtrue}}



% Initialize paths
\def\pgfcircresetpath{
    \ctikzset{bipole/name=, bipole/label/name=, bipole/label/position=90, ,bipole/annotation/name=, bipole/annotation/position=-90,
        bipole/inverted=false, bipole/kind=,
        bipole/voltage/direction=backward, bipole/voltage/label/name=, bipole/voltage/position=below,
        bipole/nodes/left=none, bipole/nodes/right=none, bipole/is voltage=false,bipole/is voltageoutsideofsymbol=false,bipole/is strokedsymbol=false,
        bipole/is current=false, bipole/current/label/name=, bipole/current/x position=after,
        bipole/current/y position=above, bipole/current/direction=forward,
        mirrored=false
    }
}

%% Helper function for path-function to ensure using anchors between nodes
\def\set@explicit@center@anchor#1{
    \pgfutil@ifundefined{pgf@sh@ns@#1}
    {
        %This coordinate is no node(but a relative position or a coordinate), no further handling needed
        }{
        \pgfutil@in@.{#1}
        \ifpgfutil@in@
            % Anchor is used, do nothing!
    \else%
        \let\tikz@moveto@waiting=\relax
        \pgfpathmoveto{\tikz@last@position}%force movement, because tikz@moveto@waiting
        \edef#1{#1.center}%ensure using center anchor
    \fi
}
}


%% Generic bipole path
\def\pgf@circ@bipole@path#1#2{

    \pgfextra{
        \set@explicit@center@anchor{\tikztostart}
        \set@explicit@center@anchor{\tikztotarget}
        \pgfsyssoftpath@getcurrentpath{\myp@th}%% save current path to extend after calculation of correct start/end coordinates
        \ctikzset{bipole/kind = #1}
        \edef\pgf@temp{\ctikzvalof{bipole/name}}
        \def\pgf@circ@temp{}
        \ifx\pgf@temp\pgf@circ@temp % if it has not a name
            \pgfmathrandominteger{\pgf@circ@rand}{1000}{9999}
            \ctikzset{bipole/name = #2\pgf@circ@rand} % create it
        \fi
    }

    (\tikztostart) coordinate (\ctikzvalof{bipole/name}start)%necessary to get correct coordinates in the case of relative start/end or constructions like ((node1)-|(node2))
    (\tikztotarget) coordinate (\ctikzvalof{bipole/name}end)
    \pgfextra{
        \pgfmathanglebetweenpoints{\pgfpointanchor{\ctikzvalof{bipole/name}start}{center}}
        {\pgfpointanchor{\ctikzvalof{bipole/name}end}{center}}
        \pgfmathround{\pgfmathresult}
        \edef\pgf@circ@direction{\pgfmathresult}%Calculate direction(angle) of path
        \pgfsyssoftpath@setcurrentpath{\myp@th}
    }
    \pgfextra{\def\pgf@temp{open}\def\pgf@circ@temp{#1}}
    \ifx\pgf@temp\pgf@circ@temp  % if it is an open
        \else
            --($(\ctikzvalof{bipole/name}start) ! .5\pgflinewidth ! (\ctikzvalof{bipole/name}end)$) %ugly workaround to get correct linejoins(node breaks path?)
        \fi
        ($(\tikztostart) ! .5 ! (\tikztotarget)$)%%positio of middle node
        node[#1shape, rotate=\pgf@circ@direction, yscale=\ctikzvalof{mirror value}, xscale=\ctikzvalof{invert value}]
        (\ctikzvalof{bipole/name}) {}
        \ifpgf@circuit@bipole@inverted
            \ifcsname pgf@anchor@#1shape@pathstart\endcsname%if special path-anchors are defined, use them!
                coordinate	(anchorstartnode) at (\ctikzvalof{bipole/name}.pathend)
                coordinate	(anchorendnode) at (\ctikzvalof{bipole/name}.pathstart)
            \else
                coordinate	(anchorstartnode) at (\ctikzvalof{bipole/name}.right)
                coordinate	(anchorendnode) at (\ctikzvalof{bipole/name}.left)
            \fi
            \else
            \ifcsname pgf@anchor@#1shape@pathstart\endcsname%if special path-anchors are defined, use them!
                coordinate	(anchorstartnode) at (\ctikzvalof{bipole/name}.pathstart)
                coordinate	(anchorendnode) at (\ctikzvalof{bipole/name}.pathend)
            \else
                coordinate	(anchorstartnode) at (\ctikzvalof{bipole/name}.left)
                coordinate	(anchorendnode) at (\ctikzvalof{bipole/name}.right)
            \fi
        \fi
        \pgfextra{\def\pgf@temp{open}\def\pgf@circ@temp{#1}}
        \ifx\pgf@temp\pgf@circ@temp  % if it is an open
        \else
            (\ctikzvalof{bipole/name}start.center) -- (anchorstartnode)
            (anchorendnode)  -- (\ctikzvalof{bipole/name}end.center)
        \fi

        \drawpoles
        \pgf@circ@ifkeyempty{bipole/label/name}\else\pgf@circ@drawlabels{label}\fi
        \pgf@circ@ifkeyempty{bipole/annotation/name}\else\pgf@circ@drawlabels{annotation}\fi
        \pgf@circ@ifkeyempty{bipole/voltage/label/name}\else\pgf@circ@drawvoltage\fi
        \pgf@circ@ifkeyempty{bipole/current/label/name}\else\pgf@circ@drawcurrent\fi
        \pgf@circ@ifkeyempty{bipole/flow/label/name}\else\pgf@circ@drawflow\fi
        \pgfextra{\def\pgf@temp{open}\def\pgf@circ@temp{#1}}
        \ifx\pgf@temp\pgf@circ@temp  % if it is an open
            (\ctikzvalof{bipole/name}end)%Move to end of path
        \else
            ($(\ctikzvalof{bipole/name}end) ! .5\pgflinewidth ! (\ctikzvalof{bipole/name}start)$) -- (\ctikzvalof{bipole/name}end)%ugly workaround to get correct linejoins(node breaks path?)
            %tikztostart and tikztotarget could not be used, because it would break if target coordinate is something like (node1-|node2)

        \fi
    % reset
    \pgfextra{
        \pgfcircresetpath
    }
    \tikztonodes%draw pending nodes an path
}


%% Path definitions
\def\pgf@circ@resistor@path#1{\ifpgf@circuit@europeanresistor\pgf@circ@bipole@path{generic}{#1}\else\pgf@circ@bipole@path{resistor}{#1}\fi}
\def\pgf@circ@vresistor@path#1{\ifpgf@circuit@europeanresistor\pgf@circ@bipole@path{tgeneric}{#1}\else\pgf@circ@bipole@path{vresistor}{#1}\fi}
\def\pgf@circ@sresistor@path#1{\ifpgf@circuit@europeanresistor\pgf@circ@bipole@path{thermistor}{#1}\else\pgf@circ@bipole@path{resistivesens}{#1}\fi}
\def\pgf@circ@potentiometer@path#1{\ifpgf@circuit@europeanresistor\pgf@circ@bipole@path{genericpotentiometer}{#1}\else\pgf@circ@bipole@path{potentiometer}{#1}\fi}
\def\pgf@circ@thermistor@path#1{\pgf@circ@bipole@path{thermistor}{#1}}
\def\pgf@circ@thermistorptc@path#1{\pgf@circ@bipole@path{thermistorptc}{#1}}
\def\pgf@circ@thermistorntc@path#1{\pgf@circ@bipole@path{thermistorntc}{#1}}
\def\pgf@circ@varistor@path#1{\pgf@circ@bipole@path{varistor}{#1}}
\def\pgf@circ@capacitor@path#1{\pgf@circ@bipole@path{capacitor}{#1}}
\def\pgf@circ@capacitivesens@path#1{\pgf@circ@bipole@path{capacitivesens}{#1}}
\def\pgf@circ@ecapacitor@path#1{\pgf@circ@bipole@path{ecapacitor}{#1}}
\def\pgf@circ@polarcapacitor@path#1{\pgf@circ@bipole@path{polarcapacitor}{#1}}
\def\pgf@circ@vcapacitor@path#1{\pgf@circ@bipole@path{vcapacitor}{#1}}
\def\pgf@circ@piezoelectric@path#1{\pgf@circ@bipole@path{piezoelectric}{#1}}
\def\pgf@circ@battery@path#1{\pgf@circ@bipole@path{battery}{#1}}
\def\pgf@circ@batteryone@path#1{\pgf@circ@bipole@path{battery1}{#1}}
\def\pgf@circ@batterytwo@path#1{\pgf@circ@bipole@path{battery2}{#1}}
\def\pgf@circ@europeaninductor@path#1{\pgf@circ@bipole@path{fullgeneric}{#1}}
\def\pgf@circ@americaninductor@path#1{\pgf@circ@bipole@path{americaninductor}{#1}}
\def\pgf@circ@cuteinductor@path#1{\pgf@circ@bipole@path{cuteinductor}{#1}}
\def\pgf@circ@cutechoke@path#1{\pgf@circ@bipole@path{cutechoke}{#1}}
\def\pgf@circ@inductor@path#1{%
    \pgfextra{
        \edef\pgf@circ@temp{\ctikzvalof{inductor}}%
        \def\pgf@temp{european}%
    }
    \ifx\pgf@temp\pgf@circ@temp%
        \pgf@circ@europeaninductor@path{#1}%
    \else%
        \pgfextra{	\def\pgf@temp{cute} }%
        \ifx\pgf@temp\pgf@circ@temp%
            \pgf@circ@cuteinductor@path{#1}%
        \else%
            \pgf@circ@americaninductor@path{#1}%
        \fi%
    \fi%
}
\def\pgf@circ@vinductor@path#1{
    \pgfextra{
        \edef\pgf@circ@temp{\ctikzvalof{inductor}}%
        \def\pgf@temp{european}%
    }
    \ifx\pgf@temp\pgf@circ@temp%
        \pgf@circ@veuropeaninductor@path{#1}%
    \else%
        \pgfextra{	\def\pgf@temp{cute} }%
        \ifx\pgf@temp\pgf@circ@temp%
            \pgf@circ@vcuteinductor@path{#1}%
        \else%
            \pgf@circ@vamericaninductor@path{#1}%
        \fi%
    \fi%
}
\def\pgf@circ@inductivesens@path#1{%
    \pgfextra{
        \edef\pgf@circ@temp{\ctikzvalof{inductor}}%
        \def\pgf@temp{european}%
    }
    \ifx\pgf@temp\pgf@circ@temp%
        \pgf@circ@europeaninductivesens@path{#1}%
    \else%
        \pgfextra{	\def\pgf@temp{cute} }%
        \ifx\pgf@temp\pgf@circ@temp%
            \pgf@circ@cuteinductivesens@path{#1}%
        \else%
            \pgf@circ@americaninductivesens@path{#1}%
        \fi%
    \fi%
}
\def\pgf@circ@veuropeaninductor@path#1{\pgf@circ@bipole@path{tfullgeneric}{#1}}
\def\pgf@circ@vamericaninductor@path#1{\pgf@circ@bipole@path{vamericaninductor}{#1}}
\def\pgf@circ@vcuteinductor@path#1{\pgf@circ@bipole@path{vcuteinductor}{#1}}
\def\pgf@circ@europeaninductivesens@path#1{\pgf@circ@bipole@path{sfullgeneric}{#1}}
\def\pgf@circ@americaninductivesens@path#1{\pgf@circ@bipole@path{samericaninductor}{#1}}
\def\pgf@circ@cuteinductivesens@path#1{\pgf@circ@bipole@path{scuteinductor}{#1}}
\def\pgf@circ@lamp@path#1{\pgf@circ@bipole@path{lamp}{#1}}
\def\pgf@circ@bulb@path#1{\pgf@circ@bipole@path{bulb}{#1}}
\def\pgf@circ@esource@path#1{\pgf@circ@bipole@path{esource}{#1}}
\def\pgf@circ@pvsource@path#1{\pgf@circ@bipole@path{pvsource}{#1}}
\def\pgf@circ@vsource@path#1{\pgf@circ@bipole@path{vsource}{#1}}
\def\pgf@circ@dcvsource@path#1{\pgf@circ@bipole@path{dcvsource}{#1}}
\def\pgf@circ@vsourceam@path#1{\pgf@circ@bipole@path{vsourceAM}{#1}}
\def\pgf@circ@vsourcesin@path#1{\pgf@circ@bipole@path{vsourcesin}{#1}}
\def\pgf@circ@isource@path#1{\pgf@circ@bipole@path{isource}{#1}}
\def\pgf@circ@oosource@path#1{\pgf@circ@bipole@path{oosource}{#1}}
\def\pgf@circ@dcisource@path#1{\pgf@circ@bipole@path{dcisource}{#1}}
\def\pgf@circ@isourcesin@path#1{\pgf@circ@bipole@path{isourcesin}{#1}}
\def\pgf@circ@vsourcesquare@path#1{\pgf@circ@bipole@path{vsourcesquare}{#1}}
\def\pgf@circ@vsourcetri@path#1{\pgf@circ@bipole@path{vsourcetri}{#1}}
\def\pgf@circ@isourceam@path#1{\pgf@circ@bipole@path{isourceAM}{#1}}
\def\pgf@circ@cvsource@path#1{\pgf@circ@bipole@path{cvsource}{#1}}
\def\pgf@circ@cvsourceam@path#1{\pgf@circ@bipole@path{cvsourceAM}{#1}}
\def\pgf@circ@cvsourcesin@path#1{\pgf@circ@bipole@path{cvsourcesin}{#1}}
\def\pgf@circ@cisource@path#1{\pgf@circ@bipole@path{cisource}{#1}}
\def\pgf@circ@cisourceam@path#1{\pgf@circ@bipole@path{cisourceAM}{#1}}
\def\pgf@circ@cisourcesin@path#1{\pgf@circ@bipole@path{cisourcesin}{#1}}
\def\pgf@circ@short@path#1{\pgf@circ@bipole@path{short}{#1}}
\def\pgf@circ@cspst@path#1{\pgf@circ@bipole@path{cspst}{#1}}
\def\pgf@circ@ospst@path#1{\pgf@circ@bipole@path{ospst}{#1}}
\def\pgf@circ@nos@path#1{\pgf@circ@bipole@path{nos}{#1}}
\def\pgf@circ@ncs@path#1{\pgf@circ@bipole@path{ncs}{#1}}
\def\pgf@circ@pushbutton@path#1{\pgf@circ@bipole@path{pushbutton}{#1}}
\def\pgf@circ@ncpushbutton@path#1{\pgf@circ@bipole@path{ncpushbutton}{#1}}
\def\pgf@circ@open@path#1{\pgf@circ@bipole@path{open}{#1}}
\def\pgf@circ@generic@path#1{\pgf@circ@bipole@path{generic}{#1}}
\def\pgf@circ@ageneric@path#1{\pgf@circ@bipole@path{ageneric}{#1}}
\def\pgf@circ@tgeneric@path#1{\pgf@circ@bipole@path{tgeneric}{#1}}
\def\pgf@circ@fullgeneric@path#1{\pgf@circ@bipole@path{fullgeneric}{#1}}
\def\pgf@circ@tfullgeneric@path#1{\pgf@circ@bipole@path{tfullgeneric}{#1}}
\def\pgf@circ@ammeter@path#1{\pgf@circ@bipole@path{ammeter}{#1}}
\def\pgf@circ@ohmmeter@path#1{\pgf@circ@bipole@path{ohmmeter}{#1}}
\def\pgf@circ@voltmeter@path#1{\pgf@circ@bipole@path{voltmeter}{#1}}
\def\pgf@circ@oscope@path#1{\pgf@circ@bipole@path{oscope}{#1}}
\def\pgf@circ@empty@path#1{}
\def\pgf@circ@photoresistor@path#1{\pgf@circ@bipole@path{photoresistor}{#1}}
\def\pgf@circ@emptythyristor@path#1{\pgf@circ@bipole@path{emptythyristor}{#1}}
\def\pgf@circ@fullthyristor@path#1{\pgf@circ@bipole@path{fullthyristor}{#1}}
\def\pgf@circ@toggleswitch@path#1{\pgf@circ@bipole@path{toggleswitch}{#1}}
\def\pgf@circ@memristor@path#1{\pgf@circ@bipole@path{memristor}{#1}}
\def\pgf@circ@emptytriac@path#1{\pgf@circ@bipole@path{emptytriac}{#1}}
\def\pgf@circ@fulltriac@path#1{\pgf@circ@bipole@path{fulltriac}{#1}}
\def\pgf@circ@tline@path#1{\pgf@circ@bipole@path{tline}{#1}}
\def\pgf@circ@mstline@path#1{\pgf@circ@bipole@path{mstline}{#1}}
\def\pgf@circ@squid@path#1{\pgf@circ@bipole@path{squid}{#1}}
\def\pgf@circ@barrier@path#1{\pgf@circ@bipole@path{barrier}{#1}}
\def\pgf@circ@thermocouple@path#1{\pgf@circ@bipole@path{thermocouple}{#1}}
\def\pgf@circ@fuse@path#1{\pgf@circ@bipole@path{fuse}{#1}}
\def\pgf@circ@afuse@path#1{\pgf@circ@bipole@path{afuse}{#1}}

\def\pgf@circ@gfsurgearrester@path#1{\ifpgf@circuit@europeangfsurgearrester\pgf@circ@europeangfsurgearrester@path{#1}\else\pgf@circ@americangfsurgearrester@path{#1}\fi}
\def\pgf@circ@europeangfsurgearrester@path#1{\pgf@circ@bipole@path{european gas filled surge arrester}{#1}}
\def\pgf@circ@americangfsurgearrester@path#1{\pgf@circ@bipole@path{american gas filled surge arrester}{#1}}

\def\pgf@circ@twoport@path#1{\pgf@circ@bipole@path{twoport}{#1}}
\def\pgf@circ@vco@path#1{\pgf@circ@bipole@path{vco}{#1}}
\def\pgf@circ@bandpass@path#1{\pgf@circ@bipole@path{bandpass}{#1}}
\def\pgf@circ@bandstop@path#1{\pgf@circ@bipole@path{bandstop}{#1}}
\def\pgf@circ@highpass@path#1{\pgf@circ@bipole@path{highpass}{#1}}
\def\pgf@circ@lowpass@path#1{\pgf@circ@bipole@path{lowpass}{#1}}
\def\pgf@circ@adc@path#1{\pgf@circ@bipole@path{adc}{#1}}
\def\pgf@circ@dac@path#1{\pgf@circ@bipole@path{dac}{#1}}
\def\pgf@circ@dsp@path#1{\pgf@circ@bipole@path{dsp}{#1}}
\def\pgf@circ@fft@path#1{\pgf@circ@bipole@path{fft}{#1}}
\def\pgf@circ@amp@path#1{\pgf@circ@bipole@path{amp}{#1}}
\def\pgf@circ@vamp@path#1{\pgf@circ@bipole@path{vamp}{#1}}
\def\pgf@circ@piattenuator@path#1{\pgf@circ@bipole@path{piattenuator}{#1}}
\def\pgf@circ@vpiattenuator@path#1{\pgf@circ@bipole@path{vpiattenuator}{#1}}
\def\pgf@circ@tattenuator@path#1{\pgf@circ@bipole@path{tattenuator}{#1}}
\def\pgf@circ@vtattenuator@path#1{\pgf@circ@bipole@path{vtattenuator}{#1}}
\def\pgf@circ@phaseshifter@path#1{\pgf@circ@bipole@path{phaseshifter}{#1}}
\def\pgf@circ@vphaseshifter@path#1{\pgf@circ@bipole@path{vphaseshifter}{#1}}
\def\pgf@circ@detector@path#1{\pgf@circ@bipole@path{detector}{#1}}

%%Mechanical
\def\pgf@circ@spring@path#1{\pgf@circ@bipole@path{spring}{#1}}
\def\pgf@circ@mass@path#1{\pgf@circ@bipole@path{mass}{#1}}
\def\pgf@circ@damper@path#1{\pgf@circ@bipole@path{damper}{#1}}
\def\pgf@circ@viscoe@path#1{\pgf@circ@bipole@path{viscoe}{#1}}

%% Styles

\def\comnpatname{\ifpgf@circuit@compat *\else\fi}
\def\compattikzset#1{\tikzset{\comnpatname#1}}

%\def\ctikzsetbipole#1#2{%
%	\tikzset{#1/.style= {to path=#2, \circuitikzbasekey, l=##1}}%
%}

\compattikzset{spring/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@spring@path, l=#1}}
\compattikzset{mass/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@mass@path, l=#1}}
\compattikzset{damper/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@damper@path, l=#1}}
\compattikzset{viscoe/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@viscoe@path, l=#1}}
\compattikzset{resistor/.style= {\circuitikzbasekey, /tikz/to path=\pgf@circ@resistor@path, l=#1}}
\compattikzset{american resistor/.style= {\circuitikzbasekey, /tikz/to path=\pgf@circ@bipole@path{resistor}{#1}, l=#1}}
\compattikzset{european resistor/.style= {\circuitikzbasekey, /tikz/to path=\pgf@circ@bipole@path{generic}{#1}, l=#1}}
\compattikzset{potentiometer/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@potentiometer@path, l=#1}}
\compattikzset{varistor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@varistor@path, l=#1}}
\compattikzset{photoresistor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@photoresistor@path, l=#1}}
\compattikzset{thermistor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@thermistor@path, l=#1}}
\compattikzset{thermistor ptc/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@thermistorptc@path, l=#1}}
\compattikzset{thermistor ntc/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@thermistorntc@path, l=#1}}
\compattikzset{american potentiometer/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@bipole@path{potentiometer}{#1}, l=#1}}
\compattikzset{european potentiometer/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@bipole@path{genericpotentiometer}{#1}, l=#1}}
\compattikzset{variable resistor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vresistor@path, l=#1}}
\compattikzset{variable american resistor/.style= {\circuitikzbasekey, /tikz/to path=\pgf@circ@bipole@path{vresistor}{#1}, l=#1}}
\compattikzset{variable european resistor/.style= {\circuitikzbasekey, /tikz/to path=\pgf@circ@bipole@path{tgeneric}{#1}, l=#1}}
\compattikzset{capacitor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@capacitor@path, l=#1}}
\compattikzset{elko/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ecapacitor@path, l=#1}}
\compattikzset{ecapacitor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ecapacitor@path, l=#1}}
\compattikzset{polar capacitor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@polarcapacitor@path, l=#1}}
\compattikzset{variable capacitor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vcapacitor@path, l=#1}}
\compattikzset{piezoelectric/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@piezoelectric@path, l=#1}}
\compattikzset{battery/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@battery@path, \circuitikzbasekey/bipole/is voltage=true,  \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{battery1/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@batteryone@path, \circuitikzbasekey/bipole/is voltage=true,  \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{battery2/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@batterytwo@path, \circuitikzbasekey/bipole/is voltage=true,  \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@inductor@path, l=#1}}
\compattikzset{gf surge arrester/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@gfsurgearrester@path, l=#1}}
\compattikzset{american gas filled surge arrester/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@americangfsurgearrester@path, l=#1}}
\compattikzset{european gas filled surge arrester/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@europeangfsurgearrester@path, l=#1}}
\compattikzset{gas filled surge arrester/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@gfsurgearrester@path, l=#1}}
\compattikzset{american inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@americaninductor@path, l=#1}}
\compattikzset{cute inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cuteinductor@path, l=#1}}
\compattikzset{cute choke/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cutechoke@path, l=#1}}
\compattikzset{european inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@europeaninductor@path, l=#1}}
\compattikzset{variable inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vinductor@path, l=#1}}
\compattikzset{variable european inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@veuropeaninductor@path, l=#1}}
\compattikzset{variable american inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vamericaninductor@path, l=#1}}
\compattikzset{variable cute inductor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vcuteinductor@path, l=#1}}
\compattikzset{tline/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@tline@path, l=#1}}
\compattikzset{transmission line/.style = {tline = #1}}
\compattikzset{TL/.style = {tline = #1}}
\compattikzset{mstline/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@mstline@path, l=#1}}
\compattikzset{european voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vsource@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{american voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vsourceam@path, \circuitikzbasekey/bipole/is voltage=true, v=#1}}
\compattikzset{european current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@isource@path, \circuitikzbasekey/bipole/is current=true, i=#1}}
\compattikzset{american current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@isourceam@path, \circuitikzbasekey/bipole/is current=true, i=#1}}
\compattikzset{european controlled voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cvsource@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{american controlled voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cvsourceam@path, \circuitikzbasekey/bipole/is voltage=true, v=#1}}
\compattikzset{european controlled current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cisource@path, \circuitikzbasekey/bipole/is current=true, i=#1}}
\compattikzset{american controlled current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cisourceam@path, \circuitikzbasekey/bipole/is current=true, i=#1}}
\compattikzset{sinusoidal voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vsourcesin@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1 }}
\compattikzset{square voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vsourcesquare@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1 }}
\compattikzset{triangle voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vsourcetri@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1 }}
\compattikzset{sinusoidal current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@isourcesin@path, \circuitikzbasekey/bipole/is current=true, i=#1}}
\compattikzset{controlled sinusoidal voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cvsourcesin@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{controlled sinusoidal current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cisourcesin@path, \circuitikzbasekey/bipole/is current=true, i=#1}}

\compattikzset{voltage source/.style = {\comnpatname \ifpgf@circuit@europeanvoltage european \else american \fi voltage source, \circuitikzbasekey/bipole/is voltage=true, v=#1}}
\compattikzset{current source/.style = {\comnpatname \ifpgf@circuit@europeancurrent european \else american \fi current source = #1, \circuitikzbasekey/bipole/is current=true}}
\compattikzset{controlled voltage source/.style = {\comnpatname \ifpgf@circuit@europeanvoltage european \else american \fi controlled voltage source, \circuitikzbasekey/bipole/is voltage=true, v=#1}}
\compattikzset{controlled current source/.style = {\comnpatname \ifpgf@circuit@europeancurrent european \else american \fi controlled current source = #1, \circuitikzbasekey/bipole/is current=true}}


\compattikzset{generic/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@generic@path, l=#1}}
\compattikzset{ageneric/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ageneric@path, l=#1}}
\compattikzset{tgeneric/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@tgeneric@path, l=#1}}
\compattikzset{fullgeneric/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fullgeneric@path, l=#1}}
\compattikzset{tfullgeneric/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@tfullgeneric@path, l=#1}}
\compattikzset{short/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@short@path}}
\compattikzset{open/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@open@path}}

\compattikzset{lamp/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@lamp@path}}
\compattikzset{bulb/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@bulb@path, l=#1}}

\compattikzset{squid/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@squid@path}}
\compattikzset{barrier/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@barrier@path}}
\compattikzset{thermocouple/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@thermocouple@path}}
\compattikzset{fuse/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fuse@path}}
\compattikzset{asymmetric fuse/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@afuse@path}}

\compattikzset{twoport/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@twoport@path}}
\compattikzset{vco/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vco@path}}
\compattikzset{bandpass/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@bandpass@path}}
\compattikzset{bandstop/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@bandstop@path}}
\compattikzset{highpass/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@highpass@path}}
\compattikzset{lowpass/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@lowpass@path}}
\compattikzset{adc/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@adc@path}}
\compattikzset{dac/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@dac@path}}
\compattikzset{dsp/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@dsp@path}}
\compattikzset{fft/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fft@path}}
\compattikzset{amp/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@amp@path}}
\compattikzset{vamp/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vamp@path}}
\compattikzset{piattenuator/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@piattenuator@path}}
\compattikzset{vpiattenuator/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vpiattenuator@path}}
\compattikzset{tattenuator/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@tattenuator@path}}
\compattikzset{vtattenuator/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vtattenuator@path}}
\compattikzset{phaseshifter/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@phaseshifter@path}}
\compattikzset{vphaseshifter/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vphaseshifter@path}}
\compattikzset{detector/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@detector@path}}

% % % % % %
% % Begin of Diodes
% % % % % %

\def\pgf@circ@fulldiode@path#1{\pgf@circ@bipole@path{fulldiode}{#1}}
\def\pgf@circ@fullzdiode@path#1{\pgf@circ@bipole@path{fullzdiode}{#1}}
\def\pgf@circ@fullzzdiode@path#1{\pgf@circ@bipole@path{fullzzdiode}{#1}}
\def\pgf@circ@fullsdiode@path#1{\pgf@circ@bipole@path{fullsdiode}{#1}}
\def\pgf@circ@fulltdiode@path#1{\pgf@circ@bipole@path{fulltdiode}{#1}}
\def\pgf@circ@fulllediode@path#1{\pgf@circ@bipole@path{fulllediode}{#1}}
\def\pgf@circ@fullpdiode@path#1{\pgf@circ@bipole@path{fullpdiode}{#1}}
\def\pgf@circ@fullvarcap@path#1{\pgf@circ@bipole@path{fullvarcap}{#1}}
\def\pgf@circ@fullbidirectionaldiode@path#1{\pgf@circ@bipole@path{fullbidirectionaldiode}{#1}}
\def\pgf@circ@emptydiode@path#1{\pgf@circ@bipole@path{emptydiode}{#1}}
\def\pgf@circ@emptyzdiode@path#1{\pgf@circ@bipole@path{emptyzdiode}{#1}}
\def\pgf@circ@emptyzzdiode@path#1{\pgf@circ@bipole@path{emptyzzdiode}{#1}}
\def\pgf@circ@emptysdiode@path#1{\pgf@circ@bipole@path{emptysdiode}{#1}}
\def\pgf@circ@emptytdiode@path#1{\pgf@circ@bipole@path{emptytdiode}{#1}}
\def\pgf@circ@emptylediode@path#1{\pgf@circ@bipole@path{emptylediode}{#1}}
\def\pgf@circ@emptypdiode@path#1{\pgf@circ@bipole@path{emptypdiode}{#1}}
\def\pgf@circ@emptyvarcap@path#1{\pgf@circ@bipole@path{emptyvarcap}{#1}}
\def\pgf@circ@emptybidirectionaldiode@path#1{\pgf@circ@bipole@path{emptybidirectionaldiode}{#1}}

\compattikzset{full diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fulldiode@path}}
\compattikzset{full Schottky diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fullsdiode@path}}
\compattikzset{full Zener diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fullzdiode@path}}
\compattikzset{full ZZener diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fullzzdiode@path}}
\compattikzset{full tunnel diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fulltdiode@path}}
\compattikzset{full photodiode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fullpdiode@path}}
\compattikzset{full led/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fulllediode@path}}
\compattikzset{full varcap/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fullvarcap@path}}
\compattikzset{full bidirectionaldiode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@fullbidirectionaldiode@path}}
\compattikzset{full thyristor/.style =  {\circuitikzbasekey, /tikz/to path=\pgf@circ@fullthyristor@path}}
\compattikzset{full triac/.style =  {\circuitikzbasekey, /tikz/to path=\pgf@circ@fulltriac@path}}

\compattikzset{empty diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptydiode@path}}
\compattikzset{empty Schottky diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptysdiode@path}}
\compattikzset{empty Zener diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptyzdiode@path}}
\compattikzset{empty ZZener diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptyzzdiode@path}}
\compattikzset{empty tunnel diode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptytdiode@path}}
\compattikzset{empty photodiode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptypdiode@path}}
\compattikzset{empty led/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptylediode@path}}
\compattikzset{empty varcap/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptyvarcap@path}}
\compattikzset{empty bidirectionaldiode/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptybidirectionaldiode@path}}
\compattikzset{empty thyristor/.style =  {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptythyristor@path}}
\compattikzset{empty triac/.style =  {\circuitikzbasekey, /tikz/to path=\pgf@circ@emptytriac@path}}

\compattikzset{stroke diode/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptydiode@path}}
\compattikzset{stroke Schottky diode/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptysdiode@path}}
\compattikzset{stroke Zener diode/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptyzdiode@path}}
\compattikzset{stroke ZZener diode/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptyzzdiode@path}}
\compattikzset{stroke tunnel diode/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptytdiode@path}}
\compattikzset{stroke photodiode/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptypdiode@path}}
\compattikzset{stroke led/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptylediode@path}}
\compattikzset{stroke varcap/.style = {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptyvarcap@path}}
\compattikzset{stroke thyristor/.style =  {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptythyristor@path}}
%\compattikzset{stroke triac/.style =  {\circuitikzbasekey,\circuitikzbasekey/bipole/is strokedsymbol=true, /tikz/to path=\pgf@circ@emptytriac@path}}

\def\pgfcircdiodestylemacro{\ifpgf@circuit@strokediode stroke \else\ifpgf@circuit@fulldiode full \else empty \fi\fi}

\compattikzset{Schottky diode/.style = {\comnpatname \pgfcircdiodestylemacro Schottky diode}}
\compattikzset{Zener diode/.style = {\comnpatname \pgfcircdiodestylemacro Zener diode}}
\compattikzset{ZZener diode/.style = {\comnpatname \pgfcircdiodestylemacro ZZener diode}}
\compattikzset{tunnel diode/.style = {\comnpatname \pgfcircdiodestylemacro tunnel diode}}
\compattikzset{photodiode/.style = {\comnpatname \pgfcircdiodestylemacro photodiode}}
\compattikzset{led/.style = {\comnpatname \pgfcircdiodestylemacro led}}
\compattikzset{varcap/.style = {\comnpatname \pgfcircdiodestylemacro varcap}}
\compattikzset{diode/.style = {\comnpatname \pgfcircdiodestylemacro diode}}
\compattikzset{thyristor/.style =  {\comnpatname \pgfcircdiodestylemacro thyristor}}
\compattikzset{triac/.style =  {\comnpatname \ifpgf@circuit@fulldiode full \else empty \fi triac}}%no stroke triac!
\compattikzset{bidirectionaldiode/.style =  {\comnpatname \ifpgf@circuit@fulldiode full \else empty \fi bidirectionaldiode}}%no stroke bidirectionaldiode! (based on triac)

%% Define Shortcuts
\compattikzset{Do/.style = {\comnpatname empty diode}}
\compattikzset{tDo/.style = {\comnpatname empty tunnel diode}}
\compattikzset{zDo/.style = {\comnpatname empty Zener diode}}
\compattikzset{zzDo/.style = {\comnpatname empty ZZener diode}}
\compattikzset{sDo/.style = {\comnpatname empty Schottky diode}}
\compattikzset{pDo/.style = {\comnpatname empty photodiode}}
\compattikzset{leDo/.style = {\comnpatname empty led}}
\compattikzset{VCo/.style = {\comnpatname empty varcap}}
\compattikzset{biDo/.style = {\comnpatname empty bidirectionaldiode}}
\compattikzset{Tyo/.style = {\comnpatname empty thyristor}}
\compattikzset{Tro/.style = {\comnpatname empty triac}}

\compattikzset{D*/.style = {\comnpatname full diode}}
\compattikzset{tD*/.style = {\comnpatname full tunnel diode}}
\compattikzset{zD*/.style = {\comnpatname full Zener diode}}
\compattikzset{zzD*/.style = {\comnpatname full ZZener diode}}
\compattikzset{sD*/.style = {\comnpatname full Schottky diode}}
\compattikzset{pD*/.style = {\comnpatname full photodiode}}
\compattikzset{leD*/.style = {\comnpatname full led}}
\compattikzset{VC*/.style = {\comnpatname full varcap}}
\compattikzset{biD*/.style = {\comnpatname full bidirectionaldiode}}
\compattikzset{Ty*/.style = {\comnpatname full thyristor}}
\compattikzset{Tr*/.style = {\comnpatname full triac}}

\compattikzset{D/.style = {\comnpatname diode}}
\compattikzset{tD/.style = {\comnpatname tunnel diode}}
\compattikzset{zD/.style = {\comnpatname Zener diode}}
\compattikzset{zzD/.style = {\comnpatname ZZener diode}}
\compattikzset{sD/.style = {\comnpatname Schottky diode}}
\compattikzset{pD/.style = {\comnpatname photodiode}}
\compattikzset{leD/.style = {\comnpatname led}}
\compattikzset{VC/.style = {\comnpatname varcap}}
\compattikzset{biD/.style = {\comnpatname bidirectionaldiode}}
\compattikzset{Ty/.style = {\comnpatname thyristor}}
\compattikzset{Tr/.style = {\comnpatname triac}}

\compattikzset{D-/.style = {\comnpatname stroke diode}}
\compattikzset{tD-/.style = {\comnpatname stroke tunnel diode}}
\compattikzset{zD-/.style = {\comnpatname stroke Zener diode}}
\compattikzset{zzD-/.style = {\comnpatname stroke ZZener diode}}
\compattikzset{sD-/.style = {\comnpatname stroke Schottky diode}}
\compattikzset{pD-/.style = {\comnpatname stroke photodiode}}
\compattikzset{leD-/.style = {\comnpatname stroke led}}
\compattikzset{VC-/.style = {\comnpatname stroke varcap}}
\compattikzset{Ty-/.style = {\comnpatname stroke thyristor}}
\compattikzset{Tr-/.style = {\comnpatname empty triac}}%no stroke triac!
\compattikzset{biD-/.style = {\comnpatname empty bidirectionaldiode}}%no stroke bidirectionaldiode! (based on triac)

% % % % % %
% % End of Diodes
% % % % % %


\compattikzset{memristor/.style =  {\circuitikzbasekey, /tikz/to path=\pgf@circ@memristor@path}}
\compattikzset{closing switch/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cspst@path, l=#1}}
\compattikzset{opening switch/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ospst@path, l=#1}}
\compattikzset{ncs/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ncs@path, l=#1}}
\compattikzset{nos/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@nos@path, l=#1}}
\compattikzset{normal closed switch/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ncs@path, l=#1}}
\compattikzset{normal open switch/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@nos@path, l=#1}}
\compattikzset{switch/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cspst@path, l=#1}}
\compattikzset{push button/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@pushbutton@path, l=#1}}
\compattikzset{nopb/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@pushbutton@path, l=#1}}
\compattikzset{normally open push button/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@pushbutton@path, l=#1}}
\compattikzset{ncpb/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ncpushbutton@path, l=#1}}
\compattikzset{normally closed push button/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ncpushbutton@path, l=#1}}
\compattikzset{toggle switch/.style =  {\circuitikzbasekey, /tikz/to path=\pgf@circ@toggleswitch@path}}

\compattikzset{ammeter/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ammeter@path}}
\compattikzset{voltmeter/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@voltmeter@path}}
\compattikzset{ohmmeter/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@ohmmeter@path}}
\tikzset{oscope/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@oscope@path, l=#1}}

% cute switches
%% closed cute switch
\def\pgf@circ@cuteclosedswitch@path#1{\pgf@circ@bipole@path{cuteclosedswitch}{#1}}
\compattikzset{cute closed switch/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cuteclosedswitch@path, l=#1}}
\compattikzset{ccsw/.style= {\comnpatname cute closed switch= #1}}

%% open cute switch
\def\pgf@circ@cuteopenswitch@path#1{\pgf@circ@bipole@path{cuteopenswitch}{#1}}
\compattikzset{cute open switch/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cuteopenswitch@path, l=#1}}
\compattikzset{cosw/.style= {\comnpatname cute open switch= #1}}

%% closing cute switch
\def\pgf@circ@cuteclosingswitch@path#1{\pgf@circ@bipole@path{cuteclosingswitch}{#1}}
\compattikzset{cute closing switch/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cuteclosingswitch@path, l=#1}}
\compattikzset{ccgsw/.style= {\comnpatname cute closing switch= #1}}

%% opening cute switch
\def\pgf@circ@cuteopeningswitch@path#1{\pgf@circ@bipole@path{cuteopeningswitch}{#1}}
\compattikzset{cute opening switch/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cuteopeningswitch@path, l=#1}}
\compattikzset{cogsw/.style= {\comnpatname cute opening switch= #1}}


% short forms
\compattikzset{esource/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@esource@path, \circuitikzbasekey/bipole/is voltage=true,\circuitikzbasekey/bipole/is voltageoutsideofsymbol=true,  v=#1}}
\compattikzset{pvsource/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@pvsource@path, \circuitikzbasekey/bipole/is voltage=true,\circuitikzbasekey/bipole/is voltageoutsideofsymbol=true,  v=#1}}
\compattikzset{dcvsource/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@dcvsource@path, \circuitikzbasekey/bipole/is voltage=true,\circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{dcisource/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@dcisource@path, \circuitikzbasekey/bipole/is current=true, l=#1}}

\compattikzset{ioosource/.style = {\circuitikzbasekey, \circuitikzbasekey/bipole/is current=true,/tikz/to path=\pgf@circ@oosource@path, i=#1}}
\compattikzset{voosource/.style = {\circuitikzbasekey, \circuitikzbasekey/bipole/is voltage=true,/tikz/to path=\pgf@circ@oosource@path, v=#1}}

\compattikzset{vsource/.style = {\comnpatname voltage source = #1}}
\compattikzset{isource/.style = {\comnpatname current source = #1}}
\compattikzset{cisource/.style = {\comnpatname controlled current source = #1}}
\compattikzset{cvsource/.style = {\comnpatname controlled voltage source = #1}}
\compattikzset{vsourcesin/.style = {\comnpatname sinusoidal voltage source = #1}}
\compattikzset{vsourcesquare/.style = {\comnpatname square voltage source = #1}}
\compattikzset{vsourcetri/.style = {triangle voltage source = #1}}
\compattikzset{isourcesin/.style = {\comnpatname sinusoidal current source = #1}}
\compattikzset{cisourcesin/.style = {\comnpatname controlled sinusoidal current source = #1}}
\compattikzset{cvsourcesin/.style = {\comnpatname controlled sinusoidal  voltage source = #1}}

\compattikzset{controlled vsource/.style = {\comnpatname controlled voltage source = #1}}
\compattikzset{controlled isource/.style = {\comnpatname controlled current source = #1}}
\compattikzset{controlled vsourcesin/.style = {\comnpatname controlled sinusoidal  voltage source = #1}}
\compattikzset{controlled isourcesin/.style = {\comnpatname controlled sinusoidal current source = #1}}

\compattikzset{R/.style= {\comnpatname resistor = #1}}
\compattikzset{vR/.style= {\comnpatname variable resistor = #1}}
\compattikzset{phR/.style= {\comnpatname photoresistor = #1}}
\compattikzset{thR/.style= {\comnpatname thermistor = #1}}
\compattikzset{thRp/.style= {\comnpatname thermistor ptc= #1}}
\compattikzset{thRn/.style= {\comnpatname thermistor ntc= #1}}
\compattikzset{pR/.style= {\comnpatname potentiometer = #1}}
\compattikzset{C/.style = {\comnpatname capacitor = #1}}
\compattikzset{eC/.style = {\comnpatname ecapacitor = #1}}
\compattikzset{pC/.style = {\comnpatname polar capacitor = #1}}
\compattikzset{vC/.style = {\comnpatname variable capacitor = #1}}
\compattikzset{PZ/.style = {\comnpatname piezoelectric = #1}}
\compattikzset{L/.style = {\comnpatname inductor = #1}}
\compattikzset{vL/.style = {\comnpatname variable inductor = #1}}
\compattikzset{V/.style = {\comnpatname voltage source = #1}}
\compattikzset{cV/.style = {\comnpatname controlled voltage source = #1}}
\compattikzset{sV/.style = {\comnpatname sinusoidal voltage source = #1}}
\compattikzset{sqV/.style = {\comnpatname square voltage source = #1}}
\compattikzset{tV/.style = {\comnpatname triangle voltage source = #1}}
\compattikzset{csV/.style = {\comnpatname controlled sinusoidal voltage source = #1}}
\def\pgf@temp#1{
    \compattikzset{V#1/.style = {\comnpatname voltage source, v#1=##1} }
    \compattikzset{cV#1/.style = {\comnpatname controlled  voltage source, v#1=##1} }
    \compattikzset{sV#1/.style = {\comnpatname sinusoidal  voltage source, v#1=##1} }
    \compattikzset{csV#1/.style = {\comnpatname controlled sinusoidal voltage source, v#1=##1} }
}
\pgf@temp{_>} \pgf@temp{_<} \pgf@temp{^>} \pgf@temp{^<}
\pgf@temp{>} \pgf@temp{<} \pgf@temp{^} \pgf@temp{_}

%current sources
\compattikzset{I/.style = {\comnpatname current source = #1}}
\compattikzset{cI/.style = {\comnpatname controlled current source = #1}}
\compattikzset{sI/.style = {\comnpatname sinusoidal current source = #1}}
\compattikzset{csI/.style = {\comnpatname controlled sinusoidal current source = #1}}
\def\pgf@temp#1{
    \compattikzset{I#1/.style = {\comnpatname current source, i#1=##1} }
    \compattikzset{cI#1/.style = {\comnpatname controlled current source, i#1=##1} }
    \compattikzset{sI#1/.style = {\comnpatname sinusoidal current source, i#1=##1} }
    \compattikzset{csI#1/.style = {\comnpatname controlled sinusoidal current source, i#1=##1} }
}
\pgf@temp{_>} \pgf@temp{_<} \pgf@temp{^>} \pgf@temp{^<}
\pgf@temp{>_} \pgf@temp{<_} \pgf@temp{>^} \pgf@temp{<^}
\pgf@temp{>} \pgf@temp{<} \pgf@temp{^} \pgf@temp{_}

% cute sources
\def\pgf@circ@vsourceC@path#1{\pgf@circ@bipole@path{vsourceC}{#1}}
\compattikzset{cute european voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vsourceC@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{vsourceC/.style= {\comnpatname cute european voltage source= #1}}
\compattikzset{ceV/.style= {\comnpatname cute european voltage source= #1}}

\def\pgf@circ@isourceC@path#1{\pgf@circ@bipole@path{isourceC}{#1}}
\compattikzset{cute european current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@isourceC@path, \circuitikzbasekey/bipole/is current=true, i=#1}}
\compattikzset{isourceC/.style= {\comnpatname cute european current source= #1}}
\compattikzset{ceI/.style= {\comnpatname cute european current source= #1}}

\def\pgf@circ@cvsourceC@path#1{\pgf@circ@bipole@path{cvsourceC}{#1}}
\compattikzset{cute european controlled voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cvsourceC@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{cvsourceC/.style= {\comnpatname cute european controlled voltage source= #1}}
\compattikzset{cceV/.style= {\comnpatname cute european controlled voltage source= #1}}

\def\pgf@circ@cisourceC@path#1{\pgf@circ@bipole@path{cisourceC}{#1}}
\compattikzset{cute european controlled current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cisourceC@path,  \circuitikzbasekey/bipole/is current=true, i=#1}}
\compattikzset{cisourceC/.style= {\comnpatname cute european controlled current source= #1}}
\compattikzset{cceI/.style= {\comnpatname cute european controlled current source= #1}}

% noise sources
\def\pgf@circ@vsourceN@path#1{\pgf@circ@bipole@path{vsourceN}{#1}}
\compattikzset{noise voltage source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@vsourceN@path, \circuitikzbasekey/bipole/is voltage=true, \circuitikzbasekey/bipole/is voltageoutsideofsymbol=true, v=#1}}
\compattikzset{vsourceN/.style= {\comnpatname noise voltage source= #1}}
\compattikzset{nV/.style= {\comnpatname noise voltage source= #1}}

\def\pgf@circ@isourceN@path#1{\pgf@circ@bipole@path{isourceN}{#1}}
\compattikzset{noise current source/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@isourceN@path, \circuitikzbasekey/bipole/is current=true, i=#1}}
\compattikzset{isourceN/.style= {\comnpatname noise current source= #1}}
\compattikzset{nI/.style= {\comnpatname noise current source= #1}}

% resistive sensor american style
\def\pgf@circ@resistivesens@path#1{\pgf@circ@bipole@path{resistivesens}{#1}}
\compattikzset{american resistive sensor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@resistivesens@path, l=#1}}
\compattikzset{european resistive sensor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@thermistorntc@path, l=#1}}
\compattikzset{resistive sensor/.style= {\circuitikzbasekey, /tikz/to path=\pgf@circ@sresistor@path, l=#1}}
\compattikzset{sR/.style= {\comnpatname resistive sensor= #1}}

\compattikzset{capacitive sensor/.style= {\circuitikzbasekey, /tikz/to path=\pgf@circ@capacitivesens@path, l=#1}}
\compattikzset{sC/.style= {\comnpatname capacitive sensor= #1}}

\compattikzset{cute inductive sensor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@cuteinductivesens@path, l=#1}}
\compattikzset{european inductive sensor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@europeaninductivesens@path, l=#1}}
\compattikzset{american inductive sensor/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@americaninductivesens@path, l=#1}}
\compattikzset{inductive sensor/.style= {\circuitikzbasekey, /tikz/to path=\pgf@circ@inductivesens@path, l=#1}}
\compattikzset{sL/.style= {\comnpatname inductive sensor= #1}}

\compattikzset{Mr/.style = {\comnpatname memristor}}

\compattikzset{cspst/.style = {\comnpatname closing switch = #1}}
\compattikzset{ospst/.style = {\comnpatname opening switch = #1}}
\compattikzset{spst/.style = {\comnpatname switch = #1}}

\compattikzset{afuse/.style = {\comnpatname asymmetric fuse=#1}}

\compattikzset{vdd/.style = {\comnpatname vcc = #1}}
\compattikzset{vss/.style = {\comnpatname vee = #1}}

% activate the to-style crossing
\def\pgf@circ@crossing@path#1{\pgf@circ@bipole@path{crossing}{#1}}
\compattikzset{crossing/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@crossing@path, l=#1}}
\compattikzset{xing/.style= {\comnpatname crossing= #1}}

%% loudspeaker and microphone

\def\pgf@circ@loudspeaker@path#1{\pgf@circ@bipole@path{loudspeaker}{#1}}
\compattikzset{loudspeaker/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@loudspeaker@path, l=#1}}

\def\pgf@circ@mic@path#1{\pgf@circ@bipole@path{mic}{#1}}
\compattikzset{mic/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@mic@path, l=#1}}

% more instrument
\def\pgf@circ@rmeter@path#1{\pgf@circ@bipole@path{rmeter}{#1}}
\compattikzset{rmeter/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@rmeter@path, l=#1}}
\def\pgf@circ@rmeterwa@path#1{\pgf@circ@bipole@path{rmeterwa}{#1}}
\compattikzset{rmeterwa/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@rmeterwa@path, l=#1}}
\def\pgf@circ@smeter@path#1{\pgf@circ@bipole@path{smeter}{#1}}
\compattikzset{smeter/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@smeter@path, l=#1}}
% current loop probes
\def\pgf@circ@iloop@path#1{\pgf@circ@bipole@path{iloop}{#1}}
\compattikzset{iloop/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@iloop@path, l=#1}}
\def\pgf@circ@iloop2@path#1{\pgf@circ@bipole@path{iloop2}{#1}}
\compattikzset{iloop2/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@iloop2@path, l=#1}}
% qucs-style probes
\def\pgf@circ@qiprobe@path#1{\pgf@circ@bipole@path{qiprobe}{#1}}
\compattikzset{qiprobe/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@qiprobe@path, l=#1}}
\def\pgf@circ@qvprobe@path#1{\pgf@circ@bipole@path{qvprobe}{#1}}
\compattikzset{qvprobe/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@qvprobe@path, l=#1}}
\def\pgf@circ@qpprobe@path#1{\pgf@circ@bipole@path{qpprobe}{#1}}
\compattikzset{qpprobe/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@qpprobe@path, l=#1}}


% Transistor like bipoles

\def\pgf@circ@trans@path#1#2{
    \pgfextra{
        \edef\pgf@temp{\pgfkeysvalueof{/tikz/circuitikz/bipole/name}}
        \def\pgf@circ@temp{#2}
        \ifx\pgf@temp\pgf@circ@temp % if it has not a name
            \pgfmathrandominteger{\pgf@circ@rand}{1000}{9999}
            \ctikzset{bipole/name = trans\pgf@circ@rand} % create it
        \fi
    }
    \ifpgf@circuit@bipole@inverted
        (\tikztostart) node[coordinate] (\ctikzvalof{bipole/name}end) {}
        (\tikztotarget) node[coordinate] (\ctikzvalof{bipole/name}start) {}
    \else
        (\tikztostart) node[coordinate] (\ctikzvalof{bipole/name}start) {}
        (\tikztotarget) node[coordinate] (\ctikzvalof{bipole/name}end) {}
    \fi
    \pgfextra{
        \pgfmathanglebetweenpoints{\pgfpointanchor{\ctikzvalof{bipole/name}start}{center}}
        {\pgfpointanchor{\ctikzvalof{bipole/name}end}{center}}
        \pgfmathadd{\pgfmathresult}{-90}
        \pgfmathround{\pgfmathresult}
        \edef\pgf@circ@direction{\pgfmathresult}
    }
    ($(\tikztostart) ! .5 ! (\tikztotarget)$)
    node[#1, /tikz/rotate=\pgf@circ@direction, xscale=\ctikzvalof{mirror value}]
    (\ctikzvalof{bipole/name}) {} node {\ctikzvalof{bipole/label/name}}
    \ifcsname pgf@anchor@#1@pathstart\endcsname%if special path-anchors are defined, use them!
        (\ctikzvalof{bipole/name}start.center) --(\ctikzvalof{bipole/name}.pathstart)
        (\ctikzvalof{bipole/name}.pathend)  -- (\ctikzvalof{bipole/name}end.center)
    \else
        (\ctikzvalof{bipole/name}start.center) --(\ctikzvalof{bipole/name}.left)
        (\ctikzvalof{bipole/name}.right)  -- (\ctikzvalof{bipole/name}end.center)
    \fi
    \pgfextra{
        \pgfcircresetpath
    }
    (\tikztotarget) 	\tikztonodes  % e si continua
}


\def\pgf@circ@definetranspath#1{
	\compattikzset{T#1/.style = {\circuitikzbasekey, /tikz/to path=\pgf@circ@trans@path{#1}{}, l=##1}}
}

\pgf@circ@definetranspath{elmech}
\pgf@circ@definetranspath{nmos}
\pgf@circ@definetranspath{pmos}
\pgf@circ@definetranspath{hemt}
\pgf@circ@definetranspath{npn}
\pgf@circ@definetranspath{pnp}
\pgf@circ@definetranspath{nfet}
\pgf@circ@definetranspath{nigfete}
\pgf@circ@definetranspath{nigfetd}
\pgf@circ@definetranspath{nigfetebulk}
\pgf@circ@definetranspath{pfet}
\pgf@circ@definetranspath{pigfete}
\pgf@circ@definetranspath{pigfetd}
\pgf@circ@definetranspath{pigfetebulk}
\pgf@circ@definetranspath{njfet}
\pgf@circ@definetranspath{pjfet}
\pgf@circ@definetranspath{pigbt}
\pgf@circ@definetranspath{nigbt}
\pgf@circ@definetranspath{Lpigbt}
\pgf@circ@definetranspath{Lnigbt}


==> pgfcircquadpoles.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the files gpl-3.0_license.txt and lppl-1-3c_license.txt for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Quadripoles

\long\def\pgfcircdeclarequadpole#1#2#3{
    \pgfdeclareshape{#1}
    {
        \anchor{center}{
            \northwest
            \pgf@x=0pt
            \pgf@y=0pt
        }
        \savedmacro{\stretto}{\def\stretto{0.4}}
        \savedanchor\northwest{%
            \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/quadpoles/#1/height}\pgf@circ@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=.5\pgf@circ@Rlen
            \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/quadpoles/#1/width}\pgf@x
        }
        \anchor{A2}{
            \northwest
            \pgf@y=-\pgf@y
        }
        \anchor{B1}{
            \northwest
            \pgf@x=-\pgf@x
        }
        \anchor{A1}{
            \northwest
        }
        \anchor{B2}{
            \northwest
            \pgf@x=-\pgf@x
            \pgf@y=-\pgf@y
        }
        %% notice for the dot anchors: I use the cute inductors as reference
        %% size; if you change one you have to change all of them.
        \anchor{inner dot A1}{
            \northwest
            \pgfmathsetlength\pgf@x{\stretto*\pgf@x +
            \ctikzvalof{bipoles/cuteinductor/height}*\pgf@circ@Rlen/2}
            \pgfmathsetlength\pgf@y{0.5*\pgf@circ@Rlen}
        }
        \anchor{outer dot A1}{
            \northwest
            \pgfmathsetlength\pgf@x{\stretto*\pgf@x -
            \ctikzvalof{bipoles/cuteinductor/height}*\pgf@circ@Rlen/2}
            \pgfmathsetlength\pgf@y{0.5*\pgf@circ@Rlen}
        }
        \anchor{inner dot A2}{
            \northwest
            \pgfmathsetlength\pgf@x{\stretto*\pgf@x +
            \ctikzvalof{bipoles/cuteinductor/height}*\pgf@circ@Rlen/2}
            \pgfmathsetlength\pgf@y{-0.5*\pgf@circ@Rlen}
        }
        \anchor{outer dot A2}{
            \northwest
            \pgfmathsetlength\pgf@x{\stretto*\pgf@x -
            \ctikzvalof{bipoles/cuteinductor/height}*\pgf@circ@Rlen/2}
            \pgfmathsetlength\pgf@y{-0.5*\pgf@circ@Rlen}
        }
        \anchor{inner dot B1}{
            \northwest
            \pgfmathsetlength\pgf@x{-\stretto*\pgf@x -
            \ctikzvalof{bipoles/cuteinductor/height}*\pgf@circ@Rlen/2}
            \pgfmathsetlength\pgf@y{0.5*\pgf@circ@Rlen}
        }
        \anchor{outer dot B1}{
            \northwest
            \pgfmathsetlength\pgf@x{-\stretto*\pgf@x +
            \ctikzvalof{bipoles/cuteinductor/height}*\pgf@circ@Rlen/2}
            \pgfmathsetlength\pgf@y{0.5*\pgf@circ@Rlen}
        }
        \anchor{inner dot B2}{
            \northwest
            \pgfmathsetlength\pgf@x{-\stretto*\pgf@x -
            \ctikzvalof{bipoles/cuteinductor/height}*\pgf@circ@Rlen/2}
            \pgfmathsetlength\pgf@y{-0.5*\pgf@circ@Rlen}
        }
        \anchor{outer dot B2}{
            \northwest
            \pgfmathsetlength\pgf@x{-\stretto*\pgf@x +
            \ctikzvalof{bipoles/cuteinductor/height}*\pgf@circ@Rlen/2}
            \pgfmathsetlength\pgf@y{-0.5*\pgf@circ@Rlen}
        }
        \anchor{north}{
            \northwest
            \pgf@x=0pt
        }
        \anchor{south}{
            \northwest
            \pgf@x=0pt
            \pgf@y=-\pgf@y
        }
        \anchor{west}{
            \northwest
            \pgf@y=0pt
        }
        \anchor{east}{
            \northwest
            \pgf@y=0pt
            \pgf@x=-\pgf@x
        }
        \anchor{south west}{
            \northwest
            \pgf@y=-\pgf@y
        }
        \anchor{north east}{
            \northwest
            \pgf@x=-\pgf@x
        }
        \anchor{north west}{
            \northwest
        }
        \anchor{south east}{
            \northwest
            \pgf@x=-\pgf@x
            \pgf@y=-\pgf@y
        }
        \anchor{base}{
            \northwest
            \pgf@x=0pt
        }
        #3
        \backgroundpath{
            \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

            \northwest
            \pgf@circ@res@up = \pgf@y
            \pgf@circ@res@down = -\pgf@y
            \pgf@circ@res@right = -\pgf@x
            \pgf@circ@res@left = \pgf@x
            #2
        }
    }
}


\def\pgf@circ@drawtransformerbasicanchor{
    \pgfkeysvalueof{/tikz/circuitikz/quadpoles/trans/height}
    \anchor{AA2}{
        \northwest
        \pgf@x=\pgfkeysvalueof{/tikz/circuitikz/quadpoles/transformer/width1}\pgf@x
        \pgf@x=.7\pgf@x
        \pgf@y=-\pgf@y
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/quadpoles/transformer/height1}\pgf@y
    }
    \anchor{BB1}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@x=\pgfkeysvalueof{/tikz/circuitikz/quadpoles/transformer/width1}\pgf@x
        \pgf@x=.7\pgf@x
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/quadpoles/transformer/height1}\pgf@y
    }
    \anchor{AA1}{
        \northwest
        \pgf@x=\pgfkeysvalueof{/tikz/circuitikz/quadpoles/transformer/width1}\pgf@x
        \pgf@x=.7\pgf@x
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/quadpoles/transformer/height1}\pgf@y
    }
    \anchor{BB2}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@x=\pgfkeysvalueof{/tikz/circuitikz/quadpoles/transformer/width1}\pgf@x
        \pgf@x=.7\pgf@x
        \pgf@y=-\pgf@y
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/quadpoles/transformer/height1}\pgf@y
    }
}

\def\pgf@circ@drawtransformerbasicbody{
    \pgfscope
        \pgfslopedattimetrue
        \pgfallowupsidedownattimetrue
        \pgftransformlineattime{.5}{%
            \pgfpoint%
            {\stretto\pgf@circ@res@left}%
            {\pgf@circ@res@up}%
            }{%
            \pgfpoint
            {\stretto\pgf@circ@res@left}%
            {\pgf@circ@res@down}%
        }

        \edef\pgf@circ@temp{\ctikzvalof{inductor}}%
        \def\pgf@temp{european}%
        \ifx\pgf@temp\pgf@circ@temp%
            \pgfnode{fullgenericshape}{center}{}{pgf@inductor1}{\pgfusepath{stroke}}
        \else%
            \def\pgf@temp{cute}
            \ifx\pgf@temp\pgf@circ@temp%
                \pgfnode{cuteinductorshape}{center}{}{pgf@inductor1}{\pgfusepath{stroke}}
            \else%
                \pgfnode{americaninductorshape}{center}{}{pgf@inductor1}{\pgfusepath{stroke}}
            \fi%
        \fi%


    \endpgfscope
    \pgfscope
        \pgfslopedattimetrue
        \pgfallowupsidedownattimetrue
        \pgftransformlineattime{.5}{%
            \pgfpoint%
            {\stretto\pgf@circ@res@right}%
            {\pgf@circ@res@down}%
            }{%
            \pgfpoint
            {\stretto\pgf@circ@res@right}%
            {\pgf@circ@res@up}%
        }

        \edef\pgf@circ@temp{\ctikzvalof{inductor}}%
        \def\pgf@temp{european}%
        \ifx\pgf@temp\pgf@circ@temp%
            \pgfnode{fullgenericshape}{center}{}{pgf@inductor2}{\pgfusepath{stroke}}
        \else%
            \def\pgf@temp{cute}
            \ifx\pgf@temp\pgf@circ@temp%
                \pgfnode{cuteinductorshape}{center}{}{pgf@inductor2}{\pgfusepath{stroke}}
            \else%
                \pgfnode{americaninductorshape}{center}{}{pgf@inductor2}{\pgfusepath{stroke}}
            \fi%
        \fi%

    \endpgfscope

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpointanchor{pgf@inductor1}{b}}

    \pgfpathmoveto{\pgfpointanchor{pgf@inductor1}{a}}
    \pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpointanchor{pgf@inductor2}{a}}

    \pgfpathmoveto{\pgfpointanchor{pgf@inductor2}{b}}
    \pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}

    \pgfusepath{draw}

}



% contrib Kristofer M. Monisit

\pgfdeclareshape{fd op amp}
{
    \anchor{center}{\pgfpointorigin}
    \savedanchor\northwest{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    }
    \savedanchor\outline{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    \ifpgf@circuit@oa@oplusup\else\pgf@y=-\pgf@y\fi
    }
    \anchor{south}{
        \northwest
        \pgf@y=-\pgf@y\pgf@x=0pt\relax
    }
    \anchor{north}{
        \northwest\pgf@x=0pt\relax
    }
    \savedanchor\left{%
        \pgf@y=0pt
    }
    \savedanchor\inOneFixed{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{in up}{
        \inOneFixed
    }
    \anchor{in down}{
        \inOneFixed
        \pgf@y=-\pgf@y
    }
    \savedanchor\inOne{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    \ifpgf@circuit@oa@iplusup\pgf@y=-\pgf@y\fi
    }
    \anchor{-}{
        \inOne
    }
    \anchor{+}{
        \inOne
        \pgf@y=-\pgf@y
    }
    \savedanchor\up{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfpointlineattime{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/up pos}}{
            \pgfpoint{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@circ@res@left}
        {\pgf@circ@res@up}}
        {\pgfpoint{.7\pgf@circ@res@right}{0pt}}
    }
    \anchor{up}{
        \up
    }
    \anchor{down}{
        \up
        \pgf@y=-\pgf@y
    }
    \anchor{out up}{
        \northwest
        \pgf@y=.5\pgf@y
        \pgf@x=-.7\pgf@x
    }
    \anchor{out down}{
        \northwest
        \pgf@y=-.5\pgf@y
        \pgf@x=-.7\pgf@x
    }
    \anchor{out +}{
        \outline
        \pgf@y=.5\pgf@y
        \pgf@x=-.7\pgf@x
    }
    \anchor{out -}{
        \outline
        \pgf@y=-.5\pgf@y
        \pgf@x=-.7\pgf@x
    }
    \anchor{west}{
        \left
    }
    \anchor{east}{
        \left
        \pgf@x=-.7\pgf@x
    }

    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-.7\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-.7\pgf@x \pgf@y=-\pgf@y }
    \backgroundpath{
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x

        % Triangle
        \pgfscope
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/quadpoles/thickness}\pgflinewidth}
            \pgftransformxshift{.7\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=.7\pgf@circ@res@step
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{0pt}}
            \pgfpathclose
            \pgf@circ@draworfill
        \endpgfscope
        % Negative input terminal
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@up}}
        \pgftext[left, at=\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@up}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/font} \ifpgf@circuit@oa@iplusup$+$\else$-$\fi}

        % Positive input terminal
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@down}}
        \pgftext[left, at=\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@down}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/font} \ifpgf@circuit@oa@iplusup$-$\else$+$\fi}

        % Negative output terminal
        \pgfpathmoveto{\pgfpoint
            {0.7\pgf@circ@res@right}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@down}}
        \pgftext[left, at=\pgfpoint{0.3\pgf@circ@res@left}{.3\pgf@circ@res@down}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/font} \ifpgf@circuit@oa@oplusup$-$\else$+$\fi}

        % Positive output terminal
        \pgfpathmoveto{\pgfpoint
            {0.7\pgf@circ@res@right}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@up}}
        \pgftext[left, at=\pgfpoint{0.3\pgf@circ@res@left}{.3\pgf@circ@res@up}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/font} \ifpgf@circuit@oa@oplusup$+$\else$-$\fi}

        \pgfsetrectcap
        % Draw them all!
        \pgfusepath{draw}

    }
}


%% instrumentation amplifier diff output

\pgfdeclareshape{fd inst amp}
{
    % when tikz calls the anchor it wants the relative position in the lengths
    % \pgf@x  \pgf@y
    % \pgfpoint* functions set that variables
    % anchors are visible outside and run on use
    \anchor{center}{\pgfpointorigin}
    % savedanchors are internals and run on node creation (not use)
    % bounding-box top left
    \savedanchor\northwest{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{nw}{
        \northwest
    }
    \anchor{south}{
        \northwest
        \pgf@y=-\pgf@y\pgf@x=0pt\relax
    }
    \anchor{north}{
        \northwest\pgf@x=0pt\relax
    }
    \savedanchor\left{%
        \pgf@y=0pt
    }
    \anchor{leftedge}
    {\left
        \pgf@x = \pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@x
    }
    \savedanchor\inOneFixed{%
          \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/height}\pgf@circ@Rlen
          \pgf@y=.5\pgf@y
          \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@y
          \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/width}\pgf@circ@Rlen
          \pgf@x=.5\pgf@x
    }
    \anchor{in up}{
        \inOneFixed
    }
    \anchor{in down}{
        \inOneFixed
        \pgf@y=-\pgf@y
    }
    \savedanchor\inOne{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/input height}\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
        \ifpgf@circuit@oa@iplusup\pgf@y=-\pgf@y\fi
    }
    \anchor{-}{
        \inOne
    }
    \anchor{+}{
        \inOne
        \pgf@y=-\pgf@y
    }
    \savedanchor\up{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfpointlineattime{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/up pos}}{
            \pgfpoint{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/port width}\pgf@circ@res@left}
        {\pgf@circ@res@up}}
        {\pgfpoint{.7\pgf@circ@res@right}{.6\pgf@circ@res@up}}
    }
    \anchor{up}{
        \up
    }
    \anchor{down}{
        \up
        \pgf@y=-\pgf@y
    }
    % reference voltage input anchors.
    \savedanchor\refv{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfpointlineattime{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/refv pos}}{
            \pgfpoint{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/port width}\pgf@circ@res@left}
        {\pgf@circ@res@up}}
        {\pgfpoint{.7\pgf@circ@res@right}{.6\pgf@circ@res@up}}
    }
    % we need both because they are normally drawn under the amp, and if you
    % mirror it vertically you need them
    \anchor{refv up}{
        \refv
    }
    \anchor{refv down}{
        \refv
        \pgf@y=-\pgf@y
    }
    \savedanchor\outport{
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/input height}\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/width}\pgf@circ@Rlen
        \pgf@x=-.5\pgf@x
        \ifpgf@circuit@oa@oplusup\else\pgf@y=-\pgf@y\fi
    }
    \anchor{out}{
        \outport
        \pgf@y=0pt
    }
    \anchor{out +}{
        \outport
    }
    \anchor{out -}{
        \outport
        \pgf@y=-\pgf@y
    }
    \savedanchor\outportfixed{
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/input height}\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/width}\pgf@circ@Rlen
        \pgf@x=-.5\pgf@x
    }
    \anchor{out up}{
        \outportfixed
    }
    \anchor{out down}{
        \outportfixed
        \pgf@y=-\pgf@y
    }
    %
    \anchor{west}{
        \left
    }
    \anchor{east}{
        \left
        \pgf@x=-\pgf@x
    }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \anchor{text}{\pgfpoint{-.5\wd\pgfnodeparttextbox}{\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox}}

    % let's start drawing the component
    \backgroundpath{
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
        %
        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        % main component, normally in thicker lines
        \pgfscope
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}
            \pgftransformxshift{.7\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=.7\pgf@circ@res@step
            %first point (near output)
            \pgfpathmoveto{\pgfpoint{1.4\pgf@circ@res@right}{0}}
            %from the exit to the top (short side)... (note that the .6 must be copied in \up and \refv anchors
            \pgfpathlineto{\pgfpoint{1.4\pgf@circ@res@right}{.6\pgf@circ@res@up}}
            % and then to the input "front up", "down", to the output short side "down"
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
            \pgfpathlineto{\pgfpoint{1.4\pgf@circ@res@right}{.6\pgf@circ@res@down}}
            % ...and close
            \pgfpathclose
            \pgf@circ@draworfill
        \endpgfscope
        % input terminal up
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/input height}\pgf@circ@res@up}}
        %
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/port width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/input height}\pgf@circ@res@up}}
        %
        \pgftext[left, at=\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/input height}\pgf@circ@res@up}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/font} \ifpgf@circuit@oa@iplusup$+$\else$-$\fi}

        % input terminal down
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/input height}\pgf@circ@res@down}}
        %
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/port width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/input height}\pgf@circ@res@down}}
        \pgftext[left, at=\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/input height}\pgf@circ@res@down}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/font} \ifpgf@circuit@oa@iplusup$-$\else$+$\fi}
        % output leads down and up
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/input height}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/input height}\pgf@circ@res@down}} %
        \pgftext[right, at=\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/port width}\pgf@circ@res@right}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/input height}\pgf@circ@res@down}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/font}\ifpgf@circuit@oa@oplusup$-\;$\else$+\;$\fi}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/input height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/input height}\pgf@circ@res@up}} %
        \pgftext[right, at=\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/port width}\pgf@circ@res@right}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/input height}\pgf@circ@res@up}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/fd inst amp/font}\ifpgf@circuit@oa@oplusup$+\;$\else$-\;$\fi}
        %
        \pgfsetrectcap
        \pgfusepath{draw}
    }
}


\pgfcircdeclarequadpole{transformer}{
    \pgf@circ@drawtransformerbasicbody
}{\pgf@circ@drawtransformerbasicanchor}

\pgfcircdeclarequadpole{transformer core}{

    \pgf@circ@drawtransformerbasicbody

    \pgfmoveto{\pgfpoint%
        {\ctikzvalof{quadpoles/transformer core/core width}\pgf@circ@res@right}%
        {\ctikzvalof{quadpoles/transformer core/core height}\pgf@circ@res@down}%
    }
    \pgflineto{
        \pgfpoint
        {\ctikzvalof{quadpoles/transformer core/core width}\pgf@circ@res@right}%
        {\ctikzvalof{quadpoles/transformer core/core height}\pgf@circ@res@up}%
    }

    \pgfmoveto{\pgfpoint%
        {\ctikzvalof{quadpoles/transformer core/core width}\pgf@circ@res@left}%
        {\ctikzvalof{quadpoles/transformer core/core height}\pgf@circ@res@down}%
    }
    \pgflineto{
        \pgfpoint
        {\ctikzvalof{quadpoles/transformer core/core width}\pgf@circ@res@left}%
        {\ctikzvalof{quadpoles/transformer core/core height}\pgf@circ@res@up}%
    }

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgflinewidth}
    \pgfusepath{draw}
}{\pgf@circ@drawtransformerbasicanchor}


\pgfcircdeclarequadpole{gyrator}{

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@left}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\stretto\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}

    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/quadpoles/thickness}\pgflinewidth}
    \pgfpathmoveto{\pgfpoint{\stretto\pgf@circ@res@left}{.7*\stretto\pgf@circ@res@down}}
    \pgfpatharc{90}{270}{.7*\stretto\pgf@circ@res@down}

    \pgfpathmoveto{\pgfpoint{\stretto\pgf@circ@res@right}{.7*\stretto\pgf@circ@res@up}}
    \pgfpatharc{-90}{90}{.7*\stretto\pgf@circ@res@down}
    \pgfusepath{draw}

}{}

%% four-port
% defines a general outer box for four-ports
% TikZ usage:
%		\draw (0,0) node[coupler](coup){\SI{-3}{dB}}
%		(coup.port1) to[short,-o] ++(-1,0)
%

\long\def\pgfcircdeclarefourport#1#2{
    \pgfdeclareshape{#1}{
        \anchor{center}{
            \northwest
            \pgf@x=0pt
            \pgf@y=0pt
        }
        \savedanchor\northwest{%
            \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/quadpoles/#1/height}\pgf@circ@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=.5\pgf@circ@Rlen
            \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/quadpoles/#1/width}\pgf@x
        }
        \anchor{north}{
            \northwest
            \pgf@x=0pt
        }
        \anchor{south}{
            \northwest
            \pgf@x=0pt
            \pgf@y=-\pgf@y
        }
        \anchor{west}{
            \northwest
            \pgf@y=0pt
        }
        \anchor{east}{
            \northwest
            \pgf@y=0pt
            \pgf@x=-\pgf@x
        }
        \anchor{south west}{
            \northwest
            \pgf@y=-\pgf@y
        }
        \anchor{north east}{
            \northwest
            \pgf@x=-\pgf@x
        }
        \anchor{north west}{
            \northwest
        }
        \anchor{south east}{
            \northwest
            \pgf@x=-\pgf@x
            \pgf@y=-\pgf@y
        }
        \anchor{port1}{
            \northwest
            \pgf@y=-0.5\pgf@y
        }
        \anchor{port2}{
            \northwest
            \pgf@x=-\pgf@x
            \pgf@y=-0.5\pgf@y
        }
        \anchor{port3}{
            \northwest
            \pgf@x=-\pgf@x
            \pgf@y=0.5\pgf@y
        }
        \anchor{port4}{
            \northwest
            \pgf@y=0.5\pgf@y
        }
        \anchor{1}{
            \northwest
            \pgf@y=-0.5\pgf@y
        }
        \anchor{2}{
            \northwest
            \pgf@x=-\pgf@x
            \pgf@y=-0.5\pgf@y
        }
        \anchor{3}{
            \northwest
            \pgf@x=-\pgf@x
            \pgf@y=0.5\pgf@y
        }
        \anchor{4}{
            \northwest
            \pgf@y=0.5\pgf@y
        }

        \anchor{text}{
            \northwest
            \advance \pgf@y by 0.5\ht\pgfnodeparttextbox
            \pgf@x=-.5\wd\pgfnodeparttextbox
        }
        \backgroundpath{
            \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

            \northwest
            \pgf@circ@res@up = \pgf@y
            \pgf@circ@res@down = -\pgf@y
            \pgf@circ@res@right = -\pgf@x
            \pgf@circ@res@left = \pgf@x

            \pgfstartlinewidth=\pgflinewidth

            % draw outer box
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
            \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \pgfusepath{draw}

            % draw inner stuff
            #2

            % draw inner text
            \pgftext[center,x=-0.15\pgf@circ@res@step,y=0]{\ctikzvalof{bipoles/twoport/text}}
        }
    }
}

% four-port
\pgfcircdeclarefourport{fourport}{}


% straight coupler
\pgfcircdeclarefourport{coupler}{
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0.5\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0.5\pgf@circ@res@up}}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0.5\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0.5\pgf@circ@res@down}}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{0.7\pgf@circ@res@left}{0.4\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{0.7\pgf@circ@res@right}{0.4\pgf@circ@res@up}}
    \pgfsetarrows{latex-latex}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.7\pgf@circ@res@left}{0.4\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0.7\pgf@circ@res@right}{0.4\pgf@circ@res@down}}
    \pgfsetarrows{latex-latex}
    \pgfusepath{draw}
}

% "bended" coupler
\pgfcircdeclarefourport{coupler2}{
    \pgfsetlinewidth{\pgfstartlinewidth}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0.5\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0.5\pgf@circ@res@up}}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0.5\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0.5\pgf@circ@res@down}}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{0.1\pgf@circ@res@left}{0pt}}
    \pgfpatharc{0}{90} {0.4\pgf@circ@res@up}
    \pgfsetarrowsend{latex}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.1\pgf@circ@res@left}{0pt}}
    \pgfpatharc{0}{-90} {0.4\pgf@circ@res@up}
    \pgfsetarrowsend{latex}
    \pgfusepath{draw}

    \pgfpathmoveto{\pgfpoint{0.1\pgf@circ@res@right}{0pt}}
    \pgfpatharc{180}{90} {0.4\pgf@circ@res@up}
    \pgfsetarrowsend{latex}
    \pgfusepath{draw}
    \pgfpathmoveto{\pgfpoint{0.1\pgf@circ@res@right}{0pt}}
    \pgfpatharc{-180}{-90} {0.4\pgf@circ@res@up}
    \pgfsetarrowsend{latex}
    \pgfusepath{draw}
}


==> pgfcircshapes.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the files gpl-3.0_license.txt and lppl-1-3c_license.txt for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Other shapes

%% Nothing

\pgfdeclareshape{emptyshape}{
    \savedanchor{\northeast}{%
        \pgf@x=.5\wd\pgfnodeparttextbox%
        \pgf@y=.5\ht\pgfnodeparttextbox%
    }
    \anchor{north}{\northeast\pgf@x=0cm\relax}
    \anchor{east}{\northeast\pgf@y=0cm\relax}
    \anchor{south}{\northeast\pgf@y=-\pgf@y \pgf@x=0cm\relax}
    \anchor{west}{\northeast\pgf@y=0cm\pgf@x=-\pgf@x}
    \anchor{north east}{\northeast}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x}
    \anchor{south east}{\northeast\pgf@y=-\pgf@y}
    \anchor{south west}{\northeast\pgf@y=-\pgf@y\pgf@x=-\pgf@x}
    \anchor{text}{\pgfpoint{-.5\wd\pgfnodeparttextbox}{\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox}}
    \anchor{center}{
        \pgfpointorigin
    }
}

%% Full terminal

\pgfdeclareshape{circ}{
    \anchor{center}{
        \pgfpointorigin
    }
    \savedanchor\northwest{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/nodes width}\pgf@circ@Rlen
        \pgf@x=-\pgf@y
    }
    \anchor{center}{ \pgf@y=0pt \pgf@x=0pt }
    \anchor{east}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{e}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{west}{ \northwest \pgf@y=0pt }
    \anchor{w}{ \northwest \pgf@y=0pt }
    \anchor{south}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{s}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{north}{ \northwest \pgf@x=0pt }
    \anchor{n}{ \northwest \pgf@x=0pt }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \anchorborder{
        \pgf@circ@res@left=\pgf@x
        \pgf@circ@res@up=\pgf@y
        \pgfpointborderellipse{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}
        }{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/nodes width}*\pgf@circ@Rlen}{\pgfkeysvalueof{/tikz/circuitikz/nodes width}*\pgf@circ@Rlen}}
    }
    \behindforegroundpath{

        \pgfscope
            \pgfpathcircle{\pgfpointorigin}{\pgfkeysvalueof{/tikz/circuitikz/nodes width}*\pgf@circ@Rlen}
            \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
            \pgfsetfillopacity{1.0}
            \pgfusepath{draw,fill}
        \endpgfscope

    }
}

%% Empty terminal

\pgfdeclareshape{ocirc}{
    \anchor{center}{
        \pgfpointorigin
    }
    \savedanchor\northwest{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/nodes width}\pgf@circ@Rlen
        \pgf@x=-\pgf@y
    }
    \anchor{center}{ \pgf@y=0pt \pgf@x=0pt }
    \anchor{east}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{e}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{west}{ \northwest \pgf@y=0pt }
    \anchor{w}{ \northwest \pgf@y=0pt }
    \anchor{south}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{s}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{north}{ \northwest \pgf@x=0pt }
    \anchor{n}{ \northwest \pgf@x=0pt }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \anchorborder{
        \pgf@circ@res@left=\pgf@x
        \pgf@circ@res@up=\pgf@y
        \pgfpointborderellipse{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}
        }{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/nodes width}*\pgf@circ@Rlen}{\pgfkeysvalueof{/tikz/circuitikz/nodes width}*\pgf@circ@Rlen}}
    }

    \behindforegroundpath{

        \pgfscope
            \pgfpathcircle{\pgfpointorigin}{\pgfkeysvalueof{/tikz/circuitikz/nodes width}*\pgf@circ@Rlen}
            \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
            \ifx\tikz@fillcolor\pgfutil@empty
                \pgfsetfillcolor{white}
            \else
                \pgfsetfillcolor{\tikz@fillcolor}
            \fi
            \pgfsetfillopacity{1.0}
            \pgfusepath{draw,fill}
        \endpgfscope

    }
}

%% Diamond terminal

\pgfdeclareshape{diamondpole}{
    \anchor{center}{
        \pgfpointorigin
    }
    \savedanchor\northwest{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/nodes width}\pgf@circ@Rlen
        \pgf@x=-\pgf@y
    }
    \anchor{center}{ \pgf@y=0pt \pgf@x=0pt }
    \anchor{east}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{e}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{west}{ \northwest \pgf@y=0pt }
    \anchor{w}{ \northwest \pgf@y=0pt }
    \anchor{south}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{s}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{north}{ \northwest \pgf@x=0pt }
    \anchor{n}{ \northwest \pgf@x=0pt }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \anchorborder{
        \pgf@circ@res@left=\pgf@x
        \pgf@circ@res@up=\pgf@y
    }
    \behindforegroundpath{
        \pgfscope
            \pgfmathsetlength{\pgf@circ@res@temp}{\pgfkeysvalueof{/tikz/circuitikz/nodes width}*\pgf@circ@Rlen}
            \pgftransformrotate{45}
            \pgfpathrectanglecorners
            {\pgfpoint{\pgf@circ@res@left-\pgf@circ@res@temp}{\pgf@circ@res@up+\pgf@circ@res@temp}}
            {\pgfpoint{\pgf@circ@res@left+\pgf@circ@res@temp}{\pgf@circ@res@up-\pgf@circ@res@temp}}
            \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
            \pgfsetfillopacity{1.0}
            \pgfusepath{draw,fill}
        \endpgfscope
    }
}

% BNC connector

\pgfdeclareshape{bnc}{
    \anchor{center}{
        \pgfpointorigin
    }
    % BNC size is 2.5 times the size of the internal "ocirc"
    \savedanchor\northwest{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/nodes width}\pgf@circ@Rlen
        \pgf@y=2.5\pgf@y
        \pgf@x=-\pgf@y
    }
    % center is on the opening
    \anchor{center}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{zero}{ \pgfpointorigin }
    \anchor{hot}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{shield}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    % geo-anchors
    \anchor{east}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{right}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{west}{ \northwest \pgf@y=0pt }
    \anchor{left}{ \northwest \pgf@y=0pt }
    \anchor{south}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{north}{ \northwest \pgf@x=0pt }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    % put the node text above and centered
    \anchor{text}{\pgfextracty{\pgf@circ@res@up}{\northwest}
        \pgfpoint{-.5\wd\pgfnodeparttextbox}{
            \dimexpr.5\dp\pgfnodeparttextbox+.5\ht\pgfnodeparttextbox+\pgf@circ@res@up\relax
        }
    }
    \anchorborder{
        \pgf@circ@res@left=\pgf@x
        \pgf@circ@res@up=\pgf@y
        \pgfpointborderellipse{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}
        }{\pgfpoint{2.5*\pgfkeysvalueof{/tikz/circuitikz/nodes width}*\pgf@circ@Rlen}{2.5*\pgfkeysvalueof{/tikz/circuitikz/nodes width}*\pgf@circ@Rlen}}
    }
    \behindforegroundpath{
        \pgfextracty{\pgf@circ@res@other}{\northwest}
        \pgf@circ@res@step=\pgfkeysvalueof{/tikz/circuitikz/nodes width}\pgf@circ@Rlen
        \pgfscope
            \pgfstartlinewidth=\pgflinewidth
            \pgfsetlinewidth{\ctikzvalof{bipoles/thickness}\pgflinewidth}
            \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
            % external circle
            \pgfscope
                % clipping path: first a rectangle bigger then the shape
                % to avoid problems with the line thickness
                \pgfpathrectanglecorners{\pgfpoint{-2\pgf@circ@res@other}{-2\pgf@circ@res@other}}
                    {\pgfpoint{2\pgf@circ@res@other}{2\pgf@circ@res@other}}
                % next the opening to the right
                \pgfpathrectanglecorners{\pgfpoint{-\pgf@circ@res@step}{-\pgf@circ@res@step}}
                    {\pgfpoint{2\pgf@circ@res@other}{\pgf@circ@res@step}}
                % do the difference and clip before drawing
                \pgfseteorule
                \pgfusepath{clip}
                \pgfpathcircle{\pgfpointorigin}{\pgf@circ@res@other}
                \pgfusepath{draw}
            \endpgfscope
            % internal circle
            \pgfpathcircle{\pgfpointorigin}{\pgf@circ@res@step}
            \pgf@circ@draworfill
            % and the contact line to the right
            \pgfsetlinewidth{\pgfstartlinewidth}
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{0pt}}
            \pgfusepath{draw}
        \endpgfscope
    }
}

%% Fill for correct rectangular joins

\pgfdeclareshape{rectjoinfill}{
    \savedanchor{\northeast}{%
        \pgf@x=.5\pgflinewidth%
        \pgf@y=.5\pgflinewidth%
    }
    \anchor{north}{\northeast\pgf@x=0cm\relax}
    \anchor{east}{\northeast\pgf@y=0cm\relax}
    \anchor{south}{\northeast\pgf@y=-\pgf@y \pgf@x=0cm\relax}
    \anchor{west}{\northeast\pgf@y=0cm\pgf@x=-\pgf@x}
    \anchor{north east}{\northeast}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x}
    \anchor{south east}{\northeast\pgf@y=-\pgf@y}
    \anchor{south west}{\northeast\pgf@y=-\pgf@y\pgf@x=-\pgf@x}
    \anchor{center}{
        \pgfpointorigin
    }
    \anchorborder{
        \pgf@circ@res@left=\pgf@x
        \pgf@circ@res@up=\pgf@y
    }
    \behindforegroundpath{
        \pgfscope
            \pgfpathrectanglecorners
            {\pgfpoint{0}{.5\pgflinewidth}}
            {\pgfpoint{0}{-.5\pgflinewidth}}
            \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
            \pgfusepath{draw,fill}
        \endpgfscope
    }
}


%% Current arrow

\pgfdeclareshape{currarrow}{
    \savedanchor{\northeast}{%
        \pgf@circ@res@step = \pgf@circ@Rlen
        \divide \pgf@circ@res@step by \pgfkeysvalueof{/tikz/circuitikz/current arrow scale}
        \pgf@x=.5\pgf@circ@res@step
        \pgf@y=\pgf@x%
    }
    \anchor{north}{\northeast\pgf@x=0cm\relax}
    \anchor{east}{\northeast\pgf@y=0cm\relax}
    \anchor{south}{\northeast\pgf@y=-\pgf@y \pgf@x=0cm\relax}
    \anchor{west}{\northeast\pgf@y=0cm\pgf@x=-\pgf@x}
    \anchor{north east}{\northeast}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x}
    \anchor{south east}{\northeast\pgf@y=-\pgf@y}
    \anchor{south west}{\northeast\pgf@y=-\pgf@y\pgf@x=-\pgf@x}
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{tip}{
        \pgfpointorigin
        \pgf@circ@res@step = \pgf@circ@Rlen
        \divide \pgf@circ@res@step by \pgfkeysvalueof{/tikz/circuitikz/current arrow scale}
        \pgf@x	=\pgf@circ@res@step
    }
    \behindforegroundpath{
        \pgfscope
            \pgf@circ@res@step = \pgf@circ@Rlen
            \divide \pgf@circ@res@step by \pgfkeysvalueof{/tikz/circuitikz/current arrow scale}

            \pgfpathmoveto{\pgfpoint{-.7\pgf@circ@res@step}{0pt}}
            \pgfpathlineto{\pgfpoint{-.7\pgf@circ@res@step}{-.8\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{1\pgf@circ@res@step}{0pt}}
            \pgfpathlineto{\pgfpoint{-.7\pgf@circ@res@step}{.8\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{-.7\pgf@circ@res@step}{0pt}}
            \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
            \pgfusepath{draw,fill}

        \endpgfscope
    }
}

%% Flow arrow

\pgfdeclareshape{flowarrow}{
    \savedanchor{\northeast}{%
        \pgf@circ@res@step = \pgf@circ@Rlen
        \divide \pgf@circ@res@step by \pgfkeysvalueof{/tikz/circuitikz/current arrow scale}
        \pgf@y=.5\pgf@circ@res@step
        \pgf@circ@res@step = \pgf@circ@Rlen
        \divide \pgf@circ@res@step by 4
        \pgf@x=\pgf@circ@res@step%
    }
    \anchor{north}{\northeast\pgf@x=0cm\relax}
    \anchor{east}{\northeast\pgf@y=0cm\relax}
    \anchor{south}{\northeast\pgf@y=-\pgf@y \pgf@x=0cm\relax}
    \anchor{west}{\northeast\pgf@y=0cm\pgf@x=-\pgf@x}
    \anchor{north east}{\northeast}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x}
    \anchor{south east}{\northeast\pgf@y=-\pgf@y}
    \anchor{south west}{\northeast\pgf@y=-\pgf@y\pgf@x=-\pgf@x}
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{tip}{
        \pgfpointorigin
        \pgf@circ@res@step = \pgf@circ@Rlen
        \divide \pgf@circ@res@step by \pgfkeysvalueof{/tikz/circuitikz/current arrow scale}
        \pgf@x	=\pgf@circ@res@step
    }
    \behindforegroundpath{
        \pgfscope
            \pgf@circ@res@step = \pgf@circ@Rlen
            \divide \pgf@circ@res@step by 4
            \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@step}{0pt}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{0pt}}
            \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
            \pgfusepath{draw}
            \pgftransformshift{\pgfpoint{\pgf@circ@res@step}{0pt}}
            \pgfnode{currarrow}{tip}{}{}{\pgfusepath{fill}}
        \endpgfscope
    }
}

%% Input arrow

\pgfdeclareshape{inputarrow}{
    \savedanchor{\northeast}{% this is really not northeast, really -northwest
        \pgf@circ@res@step = \pgf@circ@Rlen
        \divide \pgf@circ@res@step by \pgfkeysvalueof{/tikz/circuitikz/current arrow scale}
        \pgf@y=.5\pgf@circ@res@step
        \pgf@x=1.7\pgf@circ@res@step
    }
    \anchor{north}{\northeast\pgf@x=0cm\relax}
    \anchor{east}{\northeast\pgf@y=0cm\relax\pgf@x=0cm\relax}
    \anchor{south}{\northeast\pgf@y=-\pgf@y \pgf@x=0cm\relax}
    \anchor{west}{\northeast\pgf@y=0cm\pgf@x=-\pgf@x}
    \anchor{north east}{\northeast\pgf@x=0cm\relax}
    \anchor{north west}{\northeast\pgf@x=-\pgf@x}
    \anchor{south east}{\northeast\pgf@y=-\pgf@y\pgf@x=0cm\relax}
    \anchor{south west}{\northeast\pgf@y=-\pgf@y\pgf@x=-\pgf@x}
    \savedanchor{\tip}{
        \pgfpointorigin
    }
    \anchor{center}{
        \tip
    }
    \anchor{tip}{
        \tip
    }
    \behindforegroundpath{

        \pgfscope
            \pgf@circ@res@step = \pgf@circ@Rlen
            \divide \pgf@circ@res@step by 16

            \pgfpathmoveto{\pgfpoint{-1.7\pgf@circ@res@step}{0pt}}
            \pgfpathlineto{\pgfpoint{-1.7\pgf@circ@res@step}{-.8\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{0pt}{0pt}}
            \pgfpathlineto{\pgfpoint{-1.7\pgf@circ@res@step}{.8\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpoint{-1.7\pgf@circ@res@step}{0pt}}
            \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
            \pgfusepath{fill}

        \endpgfscope
    }
}


%% box

\pgfdeclareshape{box}{
    \anchor{center}{
        \pgfpointorigin
    }
    \behindforegroundpath{

        \pgfscope
            \pgf@circ@res@step = \ctikzvalof{bipoles/twoport/width}\pgf@circ@Rlen
            \pgf@circ@res@step = 0.5\pgf@circ@res@step
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
            \pgfpathrectanglecorners{\pgfpoint{-\pgf@circ@res@step}{\pgf@circ@res@step}}{\pgfpoint{\pgf@circ@res@step}{-\pgf@circ@res@step}}
            \pgf@circ@draworfill
        \endpgfscope
    }

}


% full nodes for wire crossing

\pgfdeclareshape{jump crossing}
{
    \savedanchor\northwest{%
        \pgf@y=\ctikzvalof{bipoles/crossing/size}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgf@y
    }
    \anchor{center}{ \pgf@y=0pt \pgf@x=0pt }
    \anchor{east}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{e}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{west}{ \northwest \pgf@y=0pt }
    \anchor{w}{ \northwest \pgf@y=0pt }
    \anchor{south}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{s}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{north}{ \northwest \pgf@x=0pt }
    \anchor{n}{ \northwest \pgf@x=0pt }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \behindbackgroundpath{
        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        % horizontal jumper
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0.4\pgf@circ@res@left}{0pt}}
        \pgfpatharc{0}{-180}{0.4*\pgf@circ@res@left}
        \pgfsetbeveljoin
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        % vertical, broken path
        \pgfpathmoveto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{0.5\pgf@circ@res@up}}
        \pgfpathmoveto{\pgfpoint{0pt}{0.3\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfusepath{draw}

    }
}
\pgfdeclareshape{plain crossing}
{
    \savedanchor\northwest{%
        \pgf@y=\ctikzvalof{bipoles/crossing/size}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgf@y
    }
    \anchor{center}{ \pgf@y=0pt \pgf@x=0pt }
    \anchor{east}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{e}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
    \anchor{west}{ \northwest \pgf@y=0pt }
    \anchor{w}{ \northwest \pgf@y=0pt }
    \anchor{south}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{s}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{north}{ \northwest \pgf@x=0pt }
    \anchor{n}{ \northwest \pgf@x=0pt }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \behindbackgroundpath{
        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        % horizontal jumper
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        % vertical, broken path
        \pgfpathmoveto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{0.1\pgf@circ@res@up}}
        \pgfpathmoveto{\pgfpoint{0pt}{0.1\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfusepath{draw}

    }
}

\endinput


==> pgfcirctripoles.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the files gpl-3.0_license.txt and lppl-1-3c_license.txt for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Tripoles

\pgfdeclareshape{spdt}{
    \savedanchor\northwest{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/spdt/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/spdt/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{left}{%
        \northwest
        \pgf@y=0pt
    }
    \anchor{in}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{out 1}{
        \northwest
        \pgf@x=-\pgf@x
    }
    \anchor{out 2}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@y=-\pgf@y
    }
    \anchor{center}{
        \pgf@y=0pt
        \pgf@x=0pt
    }
    \anchor{east}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{south}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{south west}{
        \northwest
        \pgf@y=-\pgf@y
    }
    \anchor{north east}{
        \northwest
        \pgf@x=-\pgf@x
    }
    \anchor{north west}{
        \northwest
    }
    \anchor{south east}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@y=-\pgf@y
    }
    \backgroundpath{
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}


        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgf@circ@res@other = \pgfkeysvalueof{/tikz/circuitikz/tripoles/spdt/margin}\pgf@circ@res@left


        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@down}}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{0pt}}

        \pgfusepath{draw}

        \pgfscope
            \pgftransformshift{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}
            \pgfnode{ocirc}{center}{}{spdt1}{\pgfusepath{stroke}}
        \endpgfscope
        \pgfscope
            \pgftransformshift{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@down}}
            \pgfnode{ocirc}{center}{}{}{\pgfusepath{stroke}}
        \endpgfscope
        \pgfscope
            \pgftransformshift{\pgfpoint{\pgf@circ@res@other}{0pt}}
            \pgfnode{ocirc}{center}{}{spdt2}{\pgfusepath{stroke}}
        \endpgfscope


        \pgfscope
            \pgfpathmoveto{\pgfpointshapeborder{spdt2}{\pgfpointorigin}}
            \pgfpathlineto{
                \pgfpointadd{\pgfpointshapeborder{spdt1}{\pgfpoint{-\pgf@circ@res@other}{-100pt}}}
                {\pgfpoint{-.05\pgf@circ@res@up}{-.05\pgf@circ@res@up}}
            }
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}
            \pgfusepath{draw}
        \endpgfscope
    }
}


% cute switch "node" shapes, matching with cute "to" shapes
% #1 -> name
% #2 -> barposition
% #3 -> arrowcode
\long\def\pgfcircdeclarecutespdt#1#2#3{
    \pgfdeclareshape{#1}
    {
        \savedanchor\northwest{%
            \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/cuteswitch/height}\pgf@circ@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/spdt/width}\pgf@circ@Rlen
            \pgf@x=.25\pgf@x
        }
        \savedanchor\midlever{
            % these values are calculated when we create the definition of the shape.
            \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/cuteswitch/height}\pgf@circ@Rlen
            \pgf@circ@res@temp=\pgfkeysvalueof{/tikz/circuitikz/nodes width}\pgf@circ@Rlen
            \pgf@circ@res@temp=\ctikzvalof{bipoles/cuteswitch/thickness}\pgf@circ@res@temp
            \pgf@circ@res@down = -.5\pgf@y
            \pgf@circ@res@up = .5\pgf@y
            \pgfextracty{\pgf@circ@res@other}{#2}
            \pgf@x=0pt
            \pgf@y=.5\pgf@circ@res@other
        }
        % mid of the lever, to stack switches
        \anchor{mid}{\midlever}

        \anchor{left}{\northwest \pgf@y=0pt }
        \anchor{in}{ \northwest \pgf@y=0pt}
        \anchor{out 1}{ \northwest \pgf@x=-\pgf@x }
        \anchor{out 2}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }

        \anchor{center}{ \pgf@y=0pt \pgf@x=0pt }
        \anchor{east}{ \northwest \pgf@y=0pt \pgf@x=-\pgf@x  }
        \anchor{west}{ \northwest \pgf@y=0pt }
        \anchor{south}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
        \anchor{north}{ \northwest \pgf@x=0pt }
        \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
        \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
        \anchor{north west}{ \northwest }
        \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }

        \backgroundpath{
            \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
            \northwest
            \pgf@circ@res@up = \pgf@y
            \pgf@circ@res@down = -\pgf@y
            \pgf@circ@res@right = -\pgf@x
            \pgf@circ@res@left = \pgf@x

            \pgfscope
            % This is the radius of the "ocirc" shape (see pgfcircshapes.tex)
            \pgf@circ@res@temp=\pgfkeysvalueof{/tikz/circuitikz/nodes width}\pgf@circ@Rlen
            \pgf@circ@res@temp=\ctikzvalof{bipoles/cuteswitch/thickness}\pgf@circ@res@temp
            \pgfsetlinewidth{2\pgf@circ@res@temp}
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfpathlineto{#2}
            \pgfsetroundcap\pgfusepath{draw}
            \endpgfscope
            \pgfscope % arrow
            #3
            \endpgfscope
            % terminals
            \pgfscope
            \pgftransformshift{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
            \pgfnode{ocirc}{center}{}{spdt1}{\pgfusepath{stroke}}
            \endpgfscope
            \pgfscope
            \pgftransformshift{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
            \pgfnode{ocirc}{center}{}{}{\pgfusepath{stroke}}
            \endpgfscope
            \pgfscope
            \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}}
            \pgfnode{ocirc}{center}{}{spdt2}{\pgfusepath{stroke}}
            \endpgfscope

        }
    }
}

\pgfcircdeclarecutespdt{cute spdt up}
{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up-1.5\pgf@circ@res@temp}}
{}

\pgfcircdeclarecutespdt{cute spdt mid}
{\pgfpoint{\pgf@circ@res@right}{0pt}}
{}

\pgfcircdeclarecutespdt{cute spdt down}
{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down+1.5\pgf@circ@res@temp}}
{}

\pgfcircdeclarecutespdt{cute spdt up arrow}
{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up-1.5\pgf@circ@res@temp}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgflinewidth}
    \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}} % in node
    \pgfpathmoveto{\pgfpointpolar{70}{1.5\pgf@circ@res@right}}
    \pgfpatharc{70}{-50}{1.5\pgf@circ@res@right}
    \pgfsetarrowsend{latexslim}
    \pgfusepath{draw}
}

\pgfcircdeclarecutespdt{cute spdt mid arrow}
{\pgfpoint{\pgf@circ@res@right}{0pt}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgflinewidth}
    \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}} % in node
    \pgfsetarrowsstart{latexslim}
    \pgfpathmoveto{\pgfpointpolar{-60}{1.5\pgf@circ@res@right}}
    \pgfpatharc{-60}{60}{1.5\pgf@circ@res@right}
    \pgfsetarrowsend{latexslim}
    \pgfusepath{draw}
}

\pgfcircdeclarecutespdt{cute spdt down arrow}
{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down+1.5\pgf@circ@res@temp}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgflinewidth}
    \pgftransformshift{\pgfpoint{\pgf@circ@res@left}{0pt}} % in node
    \pgfpathmoveto{\pgfpointpolar{-50}{1.5\pgf@circ@res@right}}
    \pgfpatharc{-50}{70}{1.5\pgf@circ@res@right}
    \pgfsetarrowsend{latexslim}
    \pgfusepath{draw}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%       Logic ports
%%
%% Code from John Kormylo at tex.stackexchange.com
%% See https://tex.stackexchange.com/questions/372993/is-it-possible-to-implement-multiple-input-logic-ports-with-circuitikz
%% Integration and fixes from Romano Giannetti and TheTeXnician <38565529+TheTeXnician@users.noreply.github.com>
%%

\newcount\pgf@circ@res@count% reserve global register

\def\pgf@circ@logicport@input#1% #1 = \pgfmathcounter
{%
    \pgfextracty{\pgf@circ@res@up}{\northeast}%
    \step
    \pgf@circ@res@step=\dimexpr 2\pgf@y -2\pgf@circ@res@up\relax
    \advance\pgf@y by -#1\pgf@circ@res@step\relax
}%

% #1 = \pgfmathcounter #2=type #3 specificic port
% type is 1 for and,nand; 2 for or,nor; 3 for xor,xnor, 4 for european.
\def\pgf@circ@logicport@baseinput#1#2#3%
{%
    % and and nand
    \ifnum #2=1\relax
        \pgfextracty{\pgf@circ@res@up}{\northeast}%
        \pgfextractx{\pgf@circ@res@left}{\southwest}%
        \step
        \pgf@circ@res@step=\dimexpr 2\pgf@y -2\pgf@circ@res@up\relax
        \advance\pgf@y by -#1\pgf@circ@res@step\relax
        \pgf@x=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american #3 port/port width}\pgf@circ@res@left
    \fi
    % or and nor
    \ifnum #2=2\relax
        \pgfextracty{\pgf@circ@res@up}{\northeast}%
        \pgfextractx{\pgf@circ@res@left}{\southwest}%
        \pgfextractx{\pgf@circ@res@right}{\northeast}%
        \step
        \pgf@circ@res@step=\dimexpr 2\pgf@y -2\pgf@circ@res@up\relax
        \advance\pgf@y by -#1\pgf@circ@res@step\relax
        \edef\pgf@circ@math@angle{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american #3 port/angle}}%
        \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american #3 port/inner}\pgf@circ@res@right
        \pgfmathsetlengthmacro{\pgf@circ@math@xradius}{\pgf@circ@res@other /(1 - cos(\pgf@circ@math@angle)}%
        \pgfmathsetlengthmacro{\pgf@circ@math@yradius}{\pgf@circ@res@up /sin(\pgf@circ@math@angle)}%
        \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american #3 port/port width}\pgf@circ@res@right
        \pgfmathsetlengthmacro{\pgf@circ@math@xorigin}{\pgf@circ@res@other + \pgf@circ@math@xradius*cos(\pgf@circ@math@angle)}%
        \pgf@circ@res@temp=\pgf@y
        \pgfmathsetmacro{\pgf@circ@math@angle}{asin(\pgf@circ@res@temp/\pgf@circ@math@yradius)}%
        \pgfmathsetlength{\pgf@circ@res@other}{\pgf@circ@math@xradius*cos(\pgf@circ@math@angle)-\pgf@circ@math@xorigin}%
        \pgf@x=\pgf@circ@res@other
    \fi
    % xor and xnor
    \ifnum #2=3\relax
        \pgfextracty{\pgf@circ@res@up}{\northeast}%
        \pgfextractx{\pgf@circ@res@left}{\southwest}%
        \pgfextractx{\pgf@circ@res@right}{\northeast}%
        \pgfkeysgetvalue{/tikz/circuitikz/tripoles/american #3 port/angle}{\pgf@circ@math@angle}%
        \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american #3 port/inner}\pgf@circ@res@right
        \pgfmathsetlengthmacro{\pgf@circ@math@xradius}{\pgf@circ@res@other /(1 - cos(\pgf@circ@math@angle)}%
        \pgfmathsetlengthmacro{\pgf@circ@math@yradius}{\pgf@circ@res@up / sin(\pgf@circ@math@angle))}%
        \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american #3 port/port width}\pgf@circ@res@right
        \pgfmathsetlengthmacro{\pgf@circ@math@xorigin}{\pgf@circ@res@other + \pgf@circ@math@xradius*cos(\pgf@circ@math@angle)}%
        \pgf@circ@res@temp=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american #3 port/distance}\pgf@circ@res@right
        \pgfmathsetlengthmacro{\pgf@circ@math@distance}{\pgf@circ@res@temp}
        % this compensates for the effect of the line width on the gap between the arcs
        \pgfmathsetlengthmacro{\pgf@circ@math@yradiusA}{\pgf@circ@math@yradius -2\pgflinewidth}%
        \pgfmathsetlengthmacro{\pgf@circ@math@xradiusA}{\pgf@circ@math@xradius -2\pgflinewidth}%

        \step
        \pgf@circ@res@step=\dimexpr 2\pgf@y -2\pgf@circ@res@up\relax
        \advance\pgf@y by -#1\pgf@circ@res@step\relax
         \pgf@circ@res@temp=\pgf@y
            \pgfmathsetmacro{\pgf@circ@math@angle}{asin(\pgf@circ@res@temp  / \pgf@circ@math@yradiusA)}%
        \pgfmathsetlength{\pgf@circ@res@other}{\pgf@circ@math@xradiusA*cos(\pgf@circ@math@angle)-\pgf@circ@math@xorigin}%
        \advance\pgf@circ@res@other by -\pgf@circ@math@distance
        \pgf@x=\pgf@circ@res@other
    \fi
    % european
    \ifnum #2=4\relax
        \pgfextracty{\pgf@circ@res@up}{\northeast}%
        \pgfextractx{\pgf@circ@res@other}{\left}%
        \step
        \pgf@circ@res@step=\dimexpr 2\pgf@y -2\pgf@circ@res@up\relax
        \advance\pgf@y by -#1\pgf@circ@res@step\relax
        \pgf@x=\pgf@circ@res@other
    \fi
}%

%%% american
\long\def\pgfcircdeclarelogicport#1#2#3{%
    \pgfdeclareshape{american #1 port}%
    {%
        \savedmacro\resize{% automatic
            \pgf@circ@res@up = \pgfkeysvalueof{/tikz/circuitikz/tripoles/american #1 port/height}\pgf@circ@Rlen
            \pgf@circ@res@up = .5\pgf@circ@res@up
            \pgf@circ@res@down = -\pgf@circ@res@up
            \pgf@circ@res@right = \pgfkeysvalueof{/tikz/circuitikz/tripoles/american #1 port/width}\pgf@circ@Rlen
            \pgf@circ@res@right = .5\pgf@circ@res@right
            \pgf@circ@res@left = -\pgf@circ@res@right
        }%
        \savedmacro\inputs{% get number of inputs
            \pgf@circ@res@count=\pgfkeysvalueof{/tikz/number inputs}\relax%
            \ifnum\pgf@circ@res@count=0
                \pgf@circ@res@count=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american #1 port/inputs}\relax%
            \fi
        \ifnum\pgf@circ@res@count<2 \pgf@circ@res@count=2\fi
    \ifnum\pgf@circ@res@count>16 \pgf@circ@res@count=16\fi
        \def\inputs{\the\pgf@circ@res@count}%
    }%
    \savedanchor\step{% 1/2 gap at edges
        \pgf@circ@res@step = \pgfkeysvalueof{/tikz/circuitikz/tripoles/american #1 port/height}\pgf@circ@Rlen
        \divide\pgf@circ@res@step by \pgf@circ@res@count
        \pgfpoint{\pgf@circ@res@left}{\dimexpr\pgf@circ@res@up+0.5\pgf@circ@res@step}%
    }%
    \savedanchor\northeast{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \savedanchor\southwest{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
    \savedanchor\left{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american #1 port/port width}\pgf@circ@res@left}{0pt}}
    \savedanchor\right{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american #1 port/port width}\pgf@circ@res@right}{0pt}}
    \savedanchor\origin{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american #1 port/origin}\pgf@circ@res@right}{0pt}}

    \anchor{center}{\origin}% for backwards compatibility
    \anchor{text}{\pgfpoint{-.5\wd\pgfnodeparttextbox}{\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox}}

    % create input anchors
    \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@american #1 port\endcsname{%
        \pgfmathloop%
        \ifnum\pgfmathcounter>\pgf@circ@res@count%
    \else%
        %\pgfutil@ifundefined{pgf@anchor@american #1 port@in \pgfmathcounter}{%
        \expandafter\xdef\csname pgf@anchor@american #1 port@in \pgfmathcounter\endcsname{%
            \noexpand\pgf@circ@logicport@input{\pgfmathcounter}% defined above
        }%
        \expandafter\xdef\csname pgf@anchor@american #1 port@bin \pgfmathcounter\endcsname{%
            \noexpand\pgf@circ@logicport@baseinput{\pgfmathcounter}{#2}{#1}% defined above
        }%
        %}{}%
        \repeatpgfmathloop%
    }

    \anchor{out}{\northeast\pgf@y=0pt}
    \anchor{bout}{\right\pgf@y=0pt}


    \anchor{left}{\left}% edges of component mius leads
    \anchor{right}{\right}

    \anchor{north east}{\northeast}% see \Compass macro
    \anchor{south west}{\southwest}
    \anchor{north}{\pgfextracty{\pgf@circ@res@up}{\northeast}%
    \pgfpoint{0cm}{\pgf@circ@res@up}}
    \anchor{north west}{\pgfextracty{\pgf@circ@res@up}{\northeast}%
        \pgfextractx{\pgf@circ@res@left}{\southwest}%
    \pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \anchor{west}{\pgfextractx{\pgf@circ@res@left}{\southwest}%
    \pgfpoint{\pgf@circ@res@left}{0cm}}
    \anchor{south}{\pgfextracty{\pgf@circ@res@down}{\southwest}%
    \pgfpoint{0cm}{\pgf@circ@res@down}}
    \anchor{south east}{\pgfextracty{\pgf@circ@res@down}{\southwest}%
        \pgfextractx{\pgf@circ@res@right}{\northeast}%
    \pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \anchor{east}{\pgfextractx{\pgf@circ@res@right}{\northeast}%
    \pgfpoint{\pgf@circ@res@right}{0cm}}

    \backgroundpath{
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
        #3
    }
}
}
%%% american and %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfcircdeclarelogicport{and}{1}{
    \pgfextracty{\pgf@circ@res@temp}{\step}%
    \pgf@circ@res@step = \dimexpr 2\pgf@circ@res@temp -2\pgf@circ@res@up\relax
    \pgf@circ@res@count = \inputs\relax
    \loop\ifnum\pgf@circ@res@count>0
        \advance\pgf@circ@res@temp by -\pgf@circ@res@step
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@temp}}%
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/american and port/port width}\pgf@circ@res@left}
        {\pgf@circ@res@temp}}
        \advance\pgf@circ@res@count by -1
        \repeat

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/american and port/port width}\pgf@circ@res@right}
    {0pt}}

    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}
    \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american and port/port width}\pgf@circ@res@left

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
    \pgfpatharc{-90}{90}{-2\pgf@circ@res@other and \pgf@circ@res@up}
    \pgfpathclose
    \pgf@circ@draworfill
    }
%%% american nand %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \pgfcircdeclarelogicport{nand}{1}{
    \pgfextracty{\pgf@circ@res@temp}{\step}%
    \pgf@circ@res@step = \dimexpr 2\pgf@circ@res@temp -2\pgf@circ@res@up\relax
    \pgf@circ@res@count = \inputs\relax
    \loop\ifnum\pgf@circ@res@count>0
        \advance\pgf@circ@res@temp by -\pgf@circ@res@step
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@temp}}%
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nand port/port width}\pgf@circ@res@left}
        {\pgf@circ@res@temp}}
        \advance\pgf@circ@res@count by -1
    \repeat

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nand port/port width}\pgf@circ@res@right} {0pt}}

    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}
    \pgf@circ@res@step = \pgfkeysvalueof{/tikz/circuitikz/tripoles/american nand port/circle width}\pgf@circ@res@right
    \pgf@circ@res@other = \pgfkeysvalueof{/tikz/circuitikz/tripoles/american nand port/port width}\pgf@circ@res@right
    \pgf@circ@res@temp = \dimexpr 2\pgf@circ@res@other - \pgf@circ@res@step\relax

    \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{-\pgf@circ@res@other}{\pgf@circ@res@down}}
    \pgfpatharc{-90}{90}{\pgf@circ@res@temp and \pgf@circ@res@up}
    \pgfpathclose

    \pgfpathellipse
    {\pgfpoint{\pgf@circ@res@other-.5\pgf@circ@res@step}{0pt}}
    {\pgfpoint{.5\pgf@circ@res@step}{0pt}}
    {\pgfpoint{0pt}{.5\pgf@circ@res@step}}

    \pgf@circ@draworfill
}
%%% american nor %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfcircdeclarelogicport{nor}{2}{
    \edef\pgf@circ@math@angle{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/angle}}%
    \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/inner}\pgf@circ@res@right
    \pgfmathsetlengthmacro{\pgf@circ@math@xradius}{\pgf@circ@res@other /(1 - cos(\pgf@circ@math@angle)}%
    \pgfmathsetlengthmacro{\pgf@circ@math@yradius}{\pgf@circ@res@up /sin(\pgf@circ@math@angle)}%
    \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/port width}\pgf@circ@res@right
    \pgfmathsetlengthmacro{\pgf@circ@math@xorigin}{\pgf@circ@res@other + \pgf@circ@math@xradius*cos(\pgf@circ@math@angle)}%

    \pgfextracty{\pgf@circ@res@temp}{\step}%
    \pgf@circ@res@step = \dimexpr 2\pgf@circ@res@temp -2\pgf@circ@res@up\relax
    \pgf@circ@res@count = \inputs\relax
    \loop\ifnum\pgf@circ@res@count>0
        \advance\pgf@circ@res@temp by -\pgf@circ@res@step
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@temp}}%
        \pgfmathsetmacro{\pgf@circ@math@angle}{asin(\pgf@circ@res@temp/\pgf@circ@math@yradius)}%
        \pgfmathsetlength{\pgf@circ@res@other}{\pgf@circ@math@xradius*cos(\pgf@circ@math@angle)-\pgf@circ@math@xorigin}%
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@temp}}%
        \advance\pgf@circ@res@count by -1
    \repeat

    \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/port width}\pgf@circ@res@right
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{0pt}}

    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}

    \edef\pgf@circ@math@angle{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/angle}}%
    \pgf@circ@res@step = \pgfkeysvalueof{/tikz/circuitikz/tripoles/american nor port/circle width}\pgf@circ@res@right
    \pgf@circ@res@temp = \dimexpr 2\pgf@circ@res@other - \pgf@circ@res@step\relax
    \advance\pgf@circ@res@other by -\pgf@circ@res@step

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}% for symmetry
    \pgfpatharc{0}{90}{\pgf@circ@res@temp and \pgf@circ@res@up}%
    \pgfpatharc{\pgf@circ@math@angle}{-\pgf@circ@math@angle}{\pgf@circ@math@xradius and \pgf@circ@math@yradius}%
    \pgfpatharc{-90}{0}{\pgf@circ@res@temp and \pgf@circ@res@up}%
    \pgfpathclose

    \pgfpathellipse
    {\pgfpoint{\pgf@circ@res@other+.5\pgf@circ@res@step}{0pt}}
    {\pgfpoint{.5\pgf@circ@res@step}{0pt}}
    {\pgfpoint{0pt}{.5\pgf@circ@res@step}}

    \pgf@circ@draworfill
}
%%% american or %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfcircdeclarelogicport{or}{2}{
    \edef\pgf@circ@math@angle{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/angle}}%
    \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/inner}\pgf@circ@res@right
    \pgfmathsetlengthmacro{\pgf@circ@math@xradius}{\pgf@circ@res@other /(1 - cos(\pgf@circ@math@angle)}%
    \pgfmathsetlengthmacro{\pgf@circ@math@yradius}{\pgf@circ@res@up /sin(\pgf@circ@math@angle)}%
    \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/port width}\pgf@circ@res@right
    \pgfmathsetlengthmacro{\pgf@circ@math@xorigin}{\pgf@circ@res@other + \pgf@circ@math@xradius*cos(\pgf@circ@math@angle)}%

    \pgfextracty{\pgf@circ@res@temp}{\step}%
    \pgf@circ@res@step = \dimexpr 2\pgf@circ@res@temp -2\pgf@circ@res@up\relax
    \pgf@circ@res@count = \inputs\relax
    \loop\ifnum\pgf@circ@res@count>0
        \advance\pgf@circ@res@temp by -\pgf@circ@res@step
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@temp}}%
        \pgfmathsetmacro{\pgf@circ@math@angle}{asin(\pgf@circ@res@temp/\pgf@circ@math@yradius)}%
        \pgfmathsetlength{\pgf@circ@res@other}{\pgf@circ@math@xradius*cos(\pgf@circ@math@angle)-\pgf@circ@math@xorigin}%
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@temp}}%
        \advance\pgf@circ@res@count by -1
    \repeat

    \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/port width}\pgf@circ@res@right
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{0pt}}

    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}

    \edef\pgf@circ@math@angle{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american or port/angle}}%

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}% for symmetry
    \pgfpatharc{0}{90}{2\pgf@circ@res@other and \pgf@circ@res@up}%
    \pgfpatharc{\pgf@circ@math@angle}{-\pgf@circ@math@angle}{\pgf@circ@math@xradius and \pgf@circ@math@yradius}%
    \pgfpatharc{-90}{0}{2\pgf@circ@res@other and \pgf@circ@res@up}%
    \pgfpathclose

    \pgf@circ@draworfill
}
%%% american xor %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfcircdeclarelogicport{xor}{3}{
    \pgfkeysgetvalue{/tikz/circuitikz/tripoles/american xor port/angle}{\pgf@circ@math@angle}%
    \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/inner}\pgf@circ@res@right
    \pgfmathsetlengthmacro{\pgf@circ@math@xradius}{\pgf@circ@res@other /(1 - cos(\pgf@circ@math@angle)}%
    \pgfmathsetlengthmacro{\pgf@circ@math@yradius}{\pgf@circ@res@up / sin(\pgf@circ@math@angle))}%
    \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/port width}\pgf@circ@res@right
    \pgfmathsetlengthmacro{\pgf@circ@math@xorigin}{\pgf@circ@res@other + \pgf@circ@math@xradius*cos(\pgf@circ@math@angle)}%
    \pgf@circ@res@temp=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/distance}\pgf@circ@res@right
    \pgfmathsetlengthmacro{\pgf@circ@math@distance}{\pgf@circ@res@temp}
    % this compensates for the effect of the line width on the gap between the arcs
    \pgfmathsetlengthmacro{\pgf@circ@math@yradiusA}{\pgf@circ@math@yradius -2\pgflinewidth}%
    \pgfmathsetlengthmacro{\pgf@circ@math@xradiusA}{\pgf@circ@math@xradius -2\pgflinewidth}%

    \pgfextracty{\pgf@circ@res@temp}{\step}%
    \pgf@circ@res@step = \dimexpr 2\pgf@circ@res@temp -2\pgf@circ@res@up\relax
    \pgf@circ@res@count = \inputs\relax
    \loop\ifnum\pgf@circ@res@count>0
        \advance\pgf@circ@res@temp by -\pgf@circ@res@step
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@temp}}%
        \pgfmathsetmacro{\pgf@circ@math@angle}{asin(\pgf@circ@res@temp  / \pgf@circ@math@yradiusA)}%
        \pgfmathsetlength{\pgf@circ@res@other}{\pgf@circ@math@xradiusA*cos(\pgf@circ@math@angle)-\pgf@circ@math@xorigin}%
        \advance\pgf@circ@res@other by -\pgf@circ@math@distance
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@temp}}%
        \advance\pgf@circ@res@count by -1
    \repeat

    \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/port width}\pgf@circ@res@right
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{0pt}}

    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}

    \edef\pgf@circ@math@angle{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/angle}}%

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}% for symmetry
    \pgfpatharc{0}{90}{2\pgf@circ@res@other and \pgf@circ@res@up}%
    \pgfpatharc{\pgf@circ@math@angle}{-\pgf@circ@math@angle}{\pgf@circ@math@xradius and \pgf@circ@math@yradius}%
    \pgfpatharc{-90}{0}{2\pgf@circ@res@other and \pgf@circ@res@up}%
    \pgfpathclose
    \pgf@circ@draworfill

    \pgfmathsetlength{\pgf@circ@res@temp}{(\pgf@circ@math@yradiusA)*sin(\pgf@circ@math@angle)}%

    \pgfpathmoveto{\pgfpoint{-\pgf@circ@res@other-\pgf@circ@math@distance}{\pgf@circ@res@temp}}% first arc
    \pgfpatharc{\pgf@circ@math@angle}{-\pgf@circ@math@angle}{\pgf@circ@math@xradiusA and \pgf@circ@math@yradiusA}%

    \pgfusepath{draw}
}
%%% american xnor %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfcircdeclarelogicport{xnor}{3}{
    \pgfkeysgetvalue{/tikz/circuitikz/tripoles/american xnor port/angle}{\pgf@circ@math@angle}%
    \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/inner}\pgf@circ@res@right
    \pgfmathsetlengthmacro{\pgf@circ@math@xradius}{\pgf@circ@res@other /(1 - cos(\pgf@circ@math@angle)}%
    \pgfmathsetlengthmacro{\pgf@circ@math@yradius}{\pgf@circ@res@up / sin(\pgf@circ@math@angle))}%
    \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/port width}\pgf@circ@res@right
    \pgfmathsetlengthmacro{\pgf@circ@math@xorigin}{\pgf@circ@res@other + \pgf@circ@math@xradius*cos(\pgf@circ@math@angle)}%
    \pgf@circ@res@temp=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xor port/distance}\pgf@circ@res@right
    \pgfmathsetlengthmacro{\pgf@circ@math@distance}{\pgf@circ@res@temp}
    % this compensates for the effect of the line width on the gap between the arcs
    \pgfmathsetlengthmacro{\pgf@circ@math@yradiusA}{\pgf@circ@math@yradius -2\pgflinewidth}%
    \pgfmathsetlengthmacro{\pgf@circ@math@xradiusA}{\pgf@circ@math@xradius -2\pgflinewidth}%

    \pgfextracty{\pgf@circ@res@temp}{\step}%
    \pgf@circ@res@step = \dimexpr 2\pgf@circ@res@temp -2\pgf@circ@res@up\relax
    \pgf@circ@res@count = \inputs\relax
    \loop\ifnum\pgf@circ@res@count>0
        \advance\pgf@circ@res@temp by -\pgf@circ@res@step
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@temp}}%
        \pgfmathsetmacro{\pgf@circ@math@angle}{asin(\pgf@circ@res@temp  / \pgf@circ@math@yradiusA)}%
        \pgfmathsetlength{\pgf@circ@res@other}{\pgf@circ@math@xradiusA*cos(\pgf@circ@math@angle)-\pgf@circ@math@xorigin}%
        \advance\pgf@circ@res@other by -\pgf@circ@math@distance
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@temp}}%
        \advance\pgf@circ@res@count by -1
    \repeat

    \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/port width}\pgf@circ@res@right
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{0pt}}

    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}

    \edef\pgf@circ@math@angle{\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/angle}}%
    \pgf@circ@res@step = \pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/circle width}\pgf@circ@res@right
    \pgf@circ@res@temp = \dimexpr 2\pgf@circ@res@other - \pgf@circ@res@step\relax
    \advance\pgf@circ@res@other by -\pgf@circ@res@step

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}% for symmetry
    \pgfpatharc{0}{90}{\pgf@circ@res@temp and \pgf@circ@res@up}%
    \pgfpatharc{\pgf@circ@math@angle}{-\pgf@circ@math@angle}{\pgf@circ@math@xradius and \pgf@circ@math@yradius}%
    \pgfpatharc{-90}{0}{\pgf@circ@res@temp and \pgf@circ@res@up}%
    \pgfpathclose

    \pgfpathellipse
    {\pgfpoint{\pgf@circ@res@other+.5\pgf@circ@res@step}{0pt}}
    {\pgfpoint{.5\pgf@circ@res@step}{0pt}}
    {\pgfpoint{0pt}{.5\pgf@circ@res@step}}
    \pgf@circ@draworfill

    \pgf@circ@res@other=\pgfkeysvalueof{/tikz/circuitikz/tripoles/american xnor port/port width}\pgf@circ@res@left
    \pgfmathsetlength{\pgf@circ@res@temp}{(\pgf@circ@math@yradiusA)*sin(\pgf@circ@math@angle)}%

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other-\pgf@circ@math@distance}{\pgf@circ@res@temp}}% first arc
    \pgfpatharc{\pgf@circ@math@angle}{-\pgf@circ@math@angle}{\pgf@circ@math@xradiusA and \pgf@circ@math@yradiusA}%

    \pgfusepath{draw}
}

%%% Original one-input ports

\pgfdeclareshape{american not port}{
    \anchor{center}{\pgfpointorigin}
    \savedanchor\northwest{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/not port/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/bipoles/not port/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    }
    \savedanchor\left{%
        \pgf@y=0pt
    }
    \anchor{in}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{east}{
        \left
        \pgf@x=-.8\pgf@x
    }
    \anchor{west}{
        \left
    }
    \anchor{south}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{south west}{
        \northwest
        \pgf@y=-\pgf@y
    }
    \anchor{north east}{
        \northwest
        \pgf@x=-\pgf@x
    }
    \anchor{north west}{
        \northwest
    }
    \anchor{south east}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@y=-\pgf@y
    }
    \backgroundpath{
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}


        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x

        \pgf@circ@res@other = \pgfkeysvalueof{/tikz/circuitikz/bipoles/not port/circle width}\pgf@circ@res@right

        \pgfscope
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}
            \pgftransformxshift{.7\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=.7\pgf@circ@res@step

            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
            \pgf@circ@draworfill
            \pgfpathellipse
            {\pgfpoint{\pgf@circ@res@step-.5\pgf@circ@res@other}{0pt}}
            {\pgfpoint{.5\pgf@circ@res@other}{0pt}}
            {\pgfpoint{0pt}{.5\pgf@circ@res@other}}
            \pgf@circ@draworfill
        \endpgfscope

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@left}{0pt}}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{0pt}}

        \pgfusepath{draw}

    }
}

\pgfdeclareshape{invschmitt}{
    \anchor{center}{\pgfpointorigin}
    \savedanchor\northwest{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/not port/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/bipoles/not port/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    }
    \savedanchor\left{%
        \pgf@y=0pt
    }
    \anchor{in}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{east}{
        \left
        \pgf@x=-.8\pgf@x
    }
    \anchor{west}{
        \left
    }
    \anchor{south}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{south west}{
        \northwest
        \pgf@y=-\pgf@y
    }
    \anchor{north east}{
        \northwest
        \pgf@x=-\pgf@x
    }
    \anchor{north west}{
        \northwest
    }
    \anchor{south east}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@y=-\pgf@y
    }
    \backgroundpath{
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x

        \pgf@circ@res@other = \pgfkeysvalueof{/tikz/circuitikz/bipoles/not port/circle width}\pgf@circ@res@right

        \pgfscope
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}
            \pgftransformxshift{.7\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=.7\pgf@circ@res@step

            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
            \pgfpathclose
            \pgf@circ@draworfill
            \pgfpathellipse
            {\pgfpoint{\pgf@circ@res@step-.5\pgf@circ@res@other}{0pt}}
            {\pgfpoint{.5\pgf@circ@res@other}{0pt}}
            {\pgfpoint{0pt}{.5\pgf@circ@res@other}}
            \pgf@circ@draworfill
        \endpgfscope

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@left}{0pt}}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{0pt}}
        \pgfusepath{draw}
        %draw inner shape

        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}

        \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left}{.3\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{.3\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{.3\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.05\pgf@circ@res@left}{.3\pgf@circ@res@up}}
        \pgfpathmoveto{\pgfpoint{.4\pgf@circ@res@left}{.3\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{.25\pgf@circ@res@left}{.3\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{.25\pgf@circ@res@left}{.3\pgf@circ@res@up}}
        \pgfusepath{draw}

    }
}

\pgfdeclareshape{schmitt}{
    \anchor{center}{\pgfpointorigin}
    \savedanchor\northwest{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/not port/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/bipoles/not port/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    }
    \savedanchor\left{%
        \pgf@y=0pt
    }
    \anchor{in}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{east}{
        \left
        \pgf@x=-.8\pgf@x
    }
    \anchor{west}{
        \left
    }
    \anchor{south}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{south west}{
        \northwest
        \pgf@y=-\pgf@y
    }
    \anchor{north east}{
        \northwest
        \pgf@x=-\pgf@x
    }
    \anchor{north west}{
        \northwest
    }
    \anchor{south east}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@y=-\pgf@y
    }
    \backgroundpath{
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}


        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x

        \pgf@circ@res@other = \pgfkeysvalueof{/tikz/circuitikz/bipoles/not port/circle width}\pgf@circ@res@right

        \pgfscope
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}
            \pgftransformxshift{.7\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=.7\pgf@circ@res@step

            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
            \pgfpathclose
            \pgf@circ@draworfill
        \endpgfscope

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@left}{0pt}}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right-\pgf@circ@res@other}{0pt}}
        \pgfusepath{draw}
        %draw inner shape

        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}

        \pgfpathmoveto{\pgfpoint{.6\pgf@circ@res@left}{.3\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{.3\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{.4\pgf@circ@res@left}{.3\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{.05\pgf@circ@res@left}{.3\pgf@circ@res@up}}
        \pgfpathmoveto{\pgfpoint{.4\pgf@circ@res@left}{.3\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{.25\pgf@circ@res@left}{.3\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{.25\pgf@circ@res@left}{.3\pgf@circ@res@up}}
        \pgfusepath{draw}

    }
}


%%% start european logic ports, from John Kormylo
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%

% #1 - name
% #2 - text inside
% #3 - number of inputs
% #4 = is it a not?

\long\def\pgfcircdeclareeurologicport#1#2#3#4{
    \pgfdeclareshape{european #1 port}
    {
        \savedmacro\resize{% automatic
            \pgf@circ@res@up = \pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/height}\pgf@circ@Rlen
            \pgf@circ@res@up = .5\pgf@circ@res@up
            \pgf@circ@res@down = -\pgf@circ@res@up
            \pgf@circ@res@right = \pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/width}\pgf@circ@Rlen
            \pgf@circ@res@right = .5\pgf@circ@res@right
            \pgf@circ@res@left = -\pgf@circ@res@right
        }%
        \savedmacro\inputs{% get number of inputs
            \pgf@circ@res@count=\pgfkeysvalueof{/tikz/number inputs}\relax%
            \ifnum\pgf@circ@res@count=0
                \pgf@circ@res@count=\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/inputs}\relax%
            \fi
        \ifnum\pgf@circ@res@count<2 \pgf@circ@res@count=2\fi
    \ifnum\pgf@circ@res@count>16 \pgf@circ@res@count=16\fi
        \def\inputs{\the\pgf@circ@res@count}%
    }%
    \savedanchor\step{% 1/2 gap at edges
        \pgf@circ@res@step = \pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/height}\pgf@circ@Rlen
        \divide\pgf@circ@res@step by #3
        \pgfpoint{\pgf@circ@res@left}{\dimexpr\pgf@circ@res@up+0.5\pgf@circ@res@step}%
    }%
    \savedanchor\northeast{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}%
    \savedanchor\southwest{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}%
    \savedanchor\left{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/reserved}\pgf@circ@res@left}{0pt}}%
    \savedanchor\right{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/reserved}\pgf@circ@res@right}{0pt}}%
    \savedanchor\origin{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/origin}\pgf@circ@res@right}{0pt}}%

    \anchor{center}{\origin}% for backwards compatibility
    % the text anchor overlaps the logic symbol
    \anchor{text}{\pgfpoint{-.5\wd\pgfnodeparttextbox}{\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox}}%
    % create input anchors
    \ifnum#3=1\relax
        \anchor{in}{\pgfpoint{\pgf@circ@res@left}{0pt}}% or \step
    \else
        \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@european #1 port\endcsname{%
            \pgfmathloop%
            \ifnum\pgfmathcounter>#3%
        \else%
            %\pgfutil@ifundefined{pgf@anchor@european #1 port@in \pgfmathcounter}{% redundant
            \expandafter\xdef\csname pgf@anchor@european #1 port@in \pgfmathcounter\endcsname{%
                \noexpand\pgf@circ@logicport@input{\pgfmathcounter}% defined above
            }%
            \expandafter\xdef\csname pgf@anchor@european #1 port@bin \pgfmathcounter\endcsname{%
                \noexpand\pgf@circ@logicport@baseinput{\pgfmathcounter}{4}{#1}% defined above
            }%
            %}{}%
            \repeatpgfmathloop%
        }
    \fi
    \anchor{out}{\northeast\pgf@y=0pt}
    \anchor{bout}{\right\pgf@y=0pt}

    \anchor{left}{\left}% edges of component minus leads
    \anchor{right}{\right}

    \anchor{north east}{\northeast}% see \Compass macro
    \anchor{south west}{\southwest}
    \anchor{north}{\pgfextracty{\pgf@circ@res@up}{\northeast}%
    \pgfpoint{0cm}{\pgf@circ@res@up}}
    \anchor{north west}{\pgfextracty{\pgf@circ@res@up}{\northeast}%
        \pgfextractx{\pgf@circ@res@left}{\southwest}%
    \pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
    \anchor{west}{\pgfextractx{\pgf@circ@res@left}{\southwest}%
    \pgfpoint{\pgf@circ@res@left}{0cm}}
    \anchor{south}{\pgfextracty{\pgf@circ@res@down}{\southwest}%
    \pgfpoint{0cm}{\pgf@circ@res@down}}
    \anchor{south east}{\pgfextracty{\pgf@circ@res@down}{\southwest}%
        \pgfextractx{\pgf@circ@res@right}{\northeast}%
    \pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \anchor{east}{\pgfextractx{\pgf@circ@res@right}{\northeast}%
    \pgfpoint{\pgf@circ@res@right}{0cm}}

    \backgroundpath{
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
        \pgfscope
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}
            \pgfpathrectanglecorners
            {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/reserved}\pgf@circ@res@left}{\pgf@circ@res@up}}
            {\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/reserved}\pgf@circ@res@right}{\pgf@circ@res@down}}
            \pgf@circ@draworfill
        \endpgfscope
        \ifnum#3=1\relax
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}%
            \pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/reserved}\pgf@circ@res@left}{0pt}}%
        \else
            \pgfextracty{\pgf@circ@res@temp}{\step}%
            \pgf@circ@res@step = \dimexpr 2\pgf@circ@res@temp -2\pgf@circ@res@up\relax
            %\pgf@circ@res@count = #3\relax% redundant
            \loop\ifnum\pgf@circ@res@count>0
                \advance\pgf@circ@res@temp by -\pgf@circ@res@step
                \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@temp}}%
                \pgfpathlineto{\pgfpoint
                    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/reserved}\pgf@circ@res@left}
                {\pgf@circ@res@temp}}
                \advance\pgf@circ@res@count by -1
                \repeat
            \fi
            %
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
            \pgfpathlineto{%
            \pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/reserved}\pgf@circ@res@right}{0pt}}
            %
            \edef\pgf@temp{not}
            \edef\pgf@circ@temp{#4}
            \ifx\pgf@temp\pgf@circ@temp % is a not
                \pgfpathmoveto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/not width}\pgf@circ@res@right}{0pt}}
                \pgfpathlineto{\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/reserved}\pgf@circ@res@right}%
                {\pgfkeysvalueof{/tikz/circuitikz/tripoles/european #1 port/not height}\pgf@circ@res@up}}
            \fi
            %
            \pgfusepath{draw}
            %
            \pgfpathmoveto{\pgfpointorigin}
            \pgftext{#2}
            %
            %
            %
        }
    }
}
\pgfcircdeclareeurologicport{and}{\&}{\pgf@circ@res@count}{}
\pgfcircdeclareeurologicport{or}{$\ge 1$}{\pgf@circ@res@count}{}
\pgfcircdeclareeurologicport{xor}{$=1$}{\pgf@circ@res@count}{}
\pgfcircdeclareeurologicport{not}{$1$}{1}{not}
\pgfcircdeclareeurologicport{nand}{\&}{\pgf@circ@res@count}{not}
\pgfcircdeclareeurologicport{nor}{$\ge 1$}{\pgf@circ@res@count}{not}
\pgfcircdeclareeurologicport{xnor}{$=1$}{\pgf@circ@res@count}{not}

%% end european logic ports

\long\def\pgfcircdeclaretransistor#1#2#3{
    \pgfdeclareshape{#1}
    {
        \anchor{center}{
            \pgfpointorigin
        }
        \savedanchor\northeast{% upper right
            \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/height}\pgf@circ@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=0pt
        }
        \savedanchor\left{%center left
            \pgf@y=0pt
            \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/width}\pgf@circ@Rlen
        }
        \anchor{text}{
            \northeast
            \pgf@y=.7\pgf@y
            \pgf@x= \pgf@circ@Rlen
            \pgf@x=0.1\pgf@x
        }
        \anchor{pathstart}{ % south
            \northeast
            \pgf@y=-\pgf@y
        }
        \anchor{pathend}{
            \northeast
        }
        \anchor{north}{
            \northeast
            \pgf@circ@res@step=\pgf@y
            \left
            \pgf@y=\pgf@circ@res@step
            \pgf@x=.5\pgf@x
        }
        \anchor{west}{
            \left
        }
        \anchor{east}{
            \northeast
            \pgf@y=0pt
        }
        \anchor{south}{
            \northeast
            \pgf@circ@res@step=\pgf@y
            \left
            \pgf@y=-\pgf@circ@res@step
            \pgf@x=.5\pgf@x
        }
        \anchor{south west}{
            \northeast
            \pgf@circ@res@step=\pgf@y
            \left
            \pgf@y=-\pgf@circ@res@step
        }
        \anchor{north east}{
            \northeast
        }
        \anchor{north west}{
            \northeast
            \pgf@circ@res@step=\pgf@y
            \left
            \pgf@y=\pgf@circ@res@step
        }
        \anchor{south east}{
            \northeast
            \pgf@y=-\pgf@y
        }
        \anchor{B}{
            \northeast
            \pgf@circ@res@step=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@y
            \left
            \pgf@y=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@circ@res@step
        }
        \anchor{base}{
            \northeast
            \pgf@circ@res@step=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@y
            \left
            \pgf@y=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@circ@res@step
        }
        \anchor{G}{
            \northeast
            \pgf@circ@res@step=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@y
            \left
            \pgf@y=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@circ@res@step
        }
        \anchor{gate}{
            \northeast
            \pgf@circ@res@step=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@y
            \left
            \pgf@y=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@circ@res@step
        }
        \anchor{nobase}{
            \left
            \pgf@x=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@x
        }
        \anchor{nogate}{
            \left
            \pgf@x=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate width}\pgf@x
        }
        \anchor{E}{
            \northeast
            \pgf@y=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@y
        }
        \anchor{emitter}{
            \northeast
            \pgf@y=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@y
        }
        \anchor{C}{
            \northeast
            \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@y
        }
        \anchor{collector}{
            \northeast
            \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@y
        }
        \anchor{S}{
            \northeast
            \pgf@y=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@y
        }
        \anchor{source}{
            \northeast
            \pgf@y=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@y
        }
        \anchor{D}{
            \northeast
            \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@y
        }
        \anchor{drain}{
            \northeast
            \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction}\pgf@y
        }
        #2
        \backgroundpath{
            \pgftransformationadjustments
            \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
            %
            \ifnum \pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/curr direction} > 0
            \pgf@circuit@trans@ntypetrue
            \else
            \pgf@circuit@trans@ntypefalse
        \fi
        \northeast
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = \pgf@x
        \left
        \pgf@circ@res@left = \pgf@x
        %
        #3
        % BODY DIODE
        \ifpgf@circuit@fet@bodydiode
            \drawbodydiode{#1}
        \fi
        %
    }
}
}

\long\def\drawbodydiode#1{
    \pgfscope
        \pgftransformshift{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/bodydiode distance}\pgf@circ@res@left}{\pgf@circ@res@up+\pgf@circ@res@down}}
        \pgftransformrotate{90}
        \pgftransformscale{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/bodydiode scale}}
        \ifpgf@circuit@fulldiode
            \pgfnode{fulldiodeshape}{center}{}{pgf@bodydiode}{\pgfusepath{fill}}
        \else
            \pgfnode{emptydiodeshape}{center}{}{pgf@bodydiode}{\pgfusepath{fill}}
        \fi
    \endpgfscope
    % Draw stroke line
    \ifpgf@circuit@strokediode
        \pgfpathmoveto{\pgfpointanchor{pgf@bodydiode}{west}}
        \pgfpathlineto{\pgfpointanchor{pgf@bodydiode}{east}}
        \pgfusepath{stroke}
    \fi
    %Draw upper connection to body diode
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/bodydiode conn}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/bodydiode distance}\pgf@circ@res@left}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/bodydiode conn}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpointanchor{pgf@bodydiode}{east}}
    \pgfusepath{draw}
    \pgfscope
        \pgftransformshift{\pgfpoint{\pgf@circ@res@right}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/bodydiode conn}\pgf@circ@res@up}}
        \pgftransformscale{0.5}
        \pgfnode{circ}{center}{}{}{\pgfusepath{fill}}
    \endpgfscope{}
    %Draw lower connection to body diode
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/bodydiode conn}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/bodydiode distance}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/bodydiode conn}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpointanchor{pgf@bodydiode}{west}}
    \pgfusepath{draw}
    \pgfscope
        \pgftransformshift{\pgfpoint{\pgf@circ@res@right}		        	       {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/bodydiode conn}\pgf@circ@res@down}}
        \pgftransformscale{0.5}
        \pgfnode{circ}{center}{}{}{\pgfusepath{fill}}
    \endpgfscope
}

\long\def\declarebpt#1{
    \pgfcircdeclaretransistor{#1}{}{
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height 2}\pgf@circ@res@up}}
        \pgfusepath{draw}

        \pgfscope
            \pgfpathmoveto{\pgfpoint
                {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint
                {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@down}}
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}
            \pgfusepath{draw}
        \endpgfscope

        \pgfpathmoveto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height 2}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
        \pgfusepath{draw}
        %draw arrow depending on type of transistor
        \pgfscope
            \pgfslopedattimetrue
            \pgfallowupsidedownattimetrue
            \pgfresetnontranslationattimefalse
            \ifpgf@circuit@trans@ntype
                \pgftransformlineattime{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/arrow pos}}{%
                    \pgfpoint%
                    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}%
                    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height 2}\pgf@circ@res@down}%
                    }{%
                    \pgfpoint{\pgf@circ@res@right}%
                    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@down}%
                }
            \else
                \pgftransformlineattime{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/arrow pos}}{%
                    \pgfpoint{\pgf@circ@res@right}%
                    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@up}%
                    }{%
                    \pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}%
                    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height 2}\pgf@circ@res@up}%
                }
            \fi
            \pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
        \endpgfscope

        \ifpgf@circuit@bpt@drawphoto
            \pgfscope
                \pgfsetarrowsstart{latexslim}
                \pgfpathmoveto{\pgfpointadd{\pgfpoint
                        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
                    {\pgf@circ@res@up+\pgf@circ@res@down}}
                {\pgfpoint{0.05\pgf@circ@res@left}{0.1\pgf@circ@res@up}}}
                \pgfpathlineto{\pgfpointadd{\pgfpoint
                        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
                    {\pgf@circ@res@up+\pgf@circ@res@down}}
                {\pgfpoint{0.5\pgf@circ@res@left}{0.3\pgf@circ@res@up}}}
                \pgfusepath{draw}
                \pgfpathmoveto{\pgfpointadd{\pgfpoint
                        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
                    {\pgf@circ@res@up+\pgf@circ@res@down}}
                {\pgfpoint{0.05\pgf@circ@res@left}{-0.1\pgf@circ@res@up}}}
                \pgfpathlineto{\pgfpointadd{\pgfpoint
                        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
                    {\pgf@circ@res@up+\pgf@circ@res@down}}
                {\pgfpoint{0.5\pgf@circ@res@left}{0.1\pgf@circ@res@up}}}
                \pgfusepath{draw}
            \endpgfscope
            \else
            \ifpgf@circuit@bpt@drawbase
                \pgfpathmoveto{\pgfpoint
                    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
                {\pgf@circ@res@up+\pgf@circ@res@down}}
                \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}{\pgf@circ@res@up+\pgf@circ@res@down}}
                \pgfusepath{draw}
            \fi
        \fi
    }
}

\declarebpt{npn}
\declarebpt{pnp}

\long\def\declareigbt#1{
    \pgfcircdeclaretransistor{#1}{}
    {
        %draw upper connection
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height 2}\pgf@circ@res@up}}
        \pgfusepath{draw}

        %draw thicker gate lines
        \pgfscope
            \pgfpathmoveto{\pgfpoint
                {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate width}\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5\pgflinewidth}}
            \pgfpathlineto{\pgfpoint
                {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate width}\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5\pgflinewidth}}
            \pgfpathmoveto{\pgfpoint
                {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5\pgflinewidth}}
            \pgfpathlineto{\pgfpoint
                {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5\pgflinewidth}}
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}
            \pgfusepath{draw}
        \endpgfscope
        %draw lower connection
        \pgfpathmoveto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height 2}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
        \pgfusepath{draw}
        %draw arrow depending on type of transiytor
        \pgfscope
            \pgfslopedattimetrue
            \pgfallowupsidedownattimetrue
            \pgfresetnontranslationattimefalse
            \ifpgf@circuit@trans@ntype
                \pgftransformlineattime{.5}{%
                    \pgfpoint%
                    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}%
                    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height 2}\pgf@circ@res@down}%
                    }{%
                    \pgfpoint{\pgf@circ@res@right}%
                    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height}\pgf@circ@res@down}%
                }
            \else
                \pgftransformlineattime{.5}{%
                    \pgfpoint{\pgf@circ@res@right}%
                    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height}\pgf@circ@res@up}%
                    }{%
                    \pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}%
                    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height 2}\pgf@circ@res@up}%
                }
            \fi
            \pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
        \endpgfscope
        %draw gate
        \ifpgf@circuit@trans@ntype
            \pgfpathmoveto{\pgfpoint
                {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate width}\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@circ@res@down}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}%
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@circ@res@down}}
        \else
            \pgfpathmoveto{\pgfpoint
                {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate width}\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}%
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@circ@res@up}}
        \fi
        \pgfusepath{draw}
    }
}

\declareigbt{pigbt}
\declareigbt{nigbt}
\declareigbt{Lnigbt}
\declareigbt{Lpigbt}


\pgfcircdeclaretransistor{nmos}{}{%
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate height}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/base width}\pgf@circ@res@left}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate height}\pgf@circ@res@up}}

    \pgfpathmoveto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/base width}\pgf@circ@res@left}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate height}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate height}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfusepath{draw}

    \pgfscope
        \pgfpathmoveto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/base height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/base height}\pgf@circ@res@down}}
        \pgfpathmoveto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate height}\pgf@circ@res@down}}
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}
        \pgfusepath{draw}
    \endpgfscope
    \ifpgf@circuit@mos@arrows
        \pgfscope
            \pgfslopedattimetrue
            \pgfallowupsidedownattimetrue
            \pgfresetnontranslationattimefalse
            \pgftransformlineattime{\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/arrow pos}}{%
                \pgfpoint%
                {\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate width}\pgf@circ@res@left}%
                {\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate height}\pgf@circ@res@down}%
                }{%
                \pgfpoint
                {\pgf@circ@res@right}%
                {\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate height}\pgf@circ@res@down}%
            }
            \pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
        \endpgfscope
    \fi

    \ifpgf@circuit@bpt@drawgate
        \pgfpathmoveto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/nmos/gate width}\pgf@circ@res@left}
        {\pgf@circ@res@up+\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}{\pgf@circ@res@up+\pgf@circ@res@down}}
        \pgfusepath{draw}
    \fi
}


\pgfcircdeclaretransistor{pmos}{}{%
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate height}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/base width}\pgf@circ@res@left}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate height}\pgf@circ@res@up}}
    \pgfusepath{draw}

    \ifpgf@circuit@mos@arrows
        \pgfscope
            \pgfslopedattimetrue
            \pgfallowupsidedownattimetrue
            \pgfresetnontranslationattimefalse
            \pgftransformlineattime{\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/arrow pos}}{%
                \pgfpoint%
                {\pgf@circ@res@right}%
                {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate height}\pgf@circ@res@up}%
                }{%
                \pgfpoint
                {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate width}\pgf@circ@res@left}%
                {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate height}\pgf@circ@res@up}%
            }
            \pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
        \endpgfscope
    \fi

    \pgfscope
        \pgfpathmoveto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/base height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/base height}\pgf@circ@res@down}}
        \pgfpathmoveto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate height}\pgf@circ@res@down}}
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}
        \pgfusepath{draw}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/base width}\pgf@circ@res@left}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate height}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate height}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}


    \pgfusepath{draw}
    \ifpgf@circuit@bpt@drawgate
        \pgfpathmoveto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate width}\pgf@circ@res@left}
        {\pgf@circ@res@up+\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}{\pgf@circ@res@up+\pgf@circ@res@down}}
        \pgfusepath{draw}
    \fi
    \pgfpathcircle{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pmos/gate width}\pgf@circ@res@left - \pgfkeysvalueof{/tikz/circuitikz/nodes width}*\pgf@circ@Rlen}
    {\pgf@circ@res@up+\pgf@circ@res@down}}{\pgfkeysvalueof{/tikz/circuitikz/nodes width}*\pgf@circ@Rlen}
    \ifpgf@circuit@pmos@emptycircle
        \pgfsetfillcolor{white}
    \fi
    \pgfusepath{draw,fill}
}

%% HEMT FET Transistor
\pgfcircdeclaretransistor{hemt}{}{%
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/hemt/gate height}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/hemt/base width}\pgf@circ@res@left}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/hemt/gate height}\pgf@circ@res@up}}

    \pgfpathmoveto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/hemt/base width}\pgf@circ@res@left}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/hemt/gate height}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/hemt/gate height}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfusepath{draw}

    \pgfscope
        \pgfpathmoveto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/hemt/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/hemt/base height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/hemt/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/hemt/base height}\pgf@circ@res@down}}
        \pgfsetlinewidth{2\pgflinewidth}
        \pgfusepath{draw}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/hemt/base width}\pgf@circ@res@left}
    {\pgf@circ@res@up+\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}{\pgf@circ@res@up+\pgf@circ@res@down}}
    \pgfusepath{draw}
}

\long\def\drawfetcore#1{
    \pgftransformationadjustments
    %top connection
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height}\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfscope
        \pgfpathmoveto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@up}}
        \ifpgf@circuit@trans@depletiontype
            \pgfpathlineto{\pgfpoint
                {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@down}}
        \else

            \pgfpathlineto{\pgfpoint
                {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@up*0.45}}
            \pgfpathmoveto{\pgfpoint
                {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@up*0.25}}
            \pgfpathlineto{\pgfpoint
                {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@down*0.25}}
            \pgfpathmoveto{\pgfpoint
                {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/nfet/base height}\pgf@circ@res@down*0.45}}
            \pgfpathlineto{\pgfpoint
                {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base height}\pgf@circ@res@down}}
        \fi
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}
        \pgfusepath{draw}
    \endpgfscope
    %Bulk connection line
    \pgfpathmoveto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
    {\pgf@circ@res@up+\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right+\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}
    {\pgf@circ@res@up+\pgf@circ@res@down}}

    %bottom connection
    \pgfpathmoveto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfusepath{draw}

    %draw thick gate line
    \pgfscope
        \pgfpathmoveto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height}\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate height}\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}
        \pgfusepath{draw}
    \endpgfscope

    \pgfscope
        \pgfslopedattimetrue
        \pgfallowupsidedownattimetrue
        \pgfresetnontranslationattimefalse

        \pgftransformlineattime{.6}{%
            \pgfpoint
            {\pgf@circ@res@right}%
            {\pgf@circ@res@up+\pgf@circ@res@down}%
            }{%
            \pgfpoint%
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/base width}\pgf@circ@res@left}%
            {\pgf@circ@res@up+\pgf@circ@res@down}%
        }
        \ifpgf@circuit@trans@ntype
    \else
        \pgftransformrotate{180}
    \fi
    \pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
\endpgfscope

% GATE CONNECTION
\ifpgf@circuit@bpt@drawgate
    \ifpgf@circuit@trans@ntype
        \pgfpathmoveto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@circ@res@down}}
    \else
        \pgfpathmoveto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/gate width}\pgf@circ@res@left}
        {-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/#1/conn height}\pgf@circ@res@down}}
    \fi
    \pgfusepath{draw}
\fi

}

\long\def\pgfdeclaretransistorwrapperaddbulk#1#2#3
{\pgfcircdeclaretransistor{#1}{
        \anchor{bulk}{\left\pgf@x=0pt}
        \anchor{B}{\left\pgf@x=0pt}%override Base anchor from npn&igbt
        #2
    }
    {#3}
}


\pgfdeclaretransistorwrapperaddbulk{nfet}{}{%
	\pgf@circuit@trans@depletiontypefalse
	\drawfetcore{nfet}
}


\pgfdeclaretransistorwrapperaddbulk{pfet}{}{%
    \pgf@circuit@trans@depletiontypefalse
    \drawfetcore{pfet}
}

% N-CHANNEL IGFET ENHANCEMENT TYPE
\pgfdeclaretransistorwrapperaddbulk{nigfete}{}{%
    \pgf@circuit@trans@depletiontypefalse
    \drawfetcore{nigfete}

    % SOURCE CONNECTION
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfusepath{draw}

    % SOLDER DOT at source-bulk connection
    \ifpgf@circuit@fet@solderdot
        \pgfscope
            \pgftransformshift{\pgfpoint{\pgf@circ@res@right}{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/nigfete/gate height}\pgf@circ@res@down}}
            \pgfnode{circ}{center}{}{}{}
    \endpgfscope{}
\fi
}




% N-CHANNEL IGFET ENHANCEMENT TYPE with Bulk connector
\pgfdeclaretransistorwrapperaddbulk{nigfetebulk}{}{%
    \pgf@circuit@trans@depletiontypefalse
    \drawfetcore{nigfetebulk}
    % SOLDER DOT at source-bulk connection
    \ifpgf@circuit@fet@solderdot
        \pgfscope
            \pgftransformshift{\pgfpoint{\pgf@circ@res@right}{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/nigfetebulk/gate height}\pgf@circ@res@down}}
            \pgfnode{circ}{center}{}{}{}
        \endpgfscope{}
    \fi
}



% N-CHANNEL IGFET DEPLETION TYPE
\pgfdeclaretransistorwrapperaddbulk{nigfetd}{}{%
    \pgf@circuit@trans@depletiontypetrue
    \drawfetcore{nigfetd}

    % SOURCE CONNECTION
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
    \pgfusepath{draw}

    % SOLDER DOT at source-bulk connection
    \ifpgf@circuit@fet@solderdot
        \pgfscope
            \pgftransformshift{\pgfpoint{\pgf@circ@res@right}{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/nigfete/gate height}\pgf@circ@res@down}}
            \pgfnode{circ}{center}{}{}{}
        \endpgfscope{}
    \fi
}

% P-CHANNEL IGFET ENHANCEMENT TYPE
\pgfdeclaretransistorwrapperaddbulk{pigfete}{}{%
    \pgf@circuit@trans@depletiontypefalse
    \drawfetcore{pigfete}
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}

    % SOURCE CONNECTION
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}


    % SOLDER DOT at source-bulk connection
    \ifpgf@circuit@fet@solderdot
        \pgfscope
            \pgftransformshift{\pgfpoint{\pgf@circ@res@right}{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/pigfete/gate height}\pgf@circ@res@up}}
            \pgfnode{circ}{center}{}{}{}
        \endpgfscope
    \fi
}

% P-CHANNEL IGFET ENHANCEMENT TYPE with bulk connector
\pgfdeclaretransistorwrapperaddbulk{pigfetebulk}{}{%
    \pgf@circuit@trans@depletiontypefalse
    \drawfetcore{pigfetebulk}
}


% P-CHANNEL IGFET DEPLETION TYPE
\pgfdeclaretransistorwrapperaddbulk{pigfetd}{}{%
    \pgf@circuit@trans@depletiontypetrue
    \drawfetcore{pigfetd}

    % SOURCE CONNECTION
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}


    % SOLDER DOT at source-bulk connection
    \ifpgf@circuit@fet@solderdot
        \pgfscope
            \pgftransformshift{\pgfpoint{\pgf@circ@res@right}{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/nigfete/gate height}\pgf@circ@res@up}}
            \pgfnode{circ}{center}{}{}{}
        \endpgfscope{}
    \fi
}

\pgfcircdeclaretransistor{njfet}{}{%
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate height 2}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate width}\pgf@circ@res@left}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate height 2}\pgf@circ@res@up}}

    \pgfpathmoveto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate width}\pgf@circ@res@left}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate height 2}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate height 2}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfusepath{draw}

    \pgfscope
        \pgfpathmoveto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate height}\pgf@circ@res@down}}
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}
        \pgfusepath{draw}
    \endpgfscope

    \pgfscope
        \pgfslopedattimetrue
        \pgfallowupsidedownattimetrue
        \pgfresetnontranslationattimefalse
        \pgftransformlineattime{.6}{%
            \pgfpoint{\pgf@circ@res@left}%
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate height 2}\pgf@circ@res@down}%
            }{%
            \pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate width}\pgf@circ@res@left}%
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate height 2}\pgf@circ@res@down}%
        }
        \pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate width}\pgf@circ@res@left}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate height 2}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/njfet/gate height 2}\pgf@circ@res@down}}
    \pgfusepath{draw}
}


\pgfcircdeclaretransistor{pjfet}{}{%
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate height 2}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate width}\pgf@circ@res@left}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate height 2}\pgf@circ@res@up}}

    \pgfpathmoveto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate width}\pgf@circ@res@left}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate height 2}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate height 2}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfusepath{draw}

    \pgfscope
        \pgfpathmoveto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate height}\pgf@circ@res@down}}
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}
        \pgfusepath{draw}
    \endpgfscope

    \pgfscope
        \pgfslopedattimetrue
        \pgfallowupsidedownattimetrue
        \pgfresetnontranslationattimefalse
        \pgftransformlineattime{.4}{%
            \pgfpoint%
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate width}\pgf@circ@res@left}%
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate height 2}\pgf@circ@res@up}%
            }{%
            \pgfpoint{\pgf@circ@res@left}%
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate height 2}\pgf@circ@res@up}%
        }
        \pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
    \endpgfscope


    \pgfpathmoveto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate width}\pgf@circ@res@left}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate height 2}\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*.5*\pgflinewidth}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/pjfet/gate height 2}\pgf@circ@res@up}}
    \pgfusepath{draw}
}


\pgfdeclaretransistorwrapperaddbulk{isfet}{}{%
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up+\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    % DRAIN CONNECTION
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/gate height}\pgf@circ@res@up}}
    % DRAIN
    \pgfpathlineto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/base width}\pgf@circ@res@left}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/gate height}\pgf@circ@res@up}}
    \pgfusepath{draw}

    % GATE, DEPLETION TYPE
    \pgfscope %% added
        \pgfpathmoveto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/base height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/base width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/base height}\pgf@circ@res@down}}
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth} %% added
        \pgfusepath{draw} %% added
    \endpgfscope %% added

    % BULK
    \pgfpathmoveto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/base width}\pgf@circ@res@left}
    {\pgf@circ@res@up+\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right+.5\pgflinewidth}
    {\pgf@circ@res@up+\pgf@circ@res@down}}

    % SOURCE
    \pgfpathmoveto{\pgfpoint
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/base width}\pgf@circ@res@left}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/gate height}\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}
    {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/gate height}\pgf@circ@res@down}}
    % SOURCE CONNECTION
    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down-\pgfverticaltransformationadjustment*.5*\pgflinewidth}}
    \pgfusepath{draw}


    % SOLDER DOT at source-bulk connection
    \ifpgf@circuit@fet@solderdot
        \pgfscope
            \pgftransformshift{\pgfpoint{\pgf@circ@res@right}{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/nigfete/gate height}\pgf@circ@res@down}}
            \pgfnode{circ}{center}{}{}{}
        \endpgfscope{}
    \fi
    % ARROW
    \pgfscope
        \pgfslopedattimetrue
        \pgfallowupsidedownattimetrue
        \pgfresetnontranslationattimefalse
        \pgftransformlineattime{.6}{%
            \pgfpoint
            {\pgf@circ@res@right}%
            {\pgf@circ@res@up+\pgf@circ@res@down}%
            }{%
            \pgfpoint%
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/base width}\pgf@circ@res@left}%
            {\pgf@circ@res@up+\pgf@circ@res@down}%
        }
        \pgfnode{currarrow}{center}{}{}{\pgfusepath{stroke}}
    \endpgfscope
    \pgfusepath{draw}

    % Wavy lines
    \pgfscope
        \pgfpathmoveto{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/waves x sep}\pgf@circ@res@up}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/waves y sep}\pgf@circ@res@up}}
        \pgfpathsine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfpathsine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfusepath{draw}

        \pgfpathmoveto{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/waves x sep}\pgf@circ@res@up}{0cm}}
        \pgfpathsine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfpathsine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfusepath{draw}

        \pgfpathmoveto{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/waves x sep}\pgf@circ@res@up}{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/waves y sep}\pgf@circ@res@up}}
        \pgfpathsine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfpathsine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfpathcosine{\pgfpoint{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave width}\pgf@circ@res@up}{-\pgfkeysvalueof{/tikz/circuitikz/tripoles/isfet/wave amp}\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope

}


%% Black thyristor

\pgfcircdeclarebipole{
	\anchor{gate}{
		\northeast
	}
	\anchor{anode}{
		\southwest
		\pgf@y=0cm
	}
	\anchor{G}{
		\northeast
	}
	\anchor{cathode}{
		\northeast
		\pgf@y=0cm
	}
}
{\ctikzvalof{tripoles/thyristor/height 2}}
{fullthyristor}{\ctikzvalof{tripoles/thyristor/height}}
{\ctikzvalof{tripoles/thyristor/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgf@circ@res@other = \ctikzvalof{tripoles/thyristor/diode width left}\pgf@circ@res@left
    \pgf@circ@res@step = \ctikzvalof{tripoles/thyristor/diode width right}\pgf@circ@res@right

    \pgfscope
        \pgftransformxshift{\pgf@circ@res@other}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}

        \pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
        \pgfusepath{draw,fill}

        \pgfsetlinewidth{\pgfstartlinewidth}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
        \pgfpathlineto{\pgfpoint{2*\pgf@circ@res@step-2*\pgf@circ@res@other}{\ctikzvalof{tripoles/thyristor/diode height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{2*\pgf@circ@res@step-2*\pgf@circ@res@other}{\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{-\pgf@circ@res@down}}

    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0pt}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}

    \pgfusepath{draw}

}

%% Empty thyristor

\pgfcircdeclarebipole{
	\anchor{gate}{
		\northeast
	}
	\anchor{anode}{
		\southwest
		\pgf@y=0cm
	}
	\anchor{G}{
		\northeast
	}
	\anchor{cathode}{
		\northeast
		\pgf@y=0cm
	}
}
{\ctikzvalof{tripoles/thyristor/height 2}}
{emptythyristor}{\ctikzvalof{tripoles/thyristor/height}}
{\ctikzvalof{tripoles/thyristor/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgf@circ@res@other = \ctikzvalof{tripoles/thyristor/diode width left}\pgf@circ@res@left
    \pgf@circ@res@step = \ctikzvalof{tripoles/thyristor/diode width right}\pgf@circ@res@right

    \pgfscope
        \pgftransformxshift{\pgf@circ@res@other}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}

        \pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
        \pgfpathclose
        \pgf@circ@draworfill
        \pgfscope
            % to allow filling, we need to draw explicitily the stroke here.
            \pgfsetlinewidth{\pgfstartlinewidth}
            \ifpgf@circuit@bipole@strokedsymbol
                \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
                \pgfpathlineto{\pgfpoint{0pt}{0pt}}
                \pgfusepath{draw}
            \fi
        \endpgfscope

        \pgfsetlinewidth{\pgfstartlinewidth}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step-\pgf@circ@res@other}{0pt}}
        \pgfpathlineto{\pgfpoint{2*\pgf@circ@res@step-2*\pgf@circ@res@other}{\ctikzvalof{tripoles/thyristor/diode height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{2*\pgf@circ@res@step-2*\pgf@circ@res@other}{\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{\pgf@circ@res@down}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{-\pgf@circ@res@down}}

    \pgfusepath{draw}

    \pgfsetlinewidth{\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0pt}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}

    \pgfusepath{draw}

}

%% Empty triac

\pgfcircdeclarebipole{
	\anchor{gate}{
		\northeast
	}
	\anchor{G}{
		\northeast
	}
	\anchor{anode}{
		\southwest
		\pgf@y=0cm
	}
	\anchor{cathode}{
		\northeast
		\pgf@y=0cm
	}
}
{\ctikzvalof{tripoles/triac/height}}
{emptytriac}
{\ctikzvalof{tripoles/triac/height}}
{\ctikzvalof{tripoles/triac/width}}
{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgf@circ@res@other = \ctikzvalof{tripoles/triac/diode width left}\pgf@circ@res@left
    \pgf@circ@res@step = \ctikzvalof{tripoles/triac/diode width right}\pgf@circ@res@right

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{0.95\pgf@circ@res@step}{0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
    \pgfpathlineto{\pgfpoint{0.95\pgf@circ@res@other}{-0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}

    \pgf@circ@draworfill

    \pgfsetlinewidth{\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{-0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}} % sqrt(1/2)

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0pt}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}

    \pgfusepath{draw}

}

%% Full triac

\pgfcircdeclarebipole{
	\anchor{gate}{
		\northeast
	}
	\anchor{G}{
		\northeast
	}
	\anchor{anode}{
		\southwest
		\pgf@y=0cm
	}
	\anchor{cathode}{
		\northeast
		\pgf@y=0cm
	}
}
{\ctikzvalof{tripoles/triac/height}}
{fulltriac}
{\ctikzvalof{tripoles/triac/height}}
{\ctikzvalof{tripoles/triac/width}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgf@circ@res@other = \ctikzvalof{tripoles/triac/diode width left}\pgf@circ@res@left
    \pgf@circ@res@step = \ctikzvalof{tripoles/triac/diode width right}\pgf@circ@res@right

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{0.95\pgf@circ@res@step}{0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
    \pgfpathlineto{\pgfpoint{0.95\pgf@circ@res@other}{-0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@step}{1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}}

    \pgfusepath{draw,fill}

    \pgfsetlinewidth{\pgfstartlinewidth}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{-0.707*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{-1.414*(\pgf@circ@res@other-\pgf@circ@res@step)}} % sqrt(1/2)
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}} % sqrt(1/2)

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0pt}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0pt}}

    \pgfusepath{draw}

}

\pgfcircdeclarebipole{
	\anchor{out 1}{
		\northeast
		\pgf@y=0cm
	}
	\anchor{out 2}{
		\northeast
		\pgf@y=.8\pgf@y
	}
}
{\ctikzvalof{tripoles/toggleswitch/height 2}}
{toggleswitch}
{\ctikzvalof{tripoles/toggleswitch/height}}
{\ctikzvalof{tripoles/toggleswitch/width}}
{

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
    \pgfpathlineto{\pgfpoint{.3\pgf@circ@res@left}{0pt}}
    \pgfusepath{draw}
    \pgfscope
        \pgfpathmoveto{\pgfpoint{.3\pgf@circ@res@left}{0pt}}
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{.5\pgf@circ@res@up}}
        \pgfusepath{draw}
    \endpgfscope

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
    \pgfpathlineto{\pgfpoint{.5\pgf@circ@res@right}{0}}

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{.8\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.5\pgf@circ@res@right}{.8\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.5\pgf@circ@res@right}{.15\pgf@circ@res@up}}
    \pgfusepath{draw}


    \pgfpathmoveto{\pgfpoint{.2\pgf@circ@res@left}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.2\pgf@circ@res@right}{\pgf@circ@res@up}}
    \pgfusepath{draw}

    \pgfsetdash{{.08\pgf@circ@res@up}{.04\pgf@circ@res@up}{.7\pgf@circ@res@up}{.04\pgf@circ@res@up}{.8\pgf@circ@res@up}}{0cm}
    \pgfpathmoveto{\pgfpoint{0}{\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0}{.8\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{.2\pgf@circ@res@left}{.6\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0}{.4\pgf@circ@res@up}}
    \pgfpathlineto{\pgfpoint{0}{.2\pgf@circ@res@up}}
    \pgfusepath{draw}
    \pgfsetdash{}{0cm}
}

%% operational and instrumentation amplifiers

\pgfdeclareshape{op amp}
{
    \anchor{center}{\pgfpointorigin}
    \savedanchor\northwest{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{south}{
        \northwest
        \pgf@y=-\pgf@y
        \pgf@x=0pt
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \savedanchor\left{%
        \pgf@y=0pt
    }
    \anchor{leftedge}
    {\left
        \pgf@x = \pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@x
    }
    \savedanchor\inOneFixed{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{in up}{
        \inOneFixed
    }
    \anchor{in down}{
        \inOneFixed
        \pgf@y=-\pgf@y
    }

    \savedanchor\inOne{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    \ifpgf@circuit@oa@iplusup\pgf@y=-\pgf@y\fi
    }
    \anchor{-}{
        \inOne
    }
    \anchor{+}{
        \inOne
        \pgf@y=-\pgf@y
    }
    \savedanchor\up{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfpointlineattime{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/up pos}}{
            \pgfpoint{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@circ@res@left}
        {\pgf@circ@res@up}}
        {\pgfpoint{.7\pgf@circ@res@right}{0pt}}
    }
    \anchor{up}{
        \up
    }
    \anchor{down}{
        \up
        \pgf@y=-\pgf@y
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \left
    }
    \anchor{east}{
        \left
        \pgf@x=-\pgf@x
    }

    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }

    \anchor{text}{\pgfpoint{-.5\wd\pgfnodeparttextbox}{\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox}}

    \backgroundpath{
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}


        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x

        \pgfscope
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}
            \pgftransformxshift{.7\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=.7\pgf@circ@res@step

            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@step}{0pt}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
            \pgfpathclose
            \pgf@circ@draworfill
        \endpgfscope

        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@up}}
        \pgftext[left, at=\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@up}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/font} \ifpgf@circuit@oa@iplusup$+$\else$-$\fi}


        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@down}}
        \pgftext[left, at=\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@circ@res@down}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/font} \ifpgf@circuit@oa@iplusup$-$\else$+$\fi}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{0pt}}
        \pgfsetrectcap
        \pgfusepath{draw}


    }
}

%op amp shape as in european standard en 60617
\pgfdeclareshape{en amp}
{
    \anchor{center}{\pgfpointorigin}
    \savedanchor\northwest{%
        \pgf@y=\ctikzvalof{tripoles/en amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/en amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{south}{
        \northwest
        \pgf@y=-\pgf@y
        \pgf@x=0pt
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \savedanchor\left{%
        \pgf@y=0pt
    }
    \anchor{leftedge}
    {
        \left
        \pgf@x = \ctikzvalof{tripoles/en amp/port width}\pgf@x
    }
    \savedanchor\inOneFixed{%
        \pgf@y=\ctikzvalof{tripoles/op amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\ctikzvalof{tripoles/op amp/input height}\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/op amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{in up}{
        \inOneFixed
    }
    \anchor{in down}{
        \inOneFixed
        \pgf@y=-\pgf@y
    }
    \savedanchor\inOne{%
        \pgf@y=\ctikzvalof{tripoles/en amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\ctikzvalof{tripoles/en amp/input height}\pgf@y
        \pgf@x=-\ctikzvalof{tripoles/en amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    \ifpgf@circuit@oa@iplusup\pgf@y=-\pgf@y\fi
    }
    \anchor{-}{
        \inOne
    }
    \anchor{+}{
        \inOne
        \pgf@y=-\pgf@y
    }
    \anchor{up}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{down}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \left
    }
    \anchor{east}{
        \left
        \pgf@x=-\pgf@x
    }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \anchor{text}{\pgfpoint{-.5\wd\pgfnodeparttextbox}{\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox}}

    \backgroundpath{
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x

        \pgfscope
            \pgfsetlinewidth{\ctikzvalof{tripoles/thickness}\pgflinewidth}
            \pgfpathmoveto{\pgfpoint{\ctikzvalof{tripoles/en amp/port width}\pgf@circ@res@left}{\pgf@circ@res@down}}
            \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/en amp/port width}\pgf@circ@res@left}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/en amp/port width}\pgf@circ@res@right}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{\ctikzvalof{tripoles/en amp/port width}\pgf@circ@res@right}{\pgf@circ@res@down}}
            \pgfpathclose
            \pgf@circ@draworfill
        \endpgfscope

        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
            {\ctikzvalof{tripoles/en amp/input height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/en amp/port width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/en amp/input height}\pgf@circ@res@up}}
        \pgftext[left, at=\pgfpoint{\ctikzvalof{tripoles/en amp/port width}\pgf@circ@res@left}{\ctikzvalof{tripoles/en amp/input height}\pgf@circ@res@up}]{\ctikzvalof{tripoles/en amp/font} \ifpgf@circuit@oa@iplusup$+$\else$-$\fi}

        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
            {\ctikzvalof{tripoles/en amp/input height}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint
            {\ctikzvalof{tripoles/en amp/port width}\pgf@circ@res@left}
            {\ctikzvalof{tripoles/en amp/input height}\pgf@circ@res@down}}
        \pgftext[left, at=\pgfpoint{\ctikzvalof{tripoles/en amp/port width}\pgf@circ@res@left}{\ctikzvalof{tripoles/en amp/input height}\pgf@circ@res@down}]{\ctikzvalof{tripoles/en amp/font} \ifpgf@circuit@oa@iplusup$-$\else$+$\fi}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{0pt}}
        \pgfsetrectcap
        \pgfusepath{draw}


        \pgftext[top, y=-.5ex, at=\pgfpoint{0pt}{\pgf@circ@res@up}]{\hbox{\ctikzvalof{tripoles/en amp/font2}\ctikzvalof{tripoles/en amp/text}}}
        % \pgftext[top, y=-.5ex, at=\pgfpoint{0pt}{\pgf@circ@res@up}]{\ctikzvalof{tripoles/en amp/font2}$\mathstrut{\triangleright}\,\mathrm{A}$}
    }
}

%%Transkonduktanzverstärker
\pgfdeclareshape{gm amp}
{
    \anchor{center}{\pgfpointorigin}
    \savedanchor\northwest{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{south}{
        \northwest
        \pgf@y=-\pgf@y
    }
    \anchor{north}{
        \northwest
    }
    \savedanchor\left{%
        \pgf@y=0pt
    }
    \anchor{leftedge}
    {\left
        \pgf@x = \pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@x
    }
    \savedanchor\inOneFixed{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{in up}{
        \inOneFixed
    }
    \anchor{in down}{
        \inOneFixed
        \pgf@y=-\pgf@y
    }
    \savedanchor\inOne{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/input height}\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    \ifpgf@circuit@oa@iplusup\pgf@y=-\pgf@y\fi
    }
    \anchor{-}{
        \inOne
    }
    \anchor{+}{
        \inOne
        \pgf@y=-\pgf@y
    }
    \savedanchor\up{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfpointlineattime{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/up pos}}{
            \pgfpoint{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/port width}\pgf@circ@res@left}
        {\pgf@circ@res@up}}
        {\pgfpoint{.7\pgf@circ@res@right}{0pt}}
    }
    \anchor{up}{
        \up
    }
    \anchor{down}{
        \up
        \pgf@y=-\pgf@y
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \left
    }
    \anchor{east}{
        \left
        \pgf@x=-\pgf@x
    }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }

    \anchor{text}{\northwest
        \pgf@x=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@x
    \pgfpoint{-.5\wd\pgfnodeparttextbox+.25\pgf@x}{\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox}}

    \backgroundpath{
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x

        \pgfscope
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}
            \pgftransformxshift{.7\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=.7\pgf@circ@res@step
            %Umrandung:
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0}} %geändert startpunkt neu am ausgangsstrich
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{.5\pgf@circ@res@up}}%vom Ausgang nach oben
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}} %neu ecke links oben nach rechts oben
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}} %bei deneigängen runter
            \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{.5\pgf@circ@res@down}}%ecke links unten nach rechts unten
            \pgfpathclose
            \pgf@circ@draworfill
        \endpgfscope

        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/input height}\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/port width}\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/input height}\pgf@circ@res@up}}
        \pgftext[left, at=\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/input height}\pgf@circ@res@up}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/font} \ifpgf@circuit@oa@iplusup$+$\else$-$\fi}


        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/input height}\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/port width}\pgf@circ@res@left}
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/input height}\pgf@circ@res@down}}
        \pgftext[left, at=\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/gm amp/input height}\pgf@circ@res@down}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/font} \ifpgf@circuit@oa@iplusup$-$\else$+$\fi}

        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{.3\pgf@circ@res@right}{0pt}} %
        \pgfsetrectcap
        \pgfusepath{draw}

    }
}

%% instrumentation amplifier

\pgfdeclareshape{inst amp}
{
    % when tikz calls the anchor it wants the relative position in the lengths
    % \pgf@x  \pgf@y
    % \pgfpoint* functions set that variables
    % anchors are visible outside and run on use
    \anchor{center}{\pgfpointorigin}
    % savedanchors are internals and run on node creation (not use)
    % bounding-box top left
    \savedanchor\northwest{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{nw}{
        \northwest
    }
    \anchor{south}{
        \northwest
        \pgf@y=-\pgf@y
    }
    \anchor{north}{
        \northwest
    }
    \savedanchor\left{%
        \pgf@y=0pt
    }
    \anchor{leftedge}
    {\left
        \pgf@x = \pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@x
    }
    \savedanchor\inOneFixed{%
          \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/height}\pgf@circ@Rlen
          \pgf@y=.5\pgf@y
          \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@y
          \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/width}\pgf@circ@Rlen
          \pgf@x=.5\pgf@x
    }
    \anchor{in up}{
        \inOneFixed
    }
    \anchor{in down}{
        \inOneFixed
        \pgf@y=-\pgf@y
    }
    \savedanchor\inOne{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/input height}\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
        \ifpgf@circuit@oa@iplusup\pgf@y=-\pgf@y\fi
    }
    \anchor{-}{
        \inOne
    }
    \anchor{+}{
        \inOne
        \pgf@y=-\pgf@y
    }
    \savedanchor\up{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfpointlineattime{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/up pos}}{
            \pgfpoint{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/port width}\pgf@circ@res@left}
        {\pgf@circ@res@up}}
        {\pgfpoint{.7\pgf@circ@res@right}{.6\pgf@circ@res@up}}
    }
    \anchor{up}{
        \up
    }
    \anchor{down}{
        \up
        \pgf@y=-\pgf@y
    }
    % reference voltage input anchors.
    \savedanchor\refv{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfpointlineattime{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/refv pos}}{
            \pgfpoint{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/port width}\pgf@circ@res@left}
        {\pgf@circ@res@up}}
        {\pgfpoint{.7\pgf@circ@res@right}{.6\pgf@circ@res@up}}
    }
    % we need both because they are normally drawn under the amp, and if you
    % mirror it vertically you need them
    \anchor{refv up}{
        \refv
    }
    \anchor{refv down}{
        \refv
        \pgf@y=-\pgf@y
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \left
    }
    \anchor{east}{
        \left
        \pgf@x=-\pgf@x
    }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }

    \anchor{text}{\pgfpoint{-.5\wd\pgfnodeparttextbox}{\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox}}

    % let's start drawing the component
    \backgroundpath{
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
        %
        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        % main component, normally in thicker lines
        \pgfscope
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}
            \pgftransformxshift{.7\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=.7\pgf@circ@res@step
            %first point (near output)
            \pgfpathmoveto{\pgfpoint{1.4\pgf@circ@res@right}{0}}
            %from the exit to the top (short side)... (note that the .6 must be copied in \up and \refv anchors
            \pgfpathlineto{\pgfpoint{1.4\pgf@circ@res@right}{.6\pgf@circ@res@up}}
            % and then to the input "front up", "down", to the output short side "down"
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
            \pgfpathlineto{\pgfpoint{1.4\pgf@circ@res@right}{.6\pgf@circ@res@down}}
            % ...and close
            \pgfpathclose
            \pgf@circ@draworfill
        \endpgfscope
        % input terminal -
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/input height}\pgf@circ@res@up}}
        %
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/port width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/input height}\pgf@circ@res@up}}
        %
        \pgftext[left, at=\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/input height}\pgf@circ@res@up}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/font} \ifpgf@circuit@oa@iplusup$+$\else$-$\fi}

        % input terminal +
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/input height}\pgf@circ@res@down}}
        %
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/port width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/input height}\pgf@circ@res@down}}
    \pgftext[left, at=\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/input height}\pgf@circ@res@down}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp/font} \ifpgf@circuit@oa@iplusup$-$\else$+$\fi}
        % output lead
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{0pt}} %
        %
        \pgfsetrectcap
        \pgfusepath{draw}
    }
}

% instrumentation amplifier, with terminals for gain resistance between inputs
\pgfdeclareshape{inst amp ra}
{
    \anchor{center}{\pgfpointorigin}
    % bounding-box top left
    \savedanchor\northwest{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{nw}{
        \northwest
    }
    \anchor{south}{
        \northwest
        \pgf@y=-\pgf@y\pgf@x=0pt\relax
    }
    \anchor{north}{
        \northwest\pgf@x=0pt\relax
    }
    \savedanchor\left{%
        \pgf@y=0pt
    }
    \anchor{leftedge}
    {\left
        \pgf@x = \pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/port width}\pgf@x
    }
    % inputs (+-)
    \savedanchor\inOneFixed{%
          \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/height}\pgf@circ@Rlen
          \pgf@y=.5\pgf@y
          \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@y
          \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/width}\pgf@circ@Rlen
          \pgf@x=.5\pgf@x
    }
    \anchor{in up}{
        \inOneFixed
    }
    \anchor{in down}{
        \inOneFixed
        \pgf@y=-\pgf@y
    }
    \savedanchor\inOne{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/input height}\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
        \ifpgf@circuit@oa@iplusup\pgf@y=-\pgf@y\fi
    }
    \anchor{-}{
        \inOne
    }
    \anchor{+}{
        \inOne
        \pgf@y=-\pgf@y
    }
    % R ampli anchors. They are by default at 20% more than R-length distance
    % you can change that with the `ra pos` key (use 0.5 for one-R).
    \savedanchor\raOneFixed{%
          \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/height}\pgf@circ@Rlen
          \pgf@y=.5\pgf@y
          \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/input height}\pgf@y
          \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/op amp/width}\pgf@circ@Rlen
          \pgf@x=.5\pgf@x
    }
    \anchor{ra up}{
        \inOneFixed
    }
    \anchor{ra down}{
        \inOneFixed
        \pgf@y=-\pgf@y
    }
    \savedanchor\raOne{%
        \pgf@y=\pgf@circ@Rlen
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/ra pos}\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
        \ifpgf@circuit@oa@iplusup\pgf@y=-\pgf@y\fi
    }
    \anchor{ra-}{
        \raOne
    }
    \anchor{ra+}{
        \raOne
        \pgf@y=-\pgf@y
    }
    % power supplies
    \savedanchor\up{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfpointlineattime{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/up pos}}{
            \pgfpoint{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/port width}\pgf@circ@res@left}
        {\pgf@circ@res@up}}
        {\pgfpoint{.7\pgf@circ@res@right}{.4\pgf@circ@res@up}}
    }
    \anchor{up}{
        \up
    }
    \anchor{down}{
        \up
        \pgf@y=-\pgf@y
    }
    % reference voltage input anchors.
    \savedanchor\refv{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/height}\pgf@circ@Rlen
        \pgf@y=0.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/width}\pgf@circ@Rlen
        \pgf@x=0.5\pgf@x
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfpointlineattime{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/refv pos}}{
            \pgfpoint{
            \pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/port width}\pgf@circ@res@left}
        {\pgf@circ@res@up}}
        {\pgfpoint{.7\pgf@circ@res@right}{.4\pgf@circ@res@up}}
    }
    % we need both because they are normally drawn under the amp, and if you
    % mirror it vertically you need them
    \anchor{refv up}{
        \refv
    }
    \anchor{refv down}{
        \refv
        \pgf@y=-\pgf@y
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \left
    }
    \anchor{east}{
        \left
        \pgf@x=-\pgf@x
    }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }

    \anchor{text}{\pgfpoint{-.5\wd\pgfnodeparttextbox}{\dimexpr.5\dp\pgfnodeparttextbox-.5\ht\pgfnodeparttextbox}}

    % drawing of the component
    \backgroundpath{
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x

        % main component, normally in thicker lines
        \pgfscope
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}
            \pgftransformxshift{.7\pgf@circ@res@left}
            \pgf@circ@res@step=\pgf@circ@res@right
            \advance\pgf@circ@res@step by -\pgf@circ@res@left
            \pgf@circ@res@step=.7\pgf@circ@res@step
            %primer punto: la linea de salida (lado componente)
            \pgfpathmoveto{\pgfpoint{1.4\pgf@circ@res@right}{0}}
            %from the exit to the top (short side)... (note that the .4 must be copied in \up anchor
            \pgfpathlineto{\pgfpoint{1.4\pgf@circ@res@right}{.4\pgf@circ@res@up}}
            % and then to the input "front up", "down", to the output short side "down"
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{0pt}{\pgf@circ@res@down}}
            \pgfpathlineto{\pgfpoint{1.4\pgf@circ@res@right}{.4\pgf@circ@res@down}}
            % ...and close
            \pgfpathclose
            \pgf@circ@draworfill
        \endpgfscope

        % ra terminal -
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/ra pos}\pgf@circ@Rlen}}
        %
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/port width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/ra pos}\pgf@circ@Rlen}}
        % ra terminal +
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
        {-\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/ra pos}\pgf@circ@Rlen}}
        %
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/port width}\pgf@circ@res@left}
        {-\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/ra pos}\pgf@circ@Rlen}}
        % input terminal -
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/input height}\pgf@circ@res@up}}
        %
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/port width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/input height}\pgf@circ@res@up}}
        %
        \pgftext[left, at=\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/input height}\pgf@circ@res@up}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/font} \ifpgf@circuit@oa@iplusup$+$\else$-$\fi}

        % input terminal +
        \pgfpathmoveto{\pgfpoint
            {\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/input height}\pgf@circ@res@down}}
        %
        \pgfpathlineto{\pgfpoint
            {\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/port width}\pgf@circ@res@left}
        {\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/input height}\pgf@circ@res@down}}
        \pgftext[left, at=\pgfpoint{\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/port width}\pgf@circ@res@left}{\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/input height}\pgf@circ@res@down}]{\pgfkeysvalueof{/tikz/circuitikz/tripoles/inst amp ra/font} \ifpgf@circuit@oa@iplusup$-$\else$+$\fi}
        % output lead
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
        \pgfpathlineto{\pgfpoint{.7\pgf@circ@res@right}{0pt}} %
        %
        \pgfsetrectcap
        \pgfusepath{draw}
    }
}
%% Potentiometer
\pgfcircdeclarebipole{
	\anchor{wiper}{
		\northeast
		\pgfpoint{0pt}{\pgf@y}
	}
	\anchor{W}{
		\northeast
		\pgfpoint{0pt}{\pgf@y}
	}
}
{\ctikzvalof{bipoles/potentiometer/height 2}}
{potentiometer}{\ctikzvalof{bipoles/potentiometer/height}}
{\ctikzvalof{bipoles/potentiometer/width}}
{
    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
    \pgftransformationadjustments
    \pgfmathsetlength{\pgf@circ@res@step}{\ctikzvalof{bipoles/resistor/width}\pgf@circ@Rlen+\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}
    \divide \pgf@circ@res@step by 12

    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left-\pgfhorizontaltransformationadjustment*0.5*\pgflinewidth}{\pgf@circ@res@zero}}

    \pgf@circ@res@other = \pgf@circ@res@left
    \advance\pgf@circ@res@other by \pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{-\pgf@circ@res@down}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{-\pgf@circ@res@down}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{-\pgf@circ@res@down}}
    \advance\pgf@circ@res@other by 2\pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@down}}
    \advance\pgf@circ@res@other by \pgf@circ@res@step
    \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{\pgf@circ@res@zero}}
    \pgfsetbeveljoin
    \pgfusepath{draw}

    \pgfscope
        %\pgfsetlinewidth{\pgfstartlinewidth}
        \pgfsetarrowsend{latexslim}
        \pgfpathmoveto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}





%% Generic tunable

\pgfcircdeclarebipole{
	\anchor{wiper}{
		\northeast
		\pgfpoint{0pt}{\pgf@y}
	}
}
{\ctikzvalof{bipoles/generic potentiometer/height 2}}
{genericpotentiometer}
{\ctikzvalof{bipoles/generic potentiometer/height}}
{\ctikzvalof{bipoles/generic potentiometer/width}}
{

    \pgf@circ@res@step = \ctikzvalof{bipoles/resistor/width}\pgf@circ@Rlen
    \divide \pgf@circ@res@step by 14

    \pgfscope
        \pgfpathrectanglecorners{\pgfpoint{\pgf@circ@res@left}{-\pgf@circ@res@down}}{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
        \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
        \pgf@circ@draworfill
    \endpgfscope
    \pgfscope
        %\pgfsetlinewidth{\pgfstartlinewidth}
        \pgfsetarrowsend{latexslim}
        \pgfpathmoveto{\pgfpoint{0pt}{\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0pt}{-\pgf@circ@res@down}}
        \pgfusepath{draw}
    \endpgfscope
}


\pgfdeclareshape{mixer}
{
    \savedanchor\northwest{
        \ifpgf@circuit@boxed
            \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/twoport/width}\pgf@circ@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/bipoles/twoport/width}\pgf@circ@Rlen
            \pgf@x=.5\pgf@x
        \else
            \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/mixer/width}\pgf@circ@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/mixer/width}\pgf@circ@Rlen
            \pgf@x=.5\pgf@x
        \fi
    }
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{left}{%
        \northwest
        \pgf@y=0pt
    }
    \anchor{1}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{2}{
        \northwest
        \pgf@y=-\pgf@y
        \pgf@x=0pt
    }
    \anchor{3}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{4}{
        \northwest
        \pgf@y=\pgf@y
        \pgf@x=0pt
    }
    \anchor{in 1}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{in1}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{in}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{in 2}{
        \northwest
        \pgf@y=-\pgf@y
        \pgf@x=0pt
    }
    \anchor{in2}{
        \northwest
        \pgf@y=-\pgf@y
        \pgf@x=0pt
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{center}{
        \pgf@y=0pt
        \pgf@x=0pt
    }
    \anchor{east}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{south}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{south west}{
        \northwest
        \pgf@y=-\pgf@y
    }
    \anchor{north east}{
        \northwest
        \pgf@x=-\pgf@x
    }
    \anchor{north west}{
        \northwest
    }
    \anchor{south east}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@y=-\pgf@y
    }
    \backgroundpath{
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

        \pgf@circ@res@step=\ctikzvalof{tripoles/mixer/width}\pgf@circ@Rlen

        \pgfscope
            \pgfstartlinewidth=\pgflinewidth

            % draw outer box
            \ifpgf@circuit@boxed
                \pgfnode{box}{center}{}{pgf@box}{\pgfusepath{draw}}
            \fi

            % draw outer circle
            \ifpgf@circuit@boxed
                \pgf@circ@res@step=.7\pgf@circ@res@step
                \pgfsetdash{}{0pt}	% draw solid circle if boxed
            \else
                \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
            \fi
            \pgfpathcircle{\pgfpoint{0}{0}} {0.5\pgf@circ@res@step}
            \pgf@circ@draworfill

            % draw inner stuff
            \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
            \pgfsetlinewidth{\pgfstartlinewidth}
            \pgfpathmoveto{\pgfpointorigin}
            \pgfpathmoveto{\pgfpointpolar{135}{0.5\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpointpolar{-45}{0.5\pgf@circ@res@step}}
            \pgfpathmoveto{\pgfpointorigin}
            \pgfpathmoveto{\pgfpointpolar{45}{0.5\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpointpolar{-135}{0.5\pgf@circ@res@step}}
            \pgfusepath{draw}

        \endpgfscope
    }
}

\pgfdeclareshape{adder}
{
    \savedanchor\northwest{
        \ifpgf@circuit@boxed
            \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/twoport/width}\pgf@circ@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/bipoles/twoport/width}\pgf@circ@Rlen
            \pgf@x=.5\pgf@x
        \else
            \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/adder/width}\pgf@circ@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/adder/width}\pgf@circ@Rlen
            \pgf@x=.5\pgf@x
        \fi
    }
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{left}{%
        \northwest
        \pgf@y=0pt
    }
    \anchor{1}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{2}{
        \northwest
        \pgf@y=-\pgf@y
        \pgf@x=0pt
    }
    \anchor{3}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{4}{
        \northwest
        \pgf@y=\pgf@y
        \pgf@x=0pt
    }
    \anchor{in 1}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{in1}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{in}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{in 2}{
        \northwest
        \pgf@y=-\pgf@y
        \pgf@x=0pt
    }
    \anchor{in2}{
        \northwest
        \pgf@y=-\pgf@y
        \pgf@x=0pt
    }
    \anchor{out}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{center}{
        \pgf@y=0pt
        \pgf@x=0pt
    }
    \anchor{east}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{south}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{south west}{
        \northwest
        \pgf@y=-\pgf@y
    }
    \anchor{north east}{
        \northwest
        \pgf@x=-\pgf@x
    }
    \anchor{north west}{
        \northwest
    }
    \anchor{south east}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@y=-\pgf@y
    }
    \backgroundpath{
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

        \pgf@circ@res@step=\ctikzvalof{tripoles/adder/width}\pgf@circ@Rlen

        \pgfscope
            \pgfstartlinewidth=\pgflinewidth

            % draw outer box
            \ifpgf@circuit@boxed
                \pgfnode{box}{center}{}{pgf@box}{\pgfusepath{draw}}
            \fi

            % draw outer circle
            \ifpgf@circuit@boxed
                \pgf@circ@res@step=.7\pgf@circ@res@step{}
                \pgfsetdash{}{0pt}	% draw solid circle if boxed
            \else
                \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
            \fi
            \pgfpathcircle{\pgfpoint{0}{0}} {0.5\pgf@circ@res@step}
            \pgf@circ@draworfill

            % draw inner stuff
            \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
            \pgfsetlinewidth{\pgfstartlinewidth}

            \pgfpathmoveto{\pgfpointorigin}
            \pgfpathmoveto{\pgfpointpolar{0}{0.3\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpointpolar{180}{0.3\pgf@circ@res@step}}
            \pgfpathmoveto{\pgfpointorigin}
            \pgfpathmoveto{\pgfpointpolar{90}{0.3\pgf@circ@res@step}}
            \pgfpathlineto{\pgfpointpolar{270}{0.3\pgf@circ@res@step}}
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/tripoles/thickness}\pgflinewidth}
            \pgfusepath{draw}

        \endpgfscope
    }
}

\pgfdeclareshape{oscillator}
{
    \savedanchor\northwest{
        \ifpgf@circuit@boxed
            \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/twoport/width}\pgf@circ@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/bipoles/twoport/width}\pgf@circ@Rlen
        \else
            \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/oscillator/width}\pgf@circ@Rlen
            \pgf@y=.5\pgf@y
            \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/oscillator/width}\pgf@circ@Rlen
        \fi
    }
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{north}{
        \northwest
        \pgf@x=.5\pgf@x
    }
    \anchor{south}{
        \northwest
        \pgf@x=.5\pgf@x
        \pgf@y=-\pgf@y
    }
    \anchor{east}{
        \northwest
        \pgf@y=0pt
        \pgf@x=0pt
    }
    \anchor{west}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y}
    \anchor{north east}{ \northwest \pgf@x=0pt\relax}
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=0pt \pgf@y=-\pgf@y }
    \anchor{text}{
        \pgf@x=-2\pgf@x
        \advance \pgf@x by -.5\wd\pgfnodeparttextbox
        \advance \pgf@y by -1.5\ht\pgfnodeparttextbox
    }
    \backgroundpath{
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

        \pgf@circ@res@step=\ctikzvalof{tripoles/oscillator/width}\pgf@circ@Rlen{}

        \pgfscope
            \pgfstartlinewidth=\pgflinewidth

            \pgftransformxshift{-0.5\pgf@circ@res@step} % The oscillator is shifted to the left, so a connection comes out of the anchor "east"

            % draw outer box
            \ifpgf@circuit@boxed{}
                \pgfnode{box}{center}{}{pgf@box}{\pgfusepath{draw}}
            \fi

            % draw outer circle
            \ifpgf@circuit@boxed
                \pgf@circ@res@step=.7\pgf@circ@res@step{}
                \pgfsetdash{}{0pt}	% draw solid circle if boxed
            \else
                \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
            \fi
            \pgfpathcircle{\pgfpoint{0}{0}} {0.5\pgf@circ@res@step}
            \pgf@circ@draworfill

            % draw inner sine waves
            \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
            \pgfsetlinewidth{\pgfstartlinewidth}
            \pgfsetcornersarced{\pgfpointorigin}% do not use rounded corners!
            \pgfpathmoveto{\pgfpoint{-0.3\pgf@circ@res@step}{0\pgf@circ@res@step}}
            \pgfpathsine{\pgfpoint{.15\pgf@circ@res@step}{.15\pgf@circ@res@step}}
            \pgfpathcosine{\pgfpoint{.15\pgf@circ@res@step}{-.15\pgf@circ@res@step}}
            \pgfpathsine{\pgfpoint{.15\pgf@circ@res@step}{-.15\pgf@circ@res@step}}
            \pgfpathcosine{\pgfpoint{.15\pgf@circ@res@step}{.15\pgf@circ@res@step}}

            \pgfusepath{draw}

        \endpgfscope
    }
}

\pgfdeclareshape{circulator}
{
	\savedanchor\northwest{
		\ifpgf@circuit@boxed
			\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/bipoles/twoport/width}\pgf@circ@Rlen
			\pgf@y=.5\pgf@y
			\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/bipoles/twoport/width}\pgf@circ@Rlen
			\pgf@x=.5\pgf@x
		\else
			\pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/circulator/width}\pgf@circ@Rlen
			\pgf@y=.5\pgf@y
			\pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/circulator/width}\pgf@circ@Rlen
			\pgf@x=.5\pgf@x
		\fi
	}
	\anchor{center}{
		\pgfpointorigin
	}
	\anchor{left}{%
		\northwest
	  	\pgf@y=0pt
	}
	\anchor{1}{
		\northwest
		\pgf@y=0pt
	}
	\anchor{2}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x
	}
	\anchor{3}{
		\northwest
		\pgf@y=-\pgf@y
		\pgf@x=0pt
	}
	\anchor{east}{
		\northwest
		\pgf@y=0pt
		\pgf@x=-\pgf@x
	}
	\anchor{west}{
		\northwest
		\pgf@y=0pt
	}
	\anchor{south}{
		\northwest
		\pgf@x=0pt
		\pgf@y=-\pgf@y
	}
	\anchor{north}{
		\northwest
		\pgf@x=0pt
	}
	\anchor{south west}{
		\northwest
		\pgf@y=-\pgf@y
	}
	\anchor{north east}{
		\northwest
		\pgf@x=-\pgf@x
	}
	\anchor{north west}{
		\northwest
	}
	\anchor{south east}{
		\northwest
		\pgf@x=-\pgf@x
		\pgf@y=-\pgf@y
	}
	\backgroundpath{
		\pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

		\pgf@circ@res@step=\ctikzvalof{tripoles/circulator/width}\pgf@circ@Rlen

		\pgfscope
			\pgfstartlinewidth=\pgflinewidth

			% draw outer box
			\ifpgf@circuit@boxed
				\pgfnode{box}{center}{}{pgf@box}{\pgfusepath{draw}}
			\fi

			% draw outer circle
			\ifpgf@circuit@boxed{}
				\pgf@circ@res@step=.7\pgf@circ@res@step{}
				\pgfsetdash{}{0pt}	% draw solid circle if boxed
			\else
				\pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
			\fi
			\pgfpathcircle{\pgfpoint{0}{0}} {0.5\pgf@circ@res@step}
                        \pgf@circ@draworfill

			% inner arrow
			\pgfsetdash{}{0pt}	% always draw solid line for inner symbol
			\pgfsetlinewidth{\pgfstartlinewidth}

			\pgfsetarrowsend{latex}
			\pgfpathmoveto{\pgfpoint{-0.25\pgf@circ@res@step}{0}}
			\pgfpatharc{180}{-90} {0.25\pgf@circ@res@step}
			\pgfpathlineto{\pgfpoint{-5pt}{-0.2\pgf@circ@res@step}}
			\pgfusepath{draw}

		\endpgfscope
	}
}


% Wilkinson divider
\pgfdeclareshape{wilkinson}{
    \anchor{center}{
        \northwest
        \pgf@x=0pt
        \pgf@y=0pt
    }
    \savedanchor\northwest{%
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/wilkinson/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x= \pgf@circ@Rlen
        \pgf@x=.5\pgf@x
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/wilkinson/width}\pgf@x
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{south}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{west}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{east}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{south west}{
        \northwest
        \pgf@y=-\pgf@y
    }
    \anchor{north east}{
        \northwest
        \pgf@x=-\pgf@x
    }
    \anchor{north west}{
        \northwest
    }
    \anchor{south east}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@y=-\pgf@y
    }
    \anchor{in}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{out1}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@y=-0.5\pgf@y
    }
    \anchor{out2}{
        \northwest
        \pgf@x=-\pgf@x
        \pgf@y=0.5\pgf@y
    }
    \anchor{text}{
        \northwest
        \advance \pgf@y by 0.5\ht\pgfnodeparttextbox
        \pgf@x=-.5\wd\pgfnodeparttextbox
    }
    \backgroundpath{
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}

        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x

        \pgfstartlinewidth=\pgflinewidth

        % draw outer box
        \pgf@circ@twoportbox

        % draw inner stuff
        \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
        \pgfsetarrows{-} %never draw arrows
        \pgfsetlinewidth{\pgfstartlinewidth}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@left}{0pt}}
        \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@right}{0.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@left}{0pt}}
        \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@right}{0.5\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{0.5\pgf@circ@res@down}}

        \pgfusepath{draw}

        \pgfsetdash{}{0pt}	% always draw solid line for inner symbol
        % draw inner resisitor - european or american style is recognised
        {
            \pgftransformshift{\pgfpoint{0.5\pgf@circ@res@right}{0pt}}
            \pgftransformrotate{90}

            % calculate size of resistor
            \ifpgf@circuit@europeanresistor
                \pgfmathparse{\pgf@circ@res@up / \pgf@circ@Rlen / \ctikzvalof{bipoles/generic/width} / 2}
                \pgftransformscale{\pgfmathresult}
                \pgfnode{genericshape}{center}{}{pgf@generic}{\pgfusepath{fill}}
            \else
                \pgfmathparse{\pgf@circ@res@up / \pgf@circ@Rlen / \ctikzvalof{bipoles/resistor/width} / 2}
                \pgftransformscale{\pgfmathresult}
                \pgfnode{resistorshape}{center}{}{pgf@resistor}{\pgfusepath{fill}}
            \fi
        }

        \pgfpathmoveto{\pgfpoint{0.5\pgf@circ@res@right}{0.5\pgf@circ@res@up}}
        \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@right}{0.25\pgf@circ@res@up}}

        \pgfpathmoveto{\pgfpoint{0.5\pgf@circ@res@right}{0.25\pgf@circ@res@down}}
        \pgfpathlineto{\pgfpoint{0.5\pgf@circ@res@right}{0.5\pgf@circ@res@down}}
        \pgfusepath{draw}

    }
}

% electromechanical device (motor/generator)
\pgfdeclareshape{elmech}
{
    \savedanchor\northwest{
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/elmech/height}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/elmech/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{text}{
        \pgfpointorigin
        \advance \pgf@x by -.5\wd\pgfnodeparttextbox
        \advance \pgf@y by -.5\ht\pgfnodeparttextbox
    }
    \anchor{left}{%
        \northwest
        \pgf@y=0pt
    }
    \anchor{right}{%
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{top}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{pathstart}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{pathend}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{bottom}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{center}{
        \pgf@y=0pt
        \pgf@x=0pt
    }
    \anchor{east}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{south}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \backgroundpath{
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
        \pgf@circ@res@step=\ctikzvalof{tripoles/elmech/width}\pgf@circ@Rlen
        \pgf@circ@res@up=\ctikzvalof{tripoles/elmech/height}\pgf@circ@Rlen
        \pgfscope
            \pgfstartlinewidth=\pgflinewidth
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
            \pgfscope % clip the bar: whole size minus the circle
                \pgfpathrectanglecorners{\pgfpoint{-.5\pgf@circ@res@step}{-.5\pgf@circ@res@up}}{\pgfpoint{.5\pgf@circ@res@step}{.5\pgf@circ@res@up}}
                \pgfpathcircle{\pgfpoint{0}{0}} {0.5\pgf@circ@res@step}
                \pgfseteorule
                \pgfusepath{clip}
                \pgfpathrectangle{\pgfpoint{-.25\pgf@circ@res@step}{-.5\pgf@circ@res@up}}{\pgfpoint{.5\pgf@circ@res@step}{\pgf@circ@res@up}}
                \pgfsetfillcolor{black}
                \pgfusepath{fill, draw}
            \endpgfscope
            \pgfpathcircle{\pgfpoint{0}{0}} {0.5\pgf@circ@res@step}
            \ifx\tikz@fillcolor\pgfutil@empty
                \pgfsetfillcolor{white}
            \else
                \pgfsetfillcolor{\tikz@fillcolor}
            \fi
            \pgfusepath{draw, fill}
        \endpgfscope
    }
}

\pgfdeclareshape{magnetron}
{
    \savedanchor\northwest{
        \pgf@y=\pgfkeysvalueof{/tikz/circuitikz/tripoles/magnetron/width}\pgf@circ@Rlen
        \pgf@y=.5\pgf@y
        \pgf@x=-\pgfkeysvalueof{/tikz/circuitikz/tripoles/magnetron/width}\pgf@circ@Rlen
        \pgf@x=.5\pgf@x
    }
    \anchor{center}{
        \pgfpointorigin
    }
    \anchor{anode}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{cathode1}{
        \northwest
        \pgf@circ@res@step=\pgf@y
        \pgfmathparse{cos(105)}
        \pgf@x=\pgfmathresult\pgf@circ@res@step
        \pgfmathparse{sin(105)}
        \pgf@y=\pgfmathresult\pgf@circ@res@step
        %\pgfpointorigin
        %\pgfpathmoveto{\pgfpointpolar{105}{\pgf@circ@res@step}}%not working in a scaled tikzpicture
    }
    \anchor{cathode2}{
        \northwest
        \pgf@circ@res@step=\pgf@y
        \pgfmathparse{cos(75)}
        \pgf@x=\pgfmathresult\pgf@circ@res@step
        \pgfmathparse{sin(75)}
        \pgf@y=\pgfmathresult\pgf@circ@res@step
        %\pgfpointorigin
        %\pgfpathmoveto{\pgfpointpolar{75}{\pgf@circ@res@step}}%not working in a scaled tikzpicture
    }
    \anchor{text}{
        \pgfpointorigin
        \advance \pgf@x by -.5\wd\pgfnodeparttextbox
        \advance \pgf@y by -.5\ht\pgfnodeparttextbox
    }
    \anchor{left}{%
        \northwest
        \pgf@y=0pt
    }
    \anchor{right}{%
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{top}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{pathstart}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{pathend}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{bottom}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{center}{
        \pgf@y=0pt
        \pgf@x=0pt
    }
    \anchor{east}{
        \northwest
        \pgf@y=0pt
        \pgf@x=-\pgf@x
    }
    \anchor{west}{
        \northwest
        \pgf@y=0pt
    }
    \anchor{south}{
        \northwest
        \pgf@x=0pt
        \pgf@y=-\pgf@y
    }
    \anchor{north}{
        \northwest
        \pgf@x=0pt
    }
    \anchor{south west}{ \northwest \pgf@y=-\pgf@y }
    \anchor{north east}{ \northwest \pgf@x=-\pgf@x }
    \anchor{north west}{ \northwest }
    \anchor{south east}{ \northwest \pgf@x=-\pgf@x \pgf@y=-\pgf@y }
    \backgroundpath{
        \pgfsetcolor{\pgfkeysvalueof{/tikz/circuitikz/color}}
        \pgf@circ@res@step=\ctikzvalof{tripoles/magnetron/width}\pgf@circ@Rlen
        \northwest
        \pgf@circ@res@up = \pgf@y
        \pgf@circ@res@down = -\pgf@y
        \pgf@circ@res@right = -\pgf@x
        \pgf@circ@res@left = \pgf@x
        \pgfmathsetlength{\pgf@circ@res@other}{sin(15)*\pgf@circ@res@up}

        \pgfscope
            \pgfstartlinewidth=\pgflinewidth
            \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}
            %create outer circle
            \pgfpathcircle{\pgfpoint{0}{0}} {\pgf@circ@res@right}
            \pgf@circ@draworfill
            %create chambers
            \foreach \angle in {45,135,225,315}{
                \pgfpathmoveto{ \pgfpointpolar{\angle}{0.6\pgf@circ@res@right}}
                \pgfpathlineto{ \pgfpointpolar{\angle}{\pgf@circ@res@right}}
            }
            \pgfsetroundcap
            \pgfusepath{draw}
            \pgfscope
                %draw connection from outside
                %anode
                \pgfsetlinewidth{\pgfstartlinewidth}
                \pgfpathmoveto{\pgfpoint{0\pgf@circ@res@left}{\pgf@circ@res@down}}
                \pgfpathlineto{\pgfpoint{0\pgf@circ@res@right}{.5\pgf@circ@res@down}}
                %cathodes
                \pgfpathmoveto{\pgfpointpolar{105}{\pgf@circ@res@up}}
                \pgfpathlineto{\pgfpoint{-\pgf@circ@res@other}{.5\pgf@circ@res@up}}
                \pgfpathmoveto{\pgfpointpolar{75}{\pgf@circ@res@up}}
                \pgfpathlineto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@up}}
                \pgfsetbuttcap
                \pgfusepath{draw}
            \endpgfscope
            %create cathode
            \pgfpathmoveto{\pgfpoint{\pgf@circ@res@other}{.5\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{0}{.15\pgf@circ@res@up}}
            \pgfpathlineto{\pgfpoint{-\pgf@circ@res@other}{.5\pgf@circ@res@up}}
            \pgfusepath{draw}
            %create anode
            \pgfpathmoveto{\pgfpoint{0.3\pgf@circ@res@left}{.5\pgf@circ@res@down}}
            \pgfpathlineto{\pgfpoint{0.3\pgf@circ@res@right}{.5\pgf@circ@res@down}}

            \pgfsetbuttcap
            \pgfusepath{draw}
        \endpgfscope
    }
}

\endinput


==> pgfcircutils.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the files gpl-3.0_license.txt and lppl-1-3c_license.txt for more details.

%\def\pgf@circ@handleSI#1{%
 % \pgf@circ@siunitx@resfalse
%
 % \edef\len{\stringlength[e]{#1}}
  %\testmatchingchar[e]{#1}{\len}{>}%
  %\ifmatchingchar%
  %  \ifnum\findchars{#1}{<}=0
	%  \def\pgf@circ@handleSI@val{\substring{#1}{1}{\findchars{#1}{<}-1}}
	  %\def\pgf@circ@handleSI@unit{\substring{#1}{\findchars{#1}{<}-1}+1}{\stringlength{#1}}
	  %\pgf@circ@siunitx@restrue
%	\else
%	\fi
  %\else
  %\fi
%}

\def\pgf@circ@handleSI#1{
    \noexpandarg
    \def\pgf@temp{}
    \StrBetween{#1}{<}{>}[\pgf@circ@handleSI@unit]
    \StrLen{\pgf@circ@handleSI@unit}[\pgf@circ@handleSI@unit@len]

    \ifnum\pgf@circ@handleSI@unit@len=0
    \pgf@circ@siunitx@resfalse
    \else
    \IfEndWith{#1}{>}{
        \pgf@circ@siunitx@restrue
        \noexpandarg
        \StrBefore{#1}{<}[\pgf@circ@handleSI@val]
        %\typeout{si |#1|}
        }{
        \pgf@circ@siunitx@resfalse
        %\typeout{no si |#1|}
    }
\fi
}

\def\pgf@circ@ifkeyempty#1{
    \pgfextra{
        \ctikzset{#1/.get=\pgf@circ@temp}
        \edef\pgf@temp{}
    }
    \ifx\pgf@circ@temp\pgf@temp
    }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%    Math routines

\def\pgf@circ@stripdecimals#1.#2\pgf@nil{#1}

\endinput


==> pgfcircvoltage.tex <==
% Copyright 2007-2009 by Massimo Redaelli
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the files gpl-3.0_license.txt and lppl-1-3c_license.txt for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Voltage management


\ctikzset{v^>/.style = {
        v = #1,
        \circuitikzbasekey/bipole/voltage/direction = forward,
        \circuitikzbasekey/bipole/voltage/position = above
    }
}

\ctikzset{v^</.style = {
        v = #1,
        \circuitikzbasekey/bipole/voltage/direction = backward,
        \circuitikzbasekey/bipole/voltage/position = above
    }
}

\ctikzset{v_>/.style = {
        v = #1,
        \circuitikzbasekey/bipole/voltage/direction = forward,
        \circuitikzbasekey/bipole/voltage/position = below
    }
}

\ctikzset{v_</.style = {
        v = #1,
        \circuitikzbasekey/bipole/voltage/direction = backward,
        \circuitikzbasekey/bipole/voltage/position = below
    }
}

\ctikzset{v_/.style = {v = #1, \circuitikzbasekey/bipole/voltage/position = below} }
\ctikzset{v^/.style = {v = #1, \circuitikzbasekey/bipole/voltage/position  = above} }
\ctikzset{v>/.style = {v = #1, \circuitikzbasekey/bipole/voltage/direction = forward} }
\ctikzset{v</.style = {v = #1, \circuitikzbasekey/bipole/voltage/direction = backward} }

% Default position varies whether the component is a voltage source
% or not
\ctikzset{v/.code = {
        \ifpgf@circuit@bipole@isvoltage
            \pgfkeys{\circuitikzbasekey/bipole/voltage/position=above,
            \circuitikzbasekey/bipole/voltage/direction=forward}
        \else
            \ifpgf@circ@oldvoltagedirection
                \pgfkeys{\circuitikzbasekey/bipole/voltage/position=below,
                \circuitikzbasekey/bipole/voltage/direction=backward}
            \else
                \pgfkeys{\circuitikzbasekey/bipole/voltage/position=below,
                \circuitikzbasekey/bipole/voltage/direction=forward}
            \fi
        \fi
        \ifpgf@circ@oldvoltagedirection
            \ifpgf@circuit@bipole@iscurrent\ifpgf@circ@fixbatteries
                \pgfkeys{\circuitikzbasekey/bipole/voltage/position=below,
                \circuitikzbasekey/bipole/voltage/direction=forward}
        \fi\fi
        \else
        \ifpgf@circuit@bipole@iscurrent
            \ifpgf@circuit@bipole@current@backward
                \pgfkeys{\circuitikzbasekey/bipole/voltage/position=below,
                \circuitikzbasekey/bipole/voltage/direction=forward}
            \else
                \pgfkeys{\circuitikzbasekey/bipole/voltage/position=below,
                \circuitikzbasekey/bipole/voltage/direction=backward}
            \fi\fi\fi
            \pgfkeys{/tikz/circuitikz/bipole/voltage/label/name=#1}
            \ctikzsetvalof{bipole/voltage/label/unit}{}
            \ifpgf@circ@siunitx
                \pgf@circ@handleSI{#1}
                \ifpgf@circ@siunitx@res
                    \edef\pgf@temp{\pgf@circ@handleSI@val}
                    \pgfkeyslet{/tikz/circuitikz/bipole/voltage/label/name}{\pgf@temp}
                    \edef\pgf@temp{\pgf@circ@handleSI@unit}
                    \pgfkeyslet{/tikz/circuitikz/bipole/voltage/label/unit}{\pgf@temp}
                \else
            \fi
            \else
        \fi
    }
}

% american voltage font selection and symbol definition
% the default font command is {} --- nothing
\def\pgf@circ@avfont{\ctikzvalof{voltage/american font}}
%
% plus and minus symbols (default is $+$ and $-$, see pgfcirc.defines.tex)
% notice that the double braces are needed  to be able
% to use \boldmath in the font (although it is semi-deprecated...)
%
\def\pgf@circ@avplus{\ctikzvalof{voltage/american plus}}
\def\pgf@circ@avminus{\ctikzvalof{voltage/american minus}}

%% Output routine for generic bipoles

\def\pgf@circ@drawvoltagegeneric{
    \pgfextra{
        \edef\pgf@temp{/tikz/circuitikz/bipoles/\pgfkeysvalueof{/tikz/circuitikz/bipole/kind}/voltage/straight label distance}
        \pgfkeysifdefined{\pgf@temp}
        {
            \edef\partheight{\ctikzvalof{bipoles/\pgfkeysvalueof{/tikz/circuitikz/bipole/kind}/voltage/straight label distance}}
            \edef\tmpdistfromline{(\partheight\pgf@circ@Rlen)}
        }
        {
            \pgfkeysifdefined{/tikz/circuitikz/bipoles/voltage/straight label distance}
            {
                \edef\partheight{\ctikzvalof{bipoles/voltage/straight label distance}}
                \edef\tmpdistfromline{(\partheight\pgf@circ@Rlen)}
            }
            {%calculate default value from part height
                \edef\pgf@temp{/tikz/circuitikz/bipoles/\pgfkeysvalueof{/tikz/circuitikz/bipole/kind}/height}
                \pgfkeysifdefined{\pgf@temp}
                {
                    \edef\partheight{0.5*\ctikzvalof{bipoles/\pgfkeysvalueof{/tikz/circuitikz/bipole/kind}/height}}
                    \edef\tmpdistfromline{(\partheight\pgf@circ@Rlen+0.2\pgf@circ@Rlen)}
                }
                {
                    \edef\tmpdistfromline{(.5\pgf@circ@Rlen)} %fallback to fixed value
                }
            }
        }
        \ifnum \ctikzvalof{mirror value}=-1
        \ifpgf@circuit@bipole@inverted
            \ifpgf@circuit@bipole@voltage@straight
                \def\distfromline{\tmpdistfromline}
            \else
                \def\distfromline{\ctikzvalof{voltage/distance from line}\pgf@circ@Rlen}
            \fi
            \else
            \ifpgf@circuit@bipole@voltage@straight
                \def\distfromline{-\tmpdistfromline}
            \else
                \def\distfromline{-\ctikzvalof{voltage/distance from line}\pgf@circ@Rlen}
            \fi
        \fi
        \else
            \ifpgf@circuit@bipole@inverted
                \ifpgf@circuit@bipole@voltage@straight
                    \def\distfromline{-\tmpdistfromline}
                \else
                    \def\distfromline{-\ctikzvalof{voltage/distance from line}\pgf@circ@Rlen}
                \fi
                \else
                \ifpgf@circuit@bipole@voltage@straight
                    \def\distfromline{\tmpdistfromline}
                \else
                    \def\distfromline{\ctikzvalof{voltage/distance from line}\pgf@circ@Rlen}
                \fi
            \fi
        \fi
        \ifpgf@circuit@bipole@voltage@below
            \def\pgf@circ@voltage@angle{90}
        \else
            \def\pgf@circ@voltage@angle{-90}
        \fi
        \edef\pgf@temp{/tikz/circuitikz/bipoles/\pgfkeysvalueof{/tikz/circuitikz/bipole/kind}/voltage/distance from node}
        \pgfkeysifdefined{\pgf@temp}
        { \edef\distacefromnode{\ctikzvalof{bipoles/\pgfkeysvalueof{/tikz/circuitikz/bipole/kind}/voltage/distance from node}} }
        { \edef\distacefromnode{\ctikzvalof{voltage/distance from node}} }
        \edef\pgf@temp{/tikz/circuitikz/bipoles/\pgfkeysvalueof{/tikz/circuitikz/bipole/kind}/voltage/bump b}
        \pgfkeysifdefined{\pgf@temp}
        { \edef\bumpb{\ctikzvalof{bipoles/\pgfkeysvalueof{/tikz/circuitikz/bipole/kind}/voltage/bump b}} }
        { \edef\bumpb{\ctikzvalof{voltage/bump b}} }
        \edef\shiftv{\ctikzvalof{voltage/shift}}
        \pgfmathsetmacro{\bumpb}{\bumpb + \shiftv} %% adjust the bump is shift
        \ifpgf@circuit@bipole@inverted
            \pgfmathsetmacro{\shiftv}{-\shiftv}
        \fi
        \ifnum \ctikzvalof{mirror value} = -1
            \pgfmathsetmacro{\shiftv}{-\shiftv}
        \fi
    }
    % %\pgf@circ@Rlen/\pgfkeysvalueof{/tikz/circuitikz/current arrow scale} is equal to the length of the currarrow
    coordinate (pgfcirc@midtmp) at ($(\tikztostart) ! \pgf@circ@Rlen/\pgfkeysvalueof{/tikz/circuitikz/current arrow scale} ! (anchorstartnode)$) %absolute move, minimum space is length of arrowhead
    coordinate (pgfcirc@midtmp) at ($(pgfcirc@midtmp) ! \distacefromnode ! (anchorstartnode)$)

    coordinate (pgfcirc@Vfrom) at ($(pgfcirc@midtmp) ! -\distfromline ! \pgf@circ@voltage@angle:(anchorstartnode)$)
    coordinate (pgfcirc@midtmp) at ($(\tikztotarget) ! \pgf@circ@Rlen/\pgfkeysvalueof{/tikz/circuitikz/current arrow scale} ! (anchorendnode)$)%absolute move, minimum space is length of arrowhead
    coordinate (pgfcirc@midtmp) at ($(pgfcirc@midtmp) ! \distacefromnode ! (anchorendnode)$)

    coordinate (pgfcirc@Vto) at ($(pgfcirc@midtmp) ! \distfromline ! \pgf@circ@voltage@angle : (anchorendnode)$)

    \ifpgf@circuit@bipole@voltage@below
        coordinate (pgfcirc@Vto) at ($(pgfcirc@Vto) ! \shiftv!90 :  (anchorendnode)$)
        coordinate (pgfcirc@Vfrom) at ($(pgfcirc@Vfrom) ! \shiftv!-90 :  (anchorstartnode)$)
        coordinate (pgfcirc@Vcont1) at ($(\ctikzvalof{bipole/name}.center) ! \bumpb ! (\ctikzvalof{bipole/name}.-110)$)
        coordinate (pgfcirc@Vcont2) at ($(\ctikzvalof{bipole/name}.center) ! \bumpb ! (\ctikzvalof{bipole/name}.-70)$)
    \else
        coordinate (pgfcirc@Vto) at ($(pgfcirc@Vto) ! -\shiftv!90 :  (anchorendnode)$)
        coordinate (pgfcirc@Vfrom) at ($(pgfcirc@Vfrom) ! -\shiftv!-90 :  (anchorstartnode)$)
        coordinate (pgfcirc@Vcont1) at ($(\ctikzvalof{bipole/name}.center) ! \bumpb ! (\ctikzvalof{bipole/name}.110)$)
        coordinate (pgfcirc@Vcont2) at ($(\ctikzvalof{bipole/name}.center) ! \bumpb ! (\ctikzvalof{bipole/name}.70)$)
    \fi

    \ifpgf@circuit@europeanvoltage
        \ifpgf@circuit@bipole@voltage@straight
            \ifpgf@circuit@bipole@voltage@backward
                (pgfcirc@Vto) --(pgfcirc@Vfrom) node[currarrow, sloped,  allow upside down, pos=1,anchor=tip] {}
            \else
                (pgfcirc@Vfrom) --(pgfcirc@Vto) node[currarrow, sloped,  allow upside down, pos=1,anchor=tip] {}
            \fi
            \else
            \ifpgf@circuit@bipole@voltage@backward
                (pgfcirc@Vto) .. controls (pgfcirc@Vcont2)  and (pgfcirc@Vcont1) ..
                node[currarrow, sloped,  allow upside down, pos=1] {}
                (pgfcirc@Vfrom)
            \else
                (pgfcirc@Vfrom) .. controls (pgfcirc@Vcont1)  and (pgfcirc@Vcont2) ..
                node[currarrow, sloped,  allow upside down, pos=1] {}
                (pgfcirc@Vto)
            \fi
        \fi
        \else
        \ifpgf@circuit@bipole@voltage@backward
            \ifpgf@circ@oldvoltagedirection
                (pgfcirc@Vfrom) node[inner sep=0, node font=\pgf@circ@avfont,
                    anchor=\pgf@circ@bipole@voltage@label@anchor]{\pgf@circ@avplus}
                (pgfcirc@Vto) node[inner sep=0, node font=\pgf@circ@avfont,
                    anchor=\pgf@circ@bipole@voltage@label@anchor]{\pgf@circ@avminus}
            \else
                (pgfcirc@Vfrom) node[inner sep=0, node font=\pgf@circ@avfont,
                    anchor=\pgf@circ@bipole@voltage@label@anchor]{\pgf@circ@avminus}
                (pgfcirc@Vto) node[inner sep=0, node font=\pgf@circ@avfont,
                    anchor=\pgf@circ@bipole@voltage@label@anchor]{\pgf@circ@avplus}
            \fi
            \else
            \ifpgf@circ@oldvoltagedirection
                (pgfcirc@Vfrom) node[inner sep=0, node font=\pgf@circ@avfont,
                    anchor=\pgf@circ@bipole@voltage@label@anchor]{\pgf@circ@avminus}
                (pgfcirc@Vto) node[inner sep=0, node font=\pgf@circ@avfont,
                    anchor=\pgf@circ@bipole@voltage@label@anchor]{\pgf@circ@avplus}
            \else
                (pgfcirc@Vfrom) node[inner sep=0, node font=\pgf@circ@avfont,
                    anchor=\pgf@circ@bipole@voltage@label@anchor]{\pgf@circ@avplus}
                (pgfcirc@Vto) node[inner sep=0, node font=\pgf@circ@avfont,
                    anchor=\pgf@circ@bipole@voltage@label@anchor]{\pgf@circ@avminus}
            \fi
        \fi
    \fi
}

%% Output routine for voltage sources
\def\pgf@circ@drawvoltagegenerator{
    % the following is affected indirectly by voltage/shift, you can move the arrow with voltage/bump a.
    % it's not perfect, but I can't find the way to do it correctly...
    \pgfextra{
        \edef\shiftv{\ctikzvalof{voltage/shift}}
        \edef\bumpa{\ctikzvalof{voltage/bump a}}
        \pgfmathsetmacro{\bumpaplus}{\bumpa + \shiftv}
    }
    \ifpgf@circuit@bipole@voltage@below
        coordinate (pgfcirc@Vfrom) at ($(\ctikzvalof{bipole/name}.center) ! \bumpaplus ! (\ctikzvalof{bipole/name}.-120)$)
        coordinate (pgfcirc@Vto) at ($(\ctikzvalof{bipole/name}.center) ! \bumpaplus ! (\ctikzvalof{bipole/name}.-60)$)
    \else
        coordinate (pgfcirc@Vfrom) at ($ (\ctikzvalof{bipole/name}.center) ! \bumpaplus ! (\ctikzvalof{bipole/name}.120)$)
        coordinate (pgfcirc@Vto) at ($ (\ctikzvalof{bipole/name}.center) ! \bumpaplus ! (\ctikzvalof{bipole/name}.60)$)
    \fi
    \ifpgf@circuit@europeanvoltage
        \ifpgf@circuit@bipole@voltage@backward
            (pgfcirc@Vto)  -- node[currarrow, sloped,  allow upside down, pos=1] {} (pgfcirc@Vfrom)
        \else
            (pgfcirc@Vfrom)  -- node[currarrow, sloped,  allow upside down, pos=1] {} (pgfcirc@Vto)
        \fi
        \else% american voltage
        \ifpgf@circuit@bipole@voltageoutsideofsymbol
            % if it is a battery, must put + and -

            \ifpgf@circ@fixbatteries
                \ifpgf@circuit@bipole@voltage@backward
                    (pgfcirc@Vfrom)  node[node font=\pgf@circ@avfont] {\pgf@circ@avplus}
                    (pgfcirc@Vto) node[node font=\pgf@circ@avfont] {\pgf@circ@avminus}
                \else
                    (pgfcirc@Vfrom)  node[node font=\pgf@circ@avfont] {\pgf@circ@avminus}
                    (pgfcirc@Vto) node[node font=\pgf@circ@avfont] {\pgf@circ@avplus}
                \fi
                \else
                \ifpgf@circuit@bipole@voltage@backward
                    (pgfcirc@Vfrom)  node[node font=\pgf@circ@avfont] {\pgf@circ@avminus}
                    (pgfcirc@Vto) node[node font=\pgf@circ@avfont] {\pgf@circ@avplus}
                \else
                    (pgfcirc@Vfrom)  node[node font=\pgf@circ@avfont] {\pgf@circ@avplus}
                    (pgfcirc@Vto) node[node font=\pgf@circ@avfont] {\pgf@circ@avminus}
                \fi
            \fi
        \fi
    \fi
}

%% Output routine
\def\pgf@circ@drawvoltage{% node name
    \pgfextra{ %WARNING: indentation is probably wrong
        \edef\pgfcircmathresult{\expandafter\pgf@circ@stripdecimals\pgf@circ@direction\pgf@nil}
        \ifnum\pgfcircmathresult >4 \ifnum\pgfcircmathresult <86
        \ifpgf@circuit@bipole@voltage@below
            \def\pgf@circ@bipole@voltage@label@anchor{north west}
        \else
            \def\pgf@circ@bipole@voltage@label@anchor{south east}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >85 \ifnum\pgfcircmathresult <95
        \ifpgf@circuit@bipole@voltage@below
            \def\pgf@circ@bipole@voltage@label@anchor{west}
        \else
            \def\pgf@circ@bipole@voltage@label@anchor{east}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >94 \ifnum\pgfcircmathresult <176
        \ifpgf@circuit@bipole@voltage@below
            \def\pgf@circ@bipole@voltage@label@anchor{south west}
        \else \def\pgf@circ@bipole@voltage@label@anchor{north east}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >175 \ifnum\pgfcircmathresult <185
        \ifpgf@circuit@bipole@voltage@below
            \def\pgf@circ@bipole@voltage@label@anchor{south}
        \else\def\pgf@circ@bipole@voltage@label@anchor{north}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >184 \ifnum\pgfcircmathresult <266
        \ifpgf@circuit@bipole@voltage@below
            \def\pgf@circ@bipole@voltage@label@anchor{south east}
        \else\def\pgf@circ@bipole@voltage@label@anchor{north west}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >265 \ifnum\pgfcircmathresult <275
        \ifpgf@circuit@bipole@voltage@below
            \def\pgf@circ@bipole@voltage@label@anchor{east}
        \else \def\pgf@circ@bipole@voltage@label@anchor{west}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >274 \ifnum\pgfcircmathresult <356
        \ifpgf@circuit@bipole@voltage@below
            \def\pgf@circ@bipole@voltage@label@anchor{north east}
        \else\def\pgf@circ@bipole@voltage@label@anchor{south west}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >-1 \ifnum\pgfcircmathresult <5
        \ifpgf@circuit@bipole@voltage@below
            \def\pgf@circ@bipole@voltage@label@anchor{north}
        \else\def\pgf@circ@bipole@voltage@label@anchor{south}
        \fi
        \fi\fi
        \ifnum\pgfcircmathresult >355 \ifnum\pgfcircmathresult <361
        \ifpgf@circuit@bipole@voltage@below
            \def\pgf@circ@bipole@voltage@label@anchor{north}
        \else\def\pgf@circ@bipole@voltage@label@anchor{south}
        \fi
        \fi\fi

        \ifnum \ctikzvalof{mirror value}=-1
            \ifpgf@circuit@bipole@voltage@below
                \pgf@circuit@bipole@voltage@belowfalse
            \else
                \pgf@circuit@bipole@voltage@belowtrue
            \fi
        \fi

        \ifpgf@circuit@bipole@inverted
            \ifpgf@circuit@bipole@voltage@below
                \pgf@circuit@bipole@voltage@belowfalse
            \else

                \pgf@circuit@bipole@voltage@belowtrue
            \fi
        \fi

        \ifpgf@circuit@bipole@voltage@below
            \def\pgf@circ@bipole@voltage@label@where{-90}
        \else
            \def\pgf@circ@bipole@voltage@label@where{90}
        \fi


        \edef\pgf@temp{/tikz/circuitikz/bipoles/\pgfkeysvalueof{/tikz/circuitikz/bipole/kind}/voltage/european label distance}
        \pgfkeysifdefined{\pgf@temp}
        { \edef\eudist{\ctikzvalof{bipoles/\pgfkeysvalueof{/tikz/circuitikz/bipole/kind}/voltage/european label distance}} }
        { \edef\eudist{\ctikzvalof{voltage/european label distance}} }
        \edef\shiftv{\ctikzvalof{voltage/shift}}
        % adjust the label distance to the shift.
        \pgfmathsetmacro{\eudistplus}{\eudist+\shiftv}

        \pgfsetcornersarced{\pgfpointorigin}% do not use rounded corners!
    }%end pgfextra

    \ifpgf@circuit@bipole@isvoltage
        \pgf@circ@drawvoltagegenerator
    \else
        \pgf@circ@drawvoltagegeneric
    \fi

    %	(\ctikzvalof{bipole/name}.\pgf@circ@bipole@voltage@label@where) %Zeile sinnlos!?
    \ifpgf@circuit@bipole@voltage@straight
        coordinate (Vlab) at ($(pgfcirc@Vto)!0.5!(pgfcirc@Vfrom) $)
        node [anchor=\pgf@circ@bipole@voltage@label@anchor, inner sep=2pt]
        at (Vlab) { \pgf@circ@finallabels{voltage/label} }
    \else
        coordinate (Vlab) at ($(\ctikzvalof{bipole/name}.center) !
        \ifpgf@circuit@europeanvoltage
            \eudistplus
        \else
            \ctikzvalof{voltage/american label distance}
        \fi !
        (\ctikzvalof{bipole/name}.\pgf@circ@bipole@voltage@label@where)$)
        node [anchor=\pgf@circ@bipole@voltage@label@anchor, inner sep=2pt] at (Vlab) { \pgf@circ@finallabels{voltage/label} }
    \fi
}%end drawvoltages
\endinput


==> t-circuitikz.tex <==
\def\pgfcircversion{0.9.0}
\def\pgfcircversiondate{2019/05/10}
\writestatus{loading}{\pgfcircversiondate{} The CircuiTikz circuit drawing package version \pgfcircversion}

\usemodule[tikz]

\startmodule[circuitikz]
\usetikzlibrary[calc]
\usetikzlibrary[arrows.meta, bending]

\unprotect

\edef\tikzatcode{\the\catcode`\@}
\edef\tikzbarcode{\the\catcode`\|}
\edef\tikzexclaimcode{\the\catcode`\!}
\catcode`\@=11
\catcode`\|=12
\catcode`\!=12

\input pgfcirc.defines.tex
\input pgfcircutils.tex

\input pgfcircshapes.tex
\input pgfcircmonopoles.tex
\input pgfcircbipoles.tex
\input pgfcirctripoles.tex
\input pgfcircquadpoles.tex

\input pgfcirclabel.tex
\input pgfcircvoltage.tex
\input pgfcirccurrent.tex
\input pgfcircflow.tex

% defaults

\setupmodule
   [current=european,
    voltage=european,
    resistor=american,
    inductor=cute,
    logic=american,
    siunitx=true,
    arrowmos=false]

\processaction
   [\currentmoduleparameter{voltage}]
   [european=>\ctikzset{voltage=european},
    american=>\ctikzset{voltage=american}]

\processaction
   [\currentmoduleparameter{current}]
   [european=>\ctikzset{ current=european},
    american=>\ctikzset{ current=american}]

\processaction
   [\currentmoduleparameter{label}]
   [straight=>\ctikzset{label/align = straight},
    align=>\ctikzset{label/align = rotate},
    smart=>\ctikzset{label/align = smart}]

\processaction
   [\currentmoduleparameter{resistor}]
   [european=>\ctikzset{ resistor=european},
    american=>\ctikzset{ resistor=american}]

\processaction
   [\currentmoduleparameter{inductor}]
   [european=>\ctikzset{ inductor=european},
    american=>\ctikzset{ inductor=american},
    cute=>\ctikzset{ inductor=cute}]

\processaction
   [\currentmoduleparameter{diode}]
   [full=>\ctikzset{ diode=full},
    empty=>\ctikzset{ diode=empty}]

\processaction
   [\currentmoduleparameter{logic}]
   [european=>\ctikzset{ logic ports=european},
    american=>\ctikzset{ logic ports=american}]

\processaction
   [\currentmoduleparameter{siunitx}]
   [true=>\def\SI#1#2{#1\,#2}
    \def\ampere{\rm{A}}
    \def\volt{\rm{V}}
    \def\ohm{\Omega}
    \def\siemens{\rm{S}}
    \def\farad{\rm{F}}
    \def\henry{\rm{H}}
    \def\second{\rm{s}}
    \def\coulomb{\rm{C}}
    \def\siemens{\rm{S}}
    \def\radians{\rm{rad}}
    \def\milli{\rm{m}}
    \def\micro{\mu}
    \def\nano{\rm{n}}
    \def\pico{\rm{p}}
    \def\kilo{\rm{k}}
    \def\mega{\rm{M}}
    \def\giga{\rm{G}}
    \def\tera{\rm{T}},
    false=>]
%   \s!default=>\pgf@circ@siunitxtrue,

\processaction
   [\currentmoduleparameter{arrowmos}]
   [true=>\pgf@circuit@mos@arrowstrue,
    false=>\pgf@circuit@mos@arrowsfalse]
%   \s!default=>\pgf@circuit@mos@arrowstrue,


\ifpgf@circ@siunitx
 % nothing! siunitx and xstrings don't work in context
\fi


% Context specific

\ctikzset{tripoles/op amp/font/.initial=\switchtobodyfont[small]}

\input pgfcircpath.tex

\catcode`\@=\tikzatcode
\catcode`\|=\tikzbarcode
\catcode`\!=\tikzexclaimcode

% define the environment
\long\def\startcircuitikz#1\stopcircuitikz{\starttikzpicture#1\stoptikzpicture}

\protect

\stopmodule

\endinput

